Ascending and descending regions of a discrete Morse function

We present an algorithm which produces a decomposition of a regular cellular complex with a discrete Morse function analogous to the Morse-Smale decomposition of a smooth manifold with respect to a smooth Morse function. The advantage of our algorithm compared to similar existing results is that it works, at least theoretically, in any dimension. Practically, there are dimensional restrictions due to the size of cellular complexes of higher dimensions, though. We prove that the algorithm is correct in the sense that it always produces a decomposition into descending and ascending regions of the critical cells in a finite number of steps, and that, after a finite number of subdivisions, all the regions are topological discs. The efficiency of the algorithm is discussed and its performance on several examples is demonstrated.

==> examples/boundary/critical.tex <==
\psdot[dotstyle=o,dotsize=0.5](0, 0)


==> examples/boundary/field.tex <==
\psline[arrows=->,linewidth=0.01](3.33333, 3.33333)(1.66667, 1.66667)
\psline[arrows=->,linewidth=0.01](3.33333, 0)(1.66667, 0)
\psline[arrows=->,linewidth=0.01](0, 3.33333)(0, 1.66667)
\psline[arrows=->,linewidth=0.01](6.66667, 3.33333)(5, 1.66667)
\psline[arrows=->,linewidth=0.01](6.66667, 0)(5, 0)
\psline[arrows=->,linewidth=0.01](10, 3.33333)(8.33333, 1.66667)
\psline[arrows=->,linewidth=0.01](10, 0)(8.33333, 0)
\psline[arrows=->,linewidth=0.01](3.33333, 6.66667)(1.66667, 5)
\psline[arrows=->,linewidth=0.01](0, 6.66667)(0, 5)
\psline[arrows=->,linewidth=0.01](6.66667, 6.66667)(5, 5)
\psline[arrows=->,linewidth=0.01](10, 6.66667)(8.33333, 5)
\psline[arrows=->,linewidth=0.01](3.33333, 10)(1.66667, 8.33333)
\psline[arrows=->,linewidth=0.01](0, 10)(0, 8.33333)
\psline[arrows=->,linewidth=0.01](6.66667, 10)(5, 8.33333)
\psline[arrows=->,linewidth=0.01](10, 10)(8.33333, 8.33333)
\psline[arrows=->,linewidth=0.01](3.33333, 1.66667)(2.22222, 1.11111)
\psline[arrows=->,linewidth=0.01](1.66667, 3.33333)(1.11111, 2.22222)
\psline[arrows=->,linewidth=0.01](6.66667, 1.66667)(5.55556, 1.11111)
\psline[arrows=->,linewidth=0.01](5, 3.33333)(4.44444, 2.22222)
\psline[arrows=->,linewidth=0.01](10, 1.66667)(8.88889, 1.11111)
\psline[arrows=->,linewidth=0.01](8.33333, 3.33333)(7.77778, 2.22222)
\psline[arrows=->,linewidth=0.01](3.33333, 5)(2.22222, 4.44444)
\psline[arrows=->,linewidth=0.01](1.66667, 6.66667)(1.11111, 5.55556)
\psline[arrows=->,linewidth=0.01](6.66667, 5)(5.55556, 4.44444)
\psline[arrows=->,linewidth=0.01](5, 6.66667)(4.44444, 5.55556)
\psline[arrows=->,linewidth=0.01](10, 5)(8.88889, 4.44444)
\psline[arrows=->,linewidth=0.01](8.33333, 6.66667)(7.77778, 5.55556)
\psline[arrows=->,linewidth=0.01](3.33333, 8.33333)(2.22222, 7.77778)
\psline[arrows=->,linewidth=0.01](1.66667, 10)(1.11111, 8.88889)
\psline[arrows=->,linewidth=0.01](6.66667, 8.33333)(5.55556, 7.77778)
\psline[arrows=->,linewidth=0.01](5, 10)(4.44444, 8.88889)
\psline[arrows=->,linewidth=0.01](10, 8.33333)(8.88889, 7.77778)
\psline[arrows=->,linewidth=0.01](8.33333, 10)(7.77778, 8.88889)


==> examples/boundary/graph.tex <==
\psline[linecolor=black,linewidth=0.01](3.33333, 0)(3.33333, 3.33333)
\psline[linecolor=black,linewidth=0.01](0, 0)(3.33333, 3.33333)
\psline[linecolor=black,linewidth=0.01](0, 0)(3.33333, 0)
\psline[linecolor=black,linewidth=0.01](0, 3.33333)(3.33333, 3.33333)
\psline[linecolor=black,linewidth=0.01](0, 0)(0, 3.33333)
\psline[linecolor=black,linewidth=0.01](6.66667, 0)(6.66667, 3.33333)
\psline[linecolor=black,linewidth=0.01](3.33333, 0)(6.66667, 3.33333)
\psline[linecolor=black,linewidth=0.01](3.33333, 0)(6.66667, 0)
\psline[linecolor=black,linewidth=0.01](3.33333, 3.33333)(6.66667, 3.33333)
\psline[linecolor=black,linewidth=0.01](10, 0)(10, 3.33333)
\psline[linecolor=black,linewidth=0.01](6.66667, 0)(10, 3.33333)
\psline[linecolor=black,linewidth=0.01](6.66667, 0)(10, 0)
\psline[linecolor=black,linewidth=0.01](6.66667, 3.33333)(10, 3.33333)
\psline[linecolor=black,linewidth=0.01](3.33333, 3.33333)(3.33333, 6.66667)
\psline[linecolor=black,linewidth=0.01](0, 3.33333)(3.33333, 6.66667)
\psline[linecolor=black,linewidth=0.01](0, 6.66667)(3.33333, 6.66667)
\psline[linecolor=black,linewidth=0.01](0, 3.33333)(0, 6.66667)
\psline[linecolor=black,linewidth=0.01](6.66667, 3.33333)(6.66667, 6.66667)
\psline[linecolor=black,linewidth=0.01](3.33333, 3.33333)(6.66667, 6.66667)
\psline[linecolor=black,linewidth=0.01](3.33333, 6.66667)(6.66667, 6.66667)
\psline[linecolor=black,linewidth=0.01](10, 3.33333)(10, 6.66667)
\psline[linecolor=black,linewidth=0.01](6.66667, 3.33333)(10, 6.66667)
\psline[linecolor=black,linewidth=0.01](6.66667, 6.66667)(10, 6.66667)
\psline[linecolor=black,linewidth=0.01](3.33333, 6.66667)(3.33333, 10)
\psline[linecolor=black,linewidth=0.01](0, 6.66667)(3.33333, 10)
\psline[linecolor=black,linewidth=0.01](0, 10)(3.33333, 10)
\psline[linecolor=black,linewidth=0.01](0, 6.66667)(0, 10)
\psline[linecolor=black,linewidth=0.01](6.66667, 6.66667)(6.66667, 10)
\psline[linecolor=black,linewidth=0.01](3.33333, 6.66667)(6.66667, 10)
\psline[linecolor=black,linewidth=0.01](3.33333, 10)(6.66667, 10)
\psline[linecolor=black,linewidth=0.01](10, 6.66667)(10, 10)
\psline[linecolor=black,linewidth=0.01](6.66667, 6.66667)(10, 10)
\psline[linecolor=black,linewidth=0.01](6.66667, 10)(10, 10)


==> examples/boundary/square/critical.tex <==
\psline[linecolor=black,linewidth=0.01](10.6, 7.06667)(10.6, 10.2)

\psdot[dotstyle=otimes,dotsize=0.5](10.6, 8.33333)

\psdot[dotstyle=o,dotsize=0.5](-0.6, -0.6)


==> examples/boundary/square/field.tex <==
\psline[arrows=->,linewidth=0.01](3.33333, -0.6)(1.66667, -0.6)
\psline[arrows=->,linewidth=0.01](6.66667, -0.6)(5, -0.6)
\psline[arrows=->,linewidth=0.01](10.6,-0.6)(8.33333, -0.6)
\psline[arrows=->,linewidth=0.01](10.6, 3.33333)(10.6, 1.66667)
\psline[arrows=->,linewidth=0.01](10.6, 6.66667)(10.6, 5)
\psline[arrows=->,linewidth=0.01](10.6, 10.6)(8.33333, 10.6)
\psline[arrows=->,linewidth=0.01](6.66667, 10.6)(5, 10.6)
\psline[arrows=->,linewidth=0.01](3.33333, 10.6)(1.66667, 10.6)
\psline[arrows=->,linewidth=0.01](-0.6, 10.6) (-0.6, 8.33333)
\psline[arrows=->,linewidth=0.01](-0.6, 6.66667)(-0.6, 5)
\psline[arrows=->,linewidth=0.01](-0.6, 3.33333)(-0.6, 1.66667)


==> examples/cart/cart_maximum_discs.tex <==
%\psset{unit=10mm}
%\begin{pspicture}(0, 0)(10, 10)
%\input {examples/cart/graph.tex}

%BOTTOM-RIGHT MAXIMUM
\input {examples/cart/ddisc1.tex}

%TOP-RIGHT MAXIMUM
\input {examples/cart/ddisc2.tex}

%CENTER SADDLE (extends to the right)
%\input {examples/cart/ddisc3.tex}

%CENTER MAXIMUM (extends to the left)
\input {examples/cart/ddisc4.tex}

%BOTTOM-LEFT MINIMUM
%\input {examples/cart/ddisc5.tex}

%TOP-LEFT MINIMUM
%\input {examples/cart/ddisc6.tex}

%LEFT SADLLE
%\input {examples/cart/ddisc7.tex}

%TOP-LEFT-CENTRAL SADDLE
%\input {examples/cart/ddisc8.tex}

%BOTTOM-LEFT-CENTRAL SADDLE
%\input {examples/cart/ddisc9.tex}

%CENTRAL MINIMUM
%\input {examples/cart/ddisc10.tex}


%\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](2.81252, 5)(2.5, 5.25)(2.5, 5)

%\psset{unit=8mm}
\psdot[dotstyle=o,dotsize=0.5,fillstyle=solid,fillcolor=black](2.60417, 5.08333)
%\psdot[dotstyle=oplus,dotsize=0.5](2.60417, 5.08333)

%\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](10, 0.25)(9.68742, 0)(10, 0)
\psdot[dotstyle=o,dotsize=0.5,fillstyle=solid,fillcolor=black](9.89581, 0.0833333)

%\psdot[dotstyle=oplus,dotsize=0.5](9.89581, 0.0833333)

%\pspolygon[linestyle=none,fillcolor=lightgray,fillstyle=solid](9.68742, 10)(9.68742, 9.75)(10, 10)
\psdot[dotstyle=o,dotsize=0.5, fillstyle=solid,fillcolor=black](9.79161, 9.91667)
% \psdot[dotstyle=oplus,dotsize=0.5](9.79161, 9.91667)
%\psset{unit=5mm}

%\end{pspicture}


==> examples/cart/cart_saddle_discs.tex <==
%\psset{unit=10mm}
%\begin{pspicture}(0, 0)(10, 10)
\input {examples/cart/graph.tex}

%BOTTOM-RIGHT MAXIMUM
%\input {examples/cart/ddisc1.tex}

%TOP-RIGHT MAXIMUM
%\input {examples/cart/ddisc2.tex}

%CENTER SADDLE (extends to the right)
\input {examples/cart/ddisc3.tex}

%CENTER MAXIMUM (extends to the left)
%\input {examples/cart/ddisc4.tex}

%BOTTOM-LEFT MINIMUM
%\input {examples/cart/ddisc5.tex}

%TOP-LEFT MINIMUM
%\input {examples/cart/ddisc6.tex}

%LEFT SADLLE
\input {examples/cart/ddisc7.tex}

%TOP-LEFT-CENTRAL SADDLE
\input {examples/cart/ddisc8.tex}

%BOTTOM-LEFT-CENTRAL SADDLE
\input {examples/cart/ddisc9.tex}

%CENTRAL MINIMUM
%\input {examples/cart/ddisc10.tex}

\psline[linewidth=0.1,linecolor=black](0, 5.25)(0, 5)
\psdot[dotstyle=o,dotsize=0.5](0, 5.125)
\psdot[dotstyle=otimes,dotsize=0.5](0, 5.125)

\psline[linewidth=0.1,linecolor=black](5, 7)(5, 6.75)
\psdot[dotstyle=o,dotsize=0.5](5, 6.875)
\psdot[dotstyle=otimes,dotsize=0.5](5, 6.875)

\psline[linewidth=0.1,linecolor=black](4.6875, 3)(5, 3)
\psdot[dotstyle=o,dotsize=0.5](4.84375, 3)
\psdot[dotstyle=otimes,dotsize=0.5](4.84375, 3)

\psline[linewidth=0.1,linecolor=black](9.68742, 5)(10, 5)
\psdot[dotstyle=o,dotsize=0.5](9.84371, 5)
\psdot[dotstyle=otimes,dotsize=0.5](9.84371, 5)

\psdot[dotstyle=o,dotsize=0.5](0, 0)
\psdot[dotstyle=o,dotsize=0.5](0, 10)
\psdot[dotstyle=o,dotsize=0.5](7.5, 5)


%\end{pspicture}


==> examples/cart/ddisc1.tex <==
\newrgbcolor{disc1}{0.6 0.6 0.6}
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 0.25)(9.68742, 0)(10, 0)
\psline[linewidth=0.03,linecolor=black](9.68742, 0)(10, 0)
\psline[linewidth=0.03,linecolor=black](10, 0.25)(9.68742, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 0)(10, 0.25)(9.68742, 0.25)
\psline[linewidth=0.03,linecolor=black](10, 0.25)(9.68742, 0.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 0)(9.68742, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 0.25)(9.68742, 0)(9.68742, 0.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.25)(9.68742, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 0.5)(9.37484, 0.25)(9.68742, 0.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.5)(9.37484, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 0.5)(9.37484, 0.25)(9.68742, 0.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.5)(9.68742, 0.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.5)(9.37484, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 0.25)(9.37484, 0.5)(9.06258, 0.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.5)(9.06258, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 0.5)(9.06258, 0.75)(9.06258, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 0.75)(9.37484, 0.5)(9.68742, 0.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.75)(9.37484, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 0.75)(9.37484, 0.75)(9.37484, 0.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.75)(9.37484, 0.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.75)(9.37484, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 0.75)(9.37484, 1)(9.37484, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 0.75)(9.06258, 0.75)(9.37484, 0.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.75)(9.06258, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 1)(9.06258, 0.75)(9.37484, 0.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 1)(9.06258, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 0.75)(9.37484, 1)(9.06258, 1)
\psline[linewidth=0.03,linecolor=black](9.37484, 1)(9.06258, 1)
\psline[linewidth=0.03,linecolor=black](9.06258, 0.75)(9.06258, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 1)(9.06258, 0.75)(9.06258, 1)
\psline[linewidth=0.03,linecolor=black](8.75, 1)(9.06258, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.25)(8.75, 1)(9.06258, 1)
\psline[linewidth=0.03,linecolor=black](8.75, 1)(9.06258, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 1)(9.06258, 1.25)(8.75, 1.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.25)(8.75, 1.25)
\psline[linewidth=0.03,linecolor=black](8.75, 1)(8.75, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 1.25)(8.75, 1)(8.75, 1.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.25)(8.75, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 1.5)(8.43742, 1.25)(8.75, 1.25)
\psline[linewidth=0.03,linecolor=black](8.75, 1.5)(8.43742, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 1.5)(8.43742, 1.5)(8.43742, 1.25)
\psline[linewidth=0.03,linecolor=black](8.75, 1.5)(8.43742, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 1.5)(8.43742, 1.75)(8.43742, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.25)(9.06258, 1.5)(8.75, 1.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.5)(8.75, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.5)(8.75, 1.5)(8.75, 1.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.5)(8.75, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 1.5)(9.06258, 1.5)(8.75, 1.75)
\psline[linewidth=0.03,linecolor=black](8.75, 1.5)(8.75, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 1.75)(8.75, 1.5)(8.75, 1.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.75)(8.75, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2)(8.43742, 1.75)(8.75, 1.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.75)(8.75, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 1.75)(8.75, 2)(8.43742, 2)
\psline[linewidth=0.03,linecolor=black](8.75, 2)(8.43742, 2)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.75)(8.43742, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 2)(8.43742, 1.75)(8.43742, 2)
\psline[linewidth=0.03,linecolor=black](8.125, 2)(8.43742, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.25)(8.125, 2)(8.43742, 2)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.25)(8.125, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 2.25)(8.125, 2)(8.43742, 2.25)
\psline[linewidth=0.03,linecolor=black](8.125, 2.25)(8.43742, 2.25)
\psline[linewidth=0.03,linecolor=black](8.125, 2.25)(8.125, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 2)(8.125, 2.25)(7.81248, 2.25)
\psline[linewidth=0.03,linecolor=black](8.125, 2.25)(7.81248, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 2.25)(7.81248, 2.5)(7.81248, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.5)(8.125, 2.25)(8.43742, 2.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.5)(8.125, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.5)(8.125, 2.5)(8.125, 2.25)
\psline[linewidth=0.03,linecolor=black](8.125, 2.5)(8.125, 2.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.5)(8.125, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.5)(8.43742, 2.75)(8.125, 2.5)
\psline[linewidth=0.03,linecolor=black](8.125, 2.5)(8.43742, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 2.5)(8.43742, 2.75)(8.125, 2.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.75)(8.125, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.75)(8.125, 3)(8.125, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 2.5)(7.81248, 2.5)(8.125, 2.25)
\psline[linewidth=0.03,linecolor=black](8.125, 2.5)(7.81248, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 2.5)(8.125, 2.5)(8.125, 2.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 2.5)(8.125, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 2.5)(8.125, 2.75)(7.81248, 2.75)
\psline[linewidth=0.03,linecolor=black](8.125, 2.75)(7.81248, 2.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 2.5)(7.81248, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.75)(7.81248, 2.5)(7.81248, 2.75)
\psline[linewidth=0.03,linecolor=black](7.5, 2.75)(7.81248, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3)(7.5, 2.75)(7.81248, 2.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 3)(7.5, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3)(7.5, 3)(7.5, 2.75)
\psline[linewidth=0.03,linecolor=black](7.5, 3)(7.5, 2.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 3)(7.5, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 3)(7.81248, 3)(7.5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 3)(7.18748, 3)(7.5, 2.75)
\psline[linewidth=0.03,linecolor=black](7.5, 3)(7.18748, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 3)(7.5, 3)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 3)(7.5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 3.25)(7.18748, 3)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.25)(7.5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 3.5)(7.18748, 3.25)(7.5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 2.75)(8.125, 3)(7.81248, 2.75)
\psline[linewidth=0.03,linecolor=black](8.125, 3)(7.81248, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 3)(7.81248, 3)(7.81248, 2.75)
\psline[linewidth=0.03,linecolor=black](8.125, 3)(7.81248, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3)(8.125, 3)(7.81248, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 3)(7.81248, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3)(7.81248, 3.25)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.25)(7.5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3.25)(7.81248, 3.5)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.5)(7.5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3.5)(7.5, 3.5)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.5, 3.5)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.5)(7.5, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3.5)(7.5, 3.75)(7.5, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 3.5)(7.18748, 3.5)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.5, 3.5)(7.18748, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 3.75)(7.18748, 3.5)(7.5, 3.5)
\psline[linewidth=0.03,linecolor=black](7.5, 3.75)(7.18748, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 3.75)(7.18748, 3.75)(7.18748, 3.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.75)(7.18748, 3.5)
\psline[linewidth=0.03,linecolor=black](7.5, 3.75)(7.18748, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 3.75)(7.18748, 4)(7.18748, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 3.75)(6.875, 3.75)(7.18748, 3.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.75)(6.875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4)(6.875, 3.75)(7.18748, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2)(8.43742, 2.25)(8.43742, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 1)(9.06258, 1.25)(9.06258, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 0.25)(9.68742, 0.5)(9.68742, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 0)(9.37484, 0.25)(9.37484, 0)
\psline[linewidth=0.03,linecolor=black](9.68742, 0)(9.37484, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 0.25)(9.06258, 0)(9.37484, 0)
\psline[linewidth=0.03,linecolor=black](9.06258, 0)(9.37484, 0)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.25)(9.06258, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 0)(9.37484, 0.25)(9.06258, 0.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 0.25)(9.37484, 0.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 0)(9.06258, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.25)(9.06258, 0)(9.06258, 0.25)
\psline[linewidth=0.03,linecolor=black](8.75, 0.25)(9.06258, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.25)(9.06258, 0.25)(9.06258, 0.5)
\psline[linewidth=0.03,linecolor=black](8.75, 0.25)(9.06258, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.5)(8.75, 0.25)(9.06258, 0.5)
\psline[linewidth=0.03,linecolor=black](8.75, 0.5)(9.06258, 0.5)
\psline[linewidth=0.03,linecolor=black](8.75, 0.25)(8.75, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 0.5)(8.75, 0.25)(8.75, 0.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.5)(8.75, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.75)(8.43742, 0.5)(8.75, 0.5)
\psline[linewidth=0.03,linecolor=black](8.75, 0.75)(8.43742, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.75)(8.43742, 0.75)(8.43742, 0.5)
\psline[linewidth=0.03,linecolor=black](8.75, 0.75)(8.43742, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 0.75)(8.75, 0.75)(8.43742, 1)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.75)(8.43742, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 1)(8.43742, 0.75)(8.43742, 1)
\psline[linewidth=0.03,linecolor=black](8.125, 1)(8.43742, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 1.25)(8.125, 1)(8.43742, 1)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.25)(8.125, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 1.25)(8.125, 1)(8.43742, 1.25)
\psline[linewidth=0.03,linecolor=black](8.125, 1.25)(8.43742, 1.25)
\psline[linewidth=0.03,linecolor=black](8.125, 1.25)(8.125, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 1)(8.125, 1.25)(7.81248, 1.25)
\psline[linewidth=0.03,linecolor=black](8.125, 1.25)(7.81248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 1.25)(7.81248, 1.5)(7.81248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 1.5)(8.125, 1.25)(8.43742, 1.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.5)(8.125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 1.5)(8.125, 1.25)(8.43742, 1.5)
\psline[linewidth=0.03,linecolor=black](8.125, 1.5)(8.43742, 1.5)
\psline[linewidth=0.03,linecolor=black](8.125, 1.5)(8.125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1.5)(8.125, 1.25)(8.125, 1.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.5)(8.125, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1.75)(7.81248, 1.5)(8.125, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 1.75)(8.125, 1.5)(8.43742, 1.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.75)(8.125, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 1.75)(8.125, 1.75)(8.125, 1.5)
\psline[linewidth=0.03,linecolor=black](8.125, 1.75)(8.125, 1.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.75)(8.125, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 1.75)(8.43742, 1.75)(8.125, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 1.75)(7.81248, 1.75)(8.125, 1.5)
\psline[linewidth=0.03,linecolor=black](8.125, 1.75)(7.81248, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1.75)(8.125, 1.75)(8.125, 2)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.75)(8.125, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1.75)(8.125, 2)(7.81248, 2)
\psline[linewidth=0.03,linecolor=black](7.81248, 2)(8.125, 2)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.75)(7.81248, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2)(7.81248, 1.75)(7.81248, 2)
\psline[linewidth=0.03,linecolor=black](7.5, 2)(7.81248, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.25)(7.5, 2)(7.81248, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 2)(8.125, 2)(7.81248, 2.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 2)(7.81248, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.25)(7.81248, 2)(7.81248, 2.25)
\psline[linewidth=0.03,linecolor=black](7.5, 2.25)(7.81248, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 2.5)(7.5, 2.25)(7.81248, 2.25)
\psline[linewidth=0.03,linecolor=black](7.5, 2.25)(7.81248, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.25)(7.81248, 2.5)(7.5, 2.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 2.5)(7.5, 2.5)
\psline[linewidth=0.03,linecolor=black](7.5, 2.25)(7.5, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.25)(7.5, 2.5)(7.18748, 2.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 2.5)(7.5, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 2.5)(7.5, 2.5)(7.18748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.5)(7.81248, 2.5)(7.5, 2.75)
\psline[linewidth=0.03,linecolor=black](7.5, 2.5)(7.5, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.5)(7.5, 2.75)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](7.5, 2.75)(7.18748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.75)(7.18748, 3)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 3)(7.18748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 3)(6.875, 3)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 3)(6.875, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3)(7.18748, 3)(7.18748, 3.25)
\psline[linewidth=0.03,linecolor=black](6.875, 3)(7.18748, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3)(7.18748, 3.25)(6.875, 3.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.25)(6.875, 3.25)
\psline[linewidth=0.03,linecolor=black](6.875, 3)(6.875, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 3.25)(6.875, 3)(6.875, 3.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.25)(6.875, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3.5)(6.56248, 3.25)(6.875, 3.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.25)(6.875, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 3.25)(6.875, 3.5)(6.56248, 3.5)
\psline[linewidth=0.03,linecolor=black](6.875, 3.5)(6.56248, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3.5)(6.875, 3.75)(6.56248, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 3.25)(7.18748, 3.5)(6.875, 3.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.5)(6.875, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 3.5)(6.875, 3.5)(6.875, 3.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.5)(6.875, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 3.5)(6.875, 3.75)(6.875, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 0.75)(8.75, 0.5)(9.06258, 0.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 0.75)(8.75, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 0.75)(8.75, 0.75)(8.75, 0.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 0.75)(8.75, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.75)(9.06258, 0.75)(8.75, 1)
\psline[linewidth=0.03,linecolor=black](8.75, 0.75)(8.75, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.75)(8.75, 1)(8.43742, 1)
\psline[linewidth=0.03,linecolor=black](8.75, 1)(8.43742, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 1)(8.43742, 1.25)(8.43742, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 0.25)(9.37484, 0.25)(9.06258, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 0)(8.75, 0.25)(8.75, 0)
\psline[linewidth=0.03,linecolor=black](9.06258, 0)(8.75, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.25)(8.43742, 0)(8.75, 0)
\psline[linewidth=0.03,linecolor=black](8.43742, 0)(8.75, 0)
\psline[linewidth=0.03,linecolor=black](8.75, 0.25)(8.43742, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 0)(8.75, 0.25)(8.43742, 0.25)
\psline[linewidth=0.03,linecolor=black](8.75, 0.25)(8.43742, 0.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 0)(8.43742, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 0.25)(8.43742, 0)(8.43742, 0.25)
\psline[linewidth=0.03,linecolor=black](8.125, 0.25)(8.43742, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 0.5)(8.125, 0.25)(8.43742, 0.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.5)(8.125, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 0.25)(8.43742, 0.5)(8.125, 0.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.5)(8.125, 0.5)
\psline[linewidth=0.03,linecolor=black](8.125, 0.25)(8.125, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 0.5)(8.125, 0.25)(8.125, 0.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 0.5)(8.125, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 0.75)(7.81248, 0.5)(8.125, 0.5)
\psline[linewidth=0.03,linecolor=black](8.125, 0.75)(7.81248, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 0.75)(7.81248, 0.75)(7.81248, 0.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 0.75)(7.81248, 0.5)
\psline[linewidth=0.03,linecolor=black](8.125, 0.75)(7.81248, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 0.75)(8.125, 1)(7.81248, 0.75)
\psline[linewidth=0.03,linecolor=black](8.125, 1)(7.81248, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 1)(7.81248, 1)(7.81248, 0.75)
\psline[linewidth=0.03,linecolor=black](8.125, 1)(7.81248, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1)(8.125, 1)(7.81248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 0.75)(7.5, 0.75)(7.81248, 0.5)
\psline[linewidth=0.03,linecolor=black](7.5, 0.75)(7.81248, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1)(7.5, 0.75)(7.81248, 0.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 1)(7.5, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 1)(7.5, 0.75)(7.81248, 1)
\psline[linewidth=0.03,linecolor=black](7.5, 1)(7.81248, 1)
\psline[linewidth=0.03,linecolor=black](7.5, 1)(7.5, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 0.75)(7.5, 1)(7.18748, 1)
\psline[linewidth=0.03,linecolor=black](7.18748, 1)(7.5, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 1)(7.5, 1)(7.18748, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 1)(7.81248, 1)(7.81248, 1.25)
\psline[linewidth=0.03,linecolor=black](7.5, 1)(7.81248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 1.25)(7.5, 1)(7.81248, 1.25)
\psline[linewidth=0.03,linecolor=black](7.5, 1.25)(7.81248, 1.25)
\psline[linewidth=0.03,linecolor=black](7.5, 1)(7.5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 1)(7.5, 1.25)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](7.5, 1.25)(7.18748, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 1.25)(7.18748, 1.5)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 1.5)(7.18748, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 1.5)(6.875, 1.5)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](6.875, 1.5)(7.18748, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1.5)(7.18748, 1.5)(7.18748, 1.75)
\psline[linewidth=0.03,linecolor=black](6.875, 1.5)(7.18748, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1.75)(6.875, 1.5)(7.18748, 1.75)
\psline[linewidth=0.03,linecolor=black](6.875, 1.75)(7.18748, 1.75)
\psline[linewidth=0.03,linecolor=black](6.875, 1.5)(6.875, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1.5)(6.875, 1.75)(6.56248, 1.75)
\psline[linewidth=0.03,linecolor=black](6.875, 1.75)(6.56248, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1.75)(6.875, 2)(6.56248, 1.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 1.75)(6.875, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 1.75)(6.875, 2)(6.56248, 2)
\psline[linewidth=0.03,linecolor=black](6.875, 2)(6.56248, 2)
\psline[linewidth=0.03,linecolor=black](6.56248, 1.75)(6.56248, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 1.75)(6.56248, 2)(6.25, 2)
\psline[linewidth=0.03,linecolor=black](6.56248, 2)(6.25, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 2)(6.25, 2.25)(6.25, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2)(6.56248, 2.25)(6.56248, 2)
\psline[linewidth=0.03,linecolor=black](6.56248, 2.25)(6.56248, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 2.25)(6.25, 2.25)(6.56248, 2)
\psline[linewidth=0.03,linecolor=black](6.56248, 2.25)(6.25, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.5)(6.25, 2.25)(6.56248, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2)(6.875, 1.75)(7.18748, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1.5)(7.5, 1.25)(7.81248, 1.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.5)(7.5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1.5)(7.5, 1.5)(7.5, 1.25)
\psline[linewidth=0.03,linecolor=black](7.5, 1.5)(7.5, 1.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.5)(7.5, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1.5)(7.81248, 1.75)(7.5, 1.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.75)(7.5, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 1.5)(7.81248, 1.75)(7.5, 1.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.75)(7.5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 1.75)(7.5, 2)(7.5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 1.5)(7.18748, 1.5)(7.5, 1.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 1.5)(7.5, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 1.5)(7.5, 1.5)(7.5, 1.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 1.5)(7.5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 1.75)(7.18748, 1.5)(7.5, 1.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 1.75)(7.5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2)(7.18748, 1.75)(7.5, 1.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 1.75)(7.5, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 1.75)(7.5, 2)(7.18748, 2)
\psline[linewidth=0.03,linecolor=black](7.5, 2)(7.18748, 2)
\psline[linewidth=0.03,linecolor=black](7.18748, 1.75)(7.18748, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2)(7.18748, 1.75)(7.18748, 2)
\psline[linewidth=0.03,linecolor=black](6.875, 2)(7.18748, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 2.25)(6.875, 2)(7.18748, 2)
\psline[linewidth=0.03,linecolor=black](7.18748, 2.25)(6.875, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2)(7.18748, 2.25)(6.875, 2.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 2.25)(6.875, 2.25)
\psline[linewidth=0.03,linecolor=black](6.875, 2)(6.875, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 2.25)(6.875, 2)(6.875, 2.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 2.25)(6.875, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2.5)(6.56248, 2.25)(6.875, 2.25)
\psline[linewidth=0.03,linecolor=black](6.875, 2.5)(6.56248, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2.5)(6.56248, 2.5)(6.56248, 2.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 2.5)(6.56248, 2.25)
\psline[linewidth=0.03,linecolor=black](6.875, 2.5)(6.56248, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 2.5)(6.875, 2.5)(6.56248, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 2.5)(6.25, 2.5)(6.56248, 2.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 2.5)(6.25, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.5)(6.56248, 2.5)(6.56248, 2.75)
\psline[linewidth=0.03,linecolor=black](6.25, 2.5)(6.56248, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.75)(6.25, 2.5)(6.56248, 2.75)
\psline[linewidth=0.03,linecolor=black](6.25, 2.75)(6.56248, 2.75)
\psline[linewidth=0.03,linecolor=black](6.25, 2.5)(6.25, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.5)(6.25, 2.75)(5.93748, 2.75)
\psline[linewidth=0.03,linecolor=black](6.25, 2.75)(5.93748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.75)(5.93748, 3)(5.93748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.75)(6.56248, 2.75)(6.56248, 3)
\psline[linewidth=0.03,linecolor=black](6.25, 2.75)(6.56248, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 3)(6.25, 2.75)(6.56248, 3)
\psline[linewidth=0.03,linecolor=black](6.25, 3)(6.56248, 3)
\psline[linewidth=0.03,linecolor=black](6.25, 3)(6.25, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3)(6.25, 2.75)(6.25, 3)
\psline[linewidth=0.03,linecolor=black](5.93748, 3)(6.25, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3)(6.25, 3)(6.25, 3.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 3)(6.25, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3.25)(5.93748, 3)(6.25, 3.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 3.25)(6.25, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 3.5)(5.93748, 3.25)(6.25, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 3.25)(6.25, 3)(6.56248, 3)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.25)(6.25, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 3)(6.56248, 3.25)(6.25, 3.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.25)(6.25, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 3.25)(6.25, 3.5)(6.25, 3.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.25)(6.25, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 3.5)(6.56248, 3.25)(6.56248, 3.5)
\psline[linewidth=0.03,linecolor=black](6.25, 3.5)(6.56248, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 3.75)(6.25, 3.5)(6.56248, 3.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.75)(6.56248, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3.75)(6.56248, 3.75)(6.56248, 3.5)
\psline[linewidth=0.03,linecolor=black](6.875, 3.75)(6.56248, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3.75)(6.56248, 4)(6.56248, 3.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 4)(6.875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 4)(6.875, 3.75)(6.875, 4)
\psline[linewidth=0.03,linecolor=black](6.875, 3.75)(6.875, 4)
\psline[linewidth=0.03,linecolor=black](6.56248, 4)(6.875, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 4.25)(6.56248, 4)(6.875, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3.75)(7.18748, 4)(6.875, 4)
\psline[linewidth=0.03,linecolor=black](7.18748, 4)(6.875, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4)(6.875, 4.25)(6.875, 4)
\psline[linewidth=0.03,linecolor=black](6.875, 4.25)(7.18748, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 4.25)(7.18748, 4)(7.18748, 4.25)
\psline[linewidth=0.03,linecolor=black](6.875, 4.25)(7.18748, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 4.5)(6.875, 4.25)(7.18748, 4.25)
\psline[linewidth=0.03,linecolor=black](6.875, 4.5)(7.18748, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4.5)(6.875, 4.5)(7.18748, 4.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.5)(6.875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4.75)(6.875, 4.5)(7.18748, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 2.25)(6.875, 2.5)(6.875, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2)(7.5, 2.25)(7.18748, 2)
\psline[linewidth=0.03,linecolor=black](7.5, 2.25)(7.18748, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.25)(7.18748, 2.25)(7.18748, 2)
\psline[linewidth=0.03,linecolor=black](7.5, 2.25)(7.18748, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 2.25)(7.18748, 2.5)(7.18748, 2.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 2.5)(7.18748, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 2.5)(6.875, 2.5)(7.18748, 2.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 2.5)(6.875, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2.5)(7.18748, 2.5)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](6.875, 2.5)(7.18748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2.75)(6.875, 2.5)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](6.875, 2.75)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](6.875, 2.75)(6.875, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2.5)(6.875, 2.75)(6.56248, 2.75)
\psline[linewidth=0.03,linecolor=black](6.875, 2.75)(6.56248, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 2.75)(6.875, 3)(6.56248, 2.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 2.75)(6.875, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 2.75)(6.875, 3)(6.56248, 3)
\psline[linewidth=0.03,linecolor=black](6.875, 3)(6.56248, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3)(6.56248, 3.25)(6.56248, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 3)(6.875, 2.75)(7.18748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 0.5)(8.43742, 0.75)(8.125, 0.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.75)(8.125, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 0.75)(8.125, 0.75)(8.125, 0.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.75)(8.125, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 0.75)(8.125, 1)(8.125, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 0.25)(8.43742, 0.5)(8.43742, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 0)(8.125, 0.25)(8.125, 0)
\psline[linewidth=0.03,linecolor=black](8.43742, 0)(8.125, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 0.25)(7.81248, 0)(8.125, 0)
\psline[linewidth=0.03,linecolor=black](7.81248, 0)(8.125, 0)
\psline[linewidth=0.03,linecolor=black](8.125, 0.25)(7.81248, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 0)(8.125, 0.25)(7.81248, 0.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 0.25)(8.125, 0.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 0)(7.81248, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 0)(7.81248, 0.25)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 0.25)(7.5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 0.25)(7.5, 0.5)(7.5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 0.25)(8.125, 0.25)(7.81248, 0.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 0.25)(7.81248, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 0.5)(7.81248, 0.25)(7.81248, 0.5)
\psline[linewidth=0.03,linecolor=black](7.5, 0.5)(7.81248, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 0.75)(7.5, 0.5)(7.81248, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 0)(7.81248, 0)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.5, 0)(7.81248, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 0)(7.5, 0)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 0)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 0)(7.5, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 0.25)(7.18748, 0)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 0.25)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 0.25)(7.18748, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 0)(7.18748, 0.25)(6.875, 0.25)
\psline[linewidth=0.03,linecolor=black](6.875, 0.25)(7.18748, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0.25)(7.18748, 0.25)(6.875, 0.5)
\psline[linewidth=0.03,linecolor=black](6.875, 0.25)(6.875, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 0.25)(6.875, 0.25)(6.875, 0.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 0.25)(6.875, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 0.25)(6.875, 0.5)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 0.25)(6.56248, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 0.25)(6.56248, 0.25)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.25, 0.25)(6.56248, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 0.5)(6.25, 0.25)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.25, 0.5)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.25, 0.25)(6.25, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 0.5)(6.25, 0.25)(6.25, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 0.75)(6.25, 0.5)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.25, 0.75)(6.25, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 0.75)(5.93748, 0.5)(6.25, 0.5)
\psline[linewidth=0.03,linecolor=black](6.25, 0.75)(5.93748, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 0.5)(6.25, 0.75)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 0.5)(5.93748, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.75)(5.93748, 0.5)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](5.625, 0.75)(5.93748, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1)(5.625, 0.75)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](5.625, 1)(5.625, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.75)(5.625, 1)(5.3125, 0.75)
\psline[linewidth=0.03,linecolor=black](5.625, 1)(5.3125, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1)(5.3125, 1)(5.3125, 0.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 0.75)(5.3125, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 0.75)(5.3125, 1)(5, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 0.5)(7.18748, 0.25)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.5, 0.5)(7.18748, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 0.25)(7.5, 0.5)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](7.5, 0.5)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 0.25)(7.18748, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0.5)(7.18748, 0.25)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](6.875, 0.5)(7.18748, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0.75)(6.875, 0.5)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](6.875, 0.5)(6.875, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0.5)(6.875, 0.75)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.875, 0.75)(6.56248, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0.75)(6.56248, 0.75)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 0.75)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.875, 0.75)(6.56248, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0.75)(6.56248, 1)(6.56248, 0.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 1)(6.56248, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 1)(6.25, 0.75)(6.56248, 0.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 1)(6.25, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 1)(6.25, 1)(6.25, 0.75)
\psline[linewidth=0.03,linecolor=black](6.25, 0.75)(6.25, 1)
\psline[linewidth=0.03,linecolor=black](6.56248, 1)(6.25, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1)(6.56248, 1)(6.25, 1.25)
\psline[linewidth=0.03,linecolor=black](6.25, 1)(6.25, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1)(6.25, 1.25)(5.93748, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 0.75)(6.25, 1)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](6.25, 1)(5.93748, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1)(5.93748, 1)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 1)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](6.25, 1)(5.93748, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1)(5.93748, 1.25)(5.93748, 1)
\psline[linewidth=0.03,linecolor=black](5.93748, 1.25)(5.93748, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 1.25)(5.625, 1.25)(5.93748, 1)
\psline[linewidth=0.03,linecolor=black](5.93748, 1.25)(5.625, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.5)(5.625, 1.25)(5.93748, 1.25)
\psline[linewidth=0.03,linecolor=black](5.625, 1.5)(5.625, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.25)(5.625, 1.5)(5.3125, 1.25)
\psline[linewidth=0.03,linecolor=black](5.625, 1.5)(5.3125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.5)(5.3125, 1.5)(5.3125, 1.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.25)(5.3125, 1.5)
\psline[linewidth=0.03,linecolor=black](5.625, 1.5)(5.3125, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.5)(5.3125, 1.75)(5.3125, 1.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.5)(5.3125, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1.5)(5.3125, 1.75)(5, 1.5)
\psline[linewidth=0.03,linecolor=black](5, 1.5)(5.3125, 1.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.5)(5, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1.5)(5, 1.5)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](5, 1.5)(5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 1.5)(4.6875, 1.25)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.25)(5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1.25)(4.6875, 1)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.25)(4.6875, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1)(4.6875, 1.25)(4.375, 1.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 1)(4.375, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 1)(4.6875, 1)(4.375, 1.25)
\psline[linewidth=0.03,linecolor=black](4.375, 1)(4.375, 1.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 1)(4.375, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1)(4.375, 1)(4.375, 0.75)
\psline[linewidth=0.03,linecolor=black](4.375, 1)(4.375, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 1)(4.06252, 0.75)(4.375, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.25)(4.375, 1)(4.375, 1.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.25)(4.375, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.25)(4.06252, 1)(4.375, 1)
\psline[linewidth=0.03,linecolor=black](4.06252, 1)(4.375, 1)
\psline[linewidth=0.03,linecolor=black](4.06252, 1)(4.06252, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1)(4.06252, 1.25)(3.75, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1)(4.06252, 0.75)(4.375, 1)
\psline[linewidth=0.03,linecolor=black](4.06252, 1)(4.06252, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0.75)(4.06252, 1)(3.75, 1)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.75)(3.75, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 0.75)(4.06252, 0.75)(3.75, 1)
\psline[linewidth=0.03,linecolor=black](3.75, 0.75)(3.75, 1)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.75)(3.75, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 0.5)(4.06252, 0.75)(3.75, 0.75)
\psline[linewidth=0.03,linecolor=black](3.75, 0.5)(3.75, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 0.75)(3.75, 0.5)(3.75, 0.75)
\psline[linewidth=0.03,linecolor=black](3.75, 0.5)(3.43752, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 0.5)(3.43752, 0.75)(3.43752, 0.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 0.75)(3.43752, 0.5)
\psline[linewidth=0.03,linecolor=black](3.75, 0.5)(3.43752, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 0.5)(3.43752, 0.5)(3.43752, 0.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 0.5)(3.43752, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 0.5)(3.125, 0.25)(3.43752, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 0.75)(3.125, 0.5)(3.43752, 0.5)
\psline[linewidth=0.03,linecolor=black](3.125, 0.5)(3.43752, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 0.5)(3.125, 0.25)(3.43752, 0.5)
\psline[linewidth=0.03,linecolor=black](3.125, 0.5)(3.125, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 0.25)(3.125, 0.5)(2.81252, 0.5)
\psline[linewidth=0.03,linecolor=black](3.125, 0.25)(2.81252, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.81252, 0.25)(3.125, 0.25)(2.81252, 0.5)
\psline[linewidth=0.03,linecolor=black](3.125, 0.25)(2.81252, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.81252, 0)(3.125, 0.25)(2.81252, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 1)(3.75, 0.75)(3.75, 1)
\psline[linewidth=0.03,linecolor=black](3.43752, 1)(3.75, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 1)(3.43752, 0.75)(3.75, 0.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 1)(3.43752, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 0.75)(3.43752, 1)(3.125, 0.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 0.75)(3.125, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 0.75)(3.125, 0.75)(3.125, 0.5)
\psline[linewidth=0.03,linecolor=black](3.125, 0.5)(3.125, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 0.5)(3.125, 0.75)(2.81252, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 1.5)(5.3125, 1.75)(5, 1.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.75)(5, 1.75)
\psline[linewidth=0.03,linecolor=black](5, 1.5)(5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1.75)(5, 1.5)(5, 1.75)
\psline[linewidth=0.03,linecolor=black](5, 1.5)(4.6875, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 1.5)(4.6875, 1.75)(4.6875, 1.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.75)(4.6875, 1.5)
\psline[linewidth=0.03,linecolor=black](5, 1.5)(4.6875, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1.25)(5, 1.5)(4.6875, 1.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.25)(4.6875, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 1.5)(4.6875, 1.25)(4.6875, 1.5)
\psline[linewidth=0.03,linecolor=black](4.375, 1.5)(4.6875, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1.25)(4.375, 1.5)(4.375, 1.25)
\psline[linewidth=0.03,linecolor=black](4.375, 1.5)(4.375, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 1.5)(4.06252, 1.25)(4.375, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1.75)(4.375, 1.5)(4.6875, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1.75)(5, 2)(5, 1.75)
\psline[linewidth=0.03,linecolor=black](5, 2)(5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 2)(4.6875, 2)(5, 1.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 2)(5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 2)(4.6875, 1.75)(5, 1.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 2)(4.6875, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1.75)(4.6875, 2)(4.375, 1.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.75)(4.375, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 1.5)(4.6875, 1.75)(4.375, 1.75)
\psline[linewidth=0.03,linecolor=black](4.375, 1.5)(4.375, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.75)(4.375, 1.5)(4.375, 1.75)
\psline[linewidth=0.03,linecolor=black](4.375, 1.5)(4.06252, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.5)(4.375, 1.5)(4.06252, 1.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.5)(4.06252, 1.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.5)(4.375, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.25)(4.375, 1.5)(4.06252, 1.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.25)(4.06252, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.25)(4.06252, 1.5)(3.75, 1.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.25)(3.75, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 1.25)(4.06252, 1.25)(3.75, 1.5)
\psline[linewidth=0.03,linecolor=black](3.75, 1.25)(3.75, 1.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.25)(3.75, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.25)(3.75, 1.25)(3.75, 1)
\psline[linewidth=0.03,linecolor=black](3.75, 1.25)(3.75, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 1.25)(3.43752, 1)(3.75, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 1.5)(3.75, 1.25)(3.75, 1.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.5)(3.75, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 1.5)(3.43752, 1.25)(3.75, 1.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.25)(3.75, 1.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.5)(3.43752, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 1.25)(3.43752, 1.5)(3.125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 1.25)(3.43752, 1)(3.75, 1.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.25)(3.43752, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 1)(3.43752, 1.25)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 1)(3.125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 1)(3.43752, 1)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](3.125, 1)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 1)(3.125, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 0.75)(3.43752, 1)(3.125, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.81252, 1)(3.125, 1)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1)(3.125, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.81252, 1)(3.125, 0.75)(3.125, 1)
\psline[linewidth=0.03,linecolor=black](3.125, 0.75)(2.81252, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 0.75)(2.81252, 1)(2.81252, 0.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 1)(2.81252, 0.75)
\psline[linewidth=0.03,linecolor=black](3.125, 0.75)(2.81252, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 0.75)(2.81252, 0.75)(2.81252, 0.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 0.75)(2.81252, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.81252, 0.75)(2.5, 0.5)(2.81252, 0.5)
\psline[linewidth=0.03,linecolor=black](2.5, 0.5)(2.81252, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.5, 0.5)(2.81252, 0.25)(2.81252, 0.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 0.25)(2.5, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.81252, 0.25)(2.5, 0.5)(2.5, 0.25)
\psline[linewidth=0.03,linecolor=black](2.5, 0.5)(2.5, 0.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 0.25)(2.5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.81252, 0)(2.81252, 0.25)(2.5, 0.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 0)(2.5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.5, 0)(2.81252, 0)(2.5, 0.25)
\psline[linewidth=0.03,linecolor=black](2.5, 0)(2.5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.18752, 0)(2.5, 0)(2.5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.5, 0.5)(2.18752, 0.25)(2.5, 0.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 0.25)(2.5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.18752, 0.25)(2.18752, 0)(2.5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.81252, 1)(2.5, 0.75)(2.81252, 0.75)
\psline[linewidth=0.03,linecolor=black](2.5, 0.75)(2.81252, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](2.5, 0.75)(2.5, 0.5)(2.81252, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.5)(4.06252, 1.75)(3.75, 1.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.5)(3.75, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.5)(3.75, 1.75)(3.75, 1.5)
\psline[linewidth=0.03,linecolor=black](3.75, 1.75)(3.75, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 1.75)(3.43752, 1.5)(3.75, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1.25)(5.3125, 1.5)(5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 1)(5.625, 1)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 1)(5.625, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.25)(5.625, 1)(5.93748, 1)
\psline[linewidth=0.03,linecolor=black](5.625, 1)(5.625, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1)(5.625, 1.25)(5.3125, 1)
\psline[linewidth=0.03,linecolor=black](5.3125, 1)(5.625, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1)(5.625, 1.25)(5.3125, 1.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 1)(5.3125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1)(5.3125, 1.25)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 1)(5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 1)(5.3125, 1)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](5, 1)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](5, 1)(5.3125, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 0.75)(5.3125, 1)(5, 1)
\psline[linewidth=0.03,linecolor=black](5, 0.75)(5, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1)(5, 0.75)(5, 1)
\psline[linewidth=0.03,linecolor=black](4.6875, 1)(5, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1)(4.6875, 0.75)(5, 0.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 1)(4.6875, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0.75)(4.6875, 1)(4.375, 0.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.75)(4.375, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 0.5)(4.6875, 0.75)(4.375, 0.75)
\psline[linewidth=0.03,linecolor=black](4.375, 0.5)(4.375, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0.75)(4.375, 0.5)(4.375, 0.75)
\psline[linewidth=0.03,linecolor=black](4.375, 0.5)(4.06252, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 0.5)(4.06252, 0.75)(4.06252, 0.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.75)(4.06252, 0.5)
\psline[linewidth=0.03,linecolor=black](4.375, 0.5)(4.06252, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0.25)(4.375, 0.5)(4.06252, 0.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.25)(4.06252, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 0.5)(4.06252, 0.25)(4.06252, 0.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.25)(3.75, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0.25)(3.75, 0.5)(3.75, 0.25)
\psline[linewidth=0.03,linecolor=black](3.75, 0.5)(3.75, 0.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.25)(3.75, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0.25)(3.75, 0.25)(3.75, 0)
\psline[linewidth=0.03,linecolor=black](3.75, 0.25)(3.75, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 0.25)(3.43752, 0)(3.75, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.75, 0.25)(3.75, 0.5)(3.43752, 0.25)
\psline[linewidth=0.03,linecolor=black](3.75, 0.25)(3.43752, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 0)(3.75, 0.25)(3.43752, 0.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 0)(3.43752, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 0.25)(3.43752, 0)(3.43752, 0.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 0)(3.125, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.43752, 0)(3.125, 0.25)(3.125, 0)
\psline[linewidth=0.03,linecolor=black](3.125, 0.25)(3.125, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](3.125, 0.25)(2.81252, 0)(3.125, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0.75)(3.75, 0.5)(4.06252, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 1)(5, 1)(5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 0.75)(6.25, 0.75)(6.56248, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 0.5)(7.5, 0.75)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](7.5, 0.75)(7.18748, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 0.75)(7.18748, 0.75)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 0.75)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 0.75)(7.5, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 0.75)(7.5, 0.75)(7.18748, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 0.75)(6.875, 0.75)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](6.875, 0.75)(7.18748, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0.75)(7.18748, 0.75)(7.18748, 1)
\psline[linewidth=0.03,linecolor=black](6.875, 0.75)(7.18748, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1)(6.875, 0.75)(7.18748, 1)
\psline[linewidth=0.03,linecolor=black](6.875, 1)(7.18748, 1)
\psline[linewidth=0.03,linecolor=black](6.875, 0.75)(6.875, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0.75)(6.875, 1)(6.56248, 1)
\psline[linewidth=0.03,linecolor=black](6.56248, 1)(6.875, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 1)(6.875, 1)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 1)(6.56248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1.25)(6.56248, 1)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](6.25, 1.25)(6.56248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1.5)(6.25, 1.25)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](6.25, 1.25)(6.25, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1.25)(6.25, 1.5)(5.93748, 1.25)
\psline[linewidth=0.03,linecolor=black](6.25, 1.5)(5.93748, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 1.25)(6.25, 1.5)(5.93748, 1.5)
\psline[linewidth=0.03,linecolor=black](6.25, 1.5)(5.93748, 1.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 1.25)(5.93748, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.5)(5.93748, 1.25)(5.93748, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1.5)(5.93748, 1.75)(5.93748, 1.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 1.75)(5.93748, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 1.75)(5.625, 1.5)(5.93748, 1.5)
\psline[linewidth=0.03,linecolor=black](5.625, 1.5)(5.93748, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.75)(5.625, 1.5)(5.93748, 1.75)
\psline[linewidth=0.03,linecolor=black](5.625, 1.75)(5.625, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1.75)(5.625, 1.5)(5.625, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1)(7.18748, 1)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](6.875, 1)(7.18748, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1.25)(6.875, 1)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](6.875, 1.25)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](6.875, 1.25)(6.875, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1)(6.875, 1.25)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](6.875, 1.25)(6.56248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1.25)(6.875, 1.5)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](6.875, 1.5)(6.56248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1.5)(6.56248, 1.5)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 1.5)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 1.5)(6.875, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 1.5)(6.875, 1.5)(6.56248, 1.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 1.5)(6.56248, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1.5)(6.56248, 1.5)(6.56248, 1.75)
\psline[linewidth=0.03,linecolor=black](6.25, 1.5)(6.56248, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1.5)(6.56248, 1.75)(6.25, 1.75)
\psline[linewidth=0.03,linecolor=black](6.25, 1.75)(6.56248, 1.75)
\psline[linewidth=0.03,linecolor=black](6.25, 1.5)(6.25, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 1.75)(6.25, 1.5)(6.25, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 1.75)(6.56248, 1.75)(6.25, 2)
\psline[linewidth=0.03,linecolor=black](6.25, 1.75)(6.25, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 1.75)(6.25, 1.75)(6.25, 2)
\psline[linewidth=0.03,linecolor=black](5.93748, 1.75)(6.25, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 2)(5.93748, 1.75)(6.25, 2)
\psline[linewidth=0.03,linecolor=black](5.93748, 2)(6.25, 2)
\psline[linewidth=0.03,linecolor=black](5.93748, 2)(5.93748, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.75)(5.93748, 1.75)(5.93748, 2)
\psline[linewidth=0.03,linecolor=black](5.625, 1.75)(5.93748, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 1.75)(5.93748, 2)(5.625, 2)
\psline[linewidth=0.03,linecolor=black](5.93748, 2)(5.625, 2)
\psline[linewidth=0.03,linecolor=black](5.625, 1.75)(5.625, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1.75)(5.625, 1.75)(5.625, 2)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.75)(5.625, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 2)(5.3125, 1.75)(5.625, 2)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.75)(5.3125, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 1.75)(5.3125, 2)(5, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 2)(5.625, 2.25)(5.625, 2)
\psline[linewidth=0.03,linecolor=black](5.625, 2.25)(5.625, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 2.25)(5.3125, 2)(5.625, 2)
\psline[linewidth=0.03,linecolor=black](5.625, 2.25)(5.3125, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 2.25)(5.3125, 2.25)(5.3125, 2)
\psline[linewidth=0.03,linecolor=black](5.3125, 2)(5.3125, 2.25)
\psline[linewidth=0.03,linecolor=black](5.625, 2.25)(5.3125, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 2.25)(5.625, 2.25)(5.3125, 2.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.25)(5.3125, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 2.25)(5.3125, 2.5)(5, 2.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.5)(5, 2.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.25)(5, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 2.25)(5.3125, 2.25)(5, 2.5)
\psline[linewidth=0.03,linecolor=black](5, 2.25)(5, 2.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.25)(5, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 2.25)(5, 2.25)(5, 2)
\psline[linewidth=0.03,linecolor=black](5, 2.25)(5, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 2.25)(4.6875, 2)(5, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 2.5)(5, 2.25)(5, 2.5)
\psline[linewidth=0.03,linecolor=black](5, 2.25)(4.6875, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 2.25)(4.6875, 2.5)(4.6875, 2.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 2.5)(4.6875, 2.25)
\psline[linewidth=0.03,linecolor=black](5, 2.25)(4.6875, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 2)(5, 2.25)(4.6875, 2.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 2)(4.6875, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 2.25)(4.6875, 2)(4.6875, 2.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 2)(4.375, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 2)(4.375, 2.25)(4.375, 2)
\psline[linewidth=0.03,linecolor=black](4.375, 2.25)(4.375, 2)
\psline[linewidth=0.03,linecolor=black](4.6875, 2)(4.375, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 1.75)(4.6875, 2)(4.375, 2)
\psline[linewidth=0.03,linecolor=black](4.375, 1.75)(4.375, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 2)(4.375, 1.75)(4.375, 2)
\psline[linewidth=0.03,linecolor=black](4.06252, 2)(4.375, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 2)(4.06252, 1.75)(4.375, 1.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.75)(4.06252, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 1.75)(4.06252, 2)(3.75, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 2.25)(4.06252, 2)(4.375, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 2.5)(4.375, 2.5)(4.6875, 2.25)
\psline[linewidth=0.03,linecolor=black](4.375, 2.5)(4.6875, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 2.5)(4.375, 2.25)(4.6875, 2.25)
\psline[linewidth=0.03,linecolor=black](4.375, 2.25)(4.375, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 2.25)(4.375, 2.5)(4.06252, 2.25)
\psline[linewidth=0.03,linecolor=black](4.375, 2.25)(4.06252, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 2)(4.375, 2.25)(4.06252, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 2.5)(5, 2.75)(5, 2.5)
\psline[linewidth=0.03,linecolor=black](5, 2.75)(5, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 2.75)(4.6875, 2.5)(5, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 2)(5.3125, 2.25)(5, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.25)(5.93748, 2)(6.25, 2)
\psline[linewidth=0.03,linecolor=black](6.25, 2.25)(5.93748, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.25)(5.93748, 2.25)(5.93748, 2)
\psline[linewidth=0.03,linecolor=black](5.93748, 2.25)(5.93748, 2)
\psline[linewidth=0.03,linecolor=black](6.25, 2.25)(5.93748, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.25)(6.25, 2.5)(5.93748, 2.25)
\psline[linewidth=0.03,linecolor=black](6.25, 2.5)(5.93748, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 2.5)(5.93748, 2.5)(5.93748, 2.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 2.5)(5.93748, 2.25)
\psline[linewidth=0.03,linecolor=black](6.25, 2.5)(5.93748, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 2.5)(6.25, 2.5)(5.93748, 2.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 2.5)(5.93748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 2.75)(5.93748, 2.5)(5.93748, 2.75)
\psline[linewidth=0.03,linecolor=black](5.625, 2.75)(5.93748, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3)(5.625, 2.75)(5.93748, 2.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 3)(5.625, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 2.75)(5.93748, 3)(5.625, 3)
\psline[linewidth=0.03,linecolor=black](5.93748, 3)(5.625, 3)
\psline[linewidth=0.03,linecolor=black](5.625, 2.75)(5.625, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 3)(5.625, 2.75)(5.625, 3)
\psline[linewidth=0.03,linecolor=black](5.3125, 3)(5.625, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 3.25)(5.3125, 3)(5.625, 3)
\psline[linewidth=0.03,linecolor=black](5.3125, 3.25)(5.625, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 3.25)(5.3125, 3.25)(5.625, 3)
\psline[linewidth=0.03,linecolor=black](5.625, 3.25)(5.3125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 3.5)(5.3125, 3.25)(5.625, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3)(5.625, 3.25)(5.625, 3)
\psline[linewidth=0.03,linecolor=black](5.93748, 3)(5.625, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3)(5.93748, 3.25)(5.625, 3.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 3.25)(5.625, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3.25)(5.625, 3.5)(5.625, 3.25)
\psline[linewidth=0.03,linecolor=black](5.625, 3.5)(5.93748, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3.5)(5.625, 3.5)(5.93748, 3.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 3.5)(5.93748, 3.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 3.5)(5.625, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3.75)(5.625, 3.5)(5.93748, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 3.5)(5.93748, 3.5)(5.93748, 3.25)
\psline[linewidth=0.03,linecolor=black](6.25, 3.5)(5.93748, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 3.5)(5.93748, 3.75)(5.93748, 3.5)
\psline[linewidth=0.03,linecolor=black](6.25, 3.5)(5.93748, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 3.75)(6.25, 3.5)(6.25, 3.75)
\psline[linewidth=0.03,linecolor=black](6.25, 3.5)(6.25, 3.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 3.75)(6.25, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 4)(5.93748, 3.75)(6.25, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 3.5)(6.56248, 3.75)(6.25, 3.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.75)(6.25, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 3.75)(6.25, 4)(6.25, 3.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.75)(6.25, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 4)(6.25, 4)(6.56248, 3.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 4)(6.25, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 4)(6.56248, 4)(6.56248, 4.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 4)(6.56248, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 4)(6.875, 4.25)(6.56248, 4.25)
\psline[linewidth=0.03,linecolor=black](6.875, 4.25)(6.56248, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 4.25)(6.875, 4.5)(6.56248, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 2.5)(5.625, 2.25)(5.93748, 2.25)
\psline[linewidth=0.03,linecolor=black](5.625, 2.25)(5.93748, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 2.25)(5.93748, 2.5)(5.625, 2.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 2.5)(5.625, 2.5)
\psline[linewidth=0.03,linecolor=black](5.625, 2.25)(5.625, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 2.5)(5.625, 2.25)(5.625, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 2.5)(5.625, 2.75)(5.625, 2.5)
\psline[linewidth=0.03,linecolor=black](5.625, 2.75)(5.625, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 2.75)(5.3125, 2.5)(5.625, 2.5)
\psline[linewidth=0.03,linecolor=black](5.625, 2.75)(5.3125, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 2.75)(5.3125, 2.75)(5.3125, 2.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.75)(5.3125, 2.5)
\psline[linewidth=0.03,linecolor=black](5.625, 2.75)(5.3125, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 2.75)(5.3125, 3)(5.3125, 2.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 3)(5.3125, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 3)(5, 2.75)(5.3125, 2.75)
\psline[linewidth=0.03,linecolor=black](5, 2.75)(5.3125, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 2.75)(5.3125, 3)(5, 3)
\psline[linewidth=0.03,linecolor=black](5.3125, 3)(5, 3)
\psline[linewidth=0.03,linecolor=black](5, 2.75)(5, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 3)(5, 2.75)(5, 3)
\psline[linewidth=0.03,linecolor=black](5, 2.75)(4.6875, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 2.75)(4.6875, 3)(4.6875, 2.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 3)(4.6875, 2.75)
\psline[linewidth=0.03,linecolor=black](5, 2.75)(4.6875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 2.5)(5, 2.75)(4.6875, 2.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 2.5)(4.6875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 2.5)(4.6875, 2.5)(4.6875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 3)(4.375, 2.75)(4.6875, 2.75)
\psline[linewidth=0.03,linecolor=black](4.375, 2.75)(4.6875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 2.75)(4.375, 2.5)(4.6875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 3)(5.3125, 3.25)(5, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 2.75)(5, 2.75)(5.3125, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 2.25)(5.625, 2.25)(5.93748, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 1.5)(6.25, 1.5)(6.56248, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 1.5)(6.875, 1.25)(7.18748, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.875, 0)(7.18748, 0)(6.875, 0.25)
\psline[linewidth=0.03,linecolor=black](6.875, 0)(6.875, 0.25)
\psline[linewidth=0.03,linecolor=black](6.875, 0)(7.18748, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 0)(6.875, 0)(6.875, 0.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 0)(6.875, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 0.25)(6.56248, 0)(6.875, 0.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 0)(6.56248, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 0.25)(6.56248, 0)(6.56248, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.56248, 0)(6.25, 0.25)(6.25, 0)
\psline[linewidth=0.03,linecolor=black](6.25, 0.25)(6.25, 0)
\psline[linewidth=0.03,linecolor=black](6.56248, 0)(6.25, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](6.25, 0.25)(5.93748, 0)(6.25, 0)
\psline[linewidth=0.03,linecolor=black](6.25, 0.25)(5.93748, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 0)(6.25, 0.25)(5.93748, 0.25)
\psline[linewidth=0.03,linecolor=black](6.25, 0.25)(5.93748, 0.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 0)(5.93748, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.25)(5.93748, 0)(5.93748, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 0.25)(6.25, 0.25)(5.93748, 0.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 0.25)(5.93748, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.25)(5.93748, 0.25)(5.93748, 0.5)
\psline[linewidth=0.03,linecolor=black](5.625, 0.25)(5.93748, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.25)(5.93748, 0.5)(5.625, 0.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 0.5)(5.625, 0.5)
\psline[linewidth=0.03,linecolor=black](5.625, 0.25)(5.625, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 0.5)(5.625, 0.25)(5.625, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 0.5)(5.625, 0.75)(5.625, 0.5)
\psline[linewidth=0.03,linecolor=black](5.625, 0.75)(5.625, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.75)(5.3125, 0.5)(5.625, 0.5)
\psline[linewidth=0.03,linecolor=black](5.625, 0.75)(5.3125, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.75)(5.3125, 0.75)(5.3125, 0.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 0.5)(5.3125, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 0.5)(5.3125, 0.75)(5, 0.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 0.75)(5, 0.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 0.5)(5, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 0.25)(5.3125, 0.5)(5, 0.5)
\psline[linewidth=0.03,linecolor=black](5, 0.25)(5, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0.5)(5, 0.25)(5, 0.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.5)(5, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0.5)(4.6875, 0.25)(5, 0.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.25)(5, 0.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.5)(4.6875, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0.5)(4.375, 0.5)(4.6875, 0.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.25)(4.375, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0.25)(4.375, 0.5)(4.375, 0.25)
\psline[linewidth=0.03,linecolor=black](4.375, 0.5)(4.375, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 0.5)(4.06252, 0.25)(4.375, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0.25)(4.6875, 0)(5, 0.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.25)(4.6875, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0)(4.6875, 0.25)(4.375, 0.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 0)(4.375, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.375, 0)(4.6875, 0)(4.375, 0.25)
\psline[linewidth=0.03,linecolor=black](4.375, 0)(4.375, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0.25)(4.375, 0)(4.375, 0.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.25)(4.375, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0.25)(4.06252, 0)(4.375, 0)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.25)(4.06252, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.06252, 0)(4.06252, 0.25)(3.75, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 0.75)(5, 0.75)(5, 0.5)
\psline[linewidth=0.03,linecolor=black](5, 0.75)(5, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 0.75)(4.6875, 0.75)(5, 0.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.75)(5, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0.75)(4.6875, 0.5)(5, 0.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.75)(4.6875, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](4.6875, 0.75)(4.375, 0.5)(4.6875, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.93748, 0)(5.625, 0.25)(5.625, 0)
\psline[linewidth=0.03,linecolor=black](5.625, 0.25)(5.625, 0)
\psline[linewidth=0.03,linecolor=black](5.93748, 0)(5.625, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.25)(5.3125, 0)(5.625, 0)
\psline[linewidth=0.03,linecolor=black](5.625, 0.25)(5.3125, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 0)(5.625, 0.25)(5.3125, 0.25)
\psline[linewidth=0.03,linecolor=black](5.625, 0.25)(5.3125, 0.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 0)(5.3125, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 0.25)(5.3125, 0)(5.3125, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.625, 0.25)(5.3125, 0.5)(5.3125, 0.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 0.5)(5.3125, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 0.5)(5, 0.25)(5.3125, 0.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5.3125, 0)(5, 0.25)(5, 0)
\psline[linewidth=0.03,linecolor=black](5, 0.25)(5, 0)
\psline[linewidth=0.03,linecolor=black](5.3125, 0)(5, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](5, 0.25)(4.6875, 0)(5, 0)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 0.5)(10, 0.25)(10, 0.5)
\psline[linewidth=0.03,linecolor=black](10, 0.25)(10, 0.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.5)(10, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 0.75)(9.68742, 0.5)(10, 0.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 0.75)(9.68742, 0.75)(10, 0.5)
\psline[linewidth=0.03,linecolor=black](10, 0.75)(10, 0.5)
\psline[linewidth=0.03,linecolor=black](10, 0.75)(9.68742, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1)(9.68742, 0.75)(10, 0.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 1)(9.68742, 0.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1)(9.37484, 1)(9.68742, 0.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 1)(9.37484, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 1)(9.68742, 1)(9.68742, 1.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 1)(9.68742, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 1)(9.68742, 1.25)(9.37484, 1.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 1.25)(9.68742, 1.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 1)(9.37484, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.25)(9.37484, 1)(9.37484, 1.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.25)(9.37484, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.5)(9.06258, 1.25)(9.37484, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 1.25)(9.68742, 1.25)(9.37484, 1.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 1.25)(9.37484, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.5)(9.37484, 1.25)(9.37484, 1.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.5)(9.37484, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 1.75)(9.06258, 1.5)(9.37484, 1.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 1.75)(9.06258, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.75)(9.06258, 1.5)(9.37484, 1.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.75)(9.37484, 1.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.75)(9.06258, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.5)(9.06258, 1.75)(8.75, 1.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.75)(8.75, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 1.75)(9.06258, 2)(8.75, 1.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 2)(8.75, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 2)(8.75, 2)(8.75, 1.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 2)(8.75, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2)(9.06258, 2)(8.75, 2.25)
\psline[linewidth=0.03,linecolor=black](8.75, 2)(8.75, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.25)(8.75, 2)(8.75, 2.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.25)(8.75, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2.5)(8.43742, 2.25)(8.75, 2.25)
\psline[linewidth=0.03,linecolor=black](8.75, 2.5)(8.43742, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2.5)(8.43742, 2.5)(8.43742, 2.25)
\psline[linewidth=0.03,linecolor=black](8.75, 2.5)(8.43742, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2.5)(8.43742, 2.75)(8.43742, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2)(9.06258, 1.75)(9.37484, 1.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 2)(9.06258, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2)(9.06258, 2)(9.06258, 1.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 2)(9.06258, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 2)(9.37484, 2)(9.06258, 2.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 2)(9.06258, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 2)(9.06258, 2.25)(8.75, 2.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 2.25)(8.75, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 2.25)(8.75, 2.5)(8.75, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 1)(9.68742, 1)(10, 0.75)
\psline[linewidth=0.03,linecolor=black](10, 1)(10, 0.75)
\psline[linewidth=0.03,linecolor=black](10, 1)(9.68742, 1)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1)(10, 1)(10, 1.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 1)(10, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1.25)(9.68742, 1)(10, 1.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.25)(10, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 1.5)(9.68742, 1.25)(10, 1.25)
\psline[linewidth=0.03,linecolor=black](10, 1.5)(9.68742, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1.5)(9.68742, 1.25)(10, 1.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.5)(10, 1.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.5)(9.68742, 1.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1.25)(9.68742, 1.5)(9.37484, 1.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.5)(9.37484, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1.5)(9.68742, 1.75)(9.37484, 1.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.75)(9.37484, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1.75)(9.37484, 1.75)(9.37484, 1.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.75)(9.37484, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1.75)(9.37484, 2)(9.37484, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1.75)(9.68742, 1.5)(10, 1.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 1.75)(10, 1.5)(10, 1.75)
\psline[linewidth=0.03,linecolor=black](10, 1.5)(10, 1.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.75)(10, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 2)(9.68742, 1.75)(10, 1.75)
\psline[linewidth=0.03,linecolor=black](10, 2)(9.68742, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 2)(9.68742, 1.75)(10, 2)
\psline[linewidth=0.03,linecolor=black](9.68742, 2)(10, 2)
\psline[linewidth=0.03,linecolor=black](9.68742, 2)(9.68742, 1.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2)(9.68742, 1.75)(9.68742, 2)
\psline[linewidth=0.03,linecolor=black](9.37484, 2)(9.68742, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 2.25)(9.37484, 2)(9.68742, 2)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.25)(9.37484, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2.25)(9.37484, 2)(9.68742, 2.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.25)(9.68742, 2.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.25)(9.37484, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2)(9.37484, 2.25)(9.06258, 2.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 2.25)(9.37484, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 2.25)(9.37484, 2.25)(9.06258, 2.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 2.25)(9.06258, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2.5)(9.06258, 2.25)(9.06258, 2.5)
\psline[linewidth=0.03,linecolor=black](8.75, 2.5)(9.06258, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 2.75)(8.75, 2.5)(9.06258, 2.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 2.75)(8.75, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2.75)(8.75, 2.5)(9.06258, 2.75)
\psline[linewidth=0.03,linecolor=black](8.75, 2.75)(9.06258, 2.75)
\psline[linewidth=0.03,linecolor=black](8.75, 2.75)(8.75, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.75)(8.75, 2.5)(8.75, 2.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.75)(8.75, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.75)(8.75, 2.75)(8.75, 3)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.75)(8.75, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 2.75)(8.75, 3)(8.43742, 3)
\psline[linewidth=0.03,linecolor=black](8.75, 3)(8.43742, 3)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.75)(8.43742, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 3)(8.43742, 2.75)(8.43742, 3)
\psline[linewidth=0.03,linecolor=black](8.125, 3)(8.43742, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.25)(8.125, 3)(8.43742, 3)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.25)(8.125, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 3)(8.43742, 3.25)(8.125, 3.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.25)(8.125, 3.25)
\psline[linewidth=0.03,linecolor=black](8.125, 3)(8.125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3.25)(8.125, 3)(8.125, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.25)(8.125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3.5)(7.81248, 3.25)(8.125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.25)(8.43742, 3.5)(8.125, 3.25)
\psline[linewidth=0.03,linecolor=black](8.125, 3.25)(8.43742, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 3.25)(8.43742, 3.5)(8.125, 3.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.5)(8.125, 3.5)
\psline[linewidth=0.03,linecolor=black](8.125, 3.25)(8.125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3.5)(8.125, 3.25)(8.125, 3.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.5)(8.125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 3.75)(7.81248, 3.5)(8.125, 3.5)
\psline[linewidth=0.03,linecolor=black](8.125, 3.75)(7.81248, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 3.75)(7.81248, 3.5)(8.125, 3.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.75)(8.125, 3.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.75)(7.81248, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 3.75)(7.81248, 3.5)(7.81248, 3.75)
\psline[linewidth=0.03,linecolor=black](7.5, 3.75)(7.81248, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4)(7.5, 3.75)(7.81248, 3.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 4)(7.5, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 3.75)(7.81248, 4)(7.5, 4)
\psline[linewidth=0.03,linecolor=black](7.5, 4)(7.81248, 4)
\psline[linewidth=0.03,linecolor=black](7.5, 3.75)(7.5, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4)(7.5, 3.75)(7.5, 4)
\psline[linewidth=0.03,linecolor=black](7.18748, 4)(7.5, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4)(7.5, 4)(7.5, 4.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 4)(7.5, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4)(7.5, 4.25)(7.18748, 4.25)
\psline[linewidth=0.03,linecolor=black](7.5, 4.25)(7.18748, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 4.25)(7.18748, 4.5)(7.18748, 4.25)
\psline[linewidth=0.03,linecolor=black](7.5, 4.25)(7.18748, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4.5)(7.5, 4.25)(7.5, 4.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.5)(7.5, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.18748, 4.75)(7.18748, 4.5)(7.5, 4.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.75)(7.5, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 4.75)(7.18748, 4.75)(7.5, 4.5)
\psline[linewidth=0.03,linecolor=black](7.5, 4.75)(7.18748, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 5)(7.18748, 4.75)(7.5, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 4)(7.81248, 4)(7.5, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4)(7.81248, 3.75)(8.125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.5)(8.43742, 3.75)(8.125, 3.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.75)(8.125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.75)(8.125, 3.75)(8.125, 3.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.75)(8.125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.75)(8.125, 4)(8.125, 3.75)
\psline[linewidth=0.03,linecolor=black](8.125, 4)(8.125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 4)(7.81248, 4)(8.125, 3.75)
\psline[linewidth=0.03,linecolor=black](8.125, 4)(7.81248, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4)(8.125, 4)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 4)(8.125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4.25)(7.81248, 4)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.25)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.25)(7.81248, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 4.25)(7.81248, 4)(7.81248, 4.25)
\psline[linewidth=0.03,linecolor=black](7.5, 4.25)(7.81248, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4.5)(7.5, 4.25)(7.81248, 4.25)
\psline[linewidth=0.03,linecolor=black](7.5, 4.25)(7.81248, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 4.25)(7.81248, 4.5)(7.5, 4.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.5)(7.5, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4.5)(7.81248, 4.75)(7.5, 4.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.75)(7.5, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4.75)(7.5, 4.75)(7.5, 4.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.75)(7.5, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4.75)(7.5, 5)(7.5, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4.5)(7.81248, 4.25)(8.125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 3)(8.43742, 3.25)(8.43742, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2.75)(9.06258, 2.75)(9.06258, 3)
\psline[linewidth=0.03,linecolor=black](8.75, 2.75)(9.06258, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 2.75)(9.06258, 3)(8.75, 3)
\psline[linewidth=0.03,linecolor=black](8.75, 3)(9.06258, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 3)(9.06258, 3)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](8.75, 3)(8.75, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.25)(8.75, 3)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.25)(8.75, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.5)(8.43742, 3.25)(8.75, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2.25)(9.68742, 2.25)(9.68742, 2.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.25)(9.68742, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2.5)(9.37484, 2.25)(9.68742, 2.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.5)(9.68742, 2.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.25)(9.37484, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2.25)(9.37484, 2.5)(9.06258, 2.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.5)(9.06258, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2.5)(9.37484, 2.75)(9.06258, 2.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.75)(9.06258, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2.75)(9.06258, 2.75)(9.06258, 2.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.75)(9.06258, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 2.75)(9.37484, 2.75)(9.06258, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2.75)(9.37484, 2.5)(9.68742, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 2.25)(9.68742, 2)(10, 2)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 2.25)(10, 2)(10, 2.25)
\psline[linewidth=0.03,linecolor=black](10, 2)(10, 2.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.25)(10, 2.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 2.25)(10, 2.25)(10, 2.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.25)(10, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 2.5)(9.68742, 2.25)(10, 2.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.5)(10, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 2.75)(9.68742, 2.5)(10, 2.5)
\psline[linewidth=0.03,linecolor=black](10, 2.75)(9.68742, 2.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 2.75)(9.68742, 2.75)(9.68742, 2.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.75)(9.68742, 2.5)
\psline[linewidth=0.03,linecolor=black](10, 2.75)(9.68742, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 2.75)(9.68742, 3)(9.68742, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 2.75)(9.37484, 2.75)(9.68742, 2.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.75)(9.37484, 2.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3)(9.37484, 2.75)(9.68742, 2.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.75)(9.68742, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 2.75)(9.68742, 3)(9.37484, 3)
\psline[linewidth=0.03,linecolor=black](9.68742, 3)(9.37484, 3)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.75)(9.37484, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3)(9.37484, 2.75)(9.37484, 3)
\psline[linewidth=0.03,linecolor=black](9.06258, 3)(9.37484, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 3.25)(9.06258, 3)(9.37484, 3)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.25)(9.06258, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3.25)(9.06258, 3)(9.37484, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.25)(9.37484, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.25)(9.06258, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3)(9.06258, 3.25)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.25)(8.75, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3.25)(9.06258, 3.5)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.5)(8.75, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3.5)(8.75, 3.5)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](8.75, 3.5)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.5)(8.75, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 3.5)(9.06258, 3.5)(8.75, 3.75)
\psline[linewidth=0.03,linecolor=black](8.75, 3.5)(8.75, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.75)(8.75, 3.5)(8.75, 3.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.75)(8.75, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4)(8.43742, 3.75)(8.75, 3.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.75)(8.75, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.75)(8.75, 4)(8.43742, 4)
\psline[linewidth=0.03,linecolor=black](8.75, 4)(8.43742, 4)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.75)(8.43742, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.75)(8.43742, 4)(8.125, 4)
\psline[linewidth=0.03,linecolor=black](8.125, 4)(8.43742, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 4)(8.43742, 4)(8.125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4)(8.75, 4)(8.43742, 4.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 4)(8.43742, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4)(8.43742, 4.25)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.25)(8.125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4.25)(8.43742, 4.5)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.5)(8.125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4.5)(8.125, 4.5)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](8.125, 4.5)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.5)(8.125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4.5)(8.125, 4.75)(8.125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 4.5)(7.81248, 4.5)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](8.125, 4.5)(7.81248, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 4.75)(7.81248, 4.5)(8.125, 4.5)
\psline[linewidth=0.03,linecolor=black](8.125, 4.75)(7.81248, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 4.75)(7.81248, 4.75)(7.81248, 4.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.75)(8.125, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.81248, 4.75)(8.125, 4.75)(7.81248, 5)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.75)(7.81248, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](7.5, 5)(7.81248, 4.75)(7.81248, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 3.5)(8.43742, 3.5)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](8.75, 3.5)(8.43742, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 3.75)(8.43742, 3.5)(8.75, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3.5)(9.06258, 3.25)(9.37484, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3)(9.37484, 3.25)(9.37484, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3)(10, 2.75)(10, 3)
\psline[linewidth=0.03,linecolor=black](10, 2.75)(10, 3)
\psline[linewidth=0.03,linecolor=black](9.68742, 3)(10, 3)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3)(10, 3)(10, 3.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 3)(10, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3.25)(9.68742, 3)(10, 3.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 3.25)(10, 3.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 3)(9.68742, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3)(9.68742, 3.25)(9.37484, 3.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 3.25)(9.37484, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3.25)(9.37484, 3.5)(9.37484, 3.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.5)(9.37484, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 3.5)(9.06258, 3.5)(9.37484, 3.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.5)(9.06258, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 3.75)(9.06258, 3.5)(9.37484, 3.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.75)(9.06258, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3.5)(9.37484, 3.75)(9.06258, 3.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.75)(9.06258, 3.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.5)(9.06258, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3.5)(9.06258, 3.75)(8.75, 3.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.75)(8.75, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 3.75)(9.06258, 4)(8.75, 3.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 4)(8.75, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 4)(8.75, 4)(8.75, 3.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 4)(8.75, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4)(9.06258, 4)(8.75, 4.25)
\psline[linewidth=0.03,linecolor=black](8.75, 4)(8.75, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4.25)(8.75, 4)(8.75, 4.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.25)(8.75, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4.5)(8.43742, 4.25)(8.75, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 3.75)(9.06258, 4)(9.06258, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 3.5)(9.68742, 3.25)(10, 3.25)
\psline[linewidth=0.03,linecolor=black](10, 3.5)(9.68742, 3.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3.25)(10, 3.5)(9.68742, 3.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 3.5)(10, 3.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 3.25)(9.68742, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 3.5)(9.68742, 3.25)(9.68742, 3.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.5)(9.68742, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 3.75)(9.37484, 3.5)(9.68742, 3.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 3.5)(10, 3.5)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 3.5)(9.68742, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 3.75)(9.68742, 3.5)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.75)(9.68742, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 4)(9.37484, 3.75)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 4)(9.37484, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4)(9.37484, 3.75)(9.68742, 4)
\psline[linewidth=0.03,linecolor=black](9.37484, 4)(9.68742, 4)
\psline[linewidth=0.03,linecolor=black](9.37484, 4)(9.37484, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 4)(9.37484, 3.75)(9.37484, 4)
\psline[linewidth=0.03,linecolor=black](9.06258, 4)(9.37484, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 4)(9.37484, 4)(9.37484, 4.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 4)(9.37484, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 4)(9.37484, 4.25)(9.06258, 4.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.25)(9.06258, 4.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 4)(9.06258, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4.25)(9.06258, 4)(9.06258, 4.25)
\psline[linewidth=0.03,linecolor=black](8.75, 4.25)(9.06258, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4.5)(8.75, 4.25)(9.06258, 4.25)
\psline[linewidth=0.03,linecolor=black](8.75, 4.5)(8.75, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4.5)(8.43742, 4.5)(8.75, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4.25)(9.06258, 4.5)(9.06258, 4.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 4.5)(9.06258, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 4.5)(8.75, 4.5)(9.06258, 4.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 4.5)(8.75, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4.75)(8.75, 4.5)(9.06258, 4.5)
\psline[linewidth=0.03,linecolor=black](8.75, 4.75)(8.75, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4.75)(8.43742, 4.5)(8.75, 4.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.5)(8.75, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4.5)(8.75, 4.75)(8.43742, 4.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.75)(8.75, 4.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.5)(8.43742, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 4.75)(8.43742, 4.5)(8.43742, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 4.75)(8.75, 4.75)(8.43742, 5)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.75)(8.43742, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 4.75)(8.43742, 4.75)(8.43742, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 4.75)(8.43742, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 5)(8.125, 4.75)(8.43742, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(8.125, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.125, 4.75)(8.125, 5)(7.81248, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 4.25)(9.37484, 4)(9.68742, 4)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.25)(9.37484, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4.25)(9.37484, 4)(9.68742, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 3.5)(10, 3.75)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](10, 3.75)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](10, 3.5)(10, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 3.75)(10, 4)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](10, 4)(9.68742, 3.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 4)(9.68742, 4)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](10, 4)(9.68742, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 4)(9.68742, 4.25)(9.68742, 4)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 4.25)(10, 4)(10, 4.25)
\psline[linewidth=0.03,linecolor=black](10, 4)(10, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 4.5)(9.68742, 4.25)(10, 4.25)
\psline[linewidth=0.03,linecolor=black](10, 4.5)(10, 4.25)
\psline[linewidth=0.03,linecolor=black](10, 4.5)(9.68742, 4.25)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 4.25)(10, 4.5)(9.68742, 4.5)
\psline[linewidth=0.03,linecolor=black](10, 4.5)(9.68742, 4.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.25)(9.68742, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4.25)(9.68742, 4.25)(9.68742, 4.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.25)(9.68742, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4.5)(9.37484, 4.25)(9.68742, 4.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.25)(9.37484, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4.25)(9.37484, 4.5)(9.06258, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 4.5)(9.68742, 4.75)(9.68742, 4.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.75)(9.68742, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 4.75)(9.37484, 4.5)(9.68742, 4.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.75)(9.37484, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 4.75)(9.37484, 4.75)(9.37484, 4.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.5)(9.37484, 4.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.75)(9.68742, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4.75)(9.68742, 4.75)(9.37484, 5)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.75)(9.37484, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 5)(9.37484, 4.75)(9.37484, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4.5)(9.37484, 4.75)(9.06258, 4.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.75)(9.06258, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.37484, 4.75)(9.06258, 4.75)(9.06258, 4.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 4.75)(9.06258, 4.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 4.75)(9.37484, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 4.75)(9.37484, 4.75)(9.06258, 5)
\psline[linewidth=0.03,linecolor=black](9.06258, 4.75)(9.06258, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4.75)(9.06258, 4.75)(9.06258, 5)
\psline[linewidth=0.03,linecolor=black](8.75, 4.75)(9.06258, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.75, 4.75)(9.06258, 5)(8.75, 5)
\psline[linewidth=0.03,linecolor=black](8.75, 4.75)(8.75, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](8.43742, 5)(8.75, 4.75)(8.75, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.06258, 4.75)(8.75, 4.75)(9.06258, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](10, 4.75)(9.68742, 4.75)(10, 4.5)
\psline[linewidth=0.03,linecolor=black](10, 4.75)(10, 4.5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 4.75)(10, 4.75)(10, 5)
\psline[linewidth=0.03,linecolor=black](10, 4.75)(10, 5)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.75)(10, 5)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 5)(9.68742, 4.75)(10, 5)
\psline[linewidth=0.03,linecolor=black](9.68742, 5)(9.68742, 4.75)
\pspolygon[linestyle=none,fillcolor=disc1,fillstyle=solid](9.68742, 4.75)(9.68742, 5)(9.37484, 5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 5)
\psdot[dotstyle=*,dotsize=0.11](10, 5)
\psdot[dotstyle=*,dotsize=0.11](10, 4.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 4.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 4.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 4.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 4.5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 4.5)
\psdot[dotstyle=*,dotsize=0.11](10, 4.5)
\psdot[dotstyle=*,dotsize=0.11](10, 4.25)
\psdot[dotstyle=*,dotsize=0.11](10, 4)
\psdot[dotstyle=*,dotsize=0.11](10, 3.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 4.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 4.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 4.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 4.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 4.5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 4.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 4.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 4)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 4)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 3.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 3.5)
\psdot[dotstyle=*,dotsize=0.11](10, 3.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 4.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 4)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 3.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 3.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 3.5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 3.25)
\psdot[dotstyle=*,dotsize=0.11](10, 3.25)
\psdot[dotstyle=*,dotsize=0.11](10, 3)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 4.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 4.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 4.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 4.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 4)
\psdot[dotstyle=*,dotsize=0.11](8.75, 4)
\psdot[dotstyle=*,dotsize=0.11](8.75, 3.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 3.5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 3.5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 3.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 3.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 3)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 3)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 2.75)
\psdot[dotstyle=*,dotsize=0.11](10, 2.75)
\psdot[dotstyle=*,dotsize=0.11](10, 2.5)
\psdot[dotstyle=*,dotsize=0.11](10, 2.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 2.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 2.5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 2.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 3.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 3)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 4.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 4.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 4.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 4.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 4)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 3.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 4.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 4.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 4.25)
\psdot[dotstyle=*,dotsize=0.11](7.5, 4)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 4)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 3.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 3.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 3.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 3.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 3.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 3.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 3)
\psdot[dotstyle=*,dotsize=0.11](8.75, 3)
\psdot[dotstyle=*,dotsize=0.11](8.75, 2.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 2.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 2.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 2.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 2.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 2)
\psdot[dotstyle=*,dotsize=0.11](10, 2)
\psdot[dotstyle=*,dotsize=0.11](10, 1.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 1.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 1.5)
\psdot[dotstyle=*,dotsize=0.11](10, 1.5)
\psdot[dotstyle=*,dotsize=0.11](10, 1.25)
\psdot[dotstyle=*,dotsize=0.11](10, 1)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 2.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 2)
\psdot[dotstyle=*,dotsize=0.11](8.75, 2.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 2.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 2)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 1.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 1.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 1.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 1.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 1.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 1)
\psdot[dotstyle=*,dotsize=0.11](10, 0.75)
\psdot[dotstyle=*,dotsize=0.11](10, 0.5)
\psdot[dotstyle=*,dotsize=0.11](5, 0)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 0.25)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 0)
\psdot[dotstyle=*,dotsize=0.11](5.625, 0)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 0)
\psdot[dotstyle=*,dotsize=0.11](4.375, 0)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 0)
\psdot[dotstyle=*,dotsize=0.11](4.375, 0.25)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 0.25)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 0.5)
\psdot[dotstyle=*,dotsize=0.11](5, 0.25)
\psdot[dotstyle=*,dotsize=0.11](5, 0.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 0.5)
\psdot[dotstyle=*,dotsize=0.11](5.625, 0.5)
\psdot[dotstyle=*,dotsize=0.11](5.625, 0.25)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 0.25)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 0)
\psdot[dotstyle=*,dotsize=0.11](6.25, 0)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 0)
\psdot[dotstyle=*,dotsize=0.11](6.875, 0)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 2.75)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 2.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 2.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 3.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 3.5)
\psdot[dotstyle=*,dotsize=0.11](5.625, 3.25)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 3)
\psdot[dotstyle=*,dotsize=0.11](5.625, 3)
\psdot[dotstyle=*,dotsize=0.11](5.625, 2.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 2.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 2.25)
\psdot[dotstyle=*,dotsize=0.11](5, 2.75)
\psdot[dotstyle=*,dotsize=0.11](4.375, 2)
\psdot[dotstyle=*,dotsize=0.11](4.375, 2.25)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 2.25)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 2.5)
\psdot[dotstyle=*,dotsize=0.11](5, 2.25)
\psdot[dotstyle=*,dotsize=0.11](5, 2.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 2.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 2.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 2.25)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 2)
\psdot[dotstyle=*,dotsize=0.11](5.625, 2)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 2)
\psdot[dotstyle=*,dotsize=0.11](6.25, 1.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 1.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 1.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 1.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 1.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 1.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 1.5)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 1.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 1)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 0.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 0)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 0)
\psdot[dotstyle=*,dotsize=0.11](3.75, 0)
\psdot[dotstyle=*,dotsize=0.11](3.75, 0.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 0.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 0.5)
\psdot[dotstyle=*,dotsize=0.11](4.375, 0.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 0.75)
\psdot[dotstyle=*,dotsize=0.11](5, 1)
\psdot[dotstyle=*,dotsize=0.11](2.5, 0)
\psdot[dotstyle=*,dotsize=0.11](2.5, 0.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 0.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 1)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 1.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 1.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 1.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 1.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 1.75)
\psdot[dotstyle=*,dotsize=0.11](4.375, 1.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 2)
\psdot[dotstyle=*,dotsize=0.11](5, 2)
\psdot[dotstyle=*,dotsize=0.11](4.375, 1.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 1.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 1.75)
\psdot[dotstyle=*,dotsize=0.11](5, 1.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 0.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 1)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 0)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 0.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 0.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 0.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 0.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 0.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 0.5)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 0.75)
\psdot[dotstyle=*,dotsize=0.11](3.75, 0.5)
\psdot[dotstyle=*,dotsize=0.11](3.75, 0.75)
\psdot[dotstyle=*,dotsize=0.11](3.75, 1)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 1)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 1.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 0.75)
\psdot[dotstyle=*,dotsize=0.11](4.375, 0.75)
\psdot[dotstyle=*,dotsize=0.11](4.375, 1)
\psdot[dotstyle=*,dotsize=0.11](4.375, 1.25)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 1)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 1.25)
\psdot[dotstyle=*,dotsize=0.11](5, 1.25)
\psdot[dotstyle=*,dotsize=0.11](5, 1.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 1.75)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 1.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 1.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 1.5)
\psdot[dotstyle=*,dotsize=0.11](5.625, 1.25)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 1)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 1.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 1.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 1)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 1)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 0.75)
\psdot[dotstyle=*,dotsize=0.11](6.875, 0.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 0.5)
\psdot[dotstyle=*,dotsize=0.11](5, 0.75)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 1)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 0.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 1)
\psdot[dotstyle=*,dotsize=0.11](5.625, 0.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 0.75)
\psdot[dotstyle=*,dotsize=0.11](6.25, 0.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 0.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 0.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 0.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 0.5)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 0.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 0.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 0.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 0.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 0)
\psdot[dotstyle=*,dotsize=0.11](7.5, 0)
\psdot[dotstyle=*,dotsize=0.11](7.5, 0.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 0.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 0.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 0)
\psdot[dotstyle=*,dotsize=0.11](8.125, 0)
\psdot[dotstyle=*,dotsize=0.11](6.875, 2.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 4.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 4.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 4.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 4)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 4)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 3.75)
\psdot[dotstyle=*,dotsize=0.11](6.25, 3.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 3.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 3.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 3)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 3)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 3)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 2.75)
\psdot[dotstyle=*,dotsize=0.11](6.25, 2.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 2.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 2.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 2.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 2.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 2.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 2)
\psdot[dotstyle=*,dotsize=0.11](7.5, 1.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 1.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 2.5)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 2.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 2.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 2)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 2)
\psdot[dotstyle=*,dotsize=0.11](6.875, 2)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 1.75)
\psdot[dotstyle=*,dotsize=0.11](6.875, 1.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 1.75)
\psdot[dotstyle=*,dotsize=0.11](6.875, 1.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 1.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 1.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 1.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 1)
\psdot[dotstyle=*,dotsize=0.11](7.5, 1)
\psdot[dotstyle=*,dotsize=0.11](7.5, 0.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 1)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 0.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 0.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 0.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 0.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 0.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 0.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 0)
\psdot[dotstyle=*,dotsize=0.11](8.75, 0)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 3.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 3.5)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 3.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 3.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 3)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 2.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 2.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 2.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 2.25)
\psdot[dotstyle=*,dotsize=0.11](7.5, 2)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 2)
\psdot[dotstyle=*,dotsize=0.11](8.125, 1.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 1.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 1.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 1.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 1.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 1.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 1)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 1)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 0.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 0.75)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 0.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 0.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 0.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 0.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 0)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 0)
\psdot[dotstyle=*,dotsize=0.11](6.875, 3.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 4)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 3.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 3.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 3.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 3.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 3.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 3.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 3.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 3)
\psdot[dotstyle=*,dotsize=0.11](7.5, 3.25)
\psdot[dotstyle=*,dotsize=0.11](7.5, 3)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 3)
\psdot[dotstyle=*,dotsize=0.11](7.5, 2.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 2.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 3)
\psdot[dotstyle=*,dotsize=0.11](8.125, 2.75)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 2.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 2.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 2.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 2.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 2.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 2.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 2.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 2)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 2)
\psdot[dotstyle=*,dotsize=0.11](8.75, 2)
\psdot[dotstyle=*,dotsize=0.11](8.75, 1.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 1.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 1.75)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 1.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 1.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 1.25)
\psdot[dotstyle=*,dotsize=0.11](8.75, 1.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 1.25)
\psdot[dotstyle=*,dotsize=0.11](8.75, 1)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 1)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 1)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 0.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 0.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 0.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 0.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 0.5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 0.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 0.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 0.25)
\psdot[dotstyle=*,dotsize=0.11](10, 0.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 0)
\psdot[dotstyle=*,dotsize=0.11](10, 0)
\psline[linewidth=0.03,linecolor=black](9.37484, 5)(9.68742, 5)
\psline[linewidth=0.03,linecolor=black](9.68742, 5)(10, 5)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.75)(10, 4.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 5)(8.75, 5)
\psline[linewidth=0.03,linecolor=black](8.75, 5)(9.06258, 5)
\psline[linewidth=0.03,linecolor=black](8.75, 4.75)(9.06258, 4.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 5)(9.37484, 4.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 5)(9.37484, 5)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.75)(9.37484, 5)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.75)(10, 4.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.5)(9.06258, 4.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.5)(9.68742, 4.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.25)(10, 4.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.25)(10, 4)
\psline[linewidth=0.03,linecolor=black](10, 3.75)(10, 4)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.25)(9.68742, 4.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 4.25)(9.68742, 4)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(7.81248, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(8.43742, 5)
\psline[linewidth=0.03,linecolor=black](8.43742, 5)(8.75, 4.75)
\psline[linewidth=0.03,linecolor=black](8.125, 4.75)(8.43742, 4.75)
\psline[linewidth=0.03,linecolor=black](8.75, 4.75)(9.06258, 4.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.25)(9.06258, 4.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.5)(8.75, 4.5)
\psline[linewidth=0.03,linecolor=black](8.75, 4.5)(9.06258, 4.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 4.25)(9.37484, 4)
\psline[linewidth=0.03,linecolor=black](9.68742, 4)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](10, 3.5)(9.68742, 3.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.75)(9.68742, 3.5)
\psline[linewidth=0.03,linecolor=black](10, 3.5)(10, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 4)(9.37484, 3.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.5)(8.75, 4.25)
\psline[linewidth=0.03,linecolor=black](8.75, 4.25)(9.06258, 4)
\psline[linewidth=0.03,linecolor=black](9.06258, 4)(9.06258, 3.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.75)(9.37484, 3.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.5)(9.68742, 3.25)
\psline[linewidth=0.03,linecolor=black](10, 3)(10, 3.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 3)(9.37484, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.5)(9.37484, 3.25)
\psline[linewidth=0.03,linecolor=black](7.5, 5)(7.81248, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 4.75)(7.81248, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 4.75)(8.43742, 4.5)
\psline[linewidth=0.03,linecolor=black](8.125, 4.75)(8.125, 4.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 4.25)(8.43742, 4.5)
\psline[linewidth=0.03,linecolor=black](8.75, 4)(8.43742, 4.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 4)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](8.75, 4)(8.75, 3.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.75)(8.75, 3.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.5)(8.75, 3.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 3.25)(9.06258, 3.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 3.25)(9.37484, 3)
\psline[linewidth=0.03,linecolor=black](9.68742, 3)(10, 2.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 3)(9.68742, 2.75)
\psline[linewidth=0.03,linecolor=black](10, 2.75)(10, 2.5)
\psline[linewidth=0.03,linecolor=black](10, 2.25)(10, 2.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.25)(10, 2)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.75)(9.68742, 2.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 3)(9.37484, 2.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.75)(9.37484, 2.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.5)(9.68742, 2.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.5)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 3)(8.75, 3.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 2.75)(9.06258, 3)
\psline[linewidth=0.03,linecolor=black](8.75, 3)(8.43742, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.5)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](7.5, 5)(7.81248, 4.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.5)(7.81248, 4.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 4.5)(7.81248, 4.25)
\psline[linewidth=0.03,linecolor=black](8.125, 4)(8.125, 4.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.75)(8.125, 4)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.5)(8.43742, 3.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 4)(8.125, 3.75)
\psline[linewidth=0.03,linecolor=black](7.5, 4.25)(7.81248, 4)
\psline[linewidth=0.03,linecolor=black](7.5, 5)(7.5, 4.75)
\psline[linewidth=0.03,linecolor=black](7.5, 4.75)(7.5, 4.5)
\psline[linewidth=0.03,linecolor=black](7.5, 4.25)(7.5, 4.5)
\psline[linewidth=0.03,linecolor=black](7.5, 4)(7.5, 4.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 4)(7.81248, 3.75)
\psline[linewidth=0.03,linecolor=black](8.125, 3.75)(8.125, 3.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.25)(8.43742, 3.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.5)(8.125, 3.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 3.25)(8.43742, 3)
\psline[linewidth=0.03,linecolor=black](8.75, 2.75)(8.75, 3)
\psline[linewidth=0.03,linecolor=black](9.06258, 2.75)(9.06258, 2.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 2.25)(9.06258, 2.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 2.25)(9.68742, 2)
\psline[linewidth=0.03,linecolor=black](10, 2)(10, 1.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.75)(10, 1.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 2)(9.68742, 1.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.75)(9.68742, 1.5)
\psline[linewidth=0.03,linecolor=black](10, 1.5)(10, 1.25)
\psline[linewidth=0.03,linecolor=black](10, 1)(10, 1.25)
\psline[linewidth=0.03,linecolor=black](8.75, 2.5)(9.06258, 2.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 2)(9.06258, 2.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 2)(9.37484, 1.75)
\psline[linewidth=0.03,linecolor=black](8.75, 2.5)(8.43742, 2.75)
\psline[linewidth=0.03,linecolor=black](8.75, 2.5)(8.75, 2.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 2)(8.75, 2.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.75)(9.06258, 2)
\psline[linewidth=0.03,linecolor=black](9.37484, 1.75)(9.37484, 1.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.25)(9.37484, 1.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.5)(9.37484, 1.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 1.25)(9.68742, 1)
\psline[linewidth=0.03,linecolor=black](9.68742, 1)(10, 0.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.75)(10, 0.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 0)(5, 0)
\psline[linewidth=0.03,linecolor=black](5, 0.25)(5.3125, 0)
\psline[linewidth=0.03,linecolor=black](5, 0.25)(5.3125, 0.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 0)(5.625, 0)
\psline[linewidth=0.03,linecolor=black](4.06252, 0)(3.75, 0)
\psline[linewidth=0.03,linecolor=black](4.06252, 0)(4.375, 0)
\psline[linewidth=0.03,linecolor=black](4.375, 0)(4.6875, 0)
\psline[linewidth=0.03,linecolor=black](5, 0.25)(4.6875, 0)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.25)(4.375, 0.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.25)(4.375, 0.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.5)(4.375, 0.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.5)(5, 0.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 0.5)(5, 0.25)
\psline[linewidth=0.03,linecolor=black](5.625, 0.25)(5.3125, 0.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 0.5)(5.625, 0.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 0)(5.625, 0.25)
\psline[linewidth=0.03,linecolor=black](5.625, 0.25)(5.93748, 0.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 0)(6.25, 0)
\psline[linewidth=0.03,linecolor=black](6.56248, 0)(6.25, 0.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 0)(6.875, 0)
\psline[linewidth=0.03,linecolor=black](4.375, 2.5)(4.6875, 2.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.75)(5, 2.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.5)(5.625, 2.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 2.25)(5.625, 2.25)
\psline[linewidth=0.03,linecolor=black](6.25, 4)(6.25, 3.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 3.75)(5.93748, 3.5)
\psline[linewidth=0.03,linecolor=black](5.625, 3.5)(5.625, 3.25)
\psline[linewidth=0.03,linecolor=black](5.625, 3.25)(5.625, 3)
\psline[linewidth=0.03,linecolor=black](5.3125, 3)(5.3125, 3.25)
\psline[linewidth=0.03,linecolor=black](5.625, 2.75)(5.3125, 3)
\psline[linewidth=0.03,linecolor=black](5.625, 2.75)(5.93748, 2.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 2.5)(5, 2.75)
\psline[linewidth=0.03,linecolor=black](5, 2.75)(5.3125, 2.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 2.5)(4.375, 2.5)
\psline[linewidth=0.03,linecolor=black](4.375, 2.25)(4.06252, 2)
\psline[linewidth=0.03,linecolor=black](4.06252, 2)(4.375, 2)
\psline[linewidth=0.03,linecolor=black](4.375, 2.25)(4.6875, 2.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 2.5)(5, 2.5)
\psline[linewidth=0.03,linecolor=black](5, 2.25)(4.6875, 2)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.25)(5, 2)
\psline[linewidth=0.03,linecolor=black](5.3125, 2.5)(5.625, 2.25)
\psline[linewidth=0.03,linecolor=black](5.625, 2.25)(5.93748, 2)
\psline[linewidth=0.03,linecolor=black](5.3125, 2)(5, 2)
\psline[linewidth=0.03,linecolor=black](5.3125, 2)(5.625, 2)
\psline[linewidth=0.03,linecolor=black](5.93748, 1.75)(6.25, 1.75)
\psline[linewidth=0.03,linecolor=black](6.25, 1.5)(6.56248, 1.5)
\psline[linewidth=0.03,linecolor=black](6.875, 1.25)(6.875, 1.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.75)(5.625, 1.75)
\psline[linewidth=0.03,linecolor=black](5.625, 1.75)(5.93748, 1.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 1.75)(6.25, 1.5)
\psline[linewidth=0.03,linecolor=black](5.625, 1.5)(5.93748, 1.5)
\psline[linewidth=0.03,linecolor=black](6.25, 1.5)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](6.875, 1)(6.56248, 1.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 0.75)(7.18748, 1)
\psline[linewidth=0.03,linecolor=black](2.81252, 0)(3.125, 0)
\psline[linewidth=0.03,linecolor=black](3.43752, 0)(3.125, 0)
\psline[linewidth=0.03,linecolor=black](3.75, 0.25)(3.43752, 0)
\psline[linewidth=0.03,linecolor=black](3.43752, 0)(3.75, 0)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.25)(3.75, 0)
\psline[linewidth=0.03,linecolor=black](3.75, 0.5)(4.06252, 0.5)
\psline[linewidth=0.03,linecolor=black](4.375, 0.5)(4.06252, 0.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 0.75)(4.375, 0.5)
\psline[linewidth=0.03,linecolor=black](5, 0.75)(4.6875, 0.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 1)(5, 1)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.25)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.75)(3.75, 1.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 0)(2.5, 0)
\psline[linewidth=0.03,linecolor=black](2.18752, 0)(2.5, 0.25)
\psline[linewidth=0.03,linecolor=black](2.5, 0)(2.81252, 0)
\psline[linewidth=0.03,linecolor=black](2.81252, 0.75)(2.5, 0.5)
\psline[linewidth=0.03,linecolor=black](3.125, 0.75)(3.125, 1)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.25)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.5)(3.75, 1.5)
\psline[linewidth=0.03,linecolor=black](3.75, 1.25)(3.43752, 1)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.5)(3.75, 1.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.75)(4.375, 1.75)
\psline[linewidth=0.03,linecolor=black](4.375, 1.75)(4.6875, 2)
\psline[linewidth=0.03,linecolor=black](5, 2)(4.6875, 2)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.75)(5, 2)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.75)(4.375, 1.5)
\psline[linewidth=0.03,linecolor=black](4.375, 1.5)(4.06252, 1.25)
\psline[linewidth=0.03,linecolor=black](4.375, 1.5)(4.6875, 1.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.75)(5, 1.75)
\psline[linewidth=0.03,linecolor=black](3.125, 0.75)(2.81252, 0.5)
\psline[linewidth=0.03,linecolor=black](3.125, 0.75)(3.43752, 1)
\psline[linewidth=0.03,linecolor=black](3.43752, 1)(3.75, 1)
\psline[linewidth=0.03,linecolor=black](3.125, 0.25)(2.81252, 0)
\psline[linewidth=0.03,linecolor=black](2.81252, 0)(2.81252, 0.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 0.25)(2.81252, 0.5)
\psline[linewidth=0.03,linecolor=black](3.125, 0.5)(2.81252, 0.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 0.75)(3.125, 0.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 0.5)(3.125, 0.25)
\psline[linewidth=0.03,linecolor=black](3.125, 0.25)(3.43752, 0.25)
\psline[linewidth=0.03,linecolor=black](3.75, 0.5)(3.43752, 0.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 0.75)(3.75, 0.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.75)(3.75, 0.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 1)(3.75, 1)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.25)(3.75, 1)
\psline[linewidth=0.03,linecolor=black](4.06252, 1.25)(4.375, 1.25)
\psline[linewidth=0.03,linecolor=black](4.375, 1)(4.06252, 0.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 0.75)(4.375, 0.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 1)(4.375, 0.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.25)(4.375, 1.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 1)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 1.25)(5, 1.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 1.5)(5, 1.25)
\psline[linewidth=0.03,linecolor=black](5.625, 1.5)(5.3125, 1.75)
\psline[linewidth=0.03,linecolor=black](5.625, 1.25)(5.3125, 1.25)
\psline[linewidth=0.03,linecolor=black](5.625, 1.5)(5.93748, 1.25)
\psline[linewidth=0.03,linecolor=black](5.625, 1.25)(5.93748, 1)
\psline[linewidth=0.03,linecolor=black](6.25, 1)(5.93748, 1.25)
\psline[linewidth=0.03,linecolor=black](6.25, 1.25)(5.93748, 1.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 1)(6.25, 1.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 0.75)(6.25, 0.75)
\psline[linewidth=0.03,linecolor=black](6.875, 0.75)(6.56248, 1)
\psline[linewidth=0.03,linecolor=black](6.875, 0.75)(7.18748, 0.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 0.75)(5, 0.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 1)(5, 0.75)
\psline[linewidth=0.03,linecolor=black](5.625, 1)(5.3125, 1)
\psline[linewidth=0.03,linecolor=black](5.625, 0.75)(5.3125, 0.75)
\psline[linewidth=0.03,linecolor=black](5.625, 1)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 0.5)(5.625, 0.75)
\psline[linewidth=0.03,linecolor=black](6.25, 0.75)(5.93748, 0.75)
\psline[linewidth=0.03,linecolor=black](6.25, 0.75)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.25, 0.25)(5.93748, 0.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 0.5)(6.25, 0.5)
\psline[linewidth=0.03,linecolor=black](6.25, 0.25)(6.56248, 0.25)
\psline[linewidth=0.03,linecolor=black](6.875, 0.5)(6.56248, 0.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 0.25)(6.875, 0.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 0.25)(6.875, 0.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 0)(6.875, 0.25)
\psline[linewidth=0.03,linecolor=black](7.5, 0)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.5, 0.75)(7.5, 0.5)
\psline[linewidth=0.03,linecolor=black](7.5, 0.5)(7.81248, 0.25)
\psline[linewidth=0.03,linecolor=black](7.5, 0.5)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 0)(7.5, 0.25)
\psline[linewidth=0.03,linecolor=black](8.125, 0.25)(8.125, 0)
\psline[linewidth=0.03,linecolor=black](6.875, 2.75)(6.875, 3)
\psline[linewidth=0.03,linecolor=black](7.18748, 2.25)(6.875, 2.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.75)(7.18748, 4.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.5)(7.18748, 4.25)
\psline[linewidth=0.03,linecolor=black](6.875, 4.5)(6.875, 4.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 4)(7.18748, 4.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 4)(6.875, 4.25)
\psline[linewidth=0.03,linecolor=black](6.875, 4.25)(6.875, 4)
\psline[linewidth=0.03,linecolor=black](6.56248, 4)(6.56248, 3.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.75)(6.25, 3.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.25)(6.56248, 3)
\psline[linewidth=0.03,linecolor=black](6.25, 3.5)(5.93748, 3.25)
\psline[linewidth=0.03,linecolor=black](6.25, 3.5)(6.25, 3.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 3)(5.93748, 3.25)
\psline[linewidth=0.03,linecolor=black](6.25, 3)(6.25, 3.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 2.75)(6.56248, 3)
\psline[linewidth=0.03,linecolor=black](5.93748, 3)(6.25, 2.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 3)(5.93748, 2.75)
\psline[linewidth=0.03,linecolor=black](6.25, 2.5)(5.93748, 2.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 2.5)(6.56248, 2.75)
\psline[linewidth=0.03,linecolor=black](6.875, 2.5)(6.56248, 2.75)
\psline[linewidth=0.03,linecolor=black](6.875, 2.5)(6.875, 2.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 2.25)(7.18748, 2)
\psline[linewidth=0.03,linecolor=black](7.5, 2)(7.5, 1.75)
\psline[linewidth=0.03,linecolor=black](7.5, 1.5)(7.5, 1.75)
\psline[linewidth=0.03,linecolor=black](6.875, 2)(7.18748, 1.75)
\psline[linewidth=0.03,linecolor=black](6.25, 2.25)(6.25, 2.5)
\psline[linewidth=0.03,linecolor=black](6.25, 2.5)(6.56248, 2.25)
\psline[linewidth=0.03,linecolor=black](6.875, 2)(6.56248, 2.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 2)(6.25, 2.25)
\psline[linewidth=0.03,linecolor=black](6.25, 2.25)(6.25, 2)
\psline[linewidth=0.03,linecolor=black](6.56248, 1.75)(6.25, 2)
\psline[linewidth=0.03,linecolor=black](6.875, 2)(6.875, 1.75)
\psline[linewidth=0.03,linecolor=black](6.875, 1.5)(6.56248, 1.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 1.75)(7.18748, 1.5)
\psline[linewidth=0.03,linecolor=black](6.875, 1.5)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 1.5)(7.5, 1.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 1)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](7.5, 1)(7.18748, 1.25)
\psline[linewidth=0.03,linecolor=black](7.5, 0.75)(7.18748, 1)
\psline[linewidth=0.03,linecolor=black](7.5, 0.75)(7.81248, 0.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 1)(7.81248, 1.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 1)(7.81248, 0.75)
\psline[linewidth=0.03,linecolor=black](8.125, 1)(8.125, 0.75)
\psline[linewidth=0.03,linecolor=black](8.125, 0.75)(8.125, 0.5)
\psline[linewidth=0.03,linecolor=black](8.125, 0.25)(7.81248, 0.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.5)(8.43742, 0.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 0)(8.125, 0.25)
\psline[linewidth=0.03,linecolor=black](8.75, 0.25)(8.75, 0)
\psline[linewidth=0.03,linecolor=black](6.875, 3.75)(6.875, 3.5)
\psline[linewidth=0.03,linecolor=black](6.875, 3.75)(6.56248, 3.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 3.25)(6.56248, 3.5)
\psline[linewidth=0.03,linecolor=black](6.875, 3.5)(6.875, 3.25)
\psline[linewidth=0.03,linecolor=black](6.875, 3)(6.56248, 3.25)
\psline[linewidth=0.03,linecolor=black](6.875, 3)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 2.5)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](7.5, 2.5)(7.18748, 2.75)
\psline[linewidth=0.03,linecolor=black](7.5, 2.25)(7.18748, 2.5)
\psline[linewidth=0.03,linecolor=black](7.5, 2.25)(7.5, 2)
\psline[linewidth=0.03,linecolor=black](7.5, 2.25)(7.81248, 2)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.75)(7.5, 2)
\psline[linewidth=0.03,linecolor=black](8.125, 1.75)(8.125, 2)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.5)(7.81248, 1.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.75)(8.125, 1.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.5)(8.125, 1.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 1.5)(7.81248, 1.25)
\psline[linewidth=0.03,linecolor=black](8.125, 1)(7.81248, 1.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.25)(8.43742, 1)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.75)(8.125, 1)
\psline[linewidth=0.03,linecolor=black](8.75, 0.75)(8.43742, 1)
\psline[linewidth=0.03,linecolor=black](8.43742, 0.5)(8.43742, 0.75)
\psline[linewidth=0.03,linecolor=black](8.75, 0.75)(8.75, 0.5)
\psline[linewidth=0.03,linecolor=black](8.75, 0.25)(8.43742, 0.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 0.25)(9.06258, 0.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 0)(8.75, 0.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.25)(9.37484, 0)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.5)(10, 0.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 1)(9.06258, 1.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.25)(8.75, 2)
\psline[linewidth=0.03,linecolor=black](6.875, 3.75)(7.18748, 4)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.5)(6.875, 3.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 4)(7.5, 3.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 4)(7.18748, 3.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.5)(7.5, 3.75)
\psline[linewidth=0.03,linecolor=black](7.5, 3.75)(7.5, 3.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.5)(7.81248, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 3.25)(8.125, 3)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.5)(7.18748, 3.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.5)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 3.25)(7.18748, 3)
\psline[linewidth=0.03,linecolor=black](7.5, 2.75)(7.18748, 3)
\psline[linewidth=0.03,linecolor=black](7.5, 3)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 3)(7.5, 3.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 3)(7.81248, 2.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 2.5)(7.5, 2.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.75)(8.125, 3)
\psline[linewidth=0.03,linecolor=black](8.125, 2.75)(8.125, 3)
\psline[linewidth=0.03,linecolor=black](8.125, 2.5)(8.125, 2.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.5)(8.43742, 2.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.5)(8.43742, 2.25)
\psline[linewidth=0.03,linecolor=black](8.125, 2.25)(7.81248, 2.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 2.5)(7.81248, 2.25)
\psline[linewidth=0.03,linecolor=black](8.125, 2)(7.81248, 2.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 2.25)(8.43742, 2)
\psline[linewidth=0.03,linecolor=black](8.125, 2)(8.43742, 1.75)
\psline[linewidth=0.03,linecolor=black](8.75, 2)(8.75, 1.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.5)(8.75, 1.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.5)(9.06258, 1.25)
\psline[linewidth=0.03,linecolor=black](8.75, 1.5)(8.43742, 1.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.75)(8.43742, 1.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.5)(8.43742, 1.25)
\psline[linewidth=0.03,linecolor=black](8.75, 1.5)(8.75, 1.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 1.25)(8.75, 1)
\psline[linewidth=0.03,linecolor=black](9.06258, 1.25)(9.06258, 1)
\psline[linewidth=0.03,linecolor=black](8.75, 1)(9.06258, 0.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.75)(9.37484, 1)
\psline[linewidth=0.03,linecolor=black](9.37484, 1)(9.37484, 0.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.75)(9.68742, 0.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 0.75)(9.37484, 0.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 0.75)(9.06258, 0.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.25)(9.06258, 0.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 0.5)(9.68742, 0.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 0.25)(9.68742, 0)
\psline[linewidth=0.03,linecolor=black](10, 0.25)(10, 0)


==> examples/cart/ddisc2.tex <==
\newrgbcolor{disc2}{0.7 0.7 0.7}
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 10)(9.68742, 9.75)(10, 10)
\psline[linewidth=0.03,linecolor=black](9.68742, 10)(10, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9.75)(9.68742, 10)(9.37484, 10)
\psline[linewidth=0.03,linecolor=black](9.68742, 10)(9.37484, 10)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.75)(9.37484, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9.75)(9.37484, 10)(9.37484, 9.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 10)(9.37484, 9.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.75)(9.37484, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9.5)(9.68742, 9.75)(9.37484, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 10)(9.06258, 9.75)(9.37484, 9.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 9.75)(9.37484, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 9.75)(9.37484, 9.5)(9.37484, 9.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.5)(9.06258, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9.5)(9.06258, 9.75)(9.06258, 9.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 9.75)(9.06258, 9.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.5)(9.06258, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9.5)(9.06258, 9.5)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 9.5)(9.06258, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 9.5)(8.75, 9.25)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](8.75, 9.25)(9.06258, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9.25)(8.75, 9)(9.06258, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 9.75)(8.75, 9.5)(9.06258, 9.5)
\psline[linewidth=0.03,linecolor=black](8.75, 9.5)(9.06258, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9.5)(8.75, 9.25)(9.06258, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 10)(9.06258, 9.75)(9.37484, 10)
\psline[linewidth=0.03,linecolor=black](9.06258, 10)(9.37484, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 9.75)(9.06258, 10)(8.75, 10)
\psline[linewidth=0.03,linecolor=black](9.06258, 10)(8.75, 10)
\psline[linewidth=0.03,linecolor=black](9.06258, 9.75)(8.75, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9.75)(9.06258, 9.75)(8.75, 10)
\psline[linewidth=0.03,linecolor=black](8.75, 9.75)(8.75, 10)
\psline[linewidth=0.03,linecolor=black](8.75, 9.75)(9.06258, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9.5)(9.06258, 9.75)(8.75, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 9.75)(8.75, 9.75)(8.75, 10)
\psline[linewidth=0.03,linecolor=black](8.43742, 9.75)(8.75, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 9.75)(8.75, 9.5)(8.75, 9.75)
\psline[linewidth=0.03,linecolor=black](8.75, 9.5)(8.43742, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9.5)(8.43742, 9.75)(8.43742, 9.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 9.75)(8.43742, 9.5)
\psline[linewidth=0.03,linecolor=black](8.75, 9.5)(8.43742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9.25)(8.75, 9.5)(8.43742, 9.5)
\psline[linewidth=0.03,linecolor=black](8.75, 9.25)(8.43742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9.25)(8.43742, 9.5)(8.43742, 9.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 9.5)(8.43742, 9.25)
\psline[linewidth=0.03,linecolor=black](8.75, 9.25)(8.43742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9)(8.75, 9.25)(8.43742, 9.25)
\psline[linewidth=0.03,linecolor=black](8.75, 9)(8.43742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9)(8.43742, 9.25)(8.43742, 9)
\psline[linewidth=0.03,linecolor=black](8.43742, 9.25)(8.43742, 9)
\psline[linewidth=0.03,linecolor=black](8.75, 9)(8.43742, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8.75)(8.75, 9)(8.43742, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 9.25)(8.125, 9)(8.43742, 9)
\psline[linewidth=0.03,linecolor=black](8.125, 9)(8.43742, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9)(8.43742, 8.75)(8.43742, 9)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.75)(8.125, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8.75)(8.125, 9)(8.125, 8.75)
\psline[linewidth=0.03,linecolor=black](8.125, 9)(8.125, 8.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.75)(8.125, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8.75)(8.125, 8.75)(8.125, 8.5)
\psline[linewidth=0.03,linecolor=black](8.125, 8.75)(8.125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 8.75)(7.81248, 8.5)(8.125, 8.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.5)(8.125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 8.5)(8.125, 8.25)(8.125, 8.5)
\psline[linewidth=0.03,linecolor=black](8.125, 8.25)(7.81248, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 8.25)(7.81248, 8.5)(7.81248, 8.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.5)(7.81248, 8.25)
\psline[linewidth=0.03,linecolor=black](8.125, 8.25)(7.81248, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 8.25)(7.81248, 8.25)(7.81248, 8)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.25)(7.81248, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 8.25)(7.5, 8)(7.81248, 8)
\psline[linewidth=0.03,linecolor=black](7.5, 8)(7.81248, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 8)(7.81248, 7.75)(7.81248, 8)
\psline[linewidth=0.03,linecolor=black](7.5, 8)(7.81248, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 8)(7.5, 7.75)(7.81248, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 7.75)(7.81248, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 8)(7.5, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7.75)(7.5, 8)(7.18748, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 7.75)(7.18748, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7.5)(7.5, 7.75)(7.18748, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 7.5)(7.18748, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 7.5)(7.5, 7.5)(7.18748, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 7.5)(7.18748, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 7.25)(7.5, 7.5)(7.18748, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7.75)(7.5, 7.5)(7.81248, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 8.25)(7.81248, 8.5)(7.5, 8.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.25)(7.5, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 8)(7.81248, 8.25)(7.5, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9)(7.81248, 8.75)(8.125, 8.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.75)(8.125, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 8.75)(7.81248, 8.5)(8.125, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 9.5)(8.125, 9.25)(8.43742, 9.25)
\psline[linewidth=0.03,linecolor=black](8.125, 9.25)(8.43742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9.25)(8.125, 9)(8.43742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 9.75)(8.125, 9.5)(8.43742, 9.5)
\psline[linewidth=0.03,linecolor=black](8.125, 9.5)(8.43742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9.5)(8.125, 9.25)(8.43742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 10)(8.43742, 9.75)(8.75, 10)
\psline[linewidth=0.03,linecolor=black](8.43742, 10)(8.75, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 9.75)(8.43742, 10)(8.125, 10)
\psline[linewidth=0.03,linecolor=black](8.43742, 10)(8.125, 10)
\psline[linewidth=0.03,linecolor=black](8.43742, 9.75)(8.125, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 9.75)(8.125, 10)(8.125, 9.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 9.75)(8.125, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9.5)(8.43742, 9.75)(8.125, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 10)(7.81248, 10)(8.125, 9.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 10)(8.125, 9.75)
\psline[linewidth=0.03,linecolor=black](8.125, 10)(7.81248, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 10)(7.81248, 9.75)(8.125, 9.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 9.75)(8.125, 9.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 9.75)(7.81248, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 9.75)(7.81248, 10)(7.5, 9.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 9.75)(7.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 9.5)(7.81248, 9.75)(7.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 9.75)(8.125, 9.5)(8.125, 9.75)
\psline[linewidth=0.03,linecolor=black](8.125, 9.5)(7.81248, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9.5)(7.81248, 9.75)(7.81248, 9.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 9.75)(7.81248, 9.5)
\psline[linewidth=0.03,linecolor=black](8.125, 9.5)(7.81248, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9.25)(8.125, 9.5)(7.81248, 9.5)
\psline[linewidth=0.03,linecolor=black](8.125, 9.25)(7.81248, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 9.25)(8.125, 9.25)(7.81248, 9.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 9.25)(8.125, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9)(8.125, 9.25)(7.81248, 9.25)
\psline[linewidth=0.03,linecolor=black](8.125, 9)(7.81248, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 9)(8.125, 9)(7.81248, 9.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 9)(8.125, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 9)(7.81248, 9)(7.81248, 8.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.75)(7.81248, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 8.75)(7.81248, 9)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.75)(7.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 8.5)(7.81248, 8.75)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.5)(7.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 8.5)(7.81248, 8.5)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.5, 8.5)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.5, 8.5)(7.81248, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 8.5)(7.5, 8.5)(7.5, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 8.5)(7.5, 8.5)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 8.5)(7.5, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 8.5)(7.18748, 8.5)(7.5, 8.25)
\psline[linewidth=0.03,linecolor=black](7.5, 8.25)(7.18748, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 8.25)(7.18748, 8.5)(7.18748, 8.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 8.5)(7.18748, 8.25)
\psline[linewidth=0.03,linecolor=black](7.5, 8.25)(7.18748, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 8)(7.5, 8.25)(7.18748, 8.25)
\psline[linewidth=0.03,linecolor=black](7.5, 8)(7.18748, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 8)(7.5, 8)(7.18748, 8.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 8)(7.5, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 8)(7.18748, 8)(7.18748, 7.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 8)(7.18748, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 8)(6.875, 7.75)(7.18748, 7.75)
\psline[linewidth=0.03,linecolor=black](6.875, 7.75)(7.18748, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 7.75)(7.18748, 7.5)(7.18748, 7.75)
\psline[linewidth=0.03,linecolor=black](6.875, 7.75)(7.18748, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 7.75)(6.875, 7.5)(7.18748, 7.5)
\psline[linewidth=0.03,linecolor=black](6.875, 7.5)(7.18748, 7.5)
\psline[linewidth=0.03,linecolor=black](6.875, 7.75)(6.875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 7.75)(6.56248, 7.5)(6.875, 7.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.5)(6.875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.5)(6.56248, 7.25)(6.875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 7.5)(7.18748, 7.25)(7.18748, 7.5)
\psline[linewidth=0.03,linecolor=black](6.875, 7.5)(7.18748, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 7.25)(7.18748, 7.25)(6.875, 7.5)
\psline[linewidth=0.03,linecolor=black](6.875, 7.25)(6.875, 7.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 7.25)(6.875, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 7.25)(6.875, 7.25)(6.875, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.25)(6.875, 7.25)(6.875, 7.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.25)(6.875, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 7.25)(6.56248, 7.25)(6.875, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.25)(6.875, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.25)(6.56248, 7)(6.875, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 7)(6.875, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 7)(6.56248, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7)(6.56248, 7.25)(6.25, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 7)(6.25, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6.75)(6.56248, 7)(6.25, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 6.75)(6.25, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 6.75)(6.56248, 6.75)(6.25, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 6.75)(6.25, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6.75)(6.25, 6.75)(6.25, 6.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 6.75)(6.25, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6.5)(6.56248, 6.75)(6.25, 6.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 6.5)(6.25, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 6.25)(6.56248, 6.5)(6.25, 6.5)
\psline[linewidth=0.03,linecolor=black](6.25, 6.25)(6.56248, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6.5)(6.25, 6.25)(6.56248, 6.25)
\psline[linewidth=0.03,linecolor=black](6.25, 6.25)(6.56248, 6.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 6.5)(6.56248, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.25)(6.56248, 6.5)(6.56248, 6.25)
\psline[linewidth=0.03,linecolor=black](6.875, 6.25)(6.56248, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6)(6.875, 6.25)(6.56248, 6.25)
\psline[linewidth=0.03,linecolor=black](6.875, 6.25)(6.56248, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.25)(6.56248, 6)(6.875, 6)
\psline[linewidth=0.03,linecolor=black](6.56248, 6)(6.875, 6)
\psline[linewidth=0.03,linecolor=black](6.875, 6.25)(6.875, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 6)(6.875, 6.25)(6.875, 6)
\psline[linewidth=0.03,linecolor=black](7.18748, 6)(6.875, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 5.75)(7.18748, 6)(6.875, 6)
\psline[linewidth=0.03,linecolor=black](7.18748, 6)(6.875, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 5.75)(7.18748, 6)(6.875, 5.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.75)(6.875, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 5.75)(6.875, 5.75)(6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.75)(6.875, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 5.5)(7.18748, 5.75)(6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.5)(6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.75)(7.18748, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 5.75)(7.18748, 5.5)(7.5, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.5)(7.5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 5.5)(7.18748, 5.25)(7.5, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.25)(7.5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 5.25)(7.5, 5.25)(7.5, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.25)(7.5, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 5.25)(7.5, 5)(7.5, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 5.25)(7.18748, 5.5)(6.875, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6)(6.875, 5.75)(6.875, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 6.25)(6.56248, 6)(6.56248, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7)(6.875, 6.75)(6.875, 7)
\psline[linewidth=0.03,linecolor=black](6.875, 6.75)(6.56248, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6.75)(6.875, 6.75)(6.56248, 7)
\psline[linewidth=0.03,linecolor=black](6.875, 6.75)(6.56248, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.75)(6.56248, 6.75)(6.56248, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 8.5)(6.875, 8.25)(7.18748, 8.25)
\psline[linewidth=0.03,linecolor=black](6.875, 8.25)(7.18748, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.25)(7.18748, 8)(7.18748, 8.25)
\psline[linewidth=0.03,linecolor=black](6.875, 8.25)(7.18748, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.25)(6.875, 8)(7.18748, 8)
\psline[linewidth=0.03,linecolor=black](6.875, 8)(7.18748, 8)
\psline[linewidth=0.03,linecolor=black](6.875, 8.25)(6.875, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8)(6.875, 8.25)(6.56248, 8)
\psline[linewidth=0.03,linecolor=black](6.875, 8)(6.56248, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 7.75)(6.875, 8)(6.56248, 8)
\psline[linewidth=0.03,linecolor=black](6.875, 7.75)(6.56248, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 7.75)(6.56248, 8)(6.56248, 7.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.75)(6.56248, 8)
\psline[linewidth=0.03,linecolor=black](6.875, 7.75)(6.56248, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.5)(6.875, 7.75)(6.56248, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.75)(6.56248, 8)(6.25, 7.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.75)(6.25, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.5)(6.56248, 7.75)(6.25, 7.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.5)(6.25, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 7.5)(6.56248, 7.5)(6.25, 7.75)
\psline[linewidth=0.03,linecolor=black](6.25, 7.5)(6.56248, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.25)(6.56248, 7.5)(6.25, 7.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.25)(6.25, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.25)(6.25, 7.5)(6.25, 7.25)
\psline[linewidth=0.03,linecolor=black](6.25, 7.5)(6.25, 7.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.25)(6.25, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 7.25)(6.25, 7.25)(6.25, 7)
\psline[linewidth=0.03,linecolor=black](6.25, 7.25)(6.25, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 7.25)(5.93748, 7)(6.25, 7)
\psline[linewidth=0.03,linecolor=black](5.93748, 7)(6.25, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 7)(6.25, 6.75)(6.25, 7)
\psline[linewidth=0.03,linecolor=black](6.25, 6.75)(5.93748, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 6.75)(5.93748, 7)(5.93748, 6.75)
\psline[linewidth=0.03,linecolor=black](6.25, 6.75)(5.93748, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 6.5)(6.25, 6.75)(5.93748, 6.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.5)(6.25, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 6.75)(5.93748, 6.5)(6.25, 6.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.5)(6.25, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 6.5)(5.93748, 6.25)(6.25, 6.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.25)(6.25, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 6.25)(6.25, 6.25)(6.25, 6.5)
\psline[linewidth=0.03,linecolor=black](6.25, 6.25)(5.93748, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 6.25)(5.93748, 6.25)(6.25, 6)
\psline[linewidth=0.03,linecolor=black](6.25, 6.25)(6.25, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6)(6.25, 6.25)(6.25, 6)
\psline[linewidth=0.03,linecolor=black](6.56248, 6)(6.25, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6)(6.25, 6)(6.25, 5.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 6)(6.25, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 5.75)(6.56248, 6)(6.25, 5.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 6)(6.56248, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 6)(6.56248, 5.75)(6.875, 5.75)
\psline[linewidth=0.03,linecolor=black](6.875, 5.75)(6.56248, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 5.75)(6.56248, 5.75)(6.875, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 7.5)(5.93748, 7.25)(6.25, 7.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 7.25)(6.25, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 7.25)(5.93748, 7)(6.25, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8)(6.875, 7.75)(7.18748, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 9.75)(7.5, 9.5)(7.81248, 9.5)
\psline[linewidth=0.03,linecolor=black](7.5, 9.5)(7.81248, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 9.5)(7.81248, 9.25)(7.81248, 9.5)
\psline[linewidth=0.03,linecolor=black](7.5, 9.5)(7.81248, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 9.25)(7.5, 9.5)(7.5, 9.25)
\psline[linewidth=0.03,linecolor=black](7.5, 9.5)(7.5, 9.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 9.25)(7.5, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 9)(7.81248, 9.25)(7.5, 9.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 9)(7.5, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 9)(7.81248, 9)(7.5, 9.25)
\psline[linewidth=0.03,linecolor=black](7.5, 9)(7.81248, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 9)(7.5, 9)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.5, 9)(7.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 9)(7.18748, 8.75)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 8.75)(7.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 8.75)(7.18748, 8.5)(7.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 9.5)(7.18748, 9.25)(7.5, 9.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 9.25)(7.5, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 9.25)(7.5, 9)(7.5, 9.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 9.25)(7.5, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 9)(7.5, 9)(7.18748, 9.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 9)(7.5, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 9)(7.18748, 9)(7.18748, 8.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 9)(7.18748, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 9)(6.875, 8.75)(7.18748, 8.75)
\psline[linewidth=0.03,linecolor=black](6.875, 8.75)(7.18748, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.75)(7.18748, 8.5)(7.18748, 8.75)
\psline[linewidth=0.03,linecolor=black](6.875, 8.75)(7.18748, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 8.5)(6.875, 8.75)(6.875, 8.5)
\psline[linewidth=0.03,linecolor=black](6.875, 8.75)(6.875, 8.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 8.5)(6.875, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.25)(7.18748, 8.5)(6.875, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.75)(6.56248, 8.5)(6.875, 8.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 8.5)(6.875, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 8.5)(6.875, 8.25)(6.875, 8.5)
\psline[linewidth=0.03,linecolor=black](6.875, 8.25)(6.56248, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.25)(6.56248, 8.5)(6.56248, 8.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 8.5)(6.56248, 8.25)
\psline[linewidth=0.03,linecolor=black](6.875, 8.25)(6.56248, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 8)(6.875, 8.25)(6.56248, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 8.5)(6.25, 8.5)(6.56248, 8.25)
\psline[linewidth=0.03,linecolor=black](6.25, 8.5)(6.56248, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.5)(6.25, 8.25)(6.56248, 8.25)
\psline[linewidth=0.03,linecolor=black](6.25, 8.25)(6.56248, 8.25)
\psline[linewidth=0.03,linecolor=black](6.25, 8.25)(6.25, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.25)(6.25, 8.5)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](6.25, 8.25)(5.93748, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 8)(6.25, 8.25)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 8)(5.93748, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8)(5.93748, 8)(5.93748, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.25)(6.56248, 8)(6.56248, 8.25)
\psline[linewidth=0.03,linecolor=black](6.25, 8.25)(6.56248, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 8)(6.25, 8.25)(6.25, 8)
\psline[linewidth=0.03,linecolor=black](6.25, 8.25)(6.25, 8)
\psline[linewidth=0.03,linecolor=black](6.56248, 8)(6.25, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 7.75)(6.56248, 8)(6.25, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.25)(5.93748, 8)(6.25, 8)
\psline[linewidth=0.03,linecolor=black](5.93748, 8)(6.25, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 8)(6.25, 7.75)(6.25, 8)
\psline[linewidth=0.03,linecolor=black](5.93748, 8)(6.25, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 8)(5.93748, 7.75)(6.25, 7.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 7.75)(6.25, 7.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 8)(5.93748, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 8)(5.625, 8)(5.93748, 7.75)
\psline[linewidth=0.03,linecolor=black](5.625, 8)(5.93748, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8)(5.625, 7.75)(5.93748, 7.75)
\psline[linewidth=0.03,linecolor=black](5.625, 7.75)(5.625, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.75)(5.625, 8)(5.3125, 7.75)
\psline[linewidth=0.03,linecolor=black](5.625, 7.75)(5.3125, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 7.5)(5.625, 7.75)(5.3125, 7.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 7.5)(5.3125, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 7.75)(5.3125, 7.5)(5.3125, 7.75)
\psline[linewidth=0.03,linecolor=black](5, 7.75)(5.3125, 7.75)
\psline[linewidth=0.03,linecolor=black](5, 7.75)(5.3125, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 7.5)(5, 7.75)(5, 7.5)
\psline[linewidth=0.03,linecolor=black](5, 7.75)(5, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 7.75)(4.6875, 7.5)(5, 7.5)
\psline[linewidth=0.03,linecolor=black](5, 7.75)(4.6875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 7.75)(4.6875, 7.75)(4.6875, 7.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 7.75)(4.6875, 7.5)
\psline[linewidth=0.03,linecolor=black](5, 7.75)(4.6875, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 7.75)(4.6875, 8)(4.6875, 7.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 8)(4.6875, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8)(4.375, 7.75)(4.6875, 7.75)
\psline[linewidth=0.03,linecolor=black](4.375, 7.75)(4.6875, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 7.75)(4.6875, 8)(4.375, 8)
\psline[linewidth=0.03,linecolor=black](4.6875, 8)(4.375, 8)
\psline[linewidth=0.03,linecolor=black](4.375, 7.75)(4.375, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 7.75)(4.375, 8)(4.06252, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8)(4.375, 8.25)(4.375, 8)
\psline[linewidth=0.03,linecolor=black](4.375, 8)(4.375, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8)(4.375, 8.25)(4.06252, 8)
\psline[linewidth=0.03,linecolor=black](4.375, 8.25)(4.06252, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.25)(4.06252, 8.25)(4.06252, 8)
\psline[linewidth=0.03,linecolor=black](4.06252, 8.25)(4.06252, 8)
\psline[linewidth=0.03,linecolor=black](4.06252, 8.25)(4.375, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 8.25)(4.375, 8.25)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 8.25)(4.06252, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 8.25)(4.06252, 8.25)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](3.75, 8.25)(4.06252, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 8.5)(3.75, 8.25)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](3.75, 8.5)(3.75, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 8.5)(3.75, 8.25)(3.75, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 8.25)(3.75, 8.25)(4.06252, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 7.75)(4.375, 7.5)(4.6875, 7.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 7.75)(4.375, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 7.75)(4.375, 7.5)(4.6875, 7.75)
\psline[linewidth=0.03,linecolor=black](4.375, 7.75)(4.375, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 7.5)(4.375, 7.75)(4.06252, 7.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 7.75)(4.375, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 7.75)(4.375, 7.75)(4.06252, 8)
\psline[linewidth=0.03,linecolor=black](4.06252, 7.75)(4.06252, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 8)(4.06252, 7.75)(4.06252, 8)
\psline[linewidth=0.03,linecolor=black](3.75, 8)(4.06252, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 8.25)(3.75, 8)(4.06252, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 8)(5, 7.75)(5.3125, 7.75)
\psline[linewidth=0.03,linecolor=black](5, 8)(5, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 8)(4.6875, 8)(5, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 7.75)(6.25, 7.5)(6.25, 7.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 7.75)(6.25, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 7.5)(5.93748, 7.75)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 7.75)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](6.25, 7.5)(5.93748, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 7.25)(6.25, 7.5)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 7.25)(5.93748, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.25)(5.93748, 7.25)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](5.625, 7.25)(5.93748, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.25)(5.93748, 7)(5.93748, 7.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 7)(5.625, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 7)(5.625, 7.25)(5.625, 7)
\psline[linewidth=0.03,linecolor=black](5.625, 7.25)(5.625, 7)
\psline[linewidth=0.03,linecolor=black](5.93748, 7)(5.625, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.75)(5.93748, 7)(5.625, 7)
\psline[linewidth=0.03,linecolor=black](5.93748, 7)(5.625, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 7)(5.625, 6.75)(5.93748, 6.75)
\psline[linewidth=0.03,linecolor=black](5.625, 6.75)(5.93748, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.75)(5.93748, 6.5)(5.93748, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.25)(5.3125, 7)(5.625, 7)
\psline[linewidth=0.03,linecolor=black](5.3125, 7)(5.625, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 7)(5.625, 6.75)(5.625, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 7.75)(5.625, 7.75)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](5.625, 7.75)(5.93748, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.75)(5.625, 7.5)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](5.625, 7.5)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](5.625, 7.5)(5.625, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.5)(5.625, 7.75)(5.3125, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.5)(5.625, 7.25)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](5.625, 7.25)(5.625, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.25)(5.625, 7.5)(5.3125, 7.5)
\psline[linewidth=0.03,linecolor=black](5.625, 7.25)(5.3125, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 7.25)(5.3125, 7.5)(5.3125, 7.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 7.5)(5.3125, 7.25)
\psline[linewidth=0.03,linecolor=black](5.625, 7.25)(5.3125, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 7)(5.625, 7.25)(5.3125, 7.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 7)(5.3125, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 7.25)(5.3125, 7)(5.3125, 7.25)
\psline[linewidth=0.03,linecolor=black](5, 7.25)(5.3125, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 7)(5.3125, 7)(5, 7.25)
\psline[linewidth=0.03,linecolor=black](5, 7)(5, 7.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 7)(5, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 7)(5, 7)(5, 6.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 7)(5, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 6.75)(5.3125, 7)(5, 6.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 7)(5.3125, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.75)(5.3125, 7)(5.3125, 6.75)
\psline[linewidth=0.03,linecolor=black](5.625, 6.75)(5.3125, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.75)(5.3125, 6.75)(5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.75)(5.3125, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.5)(5.625, 6.75)(5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.5)(5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.75)(5.625, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.75)(5.625, 6.5)(5.93748, 6.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.5)(5.93748, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.5)(5.93748, 6.25)(5.93748, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.25)(5.625, 6.5)(5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.25)(5.625, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 6.25)(5.93748, 6.25)(5.625, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 7)(5, 7.25)(4.6875, 7.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 7.25)(5, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 7.25)(5, 7.25)(4.6875, 7.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 7.25)(4.6875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 7.5)(4.6875, 7.25)(4.6875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 7.5)(5, 7.25)(5.3125, 7.25)
\psline[linewidth=0.03,linecolor=black](5, 7.25)(5.3125, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 7.25)(5.3125, 7.5)(5, 7.5)
\psline[linewidth=0.03,linecolor=black](5, 7.25)(5, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 7.5)(5, 7.25)(5, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 10)(7.5, 10)(7.5, 9.75)
\psline[linewidth=0.03,linecolor=black](7.5, 10)(7.5, 9.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 10)(7.5, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 10)(7.18748, 9.75)(7.5, 9.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 9.75)(7.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 9.75)(7.5, 9.5)(7.5, 9.75)
\psline[linewidth=0.03,linecolor=black](7.5, 9.5)(7.18748, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 9.5)(7.18748, 9.75)(7.18748, 9.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 9.75)(7.18748, 9.5)
\psline[linewidth=0.03,linecolor=black](7.5, 9.5)(7.18748, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 9.25)(7.5, 9.5)(7.18748, 9.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 9.25)(7.18748, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9.5)(7.18748, 9.25)(7.18748, 9.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 9.25)(6.875, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 9.25)(6.875, 9.5)(6.875, 9.25)
\psline[linewidth=0.03,linecolor=black](6.875, 9.5)(6.875, 9.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 9.25)(6.875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 9)(7.18748, 9.25)(6.875, 9.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 9)(6.875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9)(7.18748, 9)(6.875, 9.25)
\psline[linewidth=0.03,linecolor=black](6.875, 9)(6.875, 9.25)
\psline[linewidth=0.03,linecolor=black](6.875, 9)(7.18748, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.75)(7.18748, 9)(6.875, 9)
\psline[linewidth=0.03,linecolor=black](6.875, 8.75)(6.875, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 9)(6.875, 8.75)(6.875, 9)
\psline[linewidth=0.03,linecolor=black](6.56248, 9)(6.875, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.75)(6.56248, 9)(6.56248, 8.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 9)(6.56248, 8.75)
\psline[linewidth=0.03,linecolor=black](6.875, 8.75)(6.56248, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 8.75)(6.56248, 8.75)(6.56248, 8.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 8.75)(6.56248, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 8.75)(6.25, 8.75)(6.56248, 8.5)
\psline[linewidth=0.03,linecolor=black](6.25, 8.75)(6.56248, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.75)(6.25, 8.5)(6.56248, 8.5)
\psline[linewidth=0.03,linecolor=black](6.25, 8.5)(6.25, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.5)(6.25, 8.75)(5.93748, 8.5)
\psline[linewidth=0.03,linecolor=black](6.25, 8.5)(5.93748, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.5)(5.93748, 8.5)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 8.5)(5.93748, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 8.5)(5.625, 8.5)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](5.625, 8.5)(5.93748, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8.5)(5.625, 8.25)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](5.625, 8.25)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](5.625, 8.5)(5.625, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8.5)(5.3125, 8.25)(5.625, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8.25)(5.625, 8)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](5.625, 8.25)(5.625, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8.25)(5.625, 8)(5.625, 8.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.25)(5.625, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8)(5.3125, 8.25)(5.3125, 8)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.25)(5.3125, 8)
\psline[linewidth=0.03,linecolor=black](5.625, 8)(5.3125, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8)(5.3125, 8)(5.3125, 7.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 8)(5.3125, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8)(5, 8)(5.3125, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8.25)(5, 8)(5.3125, 8)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.25)(5, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 8)(5.3125, 8.25)(5, 8.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.25)(5, 8.25)
\psline[linewidth=0.03,linecolor=black](5, 8)(5, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8)(5, 8)(5, 8.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 8)(5, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8.25)(4.6875, 8)(5, 8.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.25)(4.6875, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.25)(4.6875, 8)(4.6875, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 8.25)(5.3125, 8.25)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](5, 8.25)(5, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8.25)(5, 8.25)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.25)(5, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8.5)(4.6875, 8.25)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.5)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.5)(4.6875, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.25)(4.6875, 8.25)(4.6875, 8.5)
\psline[linewidth=0.03,linecolor=black](4.375, 8.25)(4.6875, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.5)(4.375, 8.25)(4.6875, 8.5)
\psline[linewidth=0.03,linecolor=black](4.375, 8.5)(4.6875, 8.5)
\psline[linewidth=0.03,linecolor=black](4.375, 8.25)(4.375, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.25)(4.375, 8.5)(4.06252, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.75)(4.375, 8.5)(4.6875, 8.5)
\psline[linewidth=0.03,linecolor=black](4.375, 8.5)(4.375, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.5)(4.375, 8.75)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](4.375, 8.75)(4.06252, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.75)(4.06252, 8.75)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 8.75)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](4.375, 8.75)(4.06252, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 8.75)(4.375, 8.75)(4.06252, 9)
\psline[linewidth=0.03,linecolor=black](4.06252, 8.75)(4.06252, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9)(4.06252, 8.75)(4.06252, 9)
\psline[linewidth=0.03,linecolor=black](3.75, 9)(4.06252, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.25)(3.75, 9)(4.06252, 9)
\psline[linewidth=0.03,linecolor=black](3.75, 9.25)(3.75, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9)(3.75, 9.25)(3.43752, 9)
\psline[linewidth=0.03,linecolor=black](3.75, 9.25)(3.43752, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.25)(3.43752, 9.25)(3.43752, 9)
\psline[linewidth=0.03,linecolor=black](3.43752, 9.25)(3.43752, 9)
\psline[linewidth=0.03,linecolor=black](3.75, 9.25)(3.43752, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.25)(3.43752, 9.5)(3.43752, 9.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 9.25)(3.43752, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 9.25)(3.43752, 9.5)(3.125, 9.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 9.5)(3.125, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 9.5)(3.125, 9.5)(3.125, 9.25)
\psline[linewidth=0.03,linecolor=black](3.125, 9.5)(3.125, 9.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 9.5)(3.125, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 9.5)(3.125, 9.75)(3.125, 9.5)
\psline[linewidth=0.03,linecolor=black](3.125, 9.5)(3.125, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 9.5)(3.125, 9.75)(2.81252, 9.5)
\psline[linewidth=0.03,linecolor=black](3.125, 9.75)(2.81252, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 9.75)(2.81252, 9.75)(2.81252, 9.5)
\psline[linewidth=0.03,linecolor=black](3.125, 9.75)(2.81252, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 9.75)(2.81252, 10)(2.81252, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 9.5)(2.81252, 9.25)(3.125, 9.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 9.25)(3.125, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](2.81252, 9.25)(3.125, 9.5)(2.81252, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 9.25)(3.125, 9)(3.43752, 9)
\psline[linewidth=0.03,linecolor=black](3.125, 9)(3.43752, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 9)(3.43752, 9.25)(3.125, 9.25)
\psline[linewidth=0.03,linecolor=black](3.125, 9)(3.125, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](2.81252, 9.25)(3.125, 9)(3.125, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 8.75)(3.75, 8.5)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](3.75, 8.5)(4.06252, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 8.75)(3.75, 8.5)(4.06252, 8.75)
\psline[linewidth=0.03,linecolor=black](3.75, 8.75)(4.06252, 8.75)
\psline[linewidth=0.03,linecolor=black](3.75, 8.75)(3.75, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 8.5)(3.75, 8.5)(3.75, 8.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.5)(3.75, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 8.5)(3.75, 8.75)(3.43752, 8.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.5)(3.43752, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 8.75)(3.43752, 8.5)(3.43752, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9)(3.75, 8.75)(4.06252, 8.75)
\psline[linewidth=0.03,linecolor=black](3.75, 8.75)(3.75, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 8.75)(3.75, 9)(3.43752, 8.75)
\psline[linewidth=0.03,linecolor=black](3.75, 9)(3.43752, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 8.75)(3.75, 9)(3.43752, 9)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.75)(3.43752, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 8.75)(3.43752, 8.75)(3.43752, 9)
\psline[linewidth=0.03,linecolor=black](3.125, 8.75)(3.43752, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 9)(3.125, 8.75)(3.43752, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8.75)(4.6875, 8.5)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.75)(4.6875, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8.75)(4.375, 8.75)(4.6875, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 9)(6.25, 8.75)(6.56248, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 9)(6.875, 9)(6.875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9.5)(6.56248, 9.25)(6.875, 9.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 9.25)(6.875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 9.25)(6.56248, 9)(6.875, 9.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 9)(6.56248, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 9)(6.56248, 9.25)(6.25, 9.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 9)(6.25, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 9)(6.56248, 9)(6.25, 9.25)
\psline[linewidth=0.03,linecolor=black](6.25, 9)(6.25, 9.25)
\psline[linewidth=0.03,linecolor=black](6.25, 9)(6.56248, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.75)(6.56248, 9)(6.25, 9)
\psline[linewidth=0.03,linecolor=black](6.25, 8.75)(6.25, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 9)(6.25, 8.75)(6.25, 9)
\psline[linewidth=0.03,linecolor=black](5.93748, 9)(6.25, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.75)(5.93748, 9)(5.93748, 8.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 9)(5.93748, 8.75)
\psline[linewidth=0.03,linecolor=black](6.25, 8.75)(5.93748, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 8.75)(5.93748, 8.75)(5.93748, 8.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 8.75)(5.93748, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 8.75)(5.625, 8.75)(5.93748, 8.5)
\psline[linewidth=0.03,linecolor=black](5.625, 8.75)(5.93748, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8.75)(5.625, 8.5)(5.93748, 8.5)
\psline[linewidth=0.03,linecolor=black](5.625, 8.75)(5.625, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8.5)(5.625, 8.75)(5.3125, 8.5)
\psline[linewidth=0.03,linecolor=black](5.625, 8.5)(5.3125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8.25)(5.625, 8.5)(5.3125, 8.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.25)(5.3125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8.25)(5.3125, 8.5)(5, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 9)(5.625, 9)(5.93748, 8.75)
\psline[linewidth=0.03,linecolor=black](5.625, 9)(5.93748, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9)(5.625, 8.75)(5.93748, 8.75)
\psline[linewidth=0.03,linecolor=black](5.625, 8.75)(5.625, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8.75)(5.625, 9)(5.3125, 8.75)
\psline[linewidth=0.03,linecolor=black](5.625, 8.75)(5.3125, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 8.75)(5.3125, 8.75)(5.3125, 8.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.5)(5.3125, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8.5)(5.3125, 8.75)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](5, 8.5)(5.3125, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 8.5)(5.3125, 8.75)(5, 8.75)
\psline[linewidth=0.03,linecolor=black](5, 8.5)(5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 8.75)(5, 8.5)(5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 9)(6.25, 9)(6.25, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 9.75)(6.875, 9.75)(7.18748, 9.5)
\psline[linewidth=0.03,linecolor=black](6.875, 9.75)(7.18748, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9.75)(6.875, 9.5)(7.18748, 9.5)
\psline[linewidth=0.03,linecolor=black](6.875, 9.5)(6.875, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9.5)(6.875, 9.75)(6.56248, 9.5)
\psline[linewidth=0.03,linecolor=black](6.875, 9.5)(6.56248, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 9.25)(6.875, 9.5)(6.56248, 9.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 9.25)(6.56248, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 9.5)(6.56248, 9.25)(6.56248, 9.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 9.25)(6.25, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 9.25)(6.25, 9.5)(6.25, 9.25)
\psline[linewidth=0.03,linecolor=black](6.25, 9.5)(6.25, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 9.5)(5.93748, 9.25)(6.25, 9.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 9.25)(6.25, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 9.25)(5.93748, 9)(6.25, 9.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 9.25)(5.93748, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9)(5.93748, 9)(5.93748, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 10)(7.18748, 9.75)(7.5, 10)
\psline[linewidth=0.03,linecolor=black](7.18748, 10)(7.5, 10)
\psline[linewidth=0.03,linecolor=black](7.18748, 10)(7.18748, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9.75)(7.18748, 9.75)(7.18748, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9.75)(7.18748, 10)(6.875, 10)
\psline[linewidth=0.03,linecolor=black](7.18748, 10)(6.875, 10)
\psline[linewidth=0.03,linecolor=black](6.875, 9.75)(6.875, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 10)(6.875, 9.75)(6.875, 10)
\psline[linewidth=0.03,linecolor=black](6.875, 9.75)(6.56248, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9.75)(6.56248, 10)(6.56248, 9.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 10)(6.56248, 9.75)
\psline[linewidth=0.03,linecolor=black](6.875, 9.75)(6.56248, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 9.75)(6.56248, 9.75)(6.56248, 9.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 9.75)(6.56248, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 9.75)(6.25, 9.75)(6.56248, 9.5)
\psline[linewidth=0.03,linecolor=black](6.25, 9.75)(6.56248, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 9.75)(6.25, 9.5)(6.56248, 9.5)
\psline[linewidth=0.03,linecolor=black](6.25, 9.5)(6.25, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 9.5)(6.25, 9.75)(5.93748, 9.5)
\psline[linewidth=0.03,linecolor=black](6.25, 9.5)(5.93748, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 9.25)(6.25, 9.5)(5.93748, 9.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 9.25)(5.93748, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9.5)(5.93748, 9.25)(5.93748, 9.5)
\psline[linewidth=0.03,linecolor=black](5.625, 9.5)(5.93748, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9.5)(5.625, 9.25)(5.93748, 9.25)
\psline[linewidth=0.03,linecolor=black](5.625, 9.25)(5.93748, 9.25)
\psline[linewidth=0.03,linecolor=black](5.625, 9.5)(5.625, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9.25)(5.625, 9.5)(5.3125, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9.25)(5.625, 9)(5.93748, 9.25)
\psline[linewidth=0.03,linecolor=black](5.625, 9)(5.625, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9)(5.625, 9.25)(5.3125, 9.25)
\psline[linewidth=0.03,linecolor=black](5.625, 9)(5.3125, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 9)(5.625, 9)(5.3125, 9.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 9)(5.3125, 9.25)
\psline[linewidth=0.03,linecolor=black](5.625, 9)(5.3125, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8.75)(5.625, 9)(5.3125, 9)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.75)(5.3125, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8.75)(5.3125, 9)(5, 9)
\psline[linewidth=0.03,linecolor=black](5.3125, 9)(5, 9)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.75)(5, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 8.75)(5, 9)(5, 8.75)
\psline[linewidth=0.03,linecolor=black](5, 9)(5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 9)(4.6875, 8.75)(5, 8.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.75)(5, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9)(4.6875, 8.75)(5, 9)
\psline[linewidth=0.03,linecolor=black](4.6875, 9)(4.6875, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.75)(4.6875, 8.75)(4.6875, 9)
\psline[linewidth=0.03,linecolor=black](4.375, 8.75)(4.6875, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 9)(4.375, 8.75)(4.6875, 9)
\psline[linewidth=0.03,linecolor=black](4.375, 8.75)(4.375, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 8.75)(4.375, 9)(4.06252, 9)
\psline[linewidth=0.03,linecolor=black](4.375, 9)(4.06252, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 9)(4.06252, 9.25)(4.06252, 9)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.25)(4.06252, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 9.25)(3.75, 9.25)(4.06252, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 9)(5, 9.25)(5, 9)
\psline[linewidth=0.03,linecolor=black](5, 9.25)(5, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 9.25)(4.6875, 9)(5, 9)
\psline[linewidth=0.03,linecolor=black](5, 9.25)(4.6875, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 9.25)(4.6875, 9.25)(4.6875, 9)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.25)(4.6875, 9)
\psline[linewidth=0.03,linecolor=black](5, 9.25)(4.6875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.25)(5, 9.25)(4.6875, 9.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.25)(4.6875, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 9.5)(4.6875, 9.25)(4.6875, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.25)(4.375, 9)(4.6875, 9)
\psline[linewidth=0.03,linecolor=black](4.375, 9)(4.6875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 9)(4.6875, 9.25)(4.375, 9.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.25)(4.375, 9.25)
\psline[linewidth=0.03,linecolor=black](4.375, 9)(4.375, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 9.25)(4.375, 9)(4.375, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.25)(4.375, 9.5)(4.375, 9.25)
\psline[linewidth=0.03,linecolor=black](4.375, 9.5)(4.375, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 9.5)(4.06252, 9.25)(4.375, 9.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.25)(4.375, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 9.25)(4.375, 9.5)(4.06252, 9.5)
\psline[linewidth=0.03,linecolor=black](4.375, 9.5)(4.06252, 9.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.25)(4.06252, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.25)(4.06252, 9.25)(4.06252, 9.5)
\psline[linewidth=0.03,linecolor=black](3.75, 9.25)(4.06252, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.5)(3.75, 9.25)(4.06252, 9.5)
\psline[linewidth=0.03,linecolor=black](3.75, 9.5)(3.75, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.25)(3.75, 9.5)(3.43752, 9.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 9.5)(3.75, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 9.5)(3.75, 9.5)(3.43752, 9.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 9.5)(3.43752, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 9.75)(3.43752, 9.5)(3.43752, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 9.5)(4.06252, 9.75)(4.06252, 9.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.75)(4.06252, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 9.75)(3.75, 9.5)(4.06252, 9.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.75)(3.75, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.5)(4.06252, 9.75)(3.75, 9.75)
\psline[linewidth=0.03,linecolor=black](3.75, 9.75)(4.06252, 9.75)
\psline[linewidth=0.03,linecolor=black](3.75, 9.5)(3.75, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.5)(3.75, 9.75)(3.43752, 9.75)
\psline[linewidth=0.03,linecolor=black](3.75, 9.75)(3.43752, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.75)(3.43752, 10)(3.43752, 9.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 10)(3.43752, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 10)(3.125, 9.75)(3.43752, 9.75)
\psline[linewidth=0.03,linecolor=black](3.125, 9.75)(3.43752, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.125, 9.75)(3.43752, 10)(3.125, 10)
\psline[linewidth=0.03,linecolor=black](3.125, 9.75)(3.125, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](2.81252, 10)(3.125, 9.75)(3.125, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.75, 9.75)(4.06252, 9.75)(3.75, 10)
\psline[linewidth=0.03,linecolor=black](3.75, 9.75)(3.75, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](3.43752, 10)(3.75, 9.75)(3.75, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 9.25)(5.3125, 9)(5.3125, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.56248, 10)(6.25, 9.75)(6.56248, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 9.75)(6.56248, 10)(6.25, 10)
\psline[linewidth=0.03,linecolor=black](6.56248, 10)(6.25, 10)
\psline[linewidth=0.03,linecolor=black](6.25, 9.75)(6.25, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 10)(6.25, 9.75)(6.25, 10)
\psline[linewidth=0.03,linecolor=black](5.93748, 10)(6.25, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.25, 9.75)(5.93748, 10)(5.93748, 9.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 10)(5.93748, 9.75)
\psline[linewidth=0.03,linecolor=black](6.25, 9.75)(5.93748, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 9.5)(6.25, 9.75)(5.93748, 9.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 9.5)(5.93748, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9.5)(5.93748, 9.5)(5.93748, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 10)(5.625, 9.75)(5.93748, 9.75)
\psline[linewidth=0.03,linecolor=black](5.625, 9.75)(5.93748, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9.75)(5.625, 9.5)(5.93748, 9.75)
\psline[linewidth=0.03,linecolor=black](5.625, 9.75)(5.625, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 9.75)(5.625, 9.5)(5.625, 9.75)
\psline[linewidth=0.03,linecolor=black](5.625, 9.5)(5.3125, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 9.5)(5.625, 9.5)(5.3125, 9.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 9.5)(5.3125, 9.75)
\psline[linewidth=0.03,linecolor=black](5.625, 9.5)(5.3125, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 9.5)(5.3125, 9.5)(5.3125, 9.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 9.5)(5.3125, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 9.5)(5, 9.25)(5.3125, 9.25)
\psline[linewidth=0.03,linecolor=black](5, 9.25)(5.3125, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 9.25)(5.3125, 9.5)(5, 9.5)
\psline[linewidth=0.03,linecolor=black](5, 9.25)(5, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.5)(5, 9.25)(5, 9.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.5)(5, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.75)(4.6875, 9.5)(5, 9.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.75)(4.6875, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.75)(4.375, 9.5)(4.6875, 9.5)
\psline[linewidth=0.03,linecolor=black](4.375, 9.5)(4.6875, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 9.5)(4.6875, 9.75)(4.375, 9.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.75)(4.375, 9.75)
\psline[linewidth=0.03,linecolor=black](4.375, 9.5)(4.375, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 9.75)(4.375, 9.5)(4.375, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.75)(4.375, 10)(4.375, 9.75)
\psline[linewidth=0.03,linecolor=black](4.375, 10)(4.375, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.375, 10)(4.06252, 9.75)(4.375, 9.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.75)(4.375, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 10)(4.06252, 9.75)(4.375, 10)
\psline[linewidth=0.03,linecolor=black](4.06252, 10)(4.06252, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.06252, 9.75)(4.06252, 10)(3.75, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 9.5)(5.3125, 9.75)(5, 9.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 9.5)(5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 9.5)(5, 9.75)(5, 9.5)
\psline[linewidth=0.03,linecolor=black](5, 9.75)(5, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 9.75)(4.6875, 9.75)(5, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.93748, 10)(5.625, 10)(5.625, 9.75)
\psline[linewidth=0.03,linecolor=black](5.625, 10)(5.625, 9.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 10)(5.625, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.625, 10)(5.3125, 10)(5.625, 9.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 10)(5.625, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 10)(5.3125, 9.75)(5.625, 9.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 9.75)(5.3125, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5.3125, 9.75)(5.3125, 10)(5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](5, 9.75)(5.3125, 10)(5, 10)
\psline[linewidth=0.03,linecolor=black](5.3125, 10)(5, 10)
\psline[linewidth=0.03,linecolor=black](5, 9.75)(5, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.75)(5, 9.75)(5, 10)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.75)(5, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 10)(4.6875, 9.75)(5, 10)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.75)(4.6875, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](4.6875, 9.75)(4.6875, 10)(4.375, 10)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9.75)(10, 9.75)(10, 10)
\psline[linewidth=0.03,linecolor=black](10, 9.75)(10, 10)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.75)(10, 9.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 9.75)(9.68742, 9.75)(10, 9.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.75)(10, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 9.5)(9.68742, 9.75)(9.68742, 9.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.75)(9.68742, 9.5)
\psline[linewidth=0.03,linecolor=black](10, 9.5)(9.68742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9.25)(10, 9.5)(9.68742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9.75)(9.37484, 9.5)(9.68742, 9.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.5)(9.68742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9.5)(9.68742, 9.25)(9.68742, 9.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.5)(9.68742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9.5)(9.37484, 9.25)(9.68742, 9.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.25)(9.68742, 9.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.5)(9.37484, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9.25)(9.37484, 9.5)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.25)(9.06258, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9)(9.37484, 9.25)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 9)(9.06258, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 9)(9.37484, 9)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 9)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 9)(9.06258, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9)(9.06258, 9)(9.06258, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9)(9.06258, 9)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 9)(8.75, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 9)(8.75, 9)(9.06258, 8.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.75)(8.75, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8.75)(8.75, 9)(8.75, 8.75)
\psline[linewidth=0.03,linecolor=black](8.75, 9)(8.75, 8.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.75)(8.75, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 8.5)(9.06258, 8.75)(8.75, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 9)(8.43742, 8.75)(8.75, 8.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.75)(8.75, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8.75)(8.75, 8.5)(8.75, 8.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.75)(8.75, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8.75)(8.43742, 8.5)(8.75, 8.5)
\psline[linewidth=0.03,linecolor=black](8.75, 8.5)(8.43742, 8.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.75)(8.43742, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8.5)(8.43742, 8.75)(8.125, 8.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.5)(8.125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 8.25)(8.43742, 8.5)(8.125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 8.5)(8.43742, 8.5)(8.75, 8.25)
\psline[linewidth=0.03,linecolor=black](8.75, 8.25)(8.43742, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 8.25)(8.43742, 8.5)(8.43742, 8.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.5)(8.43742, 8.25)
\psline[linewidth=0.03,linecolor=black](8.75, 8.25)(8.43742, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8)(8.75, 8.25)(8.43742, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8.5)(8.125, 8.25)(8.43742, 8.25)
\psline[linewidth=0.03,linecolor=black](8.125, 8.25)(8.43742, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 8.25)(8.43742, 8)(8.43742, 8.25)
\psline[linewidth=0.03,linecolor=black](8.125, 8.25)(8.43742, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 8.25)(8.125, 8)(8.43742, 8)
\psline[linewidth=0.03,linecolor=black](8.125, 8)(8.43742, 8)
\psline[linewidth=0.03,linecolor=black](8.125, 8.25)(8.125, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 8)(8.125, 8.25)(7.81248, 8)
\psline[linewidth=0.03,linecolor=black](8.125, 8)(7.81248, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 7.75)(8.125, 8)(7.81248, 8)
\psline[linewidth=0.03,linecolor=black](8.125, 7.75)(7.81248, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 7.75)(8.125, 7.75)(7.81248, 8)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.75)(8.125, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 7.5)(8.125, 7.75)(7.81248, 7.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.5)(7.81248, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7.5)(7.81248, 7.5)(7.81248, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 7.5)(7.81248, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7.5)(7.81248, 7.25)(7.81248, 7.5)
\psline[linewidth=0.03,linecolor=black](7.5, 7.5)(7.81248, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7.5)(7.5, 7.25)(7.81248, 7.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.25)(7.5, 7.25)
\psline[linewidth=0.03,linecolor=black](7.5, 7.5)(7.5, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7.5)(7.18748, 7.25)(7.5, 7.25)
\psline[linewidth=0.03,linecolor=black](7.5, 7.25)(7.18748, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7.25)(7.18748, 7.25)(7.5, 7)
\psline[linewidth=0.03,linecolor=black](7.18748, 7.25)(7.5, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 7.25)(7.18748, 7)(7.5, 7)
\psline[linewidth=0.03,linecolor=black](7.18748, 7)(7.5, 7)
\psline[linewidth=0.03,linecolor=black](7.18748, 7)(7.18748, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 7)(7.18748, 7.25)(6.875, 7)
\psline[linewidth=0.03,linecolor=black](7.18748, 7)(6.875, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.75)(7.18748, 7)(6.875, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 7)(7.18748, 6.75)(7.5, 7)
\psline[linewidth=0.03,linecolor=black](7.18748, 7)(7.18748, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.75)(7.18748, 6.75)(7.18748, 7)
\psline[linewidth=0.03,linecolor=black](7.18748, 6.75)(6.875, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 6.75)(6.875, 6.75)(7.18748, 6.5)
\psline[linewidth=0.03,linecolor=black](6.875, 6.75)(7.18748, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.75)(6.875, 6.5)(7.18748, 6.5)
\psline[linewidth=0.03,linecolor=black](6.875, 6.5)(7.18748, 6.5)
\psline[linewidth=0.03,linecolor=black](6.875, 6.5)(6.875, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.5)(6.875, 6.75)(6.56248, 6.5)
\psline[linewidth=0.03,linecolor=black](6.875, 6.5)(6.56248, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.25)(6.875, 6.5)(6.56248, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.5)(6.875, 6.25)(7.18748, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 7.25)(7.5, 7.25)(7.81248, 7)
\psline[linewidth=0.03,linecolor=black](7.81248, 7)(7.5, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 7)(7.5, 7.25)(7.5, 7)
\psline[linewidth=0.03,linecolor=black](7.81248, 7)(7.5, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.75)(7.81248, 7)(7.5, 7)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.75)(7.5, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.75)(7.5, 7)(7.5, 6.75)
\psline[linewidth=0.03,linecolor=black](7.5, 7)(7.5, 6.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.75)(7.5, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.5)(7.81248, 6.75)(7.5, 6.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.5)(7.5, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 6.5)(7.81248, 6.5)(7.5, 6.75)
\psline[linewidth=0.03,linecolor=black](7.5, 6.5)(7.81248, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.25)(7.81248, 6.5)(7.5, 6.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.25)(7.5, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 6.25)(7.81248, 6.25)(7.5, 6.5)
\psline[linewidth=0.03,linecolor=black](7.5, 6.25)(7.5, 6.5)
\psline[linewidth=0.03,linecolor=black](7.5, 6.25)(7.81248, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.25)(7.5, 6.25)(7.5, 6)
\psline[linewidth=0.03,linecolor=black](7.5, 6.25)(7.5, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 6.25)(7.18748, 6)(7.5, 6)
\psline[linewidth=0.03,linecolor=black](7.18748, 6)(7.5, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 6)(7.18748, 6)(7.5, 5.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 6)(7.5, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 6)(7.18748, 5.75)(7.5, 5.75)
\psline[linewidth=0.03,linecolor=black](7.5, 5.75)(7.18748, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 5.75)(7.18748, 5.75)(7.5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 6.25)(7.5, 6.25)(7.5, 6.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 6.25)(7.5, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 6.25)(7.18748, 6)(7.5, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 7)(7.18748, 6.75)(7.5, 6.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 6.75)(7.5, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 6.75)(7.5, 6.5)(7.5, 6.75)
\psline[linewidth=0.03,linecolor=black](7.5, 6.5)(7.18748, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 6.5)(7.18748, 6.75)(7.18748, 6.5)
\psline[linewidth=0.03,linecolor=black](7.5, 6.5)(7.18748, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.18748, 6.25)(7.5, 6.5)(7.18748, 6.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 6.25)(7.18748, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.25)(7.18748, 6.25)(7.18748, 6.5)
\psline[linewidth=0.03,linecolor=black](6.875, 6.25)(7.18748, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](6.875, 6.25)(7.18748, 6)(7.18748, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 8)(8.125, 7.75)(8.43742, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9.25)(9.37484, 9)(9.68742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 9.5)(9.68742, 9.25)(10, 9.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.25)(10, 9.25)
\psline[linewidth=0.03,linecolor=black](10, 9.5)(10, 9.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9.25)(9.68742, 9)(10, 9.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.25)(9.68742, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9)(9.68742, 9)(9.68742, 9.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 9)(9.37484, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9)(9.37484, 9)(9.68742, 8.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 9)(9.68742, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9)(9.37484, 8.75)(9.68742, 8.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 8.75)(9.68742, 8.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 9)(9.37484, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 9)(9.06258, 8.75)(9.37484, 8.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.75)(9.37484, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8.75)(9.37484, 8.5)(9.37484, 8.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.75)(9.37484, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 8.5)(9.06258, 8.75)(9.06258, 8.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.75)(9.06258, 8.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 8.5)(9.06258, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8.25)(9.37484, 8.5)(9.06258, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8.75)(8.75, 8.5)(9.06258, 8.5)
\psline[linewidth=0.03,linecolor=black](8.75, 8.5)(9.06258, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 8.5)(9.06258, 8.25)(9.06258, 8.5)
\psline[linewidth=0.03,linecolor=black](8.75, 8.5)(9.06258, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8.25)(8.75, 8.5)(8.75, 8.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.25)(8.75, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8.25)(8.75, 8.25)(8.75, 8)
\psline[linewidth=0.03,linecolor=black](8.75, 8.25)(8.75, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 8.25)(8.43742, 8)(8.75, 8)
\psline[linewidth=0.03,linecolor=black](8.43742, 8)(8.75, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8)(8.75, 7.75)(8.75, 8)
\psline[linewidth=0.03,linecolor=black](8.43742, 8)(8.75, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 7.75)(8.43742, 8)(8.43742, 7.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 8)(8.43742, 7.75)
\psline[linewidth=0.03,linecolor=black](8.75, 7.75)(8.43742, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 7.5)(8.75, 7.75)(8.43742, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 8)(8.125, 7.75)(8.43742, 7.75)
\psline[linewidth=0.03,linecolor=black](8.125, 7.75)(8.43742, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 7.75)(8.43742, 7.5)(8.43742, 7.75)
\psline[linewidth=0.03,linecolor=black](8.125, 7.75)(8.43742, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 7.5)(8.125, 7.75)(8.125, 7.5)
\psline[linewidth=0.03,linecolor=black](8.125, 7.75)(8.125, 7.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 7.5)(8.125, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 7.25)(8.43742, 7.5)(8.125, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 7.75)(7.81248, 7.5)(8.125, 7.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.5)(8.125, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 7.5)(8.125, 7.25)(8.125, 7.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.5)(8.125, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 7.25)(8.125, 7.25)(7.81248, 7.5)
\psline[linewidth=0.03,linecolor=black](8.125, 7.25)(7.81248, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 7.25)(7.81248, 7.25)(7.81248, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 8.75)(9.37484, 8.5)(9.68742, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9)(10, 9)(10, 9.25)
\psline[linewidth=0.03,linecolor=black](10, 9)(10, 9.25)
\psline[linewidth=0.03,linecolor=black](10, 9)(9.68742, 9)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 9)(9.68742, 9)(10, 8.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 9)(10, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 9)(9.68742, 8.75)(10, 8.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.75)(10, 8.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 8.75)(9.68742, 8.5)(10, 8.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.75)(9.68742, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 8.5)(9.68742, 8.5)(9.68742, 8.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 8.5)(9.68742, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 8.5)(9.68742, 8.25)(9.68742, 8.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 8.5)(9.68742, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 8.25)(9.37484, 8.5)(9.37484, 8.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 8.5)(9.37484, 8.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.25)(9.37484, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 8)(9.68742, 8.25)(9.37484, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 8.5)(9.06258, 8.25)(9.37484, 8.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.25)(9.37484, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8.25)(9.37484, 8)(9.37484, 8.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.25)(9.37484, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 8)(9.06258, 8.25)(9.06258, 8)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.25)(9.06258, 8)
\psline[linewidth=0.03,linecolor=black](9.37484, 8)(9.06258, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7.75)(9.37484, 8)(9.06258, 8)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.75)(9.06258, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7.75)(9.06258, 8)(9.06258, 7.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 8)(9.06258, 7.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.75)(9.06258, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 7.5)(9.37484, 7.75)(9.06258, 7.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 7.5)(9.06258, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 7.5)(9.06258, 7.5)(9.06258, 7.75)
\psline[linewidth=0.03,linecolor=black](8.75, 7.5)(9.06258, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 7.5)(8.75, 7.25)(9.06258, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8)(8.75, 7.75)(9.06258, 7.75)
\psline[linewidth=0.03,linecolor=black](8.75, 7.75)(9.06258, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 7.75)(8.75, 7.5)(9.06258, 7.75)
\psline[linewidth=0.03,linecolor=black](8.75, 7.75)(8.75, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 7.5)(8.75, 7.5)(8.75, 7.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 7.5)(8.75, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 7.5)(8.75, 7.25)(8.75, 7.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 7.5)(8.75, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 7.25)(8.75, 7.25)(8.43742, 7.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 7.25)(8.43742, 7.5)
\psline[linewidth=0.03,linecolor=black](8.75, 7.25)(8.43742, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 7.25)(8.43742, 7.25)(8.43742, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 7.25)(8.43742, 7.25)(8.43742, 7.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 7.25)(8.125, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 7.25)(8.125, 7.25)(8.43742, 7)
\psline[linewidth=0.03,linecolor=black](8.43742, 7)(8.125, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 7)(8.125, 7.25)(8.125, 7)
\psline[linewidth=0.03,linecolor=black](8.125, 7.25)(8.125, 7)
\psline[linewidth=0.03,linecolor=black](8.43742, 7)(8.125, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 6.75)(8.43742, 7)(8.125, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 7.25)(7.81248, 7)(8.125, 7)
\psline[linewidth=0.03,linecolor=black](7.81248, 7)(8.125, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 7)(8.125, 6.75)(8.125, 7)
\psline[linewidth=0.03,linecolor=black](8.125, 6.75)(7.81248, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.75)(8.125, 6.75)(7.81248, 7)
\psline[linewidth=0.03,linecolor=black](8.125, 6.75)(7.81248, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.5)(8.125, 6.75)(7.81248, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 8)(9.06258, 8.25)(8.75, 8)
\psline[linewidth=0.03,linecolor=black](9.06258, 8)(8.75, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 7.75)(9.06258, 8)(8.75, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 8.75)(9.68742, 8.5)(10, 8.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.5)(10, 8.5)
\psline[linewidth=0.03,linecolor=black](10, 8.75)(10, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 8.5)(9.68742, 8.25)(10, 8.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 8.25)(10, 8.25)(10, 8.5)
\psline[linewidth=0.03,linecolor=black](10, 8.25)(10, 8.5)
\psline[linewidth=0.03,linecolor=black](10, 8.25)(9.68742, 8.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 8.25)(9.68742, 8.25)(10, 8)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.25)(10, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 8.25)(9.68742, 8)(10, 8)
\psline[linewidth=0.03,linecolor=black](9.68742, 8)(10, 8)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.25)(9.68742, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 8.25)(9.37484, 8)(9.68742, 8)
\psline[linewidth=0.03,linecolor=black](9.37484, 8)(9.68742, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 8)(9.37484, 7.75)(9.68742, 8)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 8)(9.68742, 7.75)(10, 8)
\psline[linewidth=0.03,linecolor=black](9.68742, 8)(9.68742, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7.75)(9.68742, 7.75)(9.68742, 8)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.75)(9.37484, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7.75)(9.37484, 7.75)(9.68742, 7.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.75)(9.68742, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7.75)(9.37484, 7.5)(9.68742, 7.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.5)(9.68742, 7.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.5)(9.37484, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7.5)(9.37484, 7.75)(9.06258, 7.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.5)(9.06258, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7.5)(9.06258, 7.5)(9.06258, 7.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 7.5)(9.06258, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 7.5)(8.75, 7.25)(9.06258, 7.25)
\psline[linewidth=0.03,linecolor=black](8.75, 7.25)(9.06258, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 7.25)(9.06258, 7)(9.06258, 7.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 7)(8.75, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 7)(8.75, 7.25)(8.75, 7)
\psline[linewidth=0.03,linecolor=black](8.75, 7.25)(8.75, 7)
\psline[linewidth=0.03,linecolor=black](9.06258, 7)(8.75, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 6.75)(9.06258, 7)(8.75, 7)
\psline[linewidth=0.03,linecolor=black](8.75, 6.75)(8.75, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6.75)(8.75, 6.75)(8.75, 7)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.75)(8.75, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6.75)(8.75, 6.5)(8.75, 6.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.75)(8.75, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6.5)(8.75, 6.5)(8.43742, 6.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.5)(8.75, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6.25)(8.75, 6.5)(8.43742, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 7.25)(8.43742, 7)(8.75, 7)
\psline[linewidth=0.03,linecolor=black](8.43742, 7)(8.75, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 7)(8.43742, 6.75)(8.75, 7)
\psline[linewidth=0.03,linecolor=black](8.43742, 7)(8.43742, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 6.75)(8.43742, 6.75)(8.43742, 7)
\psline[linewidth=0.03,linecolor=black](8.125, 6.75)(8.43742, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 6.75)(8.43742, 6.5)(8.43742, 6.75)
\psline[linewidth=0.03,linecolor=black](8.125, 6.75)(8.43742, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 6.75)(8.125, 6.5)(8.43742, 6.5)
\psline[linewidth=0.03,linecolor=black](8.125, 6.5)(8.43742, 6.5)
\psline[linewidth=0.03,linecolor=black](8.125, 6.5)(8.125, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 6.5)(8.125, 6.75)(7.81248, 6.5)
\psline[linewidth=0.03,linecolor=black](8.125, 6.5)(7.81248, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.25)(8.125, 6.5)(7.81248, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 6.5)(8.43742, 6.25)(8.43742, 6.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.25)(8.125, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6.25)(8.125, 6.5)(8.125, 6.25)
\psline[linewidth=0.03,linecolor=black](8.125, 6.5)(8.125, 6.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.25)(8.125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6)(8.43742, 6.25)(8.125, 6.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 6)(8.125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6)(8.125, 6.25)(8.125, 6)
\psline[linewidth=0.03,linecolor=black](8.43742, 6)(8.125, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 5.75)(8.43742, 6)(8.125, 6)
\psline[linewidth=0.03,linecolor=black](8.125, 5.75)(8.125, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.75)(8.125, 5.75)(8.125, 6)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.75)(8.125, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 5.75)(7.81248, 5.75)(8.125, 5.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.75)(8.125, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.75)(7.81248, 5.5)(8.125, 5.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.5)(8.125, 5.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.5)(7.81248, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.5)(7.81248, 5.75)(7.5, 5.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.5)(7.5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 5.25)(7.81248, 5.5)(7.5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.5)(7.81248, 5.25)(8.125, 5.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.5)(7.81248, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 5.25)(7.81248, 5.25)(7.81248, 5.5)
\psline[linewidth=0.03,linecolor=black](7.5, 5.25)(7.81248, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.5, 5.25)(7.5, 5)(7.81248, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 6.5)(7.81248, 6.25)(8.125, 6.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.25)(8.125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 6.25)(7.81248, 6.25)(8.125, 6)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.25)(8.125, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6.25)(7.81248, 6)(8.125, 6)
\psline[linewidth=0.03,linecolor=black](7.81248, 6)(8.125, 6)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.25)(7.81248, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6)(7.81248, 6.25)(7.5, 6)
\psline[linewidth=0.03,linecolor=black](7.81248, 6)(7.5, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.75)(7.81248, 6)(7.5, 6)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.75)(7.5, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.75)(7.5, 6)(7.5, 5.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.75)(7.5, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.75)(7.5, 5.75)(7.5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 6)(7.81248, 5.75)(8.125, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7.5)(9.68742, 7.25)(9.68742, 7.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.25)(9.37484, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7.25)(9.37484, 7.5)(9.37484, 7.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.5)(9.37484, 7.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.25)(9.37484, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7)(9.68742, 7.25)(9.37484, 7.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 7)(9.37484, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 7)(9.37484, 7)(9.37484, 7.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 7)(9.37484, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 7)(9.37484, 6.75)(9.37484, 7)
\psline[linewidth=0.03,linecolor=black](9.06258, 7)(9.37484, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 7)(9.06258, 6.75)(9.37484, 6.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.75)(9.37484, 6.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.75)(9.06258, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 6.75)(9.06258, 7)(8.75, 6.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.75)(8.75, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 6.5)(9.06258, 6.75)(8.75, 6.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.5)(8.75, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 6.5)(9.06258, 6.5)(8.75, 6.75)
\psline[linewidth=0.03,linecolor=black](8.75, 6.5)(9.06258, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 6.25)(9.06258, 6.5)(8.75, 6.5)
\psline[linewidth=0.03,linecolor=black](8.75, 6.25)(8.75, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6.25)(8.75, 6.25)(8.75, 6.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.25)(8.75, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6.25)(8.43742, 6)(8.75, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 6.75)(9.06258, 6.5)(9.37484, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 7.5)(9.06258, 7.25)(9.37484, 7.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 7.25)(9.37484, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 7.25)(9.06258, 7)(9.37484, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7.75)(10, 7.75)(10, 8)
\psline[linewidth=0.03,linecolor=black](10, 7.75)(10, 8)
\psline[linewidth=0.03,linecolor=black](10, 7.75)(9.68742, 7.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 7.75)(9.68742, 7.75)(10, 7.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.75)(10, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7.75)(9.68742, 7.5)(10, 7.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.5)(10, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7.5)(9.68742, 7.25)(10, 7.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7.25)(10, 7.25)(10, 7.5)
\psline[linewidth=0.03,linecolor=black](10, 7.25)(10, 7.5)
\psline[linewidth=0.03,linecolor=black](10, 7.25)(9.68742, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 7.25)(9.68742, 7.25)(10, 7)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.25)(10, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7.25)(9.68742, 7)(10, 7)
\psline[linewidth=0.03,linecolor=black](9.68742, 7)(10, 7)
\psline[linewidth=0.03,linecolor=black](9.68742, 7)(9.68742, 7.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7)(9.68742, 7.25)(9.37484, 7)
\psline[linewidth=0.03,linecolor=black](9.68742, 7)(9.37484, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6.75)(9.68742, 7)(9.37484, 7)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.75)(9.37484, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6.75)(9.68742, 6.75)(9.37484, 7)
\psline[linewidth=0.03,linecolor=black](9.37484, 6.75)(9.68742, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6.75)(9.37484, 6.75)(9.37484, 6.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 6.75)(9.37484, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6.75)(9.06258, 6.5)(9.37484, 6.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.5)(9.37484, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 6.5)(9.37484, 6.25)(9.37484, 6.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.5)(9.37484, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6.25)(9.06258, 6.5)(9.06258, 6.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.5)(9.06258, 6.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 6.25)(9.06258, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6)(9.37484, 6.25)(9.06258, 6.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 6)(9.06258, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6)(9.06258, 6.25)(9.06258, 6)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.25)(9.06258, 6)
\psline[linewidth=0.03,linecolor=black](9.37484, 6)(9.06258, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5.75)(9.37484, 6)(9.06258, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 6.25)(8.75, 6)(9.06258, 6)
\psline[linewidth=0.03,linecolor=black](8.75, 6)(9.06258, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 6)(9.06258, 5.75)(9.06258, 6)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.75)(8.75, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5.75)(8.75, 6)(8.75, 5.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.75)(8.75, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 5.5)(9.06258, 5.75)(8.75, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 6.5)(8.75, 6.25)(9.06258, 6.25)
\psline[linewidth=0.03,linecolor=black](8.75, 6.25)(9.06258, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 6.25)(8.75, 6)(9.06258, 6.25)
\psline[linewidth=0.03,linecolor=black](8.75, 6.25)(8.75, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6)(8.75, 6)(8.75, 6.25)
\psline[linewidth=0.03,linecolor=black](8.75, 6)(8.43742, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 6)(8.43742, 6)(8.75, 5.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 6)(8.75, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 6)(8.43742, 5.75)(8.75, 5.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.75)(8.75, 5.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.75)(8.43742, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.75)(8.43742, 6)(8.125, 5.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.75)(8.125, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.75)(8.125, 5.75)(8.125, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.75)(8.75, 5.5)(8.75, 5.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.75)(8.75, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.75)(8.43742, 5.5)(8.75, 5.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.75)(8.43742, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.5)(8.43742, 5.75)(8.125, 5.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.5)(8.125, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.5)(8.125, 5.5)(8.125, 5.25)
\psline[linewidth=0.03,linecolor=black](8.125, 5.5)(8.125, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 5.5)(7.81248, 5.25)(8.125, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 7)(9.68742, 6.75)(10, 7)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 7)(9.68742, 6.75)(10, 6.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.75)(10, 6.75)
\psline[linewidth=0.03,linecolor=black](10, 7)(10, 6.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6.75)(10, 6.5)(10, 6.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.75)(10, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6.75)(9.68742, 6.5)(10, 6.5)
\psline[linewidth=0.03,linecolor=black](10, 6.5)(9.68742, 6.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.75)(9.68742, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6.5)(9.68742, 6.75)(9.37484, 6.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.5)(9.37484, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6.25)(9.68742, 6.5)(9.37484, 6.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 6.5)(9.68742, 6.5)(10, 6.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.5)(10, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 6.25)(9.68742, 6.5)(9.68742, 6.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.5)(9.68742, 6.25)
\psline[linewidth=0.03,linecolor=black](10, 6.25)(9.68742, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6)(10, 6.25)(9.68742, 6.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 6)(9.68742, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6)(9.68742, 6)(9.68742, 6.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 6)(9.68742, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6)(9.68742, 5.75)(9.68742, 6)
\psline[linewidth=0.03,linecolor=black](9.37484, 6)(9.68742, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 5.75)(9.37484, 6)(9.37484, 5.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 5.75)(9.37484, 6)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.75)(9.37484, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 5.75)(9.37484, 5.75)(9.37484, 5.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 5.75)(9.37484, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 5.75)(9.06258, 5.5)(9.37484, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 5.75)(9.37484, 6)(9.06258, 5.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 5.75)(9.06258, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 5.75)(9.06258, 5.75)(9.06258, 5.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.5)(9.06258, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5.5)(9.06258, 5.75)(8.75, 5.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.5)(8.75, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5.5)(8.75, 5.5)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](8.75, 5.5)(8.75, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 5.5)(8.43742, 5.5)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.5)(8.75, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.5)(8.43742, 5.25)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.25)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.25)(8.43742, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.25)(8.43742, 5.5)(8.125, 5.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.25)(8.125, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 5)(8.43742, 5.25)(8.125, 5.25)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(8.125, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.25)(8.125, 5)(8.125, 5.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.25)(8.125, 5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 5)(7.81248, 5.25)(7.81248, 5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.25)(7.81248, 5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](7.81248, 5.25)(7.5, 5)(7.81248, 5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5.25)(8.43742, 5)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.25)(8.43742, 5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.125, 5)(8.43742, 5)(8.43742, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6.5)(9.37484, 6.25)(9.68742, 6.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 6.25)(9.68742, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 6.25)(9.37484, 6)(9.68742, 6.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6)(10, 6)(10, 6.25)
\psline[linewidth=0.03,linecolor=black](10, 6)(10, 6.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 6)(10, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 6)(9.68742, 5.75)(10, 6)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 6)(9.68742, 5.75)(10, 5.75)
\psline[linewidth=0.03,linecolor=black](10, 6)(10, 5.75)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 5.75)(9.68742, 5.75)(10, 5.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.75)(10, 5.5)
\psline[linewidth=0.03,linecolor=black](10, 5.75)(10, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 5.75)(9.68742, 5.5)(10, 5.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.75)(9.68742, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 5.5)(9.68742, 5.75)(9.37484, 5.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.5)(9.37484, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 5.25)(9.68742, 5.5)(9.37484, 5.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 5.25)(9.37484, 5.5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5.5)(9.37484, 5.25)(9.37484, 5.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.5)(9.37484, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5.5)(9.06258, 5.25)(9.37484, 5.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.25)(9.37484, 5.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.5)(9.06258, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5.25)(9.06258, 5.5)(8.75, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5.25)(9.06258, 5)(9.37484, 5.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 5)(9.06258, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5)(9.06258, 5.25)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 5)(8.75, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.75, 5)(9.06258, 5)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](8.75, 5)(8.75, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](8.43742, 5)(8.75, 5)(8.75, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 5.5)(10, 5.25)(10, 5.5)
\psline[linewidth=0.03,linecolor=black](10, 5.25)(10, 5.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.5)(10, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 5.25)(9.68742, 5.5)(9.68742, 5.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.5)(9.68742, 5.25)
\psline[linewidth=0.03,linecolor=black](10, 5.25)(9.68742, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 5)(10, 5.25)(9.68742, 5.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 5)(9.68742, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 5.25)(9.68742, 5)(9.68742, 5.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 5.25)(9.68742, 5)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.37484, 5)(9.68742, 5)(9.37484, 5.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 5)(9.37484, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.06258, 5)(9.37484, 5)(9.37484, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](9.68742, 5.5)(9.37484, 5.25)(9.68742, 5.25)
\pspolygon[linestyle=none,fillcolor=disc2,fillstyle=solid](10, 5.25)(9.68742, 5)(10, 5)
\psline[linewidth=0.03,linecolor=black](10, 5.25)(10, 5)
\psdot[dotstyle=*,dotsize=0.11](10, 5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 5.25)
\psdot[dotstyle=*,dotsize=0.11](10, 5.25)
\psdot[dotstyle=*,dotsize=0.11](8.75, 5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 5.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 5.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 5.5)
\psdot[dotstyle=*,dotsize=0.11](10, 5.5)
\psdot[dotstyle=*,dotsize=0.11](10, 5.75)
\psdot[dotstyle=*,dotsize=0.11](10, 6)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 5.25)
\psdot[dotstyle=*,dotsize=0.11](8.75, 5.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 5.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 5.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 5.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 5.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 6)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 6.25)
\psdot[dotstyle=*,dotsize=0.11](10, 6.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 6.5)
\psdot[dotstyle=*,dotsize=0.11](10, 6.5)
\psdot[dotstyle=*,dotsize=0.11](10, 6.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 5.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 5.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 5.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 5.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 5.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 6)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 5.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 6)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 6)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 6.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 6.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 6.5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 6.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 7)
\psdot[dotstyle=*,dotsize=0.11](10, 7)
\psdot[dotstyle=*,dotsize=0.11](10, 7.25)
\psdot[dotstyle=*,dotsize=0.11](10, 7.5)
\psdot[dotstyle=*,dotsize=0.11](10, 7.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 6.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 6.5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 6.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 6.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 7)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 7.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 7.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 6)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 5.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 5.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 5.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 5.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 5.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 6)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 6)
\psdot[dotstyle=*,dotsize=0.11](8.125, 6.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 6.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 6.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 6.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 6.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 6.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 6.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 7)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 7)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 7.25)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 7.5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 7.5)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 7.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 8)
\psdot[dotstyle=*,dotsize=0.11](10, 8)
\psdot[dotstyle=*,dotsize=0.11](10, 8.25)
\psdot[dotstyle=*,dotsize=0.11](10, 8.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 6.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 7)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 7)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 7.25)
\psdot[dotstyle=*,dotsize=0.11](8.75, 7.25)
\psdot[dotstyle=*,dotsize=0.11](8.75, 7.5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 7.5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 7.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 7.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 8)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 8)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 8.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 8.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 8.5)
\psdot[dotstyle=*,dotsize=0.11](10, 8.75)
\psdot[dotstyle=*,dotsize=0.11](10, 9)
\psdot[dotstyle=*,dotsize=0.11](8.125, 7.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 7.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 7.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 7.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 7.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 8)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 8.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 8.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 8.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 8.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 8.75)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 9)
\psdot[dotstyle=*,dotsize=0.11](10, 9.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 6.25)
\psdot[dotstyle=*,dotsize=0.11](7.5, 5.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 6)
\psdot[dotstyle=*,dotsize=0.11](7.5, 6.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 6.25)
\psdot[dotstyle=*,dotsize=0.11](7.5, 6.5)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 6.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 6.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 6.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 7)
\psdot[dotstyle=*,dotsize=0.11](6.875, 6.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 6.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 6.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 7)
\psdot[dotstyle=*,dotsize=0.11](7.5, 7)
\psdot[dotstyle=*,dotsize=0.11](7.5, 7.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 7.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 7.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 7.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 8)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 8)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 8.25)
\psdot[dotstyle=*,dotsize=0.11](8.75, 8.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 8.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 8.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 8.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 8.75)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 9)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 9)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 9.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 9.25)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 9.5)
\psdot[dotstyle=*,dotsize=0.11](10, 9.5)
\psdot[dotstyle=*,dotsize=0.11](10, 9.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 10)
\psdot[dotstyle=*,dotsize=0.11](5, 10)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 10)
\psdot[dotstyle=*,dotsize=0.11](5.625, 10)
\psdot[dotstyle=*,dotsize=0.11](5, 9.75)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 10)
\psdot[dotstyle=*,dotsize=0.11](4.375, 10)
\psdot[dotstyle=*,dotsize=0.11](4.375, 9.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 9.75)
\psdot[dotstyle=*,dotsize=0.11](5, 9.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 9.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 9.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 9.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 9.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 10)
\psdot[dotstyle=*,dotsize=0.11](6.25, 10)
\psdot[dotstyle=*,dotsize=0.11](3.75, 10)
\psdot[dotstyle=*,dotsize=0.11](3.125, 10)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 10)
\psdot[dotstyle=*,dotsize=0.11](3.75, 9.75)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 9.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 9.75)
\psdot[dotstyle=*,dotsize=0.11](3.75, 9.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 9.5)
\psdot[dotstyle=*,dotsize=0.11](4.375, 9.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 9.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 9.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 9.25)
\psdot[dotstyle=*,dotsize=0.11](5, 9.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 9.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 9)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 9)
\psdot[dotstyle=*,dotsize=0.11](5, 9)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 9)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 9.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 9.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 9.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 9.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 9.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 9.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 10)
\psdot[dotstyle=*,dotsize=0.11](6.875, 10)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 10)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 9.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 9.5)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 9.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 9.75)
\psdot[dotstyle=*,dotsize=0.11](5, 8.75)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 8.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 9)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 8.5)
\psdot[dotstyle=*,dotsize=0.11](5.625, 8.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 8.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 9)
\psdot[dotstyle=*,dotsize=0.11](6.25, 9)
\psdot[dotstyle=*,dotsize=0.11](6.25, 9.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 9.25)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 8.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 8.75)
\psdot[dotstyle=*,dotsize=0.11](3.75, 8.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 9.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 9.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 9.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 9.5)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 9.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 9)
\psdot[dotstyle=*,dotsize=0.11](3.75, 9.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 9)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 9)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 8.75)
\psdot[dotstyle=*,dotsize=0.11](4.375, 8.75)
\psdot[dotstyle=*,dotsize=0.11](4.375, 8.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 8.5)
\psdot[dotstyle=*,dotsize=0.11](5, 8.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 8.25)
\psdot[dotstyle=*,dotsize=0.11](5, 8.25)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 8)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 8.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 8.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 8.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 8.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 8.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 8.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 9)
\psdot[dotstyle=*,dotsize=0.11](6.875, 9)
\psdot[dotstyle=*,dotsize=0.11](6.875, 9.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 9.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 9.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 9.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 10)
\psdot[dotstyle=*,dotsize=0.11](5.625, 6.5)
\psdot[dotstyle=*,dotsize=0.11](5, 7.25)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 7.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 7.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 7)
\psdot[dotstyle=*,dotsize=0.11](5.625, 6.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 7)
\psdot[dotstyle=*,dotsize=0.11](5.625, 7.25)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 7.5)
\psdot[dotstyle=*,dotsize=0.11](5, 8)
\psdot[dotstyle=*,dotsize=0.11](3.75, 8.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 8.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 8.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 8.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 8)
\psdot[dotstyle=*,dotsize=0.11](4.375, 8)
\psdot[dotstyle=*,dotsize=0.11](4.375, 7.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 8)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 7.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 7.5)
\psdot[dotstyle=*,dotsize=0.11](5, 7.5)
\psdot[dotstyle=*,dotsize=0.11](5, 7.75)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 7.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 7.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 7.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 7.75)
\psdot[dotstyle=*,dotsize=0.11](6.25, 8)
\psdot[dotstyle=*,dotsize=0.11](5.625, 8)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 8)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 8.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 8.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 8.5)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 8.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 8.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 8.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 8.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 9)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 9.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 8.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 9)
\psdot[dotstyle=*,dotsize=0.11](7.5, 9.25)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 7.25)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 6.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 6.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 7)
\psdot[dotstyle=*,dotsize=0.11](6.25, 7.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 7.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 7.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 7.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 8)
\psdot[dotstyle=*,dotsize=0.11](6.875, 8)
\psdot[dotstyle=*,dotsize=0.11](6.875, 8.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 6.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 5.25)
\psdot[dotstyle=*,dotsize=0.11](7.5, 5.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 5.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 5.75)
\psdot[dotstyle=*,dotsize=0.11](6.875, 5.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 6)
\psdot[dotstyle=*,dotsize=0.11](6.875, 6)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 6)
\psdot[dotstyle=*,dotsize=0.11](6.875, 6.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 6.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 6.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 6.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 6.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 6.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 6.75)
\psdot[dotstyle=*,dotsize=0.11](6.25, 7)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 7)
\psdot[dotstyle=*,dotsize=0.11](6.875, 7)
\psdot[dotstyle=*,dotsize=0.11](6.875, 7.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 7.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 7.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 7.5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 7.75)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 8)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 8.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 8.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 8.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 8.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 9)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 9.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 9.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 9.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 9.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 9.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 10)
\psdot[dotstyle=*,dotsize=0.11](8.125, 9.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 10)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 10)
\psdot[dotstyle=*,dotsize=0.11](8.125, 9.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 9.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 8.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 8.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 7.25)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 7.5)
\psdot[dotstyle=*,dotsize=0.11](7.5, 7.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 7.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 7.75)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 7.75)
\psdot[dotstyle=*,dotsize=0.11](7.5, 8)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 8)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 8.25)
\psdot[dotstyle=*,dotsize=0.11](8.125, 8.25)
\psdot[dotstyle=*,dotsize=0.11](7.81248, 8.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 8.5)
\psdot[dotstyle=*,dotsize=0.11](8.125, 8.75)
\psdot[dotstyle=*,dotsize=0.11](8.125, 9)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 8.75)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 9)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 9.25)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 9.5)
\psdot[dotstyle=*,dotsize=0.11](8.43742, 9.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 9.75)
\psdot[dotstyle=*,dotsize=0.11](8.75, 10)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 10)
\psdot[dotstyle=*,dotsize=0.11](8.75, 9.5)
\psdot[dotstyle=*,dotsize=0.11](8.75, 9)
\psdot[dotstyle=*,dotsize=0.11](8.75, 9.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 9.25)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 9.5)
\psdot[dotstyle=*,dotsize=0.11](9.06258, 9.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 9.5)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 9.75)
\psdot[dotstyle=*,dotsize=0.11](9.37484, 10)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 10)
\psdot[dotstyle=*,dotsize=0.11](9.68742, 9.75)
\psdot[dotstyle=*,dotsize=0.11](10, 10)
\psline[linewidth=0.03,linecolor=black](9.68742, 5)(10, 5)
\psline[linewidth=0.03,linecolor=black](9.06258, 5)(9.37484, 5)
\psline[linewidth=0.03,linecolor=black](9.37484, 5)(9.68742, 5)
\psline[linewidth=0.03,linecolor=black](9.37484, 5.25)(9.68742, 5.25)
\psline[linewidth=0.03,linecolor=black](10, 5.25)(9.68742, 5)
\psline[linewidth=0.03,linecolor=black](8.43742, 5)(8.75, 5)
\psline[linewidth=0.03,linecolor=black](8.75, 5)(9.06258, 5)
\psline[linewidth=0.03,linecolor=black](9.06258, 5)(9.37484, 5.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.25)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.5)(9.37484, 5.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.5)(10, 5.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.75)(10, 5.75)
\psline[linewidth=0.03,linecolor=black](10, 6)(9.68742, 5.75)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(8.43742, 5)
\psline[linewidth=0.03,linecolor=black](8.43742, 5)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](7.5, 5)(7.81248, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(7.81248, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(8.43742, 5.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.5)(8.75, 5.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 5.75)(9.06258, 5.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.5)(9.37484, 5.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 5.75)(9.37484, 5.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 6)(9.68742, 5.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 6)(9.68742, 6.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 6)(10, 6.25)
\psline[linewidth=0.03,linecolor=black](10, 6.5)(10, 6.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.5)(9.37484, 6.25)
\psline[linewidth=0.03,linecolor=black](10, 6.5)(10, 6.75)
\psline[linewidth=0.03,linecolor=black](10, 7)(9.68742, 6.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.25)(8.125, 5.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.5)(8.125, 5.25)
\psline[linewidth=0.03,linecolor=black](8.75, 5.5)(8.43742, 5.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 5.75)(8.125, 5.5)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.75)(8.75, 5.5)
\psline[linewidth=0.03,linecolor=black](8.75, 5.5)(8.75, 5.75)
\psline[linewidth=0.03,linecolor=black](8.75, 6)(8.75, 5.75)
\psline[linewidth=0.03,linecolor=black](8.75, 6)(9.06258, 6.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 6)(9.06258, 5.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 5.75)(9.06258, 6)
\psline[linewidth=0.03,linecolor=black](9.37484, 6)(9.37484, 6.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 6.25)(9.37484, 6.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 6.75)(9.37484, 6.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 7)(9.68742, 6.75)
\psline[linewidth=0.03,linecolor=black](10, 7.25)(10, 7)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.25)(10, 7.5)
\psline[linewidth=0.03,linecolor=black](10, 7.75)(10, 7.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 6.75)(9.06258, 6.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 6)(8.75, 6.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.5)(8.75, 6.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 6.75)(9.06258, 6.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 6.75)(9.37484, 7)
\psline[linewidth=0.03,linecolor=black](9.06258, 7)(9.37484, 7.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.25)(9.37484, 7)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.25)(9.68742, 7.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.75)(7.81248, 6)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.25)(7.5, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 5.5)(7.81248, 5.25)
\psline[linewidth=0.03,linecolor=black](7.5, 5.25)(7.81248, 5.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.75)(7.5, 5.5)
\psline[linewidth=0.03,linecolor=black](8.125, 5.75)(8.125, 5.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 5.75)(8.125, 6)
\psline[linewidth=0.03,linecolor=black](8.43742, 6)(8.125, 5.75)
\psline[linewidth=0.03,linecolor=black](8.125, 6.25)(8.125, 6)
\psline[linewidth=0.03,linecolor=black](8.43742, 6)(8.43742, 6.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.25)(8.125, 6.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.25)(8.75, 6.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.25)(8.43742, 6.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.5)(8.43742, 6.75)
\psline[linewidth=0.03,linecolor=black](8.75, 6.5)(8.75, 6.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 6.75)(8.75, 7)
\psline[linewidth=0.03,linecolor=black](8.75, 6.75)(9.06258, 7)
\psline[linewidth=0.03,linecolor=black](9.06258, 7.25)(9.06258, 7)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.5)(9.06258, 7.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.75)(9.68742, 7.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 7.75)(10, 8)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.75)(9.68742, 8)
\psline[linewidth=0.03,linecolor=black](10, 8.25)(10, 8)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.25)(10, 8.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.5)(8.125, 6.75)
\psline[linewidth=0.03,linecolor=black](8.125, 6.75)(8.43742, 7)
\psline[linewidth=0.03,linecolor=black](8.125, 6.75)(8.125, 7)
\psline[linewidth=0.03,linecolor=black](8.75, 7.25)(8.43742, 7)
\psline[linewidth=0.03,linecolor=black](8.43742, 7.25)(8.43742, 7)
\psline[linewidth=0.03,linecolor=black](8.75, 7.75)(9.06258, 8)
\psline[linewidth=0.03,linecolor=black](8.75, 7.5)(8.75, 7.25)
\psline[linewidth=0.03,linecolor=black](8.75, 7.25)(9.06258, 7.5)
\psline[linewidth=0.03,linecolor=black](8.75, 7.5)(9.06258, 7.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 7.5)(9.37484, 7.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 7.75)(9.37484, 8)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.25)(9.37484, 8)
\psline[linewidth=0.03,linecolor=black](9.37484, 8)(9.37484, 8.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 8.5)(9.68742, 8.25)
\psline[linewidth=0.03,linecolor=black](10, 8.75)(9.68742, 8.5)
\psline[linewidth=0.03,linecolor=black](10, 9)(10, 8.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 8.5)(9.68742, 8.75)
\psline[linewidth=0.03,linecolor=black](8.125, 7.25)(7.81248, 7)
\psline[linewidth=0.03,linecolor=black](8.125, 7.25)(8.43742, 7.5)
\psline[linewidth=0.03,linecolor=black](8.125, 7.25)(8.125, 7.5)
\psline[linewidth=0.03,linecolor=black](8.43742, 7.5)(8.75, 7.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 7.5)(8.43742, 7.75)
\psline[linewidth=0.03,linecolor=black](8.75, 7.75)(8.75, 8)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.25)(8.75, 8)
\psline[linewidth=0.03,linecolor=black](9.37484, 8.5)(9.06258, 8.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 8.25)(9.06258, 8.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 8.75)(9.37484, 8.5)
\psline[linewidth=0.03,linecolor=black](9.68742, 9)(9.68742, 8.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 9)(10, 9.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 9)(9.68742, 9.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 8)(8.125, 7.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 6.25)(7.18748, 6)
\psline[linewidth=0.03,linecolor=black](7.18748, 6.25)(7.5, 6.5)
\psline[linewidth=0.03,linecolor=black](7.5, 5.75)(7.5, 5.5)
\psline[linewidth=0.03,linecolor=black](7.5, 6)(7.5, 5.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 6)(7.5, 6.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.25)(7.5, 6)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.25)(7.81248, 6.5)
\psline[linewidth=0.03,linecolor=black](7.5, 6.5)(7.5, 6.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.5)(7.81248, 6.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 6.75)(7.81248, 7)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.25)(7.81248, 7)
\psline[linewidth=0.03,linecolor=black](6.875, 6.25)(7.18748, 6.5)
\psline[linewidth=0.03,linecolor=black](6.875, 6.25)(6.875, 6.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 6.75)(7.18748, 6.5)
\psline[linewidth=0.03,linecolor=black](7.5, 7)(7.18748, 6.75)
\psline[linewidth=0.03,linecolor=black](6.875, 6.75)(7.18748, 7)
\psline[linewidth=0.03,linecolor=black](7.5, 7.25)(7.5, 7)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.25)(7.81248, 7.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.5)(8.125, 7.75)
\psline[linewidth=0.03,linecolor=black](8.125, 8)(8.125, 7.75)
\psline[linewidth=0.03,linecolor=black](8.75, 8.25)(8.43742, 8)
\psline[linewidth=0.03,linecolor=black](8.43742, 8)(8.43742, 8.25)
\psline[linewidth=0.03,linecolor=black](8.75, 8.5)(8.75, 8.25)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.5)(8.125, 8.25)
\psline[linewidth=0.03,linecolor=black](8.75, 8.5)(9.06258, 8.75)
\psline[linewidth=0.03,linecolor=black](8.75, 8.5)(8.75, 8.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 9)(9.06258, 8.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 9)(9.06258, 8.75)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.25)(9.37484, 9)
\psline[linewidth=0.03,linecolor=black](10, 9.5)(9.68742, 9.25)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.25)(9.68742, 9.5)
\psline[linewidth=0.03,linecolor=black](10, 9.75)(10, 9.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 10)(4.375, 10)
\psline[linewidth=0.03,linecolor=black](4.6875, 10)(5, 10)
\psline[linewidth=0.03,linecolor=black](5.3125, 10)(5, 9.75)
\psline[linewidth=0.03,linecolor=black](5.625, 10)(5.3125, 10)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.75)(5, 9.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 9.75)(5, 9.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 10)(3.75, 10)
\psline[linewidth=0.03,linecolor=black](4.06252, 10)(4.375, 10)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.75)(4.375, 10)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.75)(4.375, 9.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.75)(5, 9.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 9.5)(5, 9.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 9.75)(5.625, 9.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 10)(5.625, 9.75)
\psline[linewidth=0.03,linecolor=black](5.625, 9.5)(5.93748, 9.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 10)(6.25, 10)
\psline[linewidth=0.03,linecolor=black](6.25, 9.75)(6.56248, 10)
\psline[linewidth=0.03,linecolor=black](5, 9.25)(5.3125, 9.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 10)(3.75, 10)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.75)(3.75, 10)
\psline[linewidth=0.03,linecolor=black](2.81252, 10)(3.125, 10)
\psline[linewidth=0.03,linecolor=black](3.43752, 10)(3.125, 10)
\psline[linewidth=0.03,linecolor=black](3.75, 9.75)(3.43752, 10)
\psline[linewidth=0.03,linecolor=black](4.375, 9.5)(4.06252, 9.75)
\psline[linewidth=0.03,linecolor=black](3.125, 9.75)(3.43752, 9.75)
\psline[linewidth=0.03,linecolor=black](3.75, 9.5)(3.43752, 9.75)
\psline[linewidth=0.03,linecolor=black](3.75, 9.5)(4.06252, 9.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.25)(4.375, 9.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 9.25)(4.375, 9.5)
\psline[linewidth=0.03,linecolor=black](4.375, 9.5)(4.6875, 9.5)
\psline[linewidth=0.03,linecolor=black](5, 9.25)(4.6875, 9.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 9)(5, 9.25)
\psline[linewidth=0.03,linecolor=black](3.75, 9.25)(4.06252, 9.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 9.25)(4.375, 9)
\psline[linewidth=0.03,linecolor=black](4.375, 9)(4.6875, 9)
\psline[linewidth=0.03,linecolor=black](4.6875, 9)(5, 9)
\psline[linewidth=0.03,linecolor=black](5.625, 9.25)(5.3125, 9.25)
\psline[linewidth=0.03,linecolor=black](5.625, 9.5)(5.3125, 9.25)
\psline[linewidth=0.03,linecolor=black](5.625, 9.5)(5.93748, 9.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 9.5)(6.25, 9.75)
\psline[linewidth=0.03,linecolor=black](6.25, 9.75)(6.56248, 9.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 10)(6.875, 10)
\psline[linewidth=0.03,linecolor=black](6.875, 9.75)(7.18748, 10)
\psline[linewidth=0.03,linecolor=black](5.625, 9)(5.93748, 9.25)
\psline[linewidth=0.03,linecolor=black](6.25, 9.5)(5.93748, 9.25)
\psline[linewidth=0.03,linecolor=black](6.25, 9.5)(6.56248, 9.5)
\psline[linewidth=0.03,linecolor=black](6.875, 9.75)(6.56248, 9.5)
\psline[linewidth=0.03,linecolor=black](6.875, 9.75)(7.18748, 9.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 9)(6.25, 9.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.75)(5, 8.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.75)(5, 8.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.75)(5.625, 9)
\psline[linewidth=0.03,linecolor=black](5.93748, 9)(5.625, 9)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.5)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](5.625, 8.75)(5.3125, 8.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 8.75)(5.625, 8.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 9)(6.25, 9)
\psline[linewidth=0.03,linecolor=black](6.56248, 9.25)(6.25, 9.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 9.25)(6.875, 9.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 9)(6.875, 9.25)
\psline[linewidth=0.03,linecolor=black](6.25, 8.75)(6.56248, 9)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.75)(4.375, 8.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.75)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](3.125, 8.75)(3.43752, 8.75)
\psline[linewidth=0.03,linecolor=black](3.75, 8.75)(3.43752, 8.75)
\psline[linewidth=0.03,linecolor=black](3.125, 9)(3.43752, 9)
\psline[linewidth=0.03,linecolor=black](2.81252, 9.25)(3.125, 9.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 10)(3.125, 9.75)
\psline[linewidth=0.03,linecolor=black](3.125, 9.5)(2.81252, 9.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 9.5)(3.125, 9.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 9.25)(3.125, 9.25)
\psline[linewidth=0.03,linecolor=black](3.75, 9.25)(3.43752, 9.5)
\psline[linewidth=0.03,linecolor=black](3.75, 9)(3.43752, 9)
\psline[linewidth=0.03,linecolor=black](3.75, 9.25)(4.06252, 9)
\psline[linewidth=0.03,linecolor=black](3.75, 9)(4.06252, 8.75)
\psline[linewidth=0.03,linecolor=black](4.375, 8.75)(4.06252, 9)
\psline[linewidth=0.03,linecolor=black](4.375, 8.75)(4.6875, 8.5)
\psline[linewidth=0.03,linecolor=black](4.375, 8.5)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.25)(5, 8.5)
\psline[linewidth=0.03,linecolor=black](4.375, 8.25)(4.6875, 8.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 8.25)(5, 8.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 8)(5, 8)
\psline[linewidth=0.03,linecolor=black](5.625, 8.5)(5.3125, 8.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 8.25)(5.625, 8.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 8.5)(5.625, 8.5)
\psline[linewidth=0.03,linecolor=black](6.25, 8.75)(5.93748, 8.5)
\psline[linewidth=0.03,linecolor=black](6.25, 8.75)(6.56248, 8.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 9)(6.875, 9)
\psline[linewidth=0.03,linecolor=black](6.875, 9.5)(7.18748, 9.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 9.75)(7.5, 10)
\psline[linewidth=0.03,linecolor=black](5, 7.25)(4.6875, 7.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.5)(5.93748, 6.25)
\psline[linewidth=0.03,linecolor=black](5, 7.25)(5.3125, 7.25)
\psline[linewidth=0.03,linecolor=black](5.625, 7.5)(5.3125, 7.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.75)(5.3125, 7)
\psline[linewidth=0.03,linecolor=black](5.625, 7.25)(5.3125, 7)
\psline[linewidth=0.03,linecolor=black](5.625, 6.75)(5.93748, 6.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.75)(5.625, 7)
\psline[linewidth=0.03,linecolor=black](5.625, 7.25)(5.93748, 7.5)
\psline[linewidth=0.03,linecolor=black](5, 8)(4.6875, 8)
\psline[linewidth=0.03,linecolor=black](5, 8)(5.3125, 7.75)
\psline[linewidth=0.03,linecolor=black](4.375, 7.5)(4.6875, 7.5)
\psline[linewidth=0.03,linecolor=black](3.75, 8.25)(4.06252, 8)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.5)(3.75, 8.5)
\psline[linewidth=0.03,linecolor=black](3.75, 8.5)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](3.75, 8.25)(4.06252, 8.25)
\psline[linewidth=0.03,linecolor=black](4.375, 8.25)(4.06252, 8.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 8)(4.375, 8.25)
\psline[linewidth=0.03,linecolor=black](4.375, 7.75)(4.06252, 8)
\psline[linewidth=0.03,linecolor=black](4.375, 8)(4.06252, 8)
\psline[linewidth=0.03,linecolor=black](4.375, 7.75)(4.6875, 7.75)
\psline[linewidth=0.03,linecolor=black](5, 7.75)(4.6875, 8)
\psline[linewidth=0.03,linecolor=black](4.6875, 7.5)(5, 7.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 7.5)(5, 7.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 7.5)(5.625, 7.75)
\psline[linewidth=0.03,linecolor=black](5.625, 8)(5.3125, 7.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 7.75)(5.625, 7.75)
\psline[linewidth=0.03,linecolor=black](6.25, 7.75)(6.25, 8)
\psline[linewidth=0.03,linecolor=black](5.625, 8)(5.93748, 8)
\psline[linewidth=0.03,linecolor=black](5.625, 8)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](6.25, 8.25)(5.93748, 8)
\psline[linewidth=0.03,linecolor=black](6.25, 8.5)(5.93748, 8.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 8.5)(6.25, 8.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 8)(6.56248, 8.25)
\psline[linewidth=0.03,linecolor=black](6.875, 8.75)(6.56248, 8.5)
\psline[linewidth=0.03,linecolor=black](6.875, 8.25)(6.875, 8.5)
\psline[linewidth=0.03,linecolor=black](6.875, 8.75)(7.18748, 9)
\psline[linewidth=0.03,linecolor=black](7.18748, 9)(7.18748, 9.25)
\psline[linewidth=0.03,linecolor=black](7.5, 9.5)(7.18748, 9.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 8.75)(7.18748, 8.5)
\psline[linewidth=0.03,linecolor=black](7.5, 9)(7.18748, 8.75)
\psline[linewidth=0.03,linecolor=black](7.5, 9)(7.5, 9.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 7.25)(5.93748, 7)
\psline[linewidth=0.03,linecolor=black](5.93748, 7.25)(6.25, 7.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.5)(5.93748, 6.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.5)(5.93748, 6.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 7)(5.93748, 6.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 7)(6.25, 7.25)
\psline[linewidth=0.03,linecolor=black](6.25, 7.5)(6.25, 7.75)
\psline[linewidth=0.03,linecolor=black](6.25, 7.75)(6.56248, 8)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.5)(6.56248, 7.75)
\psline[linewidth=0.03,linecolor=black](6.875, 8)(6.875, 7.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 8)(6.875, 8.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 8.5)(6.875, 8.25)
\psline[linewidth=0.03,linecolor=black](6.875, 6.75)(6.56248, 6.5)
\psline[linewidth=0.03,linecolor=black](6.875, 6.75)(6.875, 7)
\psline[linewidth=0.03,linecolor=black](6.25, 6.25)(6.56248, 6)
\psline[linewidth=0.03,linecolor=black](6.56248, 6)(6.875, 5.75)
\psline[linewidth=0.03,linecolor=black](7.5, 5.25)(7.5, 5)
\psline[linewidth=0.03,linecolor=black](7.5, 5.25)(7.5, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.25)(7.18748, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.75)(7.5, 5.5)
\psline[linewidth=0.03,linecolor=black](6.875, 5.75)(6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.75)(7.18748, 6)
\psline[linewidth=0.03,linecolor=black](6.875, 5.75)(6.875, 6)
\psline[linewidth=0.03,linecolor=black](6.875, 6.25)(7.18748, 6)
\psline[linewidth=0.03,linecolor=black](6.56248, 6)(6.56248, 6.25)
\psline[linewidth=0.03,linecolor=black](6.875, 6.25)(6.56248, 6.5)
\psline[linewidth=0.03,linecolor=black](6.25, 6.25)(6.25, 6.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 6.5)(6.56248, 6.75)
\psline[linewidth=0.03,linecolor=black](6.25, 6.75)(6.25, 6.5)
\psline[linewidth=0.03,linecolor=black](6.25, 6.75)(6.25, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 6.75)(6.56248, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.25)(6.25, 7)
\psline[linewidth=0.03,linecolor=black](7.18748, 7.25)(6.875, 7)
\psline[linewidth=0.03,linecolor=black](6.875, 7.25)(6.875, 7)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.25)(6.56248, 7.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 7.25)(6.875, 7.5)
\psline[linewidth=0.03,linecolor=black](6.875, 7.75)(6.56248, 7.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 8)(6.875, 7.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 8)(7.18748, 8.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 8.5)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.5, 8.5)(7.5, 8.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 9)(7.5, 8.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 9)(7.81248, 9.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 9.25)(7.81248, 9.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 9.75)(7.5, 9.5)
\psline[linewidth=0.03,linecolor=black](7.5, 9.5)(7.5, 9.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 10)(7.5, 9.75)
\psline[linewidth=0.03,linecolor=black](8.125, 9.5)(8.125, 9.75)
\psline[linewidth=0.03,linecolor=black](8.125, 10)(8.125, 9.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 9.75)(8.43742, 10)
\psline[linewidth=0.03,linecolor=black](8.125, 9.5)(8.125, 9.25)
\psline[linewidth=0.03,linecolor=black](8.125, 9.5)(8.43742, 9.75)
\psline[linewidth=0.03,linecolor=black](8.125, 9.25)(8.125, 9)
\psline[linewidth=0.03,linecolor=black](8.125, 9.25)(8.43742, 9.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.75)(7.81248, 8.5)
\psline[linewidth=0.03,linecolor=black](8.125, 9)(7.81248, 8.75)
\psline[linewidth=0.03,linecolor=black](7.5, 8)(7.5, 8.25)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.5)(7.5, 8.25)
\psline[linewidth=0.03,linecolor=black](7.5, 7.5)(7.81248, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 7.5)(7.18748, 7.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 7.25)(7.18748, 7.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 7.5)(7.18748, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 7.5)(7.5, 7.75)
\psline[linewidth=0.03,linecolor=black](7.5, 8)(7.18748, 7.75)
\psline[linewidth=0.03,linecolor=black](7.81248, 7.75)(7.81248, 8)
\psline[linewidth=0.03,linecolor=black](7.5, 8)(7.81248, 8.25)
\psline[linewidth=0.03,linecolor=black](8.125, 8.25)(7.81248, 8)
\psline[linewidth=0.03,linecolor=black](8.125, 8.25)(8.125, 8.5)
\psline[linewidth=0.03,linecolor=black](7.81248, 8.5)(8.125, 8.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.75)(8.125, 8.5)
\psline[linewidth=0.03,linecolor=black](8.125, 9)(8.43742, 9.25)
\psline[linewidth=0.03,linecolor=black](8.75, 9)(8.43742, 8.75)
\psline[linewidth=0.03,linecolor=black](8.43742, 8.75)(8.43742, 9)
\psline[linewidth=0.03,linecolor=black](8.43742, 9.75)(8.75, 10)
\psline[linewidth=0.03,linecolor=black](8.75, 9.5)(8.75, 9.75)
\psline[linewidth=0.03,linecolor=black](9.06258, 10)(9.06258, 9.75)
\psline[linewidth=0.03,linecolor=black](8.75, 9.25)(8.75, 9.5)
\psline[linewidth=0.03,linecolor=black](8.75, 9.5)(9.06258, 9.75)
\psline[linewidth=0.03,linecolor=black](8.75, 9)(8.75, 9.25)
\psline[linewidth=0.03,linecolor=black](8.75, 9)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 9.5)(8.75, 9.25)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.5)(9.06258, 9.25)
\psline[linewidth=0.03,linecolor=black](9.06258, 9.75)(9.37484, 10)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.75)(9.37484, 9.5)
\psline[linewidth=0.03,linecolor=black](9.37484, 9.5)(9.37484, 9.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 10)(9.68742, 9.75)
\psline[linewidth=0.03,linecolor=black](9.68742, 9.75)(10, 10)


==> examples/cart/ddisc3.tex <==
\psline[linewidth=0.03,linecolor=black](9.68742, 5)(10, 5)
\psdot[dotstyle=*,dotsize=0.13](10, 5)
\psdot[dotstyle=*,dotsize=0.13](9.68742, 5)
\psline[linewidth=0.03,linecolor=black](9.37484, 5)(9.68742, 5)
\psdot[dotstyle=*,dotsize=0.13](9.37484, 5)
\psline[linewidth=0.03,linecolor=black](9.06258, 5)(9.37484, 5)
\psdot[dotstyle=*,dotsize=0.13](9.06258, 5)
\psline[linewidth=0.03,linecolor=black](8.75, 5)(9.06258, 5)
\psdot[dotstyle=*,dotsize=0.13](8.75, 5)
\psline[linewidth=0.03,linecolor=black](8.43742, 5)(8.75, 5)
\psdot[dotstyle=*,dotsize=0.13](8.43742, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(8.43742, 5)
\psdot[dotstyle=*,dotsize=0.13](8.125, 5)
\psline[linewidth=0.03,linecolor=black](8.125, 5)(7.81248, 5)
\psdot[dotstyle=*,dotsize=0.13](7.81248, 5)
\psline[linewidth=0.03,linecolor=black](7.5, 5)(7.81248, 5)


==> examples/cart/ddisc4.tex <==
\newrgbcolor{disc4}{0.5 0.5 0.5}
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 5)(2.5, 5.25)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.5, 5.25)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.81252, 5)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.81252, 5)(2.5, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 5)(2.81252, 5.25)(2.5, 5.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 5.25)(2.5, 5.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 5)(2.81252, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 5.25)(2.81252, 5)(3.125, 5.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 5.25)(3.125, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5.5)(2.81252, 5.25)(3.125, 5.25)
\psline[linewidth=0.03,linecolor=black](3.125, 5.5)(3.125, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5.25)(3.125, 5.5)(3.125, 5.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.25)(3.125, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5.5)(3.43752, 5.25)(3.43752, 5.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.25)(3.43752, 5.5)
\psline[linewidth=0.03,linecolor=black](3.125, 5.5)(3.43752, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5.75)(3.125, 5.5)(3.43752, 5.5)
\psline[linewidth=0.03,linecolor=black](3.125, 5.75)(3.43752, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5.75)(3.125, 5.75)(3.43752, 5.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.75)(3.43752, 5.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.75)(3.125, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5.75)(3.43752, 5.75)(3.43752, 6)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.75)(3.43752, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5.75)(3.75, 6)(3.43752, 6)
\psline[linewidth=0.03,linecolor=black](3.75, 6)(3.43752, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 6)(3.43752, 6.25)(3.43752, 6)
\psline[linewidth=0.03,linecolor=black](3.75, 6)(3.43752, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.25)(3.75, 6)(3.75, 6.25)
\psline[linewidth=0.03,linecolor=black](3.75, 6)(3.75, 6.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.25)(3.75, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.5)(3.43752, 6.25)(3.75, 6.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.5)(3.75, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 6.5)(3.43752, 6.5)(3.75, 6.25)
\psline[linewidth=0.03,linecolor=black](3.75, 6.5)(3.75, 6.25)
\psline[linewidth=0.03,linecolor=black](3.75, 6.5)(3.43752, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.75)(3.43752, 6.5)(3.75, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6.5)(3.75, 6.5)(3.75, 6.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.5)(3.75, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6.5)(4.06252, 6.75)(3.75, 6.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.75)(3.75, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6.75)(3.75, 6.75)(3.75, 6.5)
\psline[linewidth=0.03,linecolor=black](3.75, 6.75)(3.75, 6.5)
\psline[linewidth=0.03,linecolor=black](3.75, 6.75)(4.06252, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 6.75)(4.06252, 6.75)(3.75, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 6.75)(3.43752, 6.75)(3.75, 6.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.75)(3.75, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.75)(3.75, 6.75)(3.75, 7)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.75)(3.75, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.75)(3.75, 7)(3.43752, 7)
\psline[linewidth=0.03,linecolor=black](3.75, 7)(3.43752, 7)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.75)(3.43752, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7)(3.43752, 6.75)(3.43752, 7)
\psline[linewidth=0.03,linecolor=black](3.125, 7)(3.43752, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7.25)(3.125, 7)(3.43752, 7)
\psline[linewidth=0.03,linecolor=black](3.125, 7.25)(3.125, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7.25)(2.81252, 7.25)(3.125, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 7.25)(3.125, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 7.25)(3.125, 7.25)(3.125, 7.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 7.25)(3.125, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 7.25)(3.125, 7.5)(2.81252, 7.5)
\psline[linewidth=0.03,linecolor=black](3.125, 7.5)(2.81252, 7.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 7.25)(2.81252, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.5)(2.81252, 7.25)(2.81252, 7.5)
\psline[linewidth=0.03,linecolor=black](2.5, 7.5)(2.81252, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.5)(2.81252, 7.5)(2.81252, 7.75)
\psline[linewidth=0.03,linecolor=black](2.5, 7.5)(2.81252, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.75)(2.5, 7.5)(2.81252, 7.75)
\psline[linewidth=0.03,linecolor=black](2.5, 7.75)(2.81252, 7.75)
\psline[linewidth=0.03,linecolor=black](2.5, 7.5)(2.5, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.5)(2.5, 7.75)(2.18752, 7.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.75)(2.5, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 7.75)(2.5, 7.75)(2.18752, 8)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.75)(2.18752, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8)(2.18752, 7.75)(2.18752, 8)
\psline[linewidth=0.03,linecolor=black](1.875, 8)(2.18752, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 8.25)(1.875, 8)(2.18752, 8)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.25)(1.875, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 8.25)(1.875, 8.25)(1.875, 8)
\psline[linewidth=0.03,linecolor=black](1.875, 8.25)(1.875, 8)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.25)(1.875, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 8.25)(1.875, 8.5)(1.875, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8.25)(1.56258, 8.25)(1.875, 8)
\psline[linewidth=0.03,linecolor=black](1.56258, 8.25)(1.875, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8.5)(1.56258, 8.25)(1.875, 8.25)
\psline[linewidth=0.03,linecolor=black](1.875, 8.5)(1.56258, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 8.5)(1.56258, 8.25)(1.875, 8.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 8.5)(1.875, 8.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 8.25)(1.56258, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 8.25)(1.56258, 8.5)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 8.5)(1.25, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 8.5)(1.25, 8.75)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](1.25, 8.75)(1.25, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 8.75)(0.93742, 8.75)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.75)(1.25, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.75)(1.25, 8.75)(1.25, 9)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.75)(1.25, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9)(0.93742, 8.75)(1.25, 9)
\psline[linewidth=0.03,linecolor=black](0.93742, 9)(1.25, 9)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.75)(0.93742, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.75)(0.93742, 9)(0.625159, 9)
\psline[linewidth=0.03,linecolor=black](0.625159, 9)(0.93742, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 9)(0.93742, 9)(0.625159, 9.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 9)(0.625159, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 9)(0.625159, 9.25)(0.312579, 9.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.25)(0.312579, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 9.25)(0.625159, 9.5)(0.312579, 9.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.5)(0.312579, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 9.5)(0.312579, 9.5)(0.312579, 9.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.5)(0.312579, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9.5)(0.625159, 9.5)(0.312579, 9.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.5)(0.312579, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9.5)(0.312579, 9.75)(0, 9.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.75)(0, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9.75)(0.312579, 10)(0, 9.75)
\psline[linewidth=0.03,linecolor=black](0, 9.75)(0.312579, 10)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 9.75)(0.312579, 10)(0, 10)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9)(1.25, 9)(1.25, 9.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 9)(1.25, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9)(1.25, 9.25)(0.93742, 9.25)
\psline[linewidth=0.03,linecolor=black](1.25, 9.25)(0.93742, 9.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 9)(0.93742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 9.25)(0.93742, 9)(0.93742, 9.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.25)(0.93742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 9.5)(0.625159, 9.25)(0.93742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 9.25)(1.25, 9.5)(0.93742, 9.25)
\psline[linewidth=0.03,linecolor=black](1.25, 9.5)(0.93742, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 9.5)(0.93742, 9.5)(0.93742, 9.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.5)(0.93742, 9.25)
\psline[linewidth=0.03,linecolor=black](1.25, 9.5)(0.93742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 9.5)(0.93742, 9.75)(0.93742, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9.5)(0.625159, 9.5)(0.93742, 9.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.5)(0.625159, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9.75)(0.625159, 9.5)(0.93742, 9.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.5)(0.93742, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 9.5)(0.93742, 9.75)(0.625159, 9.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.75)(0.625159, 9.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.5)(0.625159, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9.75)(0.625159, 9.5)(0.625159, 9.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.75)(0.625159, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 10)(0.312579, 9.75)(0.625159, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9.75)(0.625159, 10)(0.625159, 9.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 10)(0.625159, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 10)(0.312579, 10)(0.625159, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8.75)(1.56258, 8.5)(1.875, 8.5)
\psline[linewidth=0.03,linecolor=black](1.875, 8.75)(1.56258, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 8.5)(1.875, 8.75)(1.56258, 8.75)
\psline[linewidth=0.03,linecolor=black](1.875, 8.75)(1.56258, 8.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 8.5)(1.56258, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 8.75)(1.56258, 8.5)(1.56258, 8.75)
\psline[linewidth=0.03,linecolor=black](1.25, 8.75)(1.56258, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9)(1.25, 8.75)(1.56258, 8.75)
\psline[linewidth=0.03,linecolor=black](1.25, 8.75)(1.56258, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 8.75)(1.56258, 9)(1.25, 9)
\psline[linewidth=0.03,linecolor=black](1.25, 9)(1.56258, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 9)(1.56258, 9)(1.25, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8.75)(1.875, 9)(1.56258, 8.75)
\psline[linewidth=0.03,linecolor=black](1.875, 9)(1.56258, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 9)(1.56258, 9)(1.56258, 8.75)
\psline[linewidth=0.03,linecolor=black](1.875, 9)(1.56258, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9)(1.875, 9)(1.56258, 9.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 9)(1.56258, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9)(1.56258, 9.25)(1.25, 9.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.25)(1.25, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9.25)(1.25, 9.5)(1.25, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8)(2.5, 7.75)(2.81252, 7.75)
\psline[linewidth=0.03,linecolor=black](2.5, 7.75)(2.81252, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.75)(2.81252, 8)(2.5, 8)
\psline[linewidth=0.03,linecolor=black](2.81252, 8)(2.5, 8)
\psline[linewidth=0.03,linecolor=black](2.5, 7.75)(2.5, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.75)(2.5, 8)(2.18752, 8)
\psline[linewidth=0.03,linecolor=black](2.5, 8)(2.18752, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 8)(2.18752, 8.25)(2.18752, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8)(2.81252, 8.25)(2.5, 8)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.25)(2.5, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 8)(2.81252, 8.25)(2.5, 8.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.25)(2.5, 8.25)
\psline[linewidth=0.03,linecolor=black](2.5, 8)(2.5, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 8.25)(2.5, 8)(2.5, 8.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.25)(2.5, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 8.5)(2.18752, 8.25)(2.5, 8.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.25)(2.5, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 8.25)(2.5, 8.5)(2.18752, 8.5)
\psline[linewidth=0.03,linecolor=black](2.5, 8.5)(2.18752, 8.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.25)(2.18752, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8.5)(2.18752, 8.25)(2.18752, 8.5)
\psline[linewidth=0.03,linecolor=black](1.875, 8.5)(2.18752, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8.75)(1.875, 8.5)(2.18752, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 8.5)(2.18752, 8.75)(2.18752, 8.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.75)(2.18752, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 8.75)(1.875, 8.75)(2.18752, 8.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.75)(1.875, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 9)(1.875, 8.75)(2.18752, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.25)(2.81252, 8.5)(2.5, 8.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.5)(2.5, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.5)(2.5, 8.5)(2.5, 8.25)
\psline[linewidth=0.03,linecolor=black](2.5, 8.5)(2.81252, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 8.5)(2.81252, 8.5)(2.5, 8.75)
\psline[linewidth=0.03,linecolor=black](2.5, 8.5)(2.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 8.75)(2.5, 8.5)(2.5, 8.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.75)(2.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 9)(2.18752, 8.75)(2.5, 8.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 9)(2.18752, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 9)(1.875, 9)(2.18752, 8.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 9)(1.875, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 9)(2.18752, 9)(2.18752, 9.25)
\psline[linewidth=0.03,linecolor=black](1.875, 9)(2.18752, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 9)(2.18752, 9.25)(1.875, 9.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 9.25)(1.875, 9.25)
\psline[linewidth=0.03,linecolor=black](1.875, 9)(1.875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9.25)(1.875, 9)(1.875, 9.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.25)(1.875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 9.5)(1.56258, 9.25)(1.875, 9.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.25)(1.875, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9.25)(1.875, 9.5)(1.56258, 9.5)
\psline[linewidth=0.03,linecolor=black](1.875, 9.5)(1.56258, 9.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.25)(1.56258, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 9.5)(1.56258, 9.25)(1.56258, 9.5)
\psline[linewidth=0.03,linecolor=black](1.25, 9.5)(1.56258, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9.75)(1.25, 9.5)(1.56258, 9.5)
\psline[linewidth=0.03,linecolor=black](1.25, 9.5)(1.56258, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 9.5)(1.56258, 9.75)(1.25, 9.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.75)(1.25, 9.75)
\psline[linewidth=0.03,linecolor=black](1.25, 9.5)(1.25, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9.75)(1.25, 9.5)(1.25, 9.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.75)(1.25, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9.75)(1.25, 9.75)(1.25, 10)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.75)(1.25, 10)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 10)(0.93742, 9.75)(1.25, 10)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.75)(0.93742, 10)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 9.75)(0.93742, 10)(0.625159, 10)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9.75)(1.56258, 10)(1.25, 9.75)
\psline[linewidth=0.03,linecolor=black](1.25, 9.75)(1.56258, 10)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 9.75)(1.56258, 10)(1.25, 10)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 9.5)(1.56258, 9.75)(1.56258, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 9.25)(1.875, 9.5)(1.875, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7.5)(3.125, 7.75)(2.81252, 7.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 7.5)(3.125, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 7.5)(3.125, 7.75)(2.81252, 7.75)
\psline[linewidth=0.03,linecolor=black](3.125, 7.75)(2.81252, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7.75)(2.81252, 8)(2.81252, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7)(3.43752, 7.25)(3.43752, 7)
\psline[linewidth=0.03,linecolor=black](3.43752, 7.25)(3.43752, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 7.25)(3.125, 7.25)(3.43752, 7)
\psline[linewidth=0.03,linecolor=black](3.43752, 7.25)(3.125, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7.25)(3.43752, 7.25)(3.43752, 7.5)
\psline[linewidth=0.03,linecolor=black](3.125, 7.25)(3.43752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7.5)(3.125, 7.25)(3.43752, 7.5)
\psline[linewidth=0.03,linecolor=black](3.125, 7.5)(3.43752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7.75)(3.125, 7.5)(3.43752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 6)(4.06252, 6.25)(3.75, 6.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.25)(3.75, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6.25)(4.06252, 6.5)(3.75, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5.75)(3.43752, 5.5)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.75)(3.75, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 5.75)(3.43752, 5.75)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](3.75, 5.75)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](3.75, 5.75)(3.43752, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 6)(3.43752, 5.75)(3.75, 5.75)
\psline[linewidth=0.03,linecolor=black](3.75, 6)(3.75, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5.75)(3.75, 6)(3.75, 5.75)
\psline[linewidth=0.03,linecolor=black](3.75, 6)(4.06252, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6)(3.75, 6)(4.06252, 5.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 6)(4.06252, 5.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 6)(3.75, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6.25)(3.75, 6)(4.06252, 6)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.25)(4.06252, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 6.25)(4.06252, 6.25)(4.06252, 6)
\psline[linewidth=0.03,linecolor=black](4.375, 6.25)(4.06252, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 6.25)(4.06252, 6.5)(4.06252, 6.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.5)(4.375, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6.5)(4.375, 6.25)(4.375, 6.5)
\psline[linewidth=0.03,linecolor=black](4.375, 6.25)(4.375, 6.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.5)(4.375, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6.75)(4.06252, 6.5)(4.375, 6.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.75)(4.375, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 6.75)(4.06252, 6.75)(4.375, 6.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.75)(4.375, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 7)(4.06252, 6.75)(4.375, 6.75)
\psline[linewidth=0.03,linecolor=black](4.375, 7)(4.06252, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 7)(4.06252, 6.75)(4.375, 7)
\psline[linewidth=0.03,linecolor=black](4.06252, 7)(4.375, 7)
\psline[linewidth=0.03,linecolor=black](4.06252, 7)(4.06252, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6.75)(4.06252, 7)(3.75, 7)
\psline[linewidth=0.03,linecolor=black](3.75, 7)(4.06252, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7)(4.06252, 7)(3.75, 7.25)
\psline[linewidth=0.03,linecolor=black](3.75, 7)(3.75, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7)(3.75, 7.25)(3.43752, 7.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 7.25)(3.75, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 7.25)(3.75, 7.25)(3.43752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 7)(4.375, 7)(4.375, 7.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 7)(4.375, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 7)(4.375, 7.25)(4.06252, 7.25)
\psline[linewidth=0.03,linecolor=black](4.375, 7.25)(4.06252, 7.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 7)(4.06252, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7.25)(4.06252, 7)(4.06252, 7.25)
\psline[linewidth=0.03,linecolor=black](3.75, 7.25)(4.06252, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 7.5)(3.75, 7.25)(4.06252, 7.25)
\psline[linewidth=0.03,linecolor=black](3.75, 7.25)(4.06252, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7.5)(3.75, 7.25)(4.06252, 7.5)
\psline[linewidth=0.03,linecolor=black](3.75, 7.5)(4.06252, 7.5)
\psline[linewidth=0.03,linecolor=black](3.75, 7.5)(3.75, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7.25)(3.75, 7.5)(3.43752, 7.5)
\psline[linewidth=0.03,linecolor=black](3.75, 7.5)(3.43752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7.5)(3.43752, 7.75)(3.43752, 7.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 7.75)(3.43752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 7.75)(3.125, 7.75)(3.43752, 7.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 7.75)(3.125, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 8)(3.125, 7.75)(3.43752, 7.75)
\psline[linewidth=0.03,linecolor=black](3.125, 7.75)(3.43752, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 7.75)(3.43752, 8)(3.125, 8)
\psline[linewidth=0.03,linecolor=black](3.43752, 8)(3.125, 8)
\psline[linewidth=0.03,linecolor=black](3.125, 7.75)(3.125, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8)(3.125, 7.75)(3.125, 8)
\psline[linewidth=0.03,linecolor=black](2.81252, 8)(3.125, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.25)(2.81252, 8)(3.125, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 8)(3.43752, 8.25)(3.125, 8)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.25)(3.125, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 8.25)(3.125, 8.25)(3.125, 8)
\psline[linewidth=0.03,linecolor=black](3.125, 8.25)(3.125, 8)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.25)(3.125, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 8.25)(3.43752, 8.5)(3.125, 8.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.5)(3.125, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 8.5)(3.125, 8.5)(3.125, 8.25)
\psline[linewidth=0.03,linecolor=black](3.125, 8.5)(3.125, 8.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.5)(3.125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 8.5)(3.125, 8.75)(3.125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 8.5)(2.81252, 8.5)(3.125, 8.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.5)(3.125, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 8.75)(2.81252, 8.5)(3.125, 8.5)
\psline[linewidth=0.03,linecolor=black](3.125, 8.75)(2.81252, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.75)(2.81252, 8.5)(3.125, 8.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.75)(3.125, 8.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.75)(2.81252, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.5)(2.81252, 8.75)(2.5, 8.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.75)(2.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.75)(2.5, 9)(2.5, 8.75)
\psline[linewidth=0.03,linecolor=black](2.5, 9)(2.5, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9)(2.18752, 9)(2.5, 8.75)
\psline[linewidth=0.03,linecolor=black](2.5, 9)(2.18752, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9.25)(2.18752, 9)(2.5, 9)
\psline[linewidth=0.03,linecolor=black](2.18752, 9)(2.5, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 9)(2.5, 9.25)(2.18752, 9.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 9.25)(2.5, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 9.25)(2.5, 9.25)(2.18752, 9.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 9.25)(2.18752, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 9.5)(2.18752, 9.25)(2.18752, 9.5)
\psline[linewidth=0.03,linecolor=black](1.875, 9.5)(2.18752, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 9.75)(1.875, 9.5)(2.18752, 9.5)
\psline[linewidth=0.03,linecolor=black](1.875, 9.5)(2.18752, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 9.5)(2.18752, 9.75)(1.875, 9.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 9.75)(1.875, 9.75)
\psline[linewidth=0.03,linecolor=black](1.875, 9.5)(1.875, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 9.75)(1.875, 9.5)(1.875, 9.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.75)(1.875, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 10)(1.56258, 9.75)(1.875, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 9.75)(2.18752, 10)(1.875, 9.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 10)(1.875, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 10)(1.875, 10)(1.875, 9.75)
\psline[linewidth=0.03,linecolor=black](1.875, 10)(1.875, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 10)(1.56258, 10)(1.875, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.75)(3.125, 8.75)(3.125, 9)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.75)(3.125, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.75)(3.125, 9)(2.81252, 9)
\psline[linewidth=0.03,linecolor=black](3.125, 9)(2.81252, 9)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.75)(2.81252, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9)(2.81252, 8.75)(2.81252, 9)
\psline[linewidth=0.03,linecolor=black](2.5, 9)(2.81252, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9.25)(2.5, 9)(2.81252, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 9)(2.81252, 9.25)(2.81252, 9)
\psline[linewidth=0.03,linecolor=black](2.81252, 9.25)(2.81252, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 9.25)(2.5, 9.25)(2.81252, 9)
\psline[linewidth=0.03,linecolor=black](2.5, 9.25)(2.81252, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9.25)(2.81252, 9.25)(2.81252, 9.5)
\psline[linewidth=0.03,linecolor=black](2.5, 9.25)(2.81252, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9.5)(2.5, 9.25)(2.81252, 9.5)
\psline[linewidth=0.03,linecolor=black](2.5, 9.5)(2.81252, 9.5)
\psline[linewidth=0.03,linecolor=black](2.5, 9.5)(2.5, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9.25)(2.5, 9.5)(2.18752, 9.5)
\psline[linewidth=0.03,linecolor=black](2.5, 9.5)(2.18752, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9.5)(2.18752, 9.75)(2.18752, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 9.75)(2.5, 9.5)(2.81252, 9.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 9.75)(2.5, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 9.5)(2.81252, 9.75)(2.5, 9.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 9.75)(2.5, 9.75)
\psline[linewidth=0.03,linecolor=black](2.5, 9.5)(2.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 9.75)(2.5, 9.5)(2.5, 9.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 9.75)(2.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 10)(2.18752, 9.75)(2.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 9.75)(2.81252, 10)(2.5, 9.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 10)(2.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 10)(2.5, 10)(2.5, 9.75)
\psline[linewidth=0.03,linecolor=black](2.5, 10)(2.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 10)(2.18752, 10)(2.5, 9.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 8.25)(2.81252, 8.25)(3.125, 8)
\psline[linewidth=0.03,linecolor=black](3.125, 8.25)(2.81252, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 8.5)(2.81252, 8.25)(3.125, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7.5)(4.06252, 7.5)(4.06252, 7.75)
\psline[linewidth=0.03,linecolor=black](3.75, 7.5)(4.06252, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 7.5)(4.06252, 7.75)(3.75, 7.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 7.75)(3.75, 7.75)
\psline[linewidth=0.03,linecolor=black](3.75, 7.5)(3.75, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 7.75)(3.75, 7.5)(3.75, 7.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 7.75)(3.75, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 8)(3.43752, 7.75)(3.75, 7.75)
\psline[linewidth=0.03,linecolor=black](3.75, 8)(3.43752, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 8)(3.43752, 8)(3.43752, 7.75)
\psline[linewidth=0.03,linecolor=black](3.75, 8)(3.43752, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 8)(3.75, 8.25)(3.43752, 8)
\psline[linewidth=0.03,linecolor=black](3.75, 8.25)(3.43752, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 8.25)(3.43752, 8.25)(3.43752, 8)
\psline[linewidth=0.03,linecolor=black](3.75, 8.25)(3.43752, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 8.25)(3.43752, 8.5)(3.43752, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 7.75)(3.75, 8)(3.75, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 7.25)(4.375, 7.5)(4.06252, 7.25)
\psline[linewidth=0.03,linecolor=black](4.375, 7.5)(4.06252, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 7.5)(4.06252, 7.5)(4.06252, 7.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 7.5)(4.375, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 7.5)(4.375, 7.5)(4.06252, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 6.25)(4.6875, 6.5)(4.375, 6.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.5)(4.375, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6.5)(4.375, 6.75)(4.375, 6.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.5)(4.375, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6.5)(4.6875, 6.75)(4.375, 6.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.75)(4.375, 6.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.5)(4.6875, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6.75)(4.6875, 6.5)(5, 6.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.5)(5, 6.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.75)(5, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 7)(4.6875, 6.75)(5, 6.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.75)(5, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6.75)(5, 7)(4.6875, 7)
\psline[linewidth=0.03,linecolor=black](5, 7)(4.6875, 7)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.75)(4.6875, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 7)(4.6875, 6.75)(4.6875, 7)
\psline[linewidth=0.03,linecolor=black](4.375, 7)(4.6875, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 7)(4.6875, 7)(4.6875, 7.25)
\psline[linewidth=0.03,linecolor=black](4.375, 7)(4.6875, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 7.25)(4.375, 7)(4.6875, 7.25)
\psline[linewidth=0.03,linecolor=black](4.375, 7.25)(4.6875, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 7.5)(4.375, 7.25)(4.6875, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 7)(5, 7)(4.6875, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6.5)(5, 6.5)(5, 6.75)
\psline[linewidth=0.03,linecolor=black](5, 6.5)(5, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 6.5)(5.3125, 6.75)(5, 6.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 6.75)(5, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 6.75)(5, 6.5)(5.3125, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6.75)(4.375, 7)(4.375, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 5.75)(4.06252, 6)(4.06252, 5.75)
\psline[linewidth=0.03,linecolor=black](4.375, 5.75)(4.06252, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 6)(4.375, 5.75)(4.375, 6)
\psline[linewidth=0.03,linecolor=black](4.375, 5.75)(4.375, 6)
\psline[linewidth=0.03,linecolor=black](4.06252, 6)(4.375, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 6.25)(4.06252, 6)(4.375, 6)
\psline[linewidth=0.03,linecolor=black](4.375, 6.25)(4.375, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6)(4.375, 6.25)(4.375, 6)
\psline[linewidth=0.03,linecolor=black](4.6875, 6)(4.375, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 6.25)(4.6875, 6)(4.6875, 6.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 6)(4.6875, 6.25)
\psline[linewidth=0.03,linecolor=black](4.375, 6.25)(4.6875, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6.5)(4.375, 6.25)(4.6875, 6.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.5)(4.6875, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 6.25)(4.6875, 6.5)(4.6875, 6.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.5)(5, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6.5)(5, 6.25)(5, 6.5)
\psline[linewidth=0.03,linecolor=black](5, 6.25)(5, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 6.5)(5, 6.25)(5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](5, 6.25)(5.3125, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 6.25)(5.3125, 6.25)(5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 6.25)(5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](5, 6.25)(5.3125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 6.25)(5.3125, 6)(5.3125, 6.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 6)(5.3125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 6)(5.625, 6.25)(5.3125, 6.25)
\psline[linewidth=0.03,linecolor=black](5.625, 6.25)(5.3125, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 6.25)(5.3125, 6)(5.625, 6)
\psline[linewidth=0.03,linecolor=black](5.3125, 6)(5.625, 6)
\psline[linewidth=0.03,linecolor=black](5.625, 6.25)(5.625, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 6.25)(5.625, 6.25)(5.625, 6)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.25)(5.625, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 6)(5.93748, 6.25)(5.625, 6)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.25)(5.93748, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 6.25)(5.93748, 6)(6.25, 6)
\psline[linewidth=0.03,linecolor=black](6.25, 6)(5.93748, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 6)(5.93748, 6)(6.25, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 6)(5.625, 5.75)(5.625, 6)
\psline[linewidth=0.03,linecolor=black](5.625, 5.75)(5.625, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.75)(5.93748, 6)(5.625, 6)
\psline[linewidth=0.03,linecolor=black](5.93748, 6)(5.625, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 6)(5.625, 5.75)(5.93748, 5.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 5.75)(5.625, 5.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 6)(5.93748, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 6)(5.93748, 5.75)(6.25, 5.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 5.75)(6.25, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 5.75)(6.25, 5.5)(6.25, 5.75)
\psline[linewidth=0.03,linecolor=black](6.25, 5.5)(6.25, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 5.5)(6.56248, 5.75)(6.25, 5.75)
\psline[linewidth=0.03,linecolor=black](6.25, 5.5)(6.56248, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 5.75)(6.25, 5.5)(6.56248, 5.5)
\psline[linewidth=0.03,linecolor=black](6.25, 5.5)(6.56248, 5.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.75)(6.56248, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 5.75)(6.56248, 5.5)(6.875, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 5.5)(6.56248, 5.25)(6.56248, 5.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.5)(6.56248, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 5.5)(6.56248, 5.25)(6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.25)(6.875, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 5.25)(6.875, 5.25)(6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](6.875, 5.25)(6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.25)(6.875, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 5.25)(6.875, 5)(6.875, 5.25)
\psline[linewidth=0.03,linecolor=black](6.875, 5)(6.875, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 5)(7.18748, 5.25)(6.875, 5.25)
\psline[linewidth=0.03,linecolor=black](6.875, 5)(7.18748, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](7.18748, 5.25)(6.875, 5)(7.18748, 5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.25)(7.18748, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](7.5, 5)(7.18748, 5.25)(7.18748, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 5.25)(7.18748, 5.25)(6.875, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 5.75)(5.625, 5.75)(5.93748, 5.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 5.75)(5.93748, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 5.5)(5.93748, 5.75)(5.93748, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 6.25)(5.625, 6.25)(5.3125, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6)(5, 6.25)(4.6875, 6.25)
\psline[linewidth=0.03,linecolor=black](5, 6.25)(4.6875, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 6.25)(4.6875, 6)(5, 6)
\psline[linewidth=0.03,linecolor=black](4.6875, 6)(5, 6)
\psline[linewidth=0.03,linecolor=black](5, 6.25)(5, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 6)(5, 6.25)(5, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6)(5, 5.75)(5, 6)
\psline[linewidth=0.03,linecolor=black](5, 5.75)(5, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 5.75)(5.3125, 6)(5, 6)
\psline[linewidth=0.03,linecolor=black](5.3125, 6)(5, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 6)(5, 5.75)(5.3125, 5.75)
\psline[linewidth=0.03,linecolor=black](5, 5.75)(5.3125, 5.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 6)(5.3125, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.75)(5.3125, 6)(5.3125, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 5.75)(5.3125, 5.5)(5.3125, 5.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 5.5)(5.3125, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 5.5)(5.625, 5.75)(5.3125, 5.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 5.5)(5.625, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.5)(5.625, 5.75)(5.3125, 5.5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.5)(5.3125, 5.5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.5)(5.625, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.75)(5.625, 5.5)(5.93748, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.25)(5.625, 5.5)(5.3125, 5.5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.5)(5.625, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.5)(5.625, 5.25)(5.93748, 5.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 5.5)(5.625, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 5.5)(5.625, 5.25)(5.93748, 5.25)
\psline[linewidth=0.03,linecolor=black](5.625, 5.25)(5.93748, 5.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 5.5)(5.93748, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 5.5)(5.93748, 5.5)(5.93748, 5.25)
\psline[linewidth=0.03,linecolor=black](6.25, 5.5)(5.93748, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 5.5)(5.93748, 5.25)(6.25, 5.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 5.25)(6.25, 5.25)
\psline[linewidth=0.03,linecolor=black](6.25, 5.5)(6.25, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 5.25)(6.25, 5.5)(6.25, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 5.25)(6.25, 5)(6.25, 5.25)
\psline[linewidth=0.03,linecolor=black](6.25, 5)(6.25, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 5)(6.56248, 5.25)(6.25, 5.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.25)(6.25, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 5.25)(6.25, 5)(6.56248, 5)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.25)(6.56248, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 5)(6.56248, 5.25)(6.56248, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.25)(5.93748, 5)(5.93748, 5.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 5)(5.93748, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 5)(6.25, 5)(5.93748, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 5.75)(4.6875, 6)(4.375, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5.5)(3.75, 5.75)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.5)(3.75, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5.5)(4.06252, 5.75)(3.75, 5.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.5)(4.06252, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5.5)(4.375, 5.75)(4.06252, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5.5)(3.43752, 5.25)(3.75, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 5.25)(2.5, 5.5)(2.5, 5.25)
\psline[linewidth=0.03,linecolor=black](2.5, 5.5)(2.81252, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 5.5)(2.81252, 5.25)(2.81252, 5.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 5.25)(2.81252, 5.5)
\psline[linewidth=0.03,linecolor=black](2.5, 5.5)(2.81252, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 5.75)(2.5, 5.5)(2.81252, 5.5)
\psline[linewidth=0.03,linecolor=black](2.5, 5.75)(2.81252, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 5.75)(2.5, 5.75)(2.81252, 5.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 5.75)(2.81252, 5.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 5.75)(2.5, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 6)(2.5, 5.75)(2.81252, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5.75)(2.81252, 5.75)(2.81252, 5.5)
\psline[linewidth=0.03,linecolor=black](3.125, 5.75)(2.81252, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5.75)(2.81252, 6)(2.81252, 5.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 6)(2.81252, 5.75)
\psline[linewidth=0.03,linecolor=black](3.125, 5.75)(2.81252, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5.75)(3.125, 6)(2.81252, 6)
\psline[linewidth=0.03,linecolor=black](3.125, 6)(2.81252, 6)
\psline[linewidth=0.03,linecolor=black](3.125, 5.75)(3.125, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 6)(3.125, 5.75)(3.43752, 6)
\psline[linewidth=0.03,linecolor=black](3.125, 6)(3.43752, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.25)(3.125, 6)(3.43752, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 6)(2.81252, 6.25)(2.81252, 6)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.25)(3.125, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.25)(3.125, 6)(3.125, 6.25)
\psline[linewidth=0.03,linecolor=black](3.125, 6)(3.125, 6.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.25)(3.125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.5)(2.81252, 6.25)(3.125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 6)(3.43752, 6.25)(3.125, 6.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.25)(3.125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.25)(3.43752, 6.5)(3.125, 6.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.5)(3.125, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.5)(3.125, 6.5)(3.125, 6.25)
\psline[linewidth=0.03,linecolor=black](3.125, 6.5)(3.125, 6.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.5)(3.125, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.5)(3.43752, 6.75)(3.125, 6.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.75)(3.125, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 6.75)(3.125, 6.75)(3.125, 6.5)
\psline[linewidth=0.03,linecolor=black](3.125, 6.75)(3.43752, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 6.75)(3.43752, 6.75)(3.125, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 6.5)(2.81252, 6.5)(3.125, 6.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.5)(3.125, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 6.75)(2.81252, 6.5)(3.125, 6.5)
\psline[linewidth=0.03,linecolor=black](3.125, 6.75)(2.81252, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.75)(2.81252, 6.5)(3.125, 6.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.75)(3.125, 6.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.75)(2.81252, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.5)(2.81252, 6.75)(2.5, 6.75)
\psline[linewidth=0.03,linecolor=black](2.5, 6.75)(2.81252, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 6.75)(2.81252, 6.75)(2.5, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.75)(3.125, 6.75)(3.125, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.75)(3.125, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 7)(2.81252, 6.75)(3.125, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 7)(3.125, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 7)(2.81252, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.75)(2.81252, 7)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 7)(2.5, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 7)(2.81252, 7.25)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 7.25)(2.5, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 7.25)(2.5, 7.25)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.5, 7.25)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 7.25)(2.5, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 7.25)(2.5, 7.5)(2.5, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.25)(2.18752, 7.25)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.25)(2.5, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.5)(2.18752, 7.25)(2.5, 7.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.25)(2.5, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 7.25)(2.5, 7.5)(2.18752, 7.5)
\psline[linewidth=0.03,linecolor=black](2.5, 7.5)(2.18752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 7.5)(2.18752, 7.75)(2.18752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 7.25)(2.81252, 7)(3.125, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6)(2.5, 6)(2.81252, 5.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 6)(2.5, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.25)(2.5, 6)(2.81252, 6)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.25)(2.5, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 6)(2.81252, 6.25)(2.5, 6.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.25)(2.5, 6.25)
\psline[linewidth=0.03,linecolor=black](2.5, 6)(2.5, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6.25)(2.5, 6)(2.5, 6.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.25)(2.5, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 6.5)(2.18752, 6.25)(2.5, 6.25)
\psline[linewidth=0.03,linecolor=black](2.5, 6.5)(2.18752, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 6.5)(2.18752, 6.5)(2.18752, 6.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.5)(2.18752, 6.25)
\psline[linewidth=0.03,linecolor=black](2.5, 6.5)(2.18752, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 6.5)(2.18752, 6.75)(2.18752, 6.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.75)(2.18752, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6.75)(1.875, 6.75)(2.18752, 6.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.75)(1.875, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 6.75)(2.18752, 6.75)(2.18752, 7)
\psline[linewidth=0.03,linecolor=black](1.875, 6.75)(2.18752, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 6.75)(2.18752, 7)(1.875, 7)
\psline[linewidth=0.03,linecolor=black](2.18752, 7)(1.875, 7)
\psline[linewidth=0.03,linecolor=black](1.875, 6.75)(1.875, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 7)(1.875, 6.75)(1.875, 7)
\psline[linewidth=0.03,linecolor=black](1.56258, 7)(1.875, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 7.25)(1.56258, 7)(1.875, 7)
\psline[linewidth=0.03,linecolor=black](1.875, 7.25)(1.56258, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 7.25)(1.56258, 7.25)(1.56258, 7)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.25)(1.875, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 7.25)(1.875, 7.25)(1.56258, 7.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.25)(1.56258, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 7.25)(1.56258, 7.5)(1.25, 7.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.5)(1.25, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 7.5)(1.25, 7.75)(1.25, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 7)(1.875, 7.25)(1.875, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6.5)(1.875, 6.5)(2.18752, 6.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.5)(1.875, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 6.75)(1.875, 6.5)(2.18752, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.25)(2.81252, 6.5)(2.5, 6.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.5)(2.5, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 6.5)(2.5, 6.5)(2.5, 6.25)
\psline[linewidth=0.03,linecolor=black](2.5, 6.5)(2.81252, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 6.5)(2.81252, 6.5)(2.5, 6.75)
\psline[linewidth=0.03,linecolor=black](2.5, 6.5)(2.5, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6.75)(2.5, 6.5)(2.5, 6.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.75)(2.5, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6.75)(2.5, 6.75)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.75)(2.5, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 7)(2.18752, 6.75)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.18752, 7)(2.5, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 7.25)(2.18752, 7)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.25)(2.18752, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 7.25)(1.875, 7.25)(2.18752, 7)
\psline[linewidth=0.03,linecolor=black](1.875, 7.25)(2.18752, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 7.25)(2.18752, 7.25)(2.18752, 7.5)
\psline[linewidth=0.03,linecolor=black](1.875, 7.25)(2.18752, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 7.5)(1.875, 7.25)(2.18752, 7.5)
\psline[linewidth=0.03,linecolor=black](1.875, 7.5)(2.18752, 7.5)
\psline[linewidth=0.03,linecolor=black](1.875, 7.25)(1.875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 7.25)(1.875, 7.5)(1.56258, 7.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.5)(1.875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 7.5)(1.875, 7.5)(1.56258, 7.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.5)(1.56258, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 7.75)(1.56258, 7.5)(1.56258, 7.75)
\psline[linewidth=0.03,linecolor=black](1.25, 7.75)(1.56258, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 8)(1.25, 7.75)(1.56258, 7.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 8)(1.25, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 7.75)(1.56258, 8)(1.25, 8)
\psline[linewidth=0.03,linecolor=black](1.56258, 8)(1.25, 8)
\psline[linewidth=0.03,linecolor=black](1.25, 7.75)(1.25, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8)(1.25, 7.75)(1.25, 8)
\psline[linewidth=0.03,linecolor=black](0.93742, 8)(1.25, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.25)(0.93742, 8)(1.25, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 8)(1.56258, 8.25)(1.25, 8)
\psline[linewidth=0.03,linecolor=black](1.56258, 8.25)(1.25, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 8.25)(1.25, 8.25)(1.25, 8)
\psline[linewidth=0.03,linecolor=black](1.25, 8.25)(1.25, 8)
\psline[linewidth=0.03,linecolor=black](1.25, 8.25)(1.56258, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 8.25)(1.56258, 8.25)(1.25, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 8.25)(0.93742, 8.25)(1.25, 8)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.25)(1.25, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.25)(1.25, 8.25)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.25)(1.25, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.5)(0.93742, 8.25)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.5)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.5)(0.93742, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.25)(0.93742, 8.5)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.5)(0.625159, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.5)(0.93742, 8.75)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.75)(0.625159, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.75)(0.625159, 8.75)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 8.75)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.75)(0.625159, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.75)(0.625159, 9)(0.625159, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 8.75)(0.312579, 8.75)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.75)(0.625159, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 9)(0.312579, 8.75)(0.625159, 8.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.75)(0.625159, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.75)(0.625159, 9)(0.312579, 9)
\psline[linewidth=0.03,linecolor=black](0.312579, 9)(0.625159, 9)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.75)(0.312579, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.75)(0.312579, 9)(0, 9)
\psline[linewidth=0.03,linecolor=black](0.312579, 9)(0, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9)(0, 9.25)(0, 9)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9)(0.625159, 9)(0.312579, 9.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 9)(0.312579, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9)(0.312579, 9.25)(0, 9.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.25)(0, 9.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9.25)(0.312579, 9.5)(0, 9.25)
\psline[linewidth=0.03,linecolor=black](0, 9.25)(0.312579, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 9.25)(0.312579, 9.5)(0, 9.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.5)(0, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 9.5)(0, 9.75)(0, 9.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.75)(0.93742, 8.5)(1.25, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 7.75)(1.875, 7.5)(2.18752, 7.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.75)(1.875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 7.75)(1.875, 7.5)(2.18752, 7.75)
\psline[linewidth=0.03,linecolor=black](1.875, 7.75)(2.18752, 7.75)
\psline[linewidth=0.03,linecolor=black](1.875, 7.75)(1.875, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 7.5)(1.875, 7.75)(1.56258, 7.75)
\psline[linewidth=0.03,linecolor=black](1.875, 7.75)(1.56258, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 7.75)(1.875, 8)(1.56258, 7.75)
\psline[linewidth=0.03,linecolor=black](1.875, 8)(1.56258, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8)(1.56258, 8)(1.56258, 7.75)
\psline[linewidth=0.03,linecolor=black](1.875, 8)(1.56258, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8)(1.56258, 8.25)(1.56258, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 8)(1.875, 7.75)(2.18752, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 5.25)(3.125, 5.5)(2.81252, 5.5)
\psline[linewidth=0.03,linecolor=black](3.125, 5.5)(2.81252, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5.5)(3.125, 5.75)(2.81252, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4.75)(2.81252, 5)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.75)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.75)(2.81252, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 5)(2.81252, 4.75)(3.125, 5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.75)(3.125, 5)
\psline[linewidth=0.03,linecolor=black](2.81252, 5)(3.125, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 5)(3.125, 5)(3.125, 5.25)
\psline[linewidth=0.03,linecolor=black](3.125, 5)(3.125, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5)(3.43752, 5.25)(3.125, 5.25)
\psline[linewidth=0.03,linecolor=black](3.125, 5)(3.43752, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5)(3.43752, 5.25)(3.125, 5)
\psline[linewidth=0.03,linecolor=black](3.43752, 5)(3.125, 5)
\psline[linewidth=0.03,linecolor=black](3.43752, 5)(3.43752, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5.25)(3.43752, 5)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.25)(3.75, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 5.25)(3.43752, 5.25)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](3.75, 5.25)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](3.75, 5.25)(3.43752, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5.25)(3.75, 5.25)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](3.75, 5.25)(3.75, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 5.25)(4.06252, 5.25)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.25)(3.75, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5.25)(4.06252, 5.5)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.5)(4.06252, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5.5)(4.06252, 5.25)(4.375, 5.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.5)(4.375, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 5.75)(4.06252, 5.5)(4.375, 5.5)
\psline[linewidth=0.03,linecolor=black](4.375, 5.75)(4.375, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5.5)(4.375, 5.75)(4.375, 5.5)
\psline[linewidth=0.03,linecolor=black](4.375, 5.75)(4.6875, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 5.75)(4.6875, 5.5)(4.6875, 5.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.5)(4.6875, 5.75)
\psline[linewidth=0.03,linecolor=black](4.375, 5.75)(4.6875, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 6)(4.375, 5.75)(4.6875, 5.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 6)(4.6875, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 5.75)(4.6875, 6)(4.6875, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5.5)(5, 5.75)(4.6875, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5.25)(3.75, 5.25)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.25)(3.75, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5)(4.06252, 5.25)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.25)(4.06252, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5.25)(4.06252, 5)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.25)(4.375, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 5.25)(4.06252, 5.25)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](4.375, 5.25)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.25)(4.375, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 5.5)(4.06252, 5.25)(4.375, 5.25)
\psline[linewidth=0.03,linecolor=black](4.375, 5.5)(4.375, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5.25)(4.375, 5.5)(4.375, 5.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.25)(4.375, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5.25)(4.6875, 5.5)(4.375, 5.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.25)(4.6875, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5.5)(4.6875, 5.25)(5, 5.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.25)(5, 5.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.5)(5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 5.75)(4.6875, 5.5)(5, 5.5)
\psline[linewidth=0.03,linecolor=black](5, 5.75)(5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 5.5)(5, 5.75)(5, 5.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 5.5)(5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 5.25)(5.3125, 5.5)(5, 5.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 5.25)(5.3125, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 5.25)(5.625, 5.25)(5.3125, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5.25)(5, 5.25)(5, 5.5)
\psline[linewidth=0.03,linecolor=black](5, 5.25)(5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 5.25)(5.3125, 5.25)(5, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5.25)(4.375, 5.25)(4.375, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 5)(4.375, 4.75)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](4.375, 4.75)(4.375, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4.75)(4.6875, 5)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5)(4.375, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5)(4.375, 4.75)(4.6875, 4.75)
\psline[linewidth=0.03,linecolor=black](4.375, 4.75)(4.6875, 4.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 5)(4.6875, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.75)(4.6875, 5)(4.6875, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 4.75)(4.375, 4.75)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 4.75)(4.6875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.75)(4.6875, 4.75)(4.6875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5)(4.6875, 5.25)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5)(4.6875, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5.25)(4.6875, 5)(5, 5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5)(5, 5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.25)(5, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 5.25)(4.6875, 5.25)(5, 5)
\psline[linewidth=0.03,linecolor=black](5, 5.25)(5, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 5.25)(5, 5.25)(5, 5)
\psline[linewidth=0.03,linecolor=black](5.3125, 5.25)(5, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 5)(5.3125, 5.25)(5, 5)
\psline[linewidth=0.03,linecolor=black](5.3125, 5)(5.3125, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.25)(5.3125, 5.25)(5.3125, 5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.25)(5.3125, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5)(5.625, 5.25)(5.3125, 5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.25)(5.625, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5.25)(5.625, 5)(5.93748, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 5)(5, 4.75)(5, 5)
\psline[linewidth=0.03,linecolor=black](5, 4.75)(5, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.75)(5.3125, 5)(5, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 4.75)(4.06252, 5)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.75)(4.06252, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 4.75)(4.375, 4.75)(4.06252, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4.75)(3.43752, 5)(3.125, 5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.75)(3.43752, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 5)(3.43752, 4.75)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.75)(3.75, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4.75)(3.75, 4.75)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](3.75, 4.75)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.75)(3.75, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4.75)(3.43752, 4.75)(3.75, 4.5)
\psline[linewidth=0.03,linecolor=black](3.75, 4.75)(3.75, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 4.75)(3.75, 4.75)(3.75, 4.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.75)(3.75, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 4.75)(3.75, 4.5)(4.06252, 4.5)
\psline[linewidth=0.03,linecolor=black](3.75, 4.5)(4.06252, 4.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.75)(4.06252, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4.75)(4.06252, 4.75)(4.06252, 4.5)
\psline[linewidth=0.03,linecolor=black](4.375, 4.75)(4.06252, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4.5)(4.375, 4.75)(4.06252, 4.5)
\psline[linewidth=0.03,linecolor=black](4.375, 4.75)(4.375, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4.75)(4.375, 4.5)(4.6875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4.5)(4.06252, 4.25)(4.06252, 4.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.25)(4.06252, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 4.25)(4.375, 4.5)(4.06252, 4.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.25)(4.375, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 4.25)(4.375, 4.25)(4.375, 4.5)
\psline[linewidth=0.03,linecolor=black](4.375, 4.5)(4.375, 4.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.25)(4.375, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 4.25)(4.375, 4)(4.375, 4.25)
\psline[linewidth=0.03,linecolor=black](4.375, 4.25)(4.375, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4.25)(4.375, 4)(4.6875, 4.25)
\psline[linewidth=0.03,linecolor=black](4.375, 4)(4.6875, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4)(4.6875, 4)(4.6875, 4.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 4)(4.6875, 4.25)
\psline[linewidth=0.03,linecolor=black](4.375, 4)(4.6875, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 4)(4.375, 4)(4.6875, 3.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 4)(4.6875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4)(4.6875, 4)(4.6875, 3.75)
\psline[linewidth=0.03,linecolor=black](5, 4)(4.6875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 3.75)(5, 4)(4.6875, 3.75)
\psline[linewidth=0.03,linecolor=black](5, 3.75)(5, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4)(5, 3.75)(5.3125, 3.75)
\psline[linewidth=0.03,linecolor=black](5, 4)(5.3125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 4)(5, 4)(5.3125, 3.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 4)(5.3125, 3.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 4)(5, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4)(5.3125, 4)(5.3125, 4.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 4)(5.3125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 4)(5.625, 4)(5.3125, 4.25)
\psline[linewidth=0.03,linecolor=black](5.625, 4)(5.3125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4)(5.625, 4.25)(5.3125, 4.25)
\psline[linewidth=0.03,linecolor=black](5.625, 4.25)(5.625, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.25)(5.625, 4)(5.93748, 4.25)
\psline[linewidth=0.03,linecolor=black](5.625, 4.25)(5.93748, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.25)(5.93748, 4.25)(5.93748, 4.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 4.5)(5.93748, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 4.5)(5.93748, 4.25)(6.25, 4.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 4.5)(6.25, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 4.75)(5.93748, 4.5)(6.25, 4.5)
\psline[linewidth=0.03,linecolor=black](6.25, 4.75)(6.25, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 4.5)(6.25, 4.75)(6.25, 4.5)
\psline[linewidth=0.03,linecolor=black](6.56248, 4.5)(6.25, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 4.75)(6.56248, 4.5)(6.56248, 4.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 4.5)(6.56248, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 4.5)(6.875, 4.5)(6.56248, 4.75)
\psline[linewidth=0.03,linecolor=black](6.875, 4.5)(6.56248, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 4.5)(6.875, 4.75)(6.56248, 4.75)
\psline[linewidth=0.03,linecolor=black](6.875, 4.5)(6.875, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 4.5)(7.18748, 4.75)(6.875, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4)(5.3125, 4)(5.3125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 4)(5, 4)(4.6875, 4.25)
\psline[linewidth=0.03,linecolor=black](5, 4)(4.6875, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4)(5, 4.25)(4.6875, 4.25)
\psline[linewidth=0.03,linecolor=black](5, 4)(5, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.25)(5, 4)(5.3125, 4.25)
\psline[linewidth=0.03,linecolor=black](5, 4.25)(5.3125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.25)(5.3125, 4.25)(5.3125, 4.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 4.25)(5.3125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 4.25)(5.625, 4.25)(5.3125, 4.5)
\psline[linewidth=0.03,linecolor=black](5.625, 4.25)(5.3125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.25)(5.625, 4.5)(5.3125, 4.5)
\psline[linewidth=0.03,linecolor=black](5.625, 4.25)(5.625, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.5)(5.625, 4.25)(5.93748, 4.5)
\psline[linewidth=0.03,linecolor=black](5.625, 4.5)(5.93748, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.5)(5.93748, 4.5)(5.93748, 4.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 4.5)(5.93748, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 4.5)(6.25, 4.75)(5.93748, 4.75)
\psline[linewidth=0.03,linecolor=black](6.25, 4.75)(5.93748, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 4.75)(6.25, 5)(5.93748, 4.75)
\psline[linewidth=0.03,linecolor=black](6.25, 5)(6.25, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 5)(6.25, 4.75)(6.56248, 4.75)
\psline[linewidth=0.03,linecolor=black](6.25, 5)(6.56248, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 5)(6.25, 5)(6.56248, 4.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 5)(6.56248, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 4.75)(6.56248, 5)(6.56248, 4.75)
\psline[linewidth=0.03,linecolor=black](6.875, 4.75)(6.56248, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 4.75)(6.875, 5)(6.56248, 5)
\psline[linewidth=0.03,linecolor=black](6.875, 4.75)(6.875, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 4.75)(7.18748, 4.75)(6.875, 5)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.75)(6.875, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 5)(7.18748, 4.75)(7.18748, 5)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.75)(7.18748, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](7.18748, 4.75)(7.5, 5)(7.18748, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4.5)(4.375, 4.25)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](4.375, 4.25)(4.6875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4.25)(4.6875, 4.25)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 4.25)(4.6875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 4.25)(5, 4.25)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](5, 4.25)(4.6875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.25)(5, 4.5)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](5, 4.5)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](5, 4.25)(5, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.5)(5, 4.25)(5.3125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.5)(5, 4.75)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](5, 4.75)(5, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.75)(5, 4.5)(5.3125, 4.5)
\psline[linewidth=0.03,linecolor=black](5, 4.75)(5.3125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.75)(5.3125, 4.5)(5.3125, 4.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 4.5)(5.3125, 4.75)
\psline[linewidth=0.03,linecolor=black](5, 4.75)(5.3125, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 4.75)(5.3125, 4.75)(5.3125, 5)
\psline[linewidth=0.03,linecolor=black](5.3125, 4.75)(5.3125, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 4.75)(5.625, 4.75)(5.3125, 5)
\psline[linewidth=0.03,linecolor=black](5.625, 4.75)(5.3125, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.75)(5.625, 5)(5.3125, 5)
\psline[linewidth=0.03,linecolor=black](5.625, 4.75)(5.625, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 5)(5.625, 4.75)(5.93748, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 4.5)(5.625, 4.5)(5.3125, 4.75)
\psline[linewidth=0.03,linecolor=black](5.625, 4.5)(5.3125, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.5)(5.625, 4.75)(5.3125, 4.75)
\psline[linewidth=0.03,linecolor=black](5.625, 4.5)(5.625, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.75)(5.625, 4.5)(5.93748, 4.75)
\psline[linewidth=0.03,linecolor=black](5.625, 4.75)(5.93748, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4.75)(5.93748, 4.75)(5.93748, 5)
\psline[linewidth=0.03,linecolor=black](5.93748, 4.75)(5.93748, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 4.75)(6.25, 5)(5.93748, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4.75)(4.06252, 4.75)(3.75, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 5)(2.81252, 4.75)(3.125, 4.75)
\psline[linewidth=0.03,linecolor=black](3.125, 4.75)(2.81252, 4.75)
\psline[linewidth=0.03,linecolor=black](3.125, 5)(3.125, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4.75)(3.125, 5)(3.125, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 4.75)(2.81252, 4.75)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](3.125, 4.75)(3.125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4.75)(3.125, 4.75)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.75)(3.125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4.5)(3.43752, 4.75)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.5)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.5)(3.43752, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4.5)(3.43752, 4.75)(3.43752, 4.5)
\psline[linewidth=0.03,linecolor=black](3.75, 4.5)(3.43752, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4.25)(3.75, 4.5)(3.43752, 4.5)
\psline[linewidth=0.03,linecolor=black](3.75, 4.25)(3.75, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4.25)(4.06252, 4.25)(3.75, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4.25)(3.43752, 4.5)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.25)(3.43752, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4.25)(3.75, 4.25)(3.43752, 4.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.25)(3.75, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4)(3.75, 4.25)(3.43752, 4.25)
\psline[linewidth=0.03,linecolor=black](3.75, 4)(3.75, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4)(4.06252, 4.25)(3.75, 4.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.25)(3.75, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 4.25)(3.75, 4)(4.06252, 4)
\psline[linewidth=0.03,linecolor=black](3.75, 4)(4.06252, 4)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.25)(4.06252, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4)(4.06252, 4.25)(4.06252, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4)(4.06252, 3.75)(4.06252, 4)
\psline[linewidth=0.03,linecolor=black](4.06252, 3.75)(4.06252, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3.75)(4.375, 4)(4.06252, 4)
\psline[linewidth=0.03,linecolor=black](4.375, 4)(4.06252, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 3.75)(4.375, 4)(4.06252, 3.75)
\psline[linewidth=0.03,linecolor=black](4.375, 3.75)(4.06252, 3.75)
\psline[linewidth=0.03,linecolor=black](4.375, 3.75)(4.375, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 4)(4.375, 3.75)(4.6875, 3.75)
\psline[linewidth=0.03,linecolor=black](4.375, 3.75)(4.6875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 3.75)(4.6875, 3.5)(4.6875, 3.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.5)(4.6875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 3.5)(5, 3.75)(4.6875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3.5)(4.375, 3.75)(4.06252, 3.75)
\psline[linewidth=0.03,linecolor=black](4.375, 3.75)(4.06252, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 3.75)(4.06252, 3.5)(4.375, 3.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 3.5)(4.375, 3.5)
\psline[linewidth=0.03,linecolor=black](4.375, 3.75)(4.375, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 3.5)(4.375, 3.75)(4.375, 3.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.5)(4.375, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 3.25)(4.6875, 3.5)(4.375, 3.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.5)(4.6875, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 3.5)(4.6875, 3.25)(5, 3.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.25)(5, 3.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.5)(5, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 3.75)(4.6875, 3.5)(5, 3.5)
\psline[linewidth=0.03,linecolor=black](5, 3.75)(5, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 3.75)(5, 3.5)(5.3125, 3.5)
\psline[linewidth=0.03,linecolor=black](5, 3.75)(5.3125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 3.75)(5, 3.75)(5.3125, 3.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 3.75)(5.3125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 3.5)(5.3125, 3.75)(5.3125, 3.5)
\psline[linewidth=0.03,linecolor=black](5.625, 3.5)(5.3125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 3.5)(5.625, 3.75)(5.3125, 3.75)
\psline[linewidth=0.03,linecolor=black](5.625, 3.75)(5.3125, 3.75)
\psline[linewidth=0.03,linecolor=black](5.625, 3.5)(5.625, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 3.5)(5.93748, 3.75)(5.625, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 3.75)(5.625, 4)(5.3125, 3.75)
\psline[linewidth=0.03,linecolor=black](5.625, 4)(5.625, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 3.75)(5.625, 4)(5.625, 3.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 3.75)(5.625, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 4)(5.625, 4)(5.93748, 3.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 4)(5.93748, 3.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 4)(5.625, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.625, 4)(5.93748, 4)(5.93748, 4.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 4)(5.93748, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 4)(6.25, 4)(5.93748, 4.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 4.25)(6.25, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.93748, 4.25)(6.25, 4)(6.25, 4.25)
\psline[linewidth=0.03,linecolor=black](6.25, 4)(6.25, 4.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 4.25)(6.25, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 4.5)(5.93748, 4.25)(6.25, 4.25)
\psline[linewidth=0.03,linecolor=black](6.25, 4.5)(6.25, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 4.5)(6.25, 4.5)(6.25, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 4)(6.56248, 4.25)(6.25, 4.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 4.25)(6.25, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.56248, 4.25)(6.56248, 4.5)(6.25, 4.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 4.25)(6.56248, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.875, 4.5)(6.56248, 4.5)(6.56248, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](6.25, 4)(5.93748, 4)(5.93748, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 3.5)(4.6875, 3.25)(5, 3.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.25)(5, 3.25)
\psline[linewidth=0.03,linecolor=black](5, 3.5)(5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 3.25)(5, 3.5)(5, 3.25)
\psline[linewidth=0.03,linecolor=black](5, 3.5)(5.3125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 3.5)(5.3125, 3.25)(5.3125, 3.5)
\psline[linewidth=0.03,linecolor=black](5.3125, 3.25)(5.3125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5.3125, 3.25)(5.625, 3.5)(5.3125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 3.25)(5, 3)(5, 3.25)
\psline[linewidth=0.03,linecolor=black](5, 3)(5, 3.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.25)(5, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 3.25)(4.6875, 3)(5, 3)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.25)(4.6875, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 3)(4.6875, 3.25)(4.375, 3)
\psline[linewidth=0.03,linecolor=black](4.6875, 3)(4.375, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 2.75)(4.6875, 3)(4.375, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](5, 3)(5.3125, 3.25)(5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3.5)(4.375, 3.25)(4.375, 3.5)
\psline[linewidth=0.03,linecolor=black](4.375, 3.25)(4.375, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 3.25)(4.6875, 3.25)(4.375, 3.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.25)(4.375, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.6875, 3.25)(4.375, 3.25)(4.375, 3)
\psline[linewidth=0.03,linecolor=black](4.375, 3.25)(4.375, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 3.25)(4.06252, 3)(4.375, 3)
\psline[linewidth=0.03,linecolor=black](4.06252, 3)(4.375, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3)(4.375, 2.75)(4.375, 3)
\psline[linewidth=0.03,linecolor=black](4.375, 2.75)(4.06252, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 2.75)(4.06252, 3)(4.06252, 2.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 3)(4.06252, 2.75)
\psline[linewidth=0.03,linecolor=black](4.375, 2.75)(4.06252, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 2.5)(4.375, 2.75)(4.06252, 2.75)
\psline[linewidth=0.03,linecolor=black](4.375, 2.5)(4.06252, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 2.5)(4.06252, 2.75)(4.06252, 2.5)
\psline[linewidth=0.03,linecolor=black](4.375, 2.5)(4.06252, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 2.25)(4.375, 2.5)(4.06252, 2.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 2.25)(4.06252, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.25)(4.06252, 2.25)(4.06252, 2.5)
\psline[linewidth=0.03,linecolor=black](3.75, 2.25)(4.06252, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.25)(4.06252, 2)(4.06252, 2.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 2)(3.75, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 2)(3.75, 2.25)(3.75, 2)
\psline[linewidth=0.03,linecolor=black](3.75, 2.25)(3.75, 2)
\psline[linewidth=0.03,linecolor=black](4.06252, 2)(3.75, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 1.75)(4.06252, 2)(3.75, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.25)(3.43752, 2)(3.75, 2)
\psline[linewidth=0.03,linecolor=black](3.43752, 2)(3.75, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 2)(3.75, 1.75)(3.75, 2)
\psline[linewidth=0.03,linecolor=black](3.43752, 2)(3.75, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 2)(3.43752, 1.75)(3.75, 1.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.75)(3.75, 1.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 2)(3.43752, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 1.75)(3.43752, 2)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.75)(3.125, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 1.5)(3.43752, 1.75)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.5)(3.125, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 1.5)(3.43752, 1.5)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](3.125, 1.5)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](3.125, 1.5)(3.43752, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 1.5)(3.125, 1.5)(3.125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1.5)(3.125, 1.5)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.5)(3.125, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 1.5)(2.81252, 1.5)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.5)(3.125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1.5)(2.81252, 1.25)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.25)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.25)(2.81252, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1.25)(2.81252, 1.5)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.25)(2.5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1)(2.81252, 1.25)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1)(2.5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 1)(2.81252, 1)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.5, 1)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.5, 1)(2.81252, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 0.75)(2.81252, 1)(2.5, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1)(2.5, 1)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 1)(2.5, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1)(2.5, 0.75)(2.5, 1)
\psline[linewidth=0.03,linecolor=black](2.5, 0.75)(2.18752, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 0.75)(2.18752, 1)(2.18752, 0.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 1)(2.18752, 0.75)
\psline[linewidth=0.03,linecolor=black](2.5, 0.75)(2.18752, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 0.5)(2.5, 0.75)(2.18752, 0.75)
\psline[linewidth=0.03,linecolor=black](2.5, 0.5)(2.18752, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 0.5)(2.5, 0.5)(2.18752, 0.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 0.5)(2.18752, 0.75)
\psline[linewidth=0.03,linecolor=black](2.5, 0.5)(2.18752, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 0.25)(2.5, 0.5)(2.18752, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0.5)(2.18752, 0.5)(2.18752, 0.75)
\psline[linewidth=0.03,linecolor=black](1.875, 0.5)(2.18752, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0.5)(2.18752, 0.25)(2.18752, 0.5)
\psline[linewidth=0.03,linecolor=black](1.875, 0.5)(2.18752, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 0.25)(1.875, 0.5)(1.875, 0.25)
\psline[linewidth=0.03,linecolor=black](1.875, 0.5)(1.875, 0.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 0.25)(1.875, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 0)(2.18752, 0.25)(1.875, 0.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 0)(1.875, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0)(2.18752, 0)(1.875, 0.25)
\psline[linewidth=0.03,linecolor=black](1.875, 0)(1.875, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0)(1.875, 0)(1.875, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0.5)(1.56258, 0.25)(1.875, 0.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.25)(1.875, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0.25)(1.56258, 0)(1.875, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1)(1.875, 0.75)(2.18752, 0.75)
\psline[linewidth=0.03,linecolor=black](1.875, 0.75)(2.18752, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0.75)(1.875, 0.5)(2.18752, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1.25)(2.81252, 1)(3.125, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 1.75)(3.43752, 1.5)(3.75, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3)(3.75, 2.75)(4.06252, 2.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 2.75)(3.75, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 2.75)(3.75, 2.75)(4.06252, 2.5)
\psline[linewidth=0.03,linecolor=black](3.75, 2.75)(4.06252, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.75)(3.75, 2.5)(4.06252, 2.5)
\psline[linewidth=0.03,linecolor=black](3.75, 2.5)(4.06252, 2.5)
\psline[linewidth=0.03,linecolor=black](3.75, 2.5)(3.75, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.5)(3.75, 2.75)(3.43752, 2.5)
\psline[linewidth=0.03,linecolor=black](3.75, 2.5)(3.43752, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.25)(3.75, 2.5)(3.43752, 2.5)
\psline[linewidth=0.03,linecolor=black](3.75, 2.25)(3.43752, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 2.25)(3.75, 2.25)(3.43752, 2.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 2.25)(3.43752, 2.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 2.25)(3.75, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 2)(3.75, 2.25)(3.43752, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.25)(3.43752, 2.25)(3.43752, 2.5)
\psline[linewidth=0.03,linecolor=black](3.125, 2.25)(3.43752, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.25)(3.43752, 2)(3.43752, 2.25)
\psline[linewidth=0.03,linecolor=black](3.125, 2.25)(3.43752, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 2)(3.125, 2.25)(3.125, 2)
\psline[linewidth=0.03,linecolor=black](3.125, 2.25)(3.125, 2)
\psline[linewidth=0.03,linecolor=black](3.43752, 2)(3.125, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 2)(3.125, 2)(3.125, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.25)(2.81252, 2)(3.125, 2)
\psline[linewidth=0.03,linecolor=black](3.125, 2)(2.81252, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2)(2.81252, 2)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 2)(3.125, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2)(2.81252, 1.75)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.75)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.75)(2.81252, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1.75)(2.81252, 2)(2.5, 1.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.75)(2.5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1.5)(2.81252, 1.75)(2.5, 1.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.5)(2.5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 1.5)(2.81252, 1.5)(2.5, 1.75)
\psline[linewidth=0.03,linecolor=black](2.5, 1.5)(2.81252, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1.5)(2.5, 1.5)(2.5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 1.75)(2.81252, 1.5)(3.125, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.5)(3.75, 2.25)(4.06252, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 4.75)(2.81252, 4.75)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.5, 4.75)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.75)(2.5, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 4.5)(2.81252, 4.75)(2.5, 4.75)
\psline[linewidth=0.03,linecolor=black](2.5, 4.5)(2.5, 4.75)
\psline[linewidth=0.03,linecolor=black](2.5, 4.5)(2.81252, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4.5)(2.81252, 4.75)(2.5, 4.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.5)(2.5, 4.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.5)(2.81252, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4.75)(2.81252, 4.5)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.5)(3.125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4.5)(2.81252, 4.25)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.25)(3.125, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 4.5)(2.81252, 4.25)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.25)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](3.125, 4.5)(3.125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4.25)(3.125, 4.5)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.25)(3.125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4)(3.43752, 4.25)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 4)(3.43752, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4)(3.75, 4)(3.43752, 4.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 4)(3.75, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4)(3.43752, 4)(3.43752, 3.75)
\psline[linewidth=0.03,linecolor=black](3.75, 4)(3.43752, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 3.75)(3.75, 4)(3.43752, 3.75)
\psline[linewidth=0.03,linecolor=black](3.75, 3.75)(3.43752, 3.75)
\psline[linewidth=0.03,linecolor=black](3.75, 4)(3.75, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 4)(3.75, 3.75)(4.06252, 3.75)
\psline[linewidth=0.03,linecolor=black](3.75, 3.75)(4.06252, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 3.75)(4.06252, 3.5)(4.06252, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 3.5)(3.75, 3.75)(3.43752, 3.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.5)(3.75, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 3.75)(3.43752, 3.5)(3.75, 3.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.5)(3.75, 3.5)
\psline[linewidth=0.03,linecolor=black](3.75, 3.75)(3.75, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3.5)(3.75, 3.75)(3.75, 3.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 3.5)(3.75, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 3.25)(4.06252, 3.5)(3.75, 3.5)
\psline[linewidth=0.03,linecolor=black](3.75, 3.25)(4.06252, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 3.25)(4.06252, 3.25)(4.06252, 3.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 3.25)(4.06252, 3.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 3.25)(3.75, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3.25)(3.75, 3.25)(4.06252, 3)
\psline[linewidth=0.03,linecolor=black](4.06252, 3)(3.75, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3)(3.75, 3.25)(3.75, 3)
\psline[linewidth=0.03,linecolor=black](3.75, 3.25)(3.75, 3)
\psline[linewidth=0.03,linecolor=black](4.06252, 3)(3.75, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.75)(4.06252, 3)(3.75, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 3.25)(3.43752, 3)(3.75, 3)
\psline[linewidth=0.03,linecolor=black](3.43752, 3)(3.75, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 3)(3.75, 2.75)(3.75, 3)
\psline[linewidth=0.03,linecolor=black](3.75, 2.75)(3.43752, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 2.75)(3.43752, 3)(3.43752, 2.75)
\psline[linewidth=0.03,linecolor=black](3.75, 2.75)(3.43752, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 2.5)(3.75, 2.75)(3.43752, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.06252, 3.25)(4.375, 3.25)(4.06252, 3.5)
\psline[linewidth=0.03,linecolor=black](4.375, 3.25)(4.06252, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](4.375, 3.25)(4.06252, 3.25)(4.06252, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 3.5)(3.75, 3.25)(3.75, 3.5)
\psline[linewidth=0.03,linecolor=black](3.75, 3.25)(3.43752, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 3.25)(3.43752, 3.5)(3.43752, 3.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.25)(3.43752, 3.5)
\psline[linewidth=0.03,linecolor=black](3.75, 3.25)(3.43752, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.75, 3.25)(3.43752, 3.25)(3.43752, 3)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.25)(3.43752, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 3.25)(3.125, 3)(3.43752, 3)
\psline[linewidth=0.03,linecolor=black](3.43752, 3)(3.125, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 3)(3.125, 3)(3.43752, 2.75)
\psline[linewidth=0.03,linecolor=black](3.125, 3)(3.43752, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 3)(3.125, 2.75)(3.43752, 2.75)
\psline[linewidth=0.03,linecolor=black](3.125, 2.75)(3.43752, 2.75)
\psline[linewidth=0.03,linecolor=black](3.125, 3)(3.125, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 3)(2.81252, 2.75)(3.125, 2.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 2.75)(3.125, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.75)(2.81252, 2.75)(3.125, 2.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 2.75)(3.125, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.5)(2.81252, 2.75)(2.81252, 2.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 2.75)(2.81252, 2.5)
\psline[linewidth=0.03,linecolor=black](3.125, 2.5)(2.81252, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.25)(3.125, 2.5)(2.81252, 2.5)
\psline[linewidth=0.03,linecolor=black](3.125, 2.25)(2.81252, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2.25)(3.125, 2.25)(2.81252, 2.5)
\psline[linewidth=0.03,linecolor=black](3.125, 2.25)(2.81252, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2)(3.125, 2.25)(2.81252, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2.75)(2.5, 2.5)(2.81252, 2.5)
\psline[linewidth=0.03,linecolor=black](2.5, 2.5)(2.81252, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 2.5)(2.81252, 2.25)(2.81252, 2.5)
\psline[linewidth=0.03,linecolor=black](2.5, 2.5)(2.81252, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2.25)(2.5, 2.5)(2.5, 2.25)
\psline[linewidth=0.03,linecolor=black](2.5, 2.5)(2.5, 2.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 2.25)(2.5, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2)(2.81252, 2.25)(2.5, 2.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 2)(2.5, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 2)(2.81252, 2)(2.5, 2.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 2)(2.5, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2)(2.5, 2)(2.5, 1.75)
\psline[linewidth=0.03,linecolor=black](2.5, 2)(2.5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 2)(2.18752, 1.75)(2.5, 1.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.75)(2.5, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1.75)(2.5, 1.5)(2.5, 1.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.75)(2.5, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1.75)(2.18752, 1.5)(2.5, 1.5)
\psline[linewidth=0.03,linecolor=black](2.5, 1.5)(2.18752, 1.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.75)(2.18752, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1.75)(1.875, 1.5)(2.18752, 1.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.5)(1.875, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1.5)(1.875, 1.5)(2.18752, 1.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.25)(1.875, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1.25)(1.875, 1.5)(1.875, 1.25)
\psline[linewidth=0.03,linecolor=black](1.875, 1.5)(1.875, 1.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.25)(1.875, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1)(2.18752, 1.25)(1.875, 1.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 1)(1.875, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 1)(2.18752, 1)(1.875, 1.25)
\psline[linewidth=0.03,linecolor=black](1.875, 1)(1.875, 1.25)
\psline[linewidth=0.03,linecolor=black](1.875, 1)(2.18752, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0.75)(2.18752, 1)(1.875, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1)(1.875, 1)(1.875, 1.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 1)(1.875, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1)(1.875, 0.75)(1.875, 1)
\psline[linewidth=0.03,linecolor=black](1.875, 0.75)(1.56258, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0.75)(1.56258, 1)(1.56258, 0.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.75)(1.56258, 1)
\psline[linewidth=0.03,linecolor=black](1.875, 0.75)(1.56258, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0.5)(1.875, 0.75)(1.56258, 0.75)
\psline[linewidth=0.03,linecolor=black](1.875, 0.5)(1.56258, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0.5)(1.875, 0.5)(1.56258, 0.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.5)(1.875, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 0.5)(1.56258, 0.5)(1.56258, 0.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.25)(1.56258, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0.25)(1.56258, 0.5)(1.25, 0.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.25)(1.25, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0)(1.56258, 0.25)(1.25, 0.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 0)(1.25, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0)(1.25, 0.25)(1.25, 0)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0.75)(1.56258, 1)(1.25, 0.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.75)(1.25, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0.5)(1.56258, 0.75)(1.25, 0.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.5)(1.25, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 0.5)(1.25, 0.75)(1.25, 0.5)
\psline[linewidth=0.03,linecolor=black](1.25, 0.75)(1.25, 0.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.5)(1.25, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 0.25)(1.56258, 0.5)(1.25, 0.5)
\psline[linewidth=0.03,linecolor=black](1.25, 0.25)(1.25, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 0.25)(1.25, 0.25)(1.25, 0.5)
\psline[linewidth=0.03,linecolor=black](1.25, 0.25)(0.93742, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 0.25)(0.93742, 0.25)(1.25, 0)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.25)(1.25, 0)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 0.25)(0.93742, 0)(1.25, 0)
\psline[linewidth=0.03,linecolor=black](0.93742, 0)(0.93742, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 0)(0.93742, 0.25)(0.625159, 0)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 0.75)(0.93742, 0.5)(1.25, 0.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.5)(1.25, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 0.5)(0.93742, 0.25)(1.25, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 1.5)(1.56258, 1.25)(1.875, 1.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.25)(1.875, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1.25)(1.56258, 1)(1.875, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 1.5)(2.18752, 1.5)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.5)(2.5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1.5)(2.18752, 1.25)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.25)(2.5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1.25)(2.18752, 1)(2.5, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 2.5)(2.18752, 2.25)(2.5, 2.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.25)(2.5, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2.25)(2.5, 2)(2.5, 2.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.25)(2.5, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2.25)(2.18752, 2)(2.5, 2)
\psline[linewidth=0.03,linecolor=black](2.18752, 2)(2.5, 2)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.25)(2.18752, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2)(2.18752, 2.25)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](2.18752, 2)(1.875, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 1.75)(2.18752, 2)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.75)(1.875, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 1.75)(2.18752, 1.75)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](1.875, 1.75)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.75)(1.875, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 1.5)(2.18752, 1.75)(1.875, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1.75)(1.875, 1.75)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.75)(1.875, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1.75)(1.875, 1.5)(1.875, 1.75)
\psline[linewidth=0.03,linecolor=black](1.875, 1.5)(1.56258, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 1.5)(1.56258, 1.75)(1.56258, 1.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.5)(1.56258, 1.75)
\psline[linewidth=0.03,linecolor=black](1.875, 1.5)(1.56258, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 1.5)(1.56258, 1.5)(1.56258, 1.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.25)(1.56258, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1.25)(1.56258, 1.5)(1.25, 1.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.25)(1.25, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1)(1.56258, 1.25)(1.25, 1.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 1)(1.25, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1)(1.25, 1.25)(1.25, 1)
\psline[linewidth=0.03,linecolor=black](1.56258, 1)(1.25, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 0.75)(1.56258, 1)(1.25, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1.5)(1.56258, 1.75)(1.25, 1.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.5)(1.25, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1.5)(1.25, 1.5)(1.25, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2)(2.18752, 1.75)(2.5, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.75)(3.43752, 2.5)(3.43752, 2.75)
\psline[linewidth=0.03,linecolor=black](3.125, 2.75)(3.43752, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.75)(3.125, 2.5)(3.43752, 2.5)
\psline[linewidth=0.03,linecolor=black](3.125, 2.5)(3.43752, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 2.5)(3.125, 2.25)(3.43752, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 3.25)(3.43752, 3.5)(3.125, 3.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.25)(3.125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 3)(3.43752, 3.25)(3.125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4.25)(2.81252, 4)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 4)(3.125, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4)(3.125, 4)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](3.125, 4)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 4)(3.125, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4)(2.81252, 3.75)(3.125, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 4)(3.43752, 4)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](3.125, 4)(3.43752, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 3.75)(3.43752, 4)(3.125, 4)
\psline[linewidth=0.03,linecolor=black](3.125, 3.75)(3.125, 4)
\psline[linewidth=0.03,linecolor=black](3.43752, 4)(3.125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 4)(3.125, 3.75)(3.43752, 3.75)
\psline[linewidth=0.03,linecolor=black](3.125, 3.75)(3.43752, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 3.75)(3.43752, 3.5)(3.43752, 3.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.5)(3.125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 3.5)(3.125, 3.75)(3.125, 3.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.5)(3.125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.43752, 3.5)(3.125, 3.5)(3.125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.75)(3.125, 3.75)(3.125, 4)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.75)(3.125, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 3.75)(2.81252, 3.75)(3.125, 3.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.75)(3.125, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.75)(2.81252, 3.5)(3.125, 3.5)
\psline[linewidth=0.03,linecolor=black](3.125, 3.5)(2.81252, 3.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.5)(2.81252, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.5)(2.81252, 3.75)(2.5, 3.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.5)(2.5, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 3.25)(2.81252, 3.5)(2.5, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 3.5)(2.81252, 3.5)(3.125, 3.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.5)(3.125, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.5)(2.81252, 3.25)(3.125, 3.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.25)(3.125, 3.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.5)(2.81252, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.5)(2.5, 3.25)(2.81252, 3.25)
\psline[linewidth=0.03,linecolor=black](2.5, 3.25)(2.81252, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.25)(2.5, 3.25)(2.81252, 3)
\psline[linewidth=0.03,linecolor=black](2.81252, 3)(2.5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3)(2.5, 3.25)(2.5, 3)
\psline[linewidth=0.03,linecolor=black](2.5, 3.25)(2.5, 3)
\psline[linewidth=0.03,linecolor=black](2.81252, 3)(2.5, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2.75)(2.81252, 3)(2.5, 3)
\psline[linewidth=0.03,linecolor=black](2.81252, 2.75)(2.5, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 2.75)(2.81252, 2.75)(2.5, 3)
\psline[linewidth=0.03,linecolor=black](2.5, 2.75)(2.81252, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2.75)(2.5, 2.75)(2.5, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 3.25)(2.18752, 3)(2.5, 3)
\psline[linewidth=0.03,linecolor=black](2.18752, 3)(2.5, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3)(2.5, 2.75)(2.5, 3)
\psline[linewidth=0.03,linecolor=black](2.18752, 3)(2.5, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3)(2.18752, 2.75)(2.5, 2.75)
\psline[linewidth=0.03,linecolor=black](2.5, 2.75)(2.18752, 2.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 3)(2.18752, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2.75)(2.18752, 3)(1.875, 2.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.75)(1.875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 2.5)(2.18752, 2.75)(1.875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 2.75)(2.18752, 2.75)(2.5, 2.5)
\psline[linewidth=0.03,linecolor=black](2.5, 2.5)(2.18752, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 2.5)(2.18752, 2.75)(2.18752, 2.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.75)(2.18752, 2.5)
\psline[linewidth=0.03,linecolor=black](2.5, 2.5)(2.18752, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2.25)(2.5, 2.5)(2.18752, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2.75)(1.875, 2.5)(2.18752, 2.5)
\psline[linewidth=0.03,linecolor=black](1.875, 2.5)(2.18752, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 2.5)(2.18752, 2.25)(2.18752, 2.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.25)(1.875, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2.25)(1.875, 2.5)(1.875, 2.25)
\psline[linewidth=0.03,linecolor=black](1.875, 2.5)(1.875, 2.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.25)(1.875, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 2.25)(1.875, 2.25)(1.875, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 2.5)(1.56258, 2.25)(1.875, 2.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.25)(1.875, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 2.25)(1.56258, 2.25)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.25)(1.875, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2.25)(1.56258, 2)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](1.56258, 2)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.25)(1.56258, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2.25)(1.25, 2)(1.56258, 2)
\psline[linewidth=0.03,linecolor=black](1.25, 2)(1.56258, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 2)(1.56258, 1.75)(1.56258, 2)
\psline[linewidth=0.03,linecolor=black](1.25, 2)(1.56258, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 1.75)(1.25, 2)(1.25, 1.75)
\psline[linewidth=0.03,linecolor=black](1.25, 2)(1.25, 1.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.75)(1.25, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 1.5)(1.56258, 1.75)(1.25, 1.75)
\psline[linewidth=0.03,linecolor=black](1.25, 1.5)(1.25, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1.5)(1.25, 1.5)(1.25, 1.75)
\psline[linewidth=0.03,linecolor=black](1.25, 1.5)(0.93742, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 1.5)(0.93742, 1.5)(1.25, 1.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.5)(1.25, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1.5)(0.93742, 1.25)(1.25, 1.25)
\psline[linewidth=0.03,linecolor=black](1.25, 1.25)(0.93742, 1.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.5)(0.93742, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1.25)(0.93742, 1.5)(0.625159, 1.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.25)(0.625159, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1.25)(0.625159, 1.25)(0.625159, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 1.25)(0.93742, 1.25)(1.25, 1)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.25)(1.25, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1.25)(0.93742, 1)(1.25, 1)
\psline[linewidth=0.03,linecolor=black](0.93742, 1)(1.25, 1)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.25)(0.93742, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1)(0.93742, 1.25)(0.625159, 1)
\psline[linewidth=0.03,linecolor=black](0.93742, 1)(0.625159, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 0.75)(0.93742, 1)(0.625159, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1)(1.25, 0.75)(1.25, 1)
\psline[linewidth=0.03,linecolor=black](1.25, 0.75)(0.93742, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 0.75)(0.93742, 1)(0.93742, 0.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 1)(0.93742, 0.75)
\psline[linewidth=0.03,linecolor=black](1.25, 0.75)(0.93742, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 0.5)(1.25, 0.75)(0.93742, 0.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.5)(0.93742, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 0.5)(0.93742, 0.5)(0.93742, 0.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.5)(0.93742, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 0.5)(0.93742, 0.25)(0.93742, 0.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.25)(0.625159, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 0.25)(0.625159, 0.5)(0.625159, 0.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.5)(0.625159, 0.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.25)(0.625159, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 0)(0.93742, 0.25)(0.625159, 0.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 0)(0.625159, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0)(0.625159, 0)(0.625159, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 0.5)(0.312579, 0.25)(0.625159, 0.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.25)(0.625159, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0.25)(0.312579, 0)(0.625159, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1)(0.625159, 0.75)(0.93742, 0.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.75)(0.93742, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 0.75)(0.625159, 0.5)(0.93742, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 2)(0.93742, 1.75)(1.25, 1.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.75)(1.25, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1.75)(0.93742, 1.5)(1.25, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2)(1.56258, 1.75)(1.875, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.25)(3.125, 3)(3.125, 3.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.25)(3.125, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](3.125, 3)(2.81252, 3.25)(2.81252, 3)
\psline[linewidth=0.03,linecolor=black](3.125, 3)(2.81252, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 2.75)(3.125, 3)(2.81252, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4.25)(2.81252, 4.5)(2.5, 4.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.25)(2.5, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4.25)(2.5, 4.5)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.25)(2.5, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 4)(2.81252, 4.25)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 4)(2.5, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 4)(2.81252, 4)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.5, 4)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.5, 4)(2.81252, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.75)(2.81252, 4)(2.5, 4)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.75)(2.5, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.81252, 3.75)(2.5, 4)(2.5, 3.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.75)(2.5, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 3.5)(2.81252, 3.75)(2.5, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4)(2.5, 4)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.5, 4)(2.18752, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 4)(2.18752, 4)(2.5, 3.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 4)(2.5, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4)(2.18752, 3.75)(2.5, 3.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 3.75)(2.5, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3.75)(2.5, 3.5)(2.5, 3.75)
\psline[linewidth=0.03,linecolor=black](2.5, 3.5)(2.18752, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 3.5)(2.18752, 3.75)(2.18752, 3.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 3.75)(2.18752, 3.5)
\psline[linewidth=0.03,linecolor=black](2.5, 3.5)(2.18752, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 3.25)(2.5, 3.5)(2.18752, 3.5)
\psline[linewidth=0.03,linecolor=black](2.5, 3.25)(2.18752, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3.25)(2.5, 3.25)(2.18752, 3.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 3.25)(2.18752, 3.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 3.25)(2.5, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3)(2.5, 3.25)(2.18752, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 3.25)(2.18752, 3.25)(2.18752, 3.5)
\psline[linewidth=0.03,linecolor=black](1.875, 3.25)(2.18752, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 3.25)(2.18752, 3)(2.18752, 3.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 3)(1.875, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3)(1.875, 3.25)(1.875, 3)
\psline[linewidth=0.03,linecolor=black](1.875, 3.25)(1.875, 3)
\psline[linewidth=0.03,linecolor=black](2.18752, 3)(1.875, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3)(1.875, 3)(1.875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 3.25)(1.56258, 3)(1.875, 3)
\psline[linewidth=0.03,linecolor=black](1.875, 3)(1.56258, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 3)(1.56258, 3)(1.875, 2.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 3)(1.875, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3)(1.56258, 2.75)(1.875, 2.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.75)(1.875, 2.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.75)(1.56258, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2.75)(1.56258, 3)(1.25, 2.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.75)(1.25, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2.75)(1.25, 2.75)(1.25, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2.75)(1.875, 2.5)(1.875, 2.75)
\psline[linewidth=0.03,linecolor=black](1.875, 2.5)(1.56258, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 2.5)(1.56258, 2.75)(1.56258, 2.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.75)(1.56258, 2.5)
\psline[linewidth=0.03,linecolor=black](1.875, 2.5)(1.56258, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2.25)(1.875, 2.5)(1.56258, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2.5)(1.56258, 2.75)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.5)(1.25, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 2.25)(1.56258, 2.5)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.25)(1.25, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 2.25)(1.56258, 2.25)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](1.25, 2.25)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](1.25, 2.25)(1.56258, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 2)(1.56258, 2.25)(1.25, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 2.25)(1.25, 2.25)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.25)(1.25, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 2.25)(1.25, 2)(1.25, 2.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.25)(1.25, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 2)(0.93742, 2.25)(0.93742, 2)
\psline[linewidth=0.03,linecolor=black](1.25, 2)(0.93742, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 2)(0.93742, 2)(0.93742, 1.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 2)(0.93742, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 2)(0.625159, 1.75)(0.93742, 1.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.75)(0.93742, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 1.75)(0.93742, 1.5)(0.93742, 1.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.5)(0.625159, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1.5)(0.625159, 1.75)(0.625159, 1.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.75)(0.625159, 1.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.5)(0.625159, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 1.5)(0.625159, 1.5)(0.625159, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 1.75)(0.312579, 1.5)(0.625159, 1.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.5)(0.312579, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 1.5)(0.312579, 1.5)(0.625159, 1.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.5)(0.625159, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1.5)(0.312579, 1.25)(0.625159, 1.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.25)(0.312579, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 1.25)(0.312579, 1.25)(0.625159, 1)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.25)(0.625159, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1.25)(0.312579, 1)(0.625159, 1)
\psline[linewidth=0.03,linecolor=black](0.312579, 1)(0.625159, 1)
\psline[linewidth=0.03,linecolor=black](0.312579, 1)(0.312579, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1)(0.312579, 1.25)(0, 1)
\psline[linewidth=0.03,linecolor=black](0.312579, 1)(0, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0.75)(0.312579, 1)(0, 1)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.75)(0, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 0.75)(0.312579, 0.75)(0, 1)
\psline[linewidth=0.03,linecolor=black](0, 0.75)(0.312579, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0.5)(0.312579, 0.75)(0, 0.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.5)(0, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0.5)(0, 0.75)(0, 0.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.5)(0, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 0.25)(0.312579, 0.5)(0, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1)(0.625159, 0.75)(0.625159, 1)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.75)(0.312579, 1)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0.75)(0.625159, 0.75)(0.312579, 1)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.75)(0.625159, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 0.5)(0.625159, 0.75)(0.312579, 0.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.5)(0.312579, 0.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0.5)(0.625159, 0.5)(0.312579, 0.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.5)(0.625159, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 0.5)(0.312579, 0.5)(0.312579, 0.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.25)(0.312579, 0.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0.25)(0.312579, 0.5)(0, 0.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.25)(0, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0)(0.312579, 0.25)(0, 0.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 0)(0, 0.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 0)(0, 0.25)(0, 0)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3.75)(1.875, 3.5)(2.18752, 3.5)
\psline[linewidth=0.03,linecolor=black](1.875, 3.5)(2.18752, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 3.5)(1.875, 3.25)(2.18752, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4.5)(2.5, 4.5)(2.5, 4.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.5)(2.5, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 4.5)(2.18752, 4.5)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.5)(2.5, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4.5)(2.18752, 4.25)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.25)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.5)(2.18752, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4.5)(1.875, 4.25)(2.18752, 4.25)
\psline[linewidth=0.03,linecolor=black](1.875, 4.25)(2.18752, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4.25)(1.875, 4)(2.18752, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4.25)(2.18752, 4)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.25)(2.18752, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4)(2.18752, 4)(2.18752, 4.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 4)(1.875, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4)(1.875, 4)(2.18752, 3.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 3.75)(1.875, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 3.75)(1.875, 4)(1.875, 3.75)
\psline[linewidth=0.03,linecolor=black](1.875, 4)(1.875, 3.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 3.75)(1.875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 3.5)(2.18752, 3.75)(1.875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4)(1.56258, 3.75)(1.875, 3.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 3.75)(1.875, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3.75)(1.875, 3.5)(1.875, 3.75)
\psline[linewidth=0.03,linecolor=black](1.875, 3.5)(1.56258, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 3.5)(1.56258, 3.75)(1.56258, 3.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 3.75)(1.56258, 3.5)
\psline[linewidth=0.03,linecolor=black](1.875, 3.5)(1.56258, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 3.25)(1.875, 3.5)(1.56258, 3.5)
\psline[linewidth=0.03,linecolor=black](1.875, 3.25)(1.56258, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3.25)(1.875, 3.25)(1.56258, 3.5)
\psline[linewidth=0.03,linecolor=black](1.875, 3.25)(1.56258, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3)(1.875, 3.25)(1.56258, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3.75)(1.25, 3.5)(1.56258, 3.5)
\psline[linewidth=0.03,linecolor=black](1.25, 3.5)(1.56258, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 3.5)(1.56258, 3.25)(1.56258, 3.5)
\psline[linewidth=0.03,linecolor=black](1.25, 3.5)(1.56258, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3.25)(1.25, 3.5)(1.25, 3.25)
\psline[linewidth=0.03,linecolor=black](1.25, 3.5)(1.25, 3.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 3.25)(1.25, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3)(1.56258, 3.25)(1.25, 3.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 3)(1.25, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 3)(1.56258, 3)(1.25, 3.25)
\psline[linewidth=0.03,linecolor=black](1.25, 3)(1.25, 3.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 3)(1.25, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 2.75)(1.56258, 3)(1.25, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3)(1.25, 3)(1.25, 3.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 3)(1.25, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3)(1.25, 2.75)(1.25, 3)
\psline[linewidth=0.03,linecolor=black](0.93742, 3)(1.25, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3)(0.93742, 2.75)(1.25, 2.75)
\psline[linewidth=0.03,linecolor=black](1.25, 2.75)(0.93742, 2.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 3)(0.93742, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 2.75)(0.93742, 3)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.75)(0.625159, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 2.5)(0.93742, 2.75)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 2.5)(0.625159, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 2.5)(0.625159, 2.5)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.5)(0.625159, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 2.5)(0.625159, 2.25)(0.625159, 2.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.5)(0.625159, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 2.25)(0.312579, 2.5)(0.312579, 2.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.25)(0.312579, 2.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 2.25)(0.312579, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 2.25)(0.312579, 2.25)(0.312579, 2)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.25)(0.312579, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 2.25)(0, 2)(0.312579, 2)
\psline[linewidth=0.03,linecolor=black](0, 2)(0.312579, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 2)(0.312579, 1.75)(0.312579, 2)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.75)(0, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1.75)(0, 2)(0, 1.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.75)(0, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 1.5)(0.312579, 1.75)(0, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 2.25)(0.312579, 2.5)(0, 2.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.25)(0, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 2)(0.312579, 2.25)(0, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 2.75)(0.93742, 2.75)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.75)(1.25, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 2.75)(0.93742, 2.5)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.5)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.5)(0.93742, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 2.5)(0.93742, 2.75)(0.625159, 2.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.5)(0.625159, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 2.25)(0.93742, 2.5)(0.625159, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 2.5)(0.93742, 2.25)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.5)(0.93742, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 2.25)(0.93742, 2.25)(0.93742, 2.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.25)(0.625159, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 2.25)(0.625159, 2.25)(0.93742, 2)
\psline[linewidth=0.03,linecolor=black](0.625159, 2.25)(0.93742, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 2.25)(0.625159, 2)(0.93742, 2)
\psline[linewidth=0.03,linecolor=black](0.625159, 2)(0.93742, 2)
\psline[linewidth=0.03,linecolor=black](0.625159, 2)(0.625159, 2.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 2)(0.625159, 2.25)(0.312579, 2)
\psline[linewidth=0.03,linecolor=black](0.625159, 2)(0.312579, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 1.75)(0.625159, 2)(0.312579, 2)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.75)(0.312579, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1.75)(0.625159, 1.75)(0.312579, 2)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.75)(0.312579, 1.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 1.75)(0.312579, 1.75)(0.312579, 1.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.75)(0.312579, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1.75)(0, 1.5)(0.312579, 1.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.5)(0, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1.5)(0, 1.5)(0.312579, 1.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.25)(0, 1.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 1.25)(0, 1.5)(0, 1.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.25)(0, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 1)(0.312579, 1.25)(0, 1.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 2)(0.625159, 1.75)(0.93742, 2)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 3.5)(0.93742, 3.25)(1.25, 3.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 3.25)(1.25, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3.25)(0.93742, 3)(1.25, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 5)(2.5, 4.75)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5)(2.5, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 5)(2.18752, 4.75)(2.5, 4.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.75)(2.5, 4.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 5)(2.18752, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4.75)(2.18752, 5)(1.875, 4.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.75)(1.875, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4.5)(2.18752, 4.75)(1.875, 4.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.5)(1.875, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4.5)(1.875, 4.75)(1.875, 4.5)
\psline[linewidth=0.03,linecolor=black](1.875, 4.75)(1.875, 4.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.5)(1.875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4.25)(2.18752, 4.5)(1.875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4.75)(1.56258, 4.75)(1.875, 4.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.75)(1.875, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 4.75)(1.56258, 4.5)(1.875, 4.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.5)(1.875, 4.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.75)(1.56258, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 4.5)(1.56258, 4.75)(1.25, 4.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.5)(1.25, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4.25)(1.56258, 4.5)(1.25, 4.5)
\psline[linewidth=0.03,linecolor=black](1.25, 4.25)(1.25, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4.25)(1.25, 4.5)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](1.25, 4.25)(0.93742, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 4.25)(1.25, 4.25)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 4.25)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 4.25)(1.25, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 4)(1.25, 4.25)(0.93742, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.25)(0.93742, 4.25)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.25)(0.93742, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.25)(0.93742, 4)(0.93742, 4.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.25)(0.93742, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 4)(0.625159, 4.25)(0.625159, 4)
\psline[linewidth=0.03,linecolor=black](0.625159, 4)(0.625159, 4.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 4)(0.625159, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 4)(0.625159, 4)(0.625159, 3.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 4)(0.625159, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4)(0.312579, 3.75)(0.625159, 3.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.75)(0.625159, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.75)(0.312579, 3.5)(0.625159, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4)(0.625159, 4.25)(0.312579, 4)
\psline[linewidth=0.03,linecolor=black](0.625159, 4)(0.312579, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4)(0.312579, 4)(0.312579, 3.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.75)(0.312579, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.75)(0.312579, 4)(0, 3.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.75)(0, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.5)(0.312579, 3.75)(0, 3.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.5)(0, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 3.5)(0.312579, 3.5)(0, 3.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.5)(0, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.5)(0, 3.5)(0, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 4.5)(1.875, 4.25)(1.875, 4.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.5)(1.875, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4.25)(1.56258, 4.5)(1.56258, 4.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.5)(1.56258, 4.25)
\psline[linewidth=0.03,linecolor=black](1.875, 4.25)(1.56258, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4)(1.875, 4.25)(1.56258, 4.25)
\psline[linewidth=0.03,linecolor=black](1.875, 4)(1.56258, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4)(1.56258, 4.25)(1.56258, 4)
\psline[linewidth=0.03,linecolor=black](1.875, 4)(1.56258, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3.75)(1.875, 4)(1.56258, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 4.5)(1.25, 4.25)(1.56258, 4.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.25)(1.25, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 4.25)(1.25, 4.25)(1.56258, 4)
\psline[linewidth=0.03,linecolor=black](1.25, 4.25)(1.56258, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4.25)(1.25, 4)(1.56258, 4)
\psline[linewidth=0.03,linecolor=black](1.25, 4)(1.56258, 4)
\psline[linewidth=0.03,linecolor=black](1.25, 4.25)(1.25, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4.25)(0.93742, 4)(1.25, 4)
\psline[linewidth=0.03,linecolor=black](0.93742, 4)(1.25, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4)(0.93742, 4)(1.25, 3.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 4)(1.25, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 4)(0.93742, 3.75)(1.25, 3.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 3.75)(1.25, 3.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 4)(0.93742, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3.75)(0.93742, 4)(0.625159, 3.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 3.75)(0.625159, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 3.5)(0.93742, 3.75)(0.625159, 3.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 3.5)(0.625159, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.5)(0.625159, 3.5)(0.625159, 3.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.5)(0.625159, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.5)(0.625159, 3.25)(0.625159, 3.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.5)(0.625159, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.5)(0.312579, 3.25)(0.625159, 3.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 3.25)(0.312579, 3.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.5)(0.312579, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.25)(0.312579, 3.5)(0, 3.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.25)(0, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.25)(0, 3.25)(0, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 3.25)(0.312579, 3.25)(0.625159, 3)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.25)(0.625159, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3.25)(0.312579, 3)(0.625159, 3)
\psline[linewidth=0.03,linecolor=black](0.625159, 3)(0.312579, 3)
\psline[linewidth=0.03,linecolor=black](0.312579, 3)(0.312579, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3)(0.312579, 3.25)(0, 3)
\psline[linewidth=0.03,linecolor=black](0.312579, 3)(0, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 2.75)(0.312579, 3)(0, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 3)(0.312579, 3)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 3)(0.625159, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 3)(0.312579, 2.75)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.75)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.75)(0.312579, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 2.75)(0.312579, 3)(0, 2.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.75)(0, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 2.5)(0.312579, 2.75)(0, 2.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.5)(0, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 2.5)(0, 2.75)(0, 2.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.5)(0, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 2.25)(0.312579, 2.5)(0, 2.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 2.75)(0.312579, 2.5)(0.625159, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3.75)(1.25, 3.5)(1.25, 3.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 3.75)(1.25, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 3.5)(0.93742, 3.75)(0.93742, 3.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 3.75)(0.93742, 3.5)
\psline[linewidth=0.03,linecolor=black](1.25, 3.5)(0.93742, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3.25)(1.25, 3.5)(0.93742, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3.75)(0.625159, 3.5)(0.93742, 3.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 3.5)(0.93742, 3.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 3.5)(0.93742, 3.25)(0.93742, 3.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 3.5)(0.93742, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 3.25)(0.93742, 3.25)(0.625159, 3.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 3.25)(0.93742, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3)(0.93742, 3.25)(0.625159, 3.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 3)(0.625159, 3.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3)(0.625159, 3.25)(0.625159, 3)
\psline[linewidth=0.03,linecolor=black](0.93742, 3)(0.625159, 3)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 3)(0.625159, 3)(0.625159, 2.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4)(1.56258, 3.75)(1.56258, 4)
\psline[linewidth=0.03,linecolor=black](1.56258, 3.75)(1.25, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 3.75)(1.25, 4)(1.25, 3.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 3.75)(1.25, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 3.5)(1.56258, 3.75)(1.25, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 4.75)(2.18752, 4.5)(2.5, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 5.25)(2.18752, 5)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5.25)(2.18752, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 5)(2.18752, 5.25)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5.25)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5)(1.875, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 4.75)(2.18752, 5)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](1.875, 4.75)(1.875, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 4.75)(1.875, 4.75)(1.875, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 5.25)(1.875, 5.25)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](1.875, 5.25)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5.25)(1.875, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 5.25)(1.875, 5.5)(1.875, 5.25)
\psline[linewidth=0.03,linecolor=black](1.875, 5.5)(1.875, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.5)(1.56258, 5.5)(1.875, 5.25)
\psline[linewidth=0.03,linecolor=black](1.875, 5.5)(1.56258, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.75)(1.56258, 5.5)(1.875, 5.5)
\psline[linewidth=0.03,linecolor=black](1.875, 5.75)(1.56258, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.75)(1.56258, 5.75)(1.56258, 5.5)
\psline[linewidth=0.03,linecolor=black](1.875, 5.75)(1.56258, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5.75)(1.875, 5.75)(1.56258, 6)
\psline[linewidth=0.03,linecolor=black](1.56258, 5.75)(1.56258, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5.75)(1.56258, 6)(1.25, 6)
\psline[linewidth=0.03,linecolor=black](1.56258, 6)(1.25, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6)(1.25, 6.25)(1.25, 6)
\psline[linewidth=0.03,linecolor=black](1.25, 6.25)(1.25, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 6.25)(0.93742, 6.25)(1.25, 6)
\psline[linewidth=0.03,linecolor=black](1.25, 6.25)(0.93742, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.25)(1.25, 6.25)(1.25, 6.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.25)(1.25, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.5)(0.93742, 6.25)(1.25, 6.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.5)(1.25, 6.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.5)(0.93742, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.25)(0.93742, 6.5)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.5)(0.625159, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.5)(0.93742, 6.75)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.75)(0.625159, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.75)(0.625159, 6.75)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 6.75)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.75)(0.625159, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.75)(0.93742, 7)(0.625159, 6.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 7)(0.625159, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 6.75)(0.93742, 7)(0.625159, 7)
\psline[linewidth=0.03,linecolor=black](0.625159, 7)(0.93742, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 7)(0.93742, 7)(0.625159, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 6.75)(0.312579, 6.75)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.75)(0.625159, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6.75)(0.625159, 6.75)(0.625159, 7)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.75)(0.625159, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7)(0.312579, 6.75)(0.625159, 7)
\psline[linewidth=0.03,linecolor=black](0.312579, 7)(0.625159, 7)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.75)(0.312579, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6.75)(0.312579, 7)(0, 7)
\psline[linewidth=0.03,linecolor=black](0.312579, 7)(0, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7)(0, 7.25)(0, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7)(0.625159, 7)(0.625159, 7.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 7)(0.625159, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7.25)(0.312579, 7)(0.625159, 7.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.25)(0.625159, 7.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 7)(0.312579, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7)(0.312579, 7.25)(0, 7.25)
\psline[linewidth=0.03,linecolor=black](0, 7.25)(0.312579, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 7.25)(0.312579, 7.25)(0, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 7.5)(0.312579, 7.25)(0.625159, 7.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.25)(0.625159, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7.25)(0.625159, 7.5)(0.312579, 7.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.5)(0.312579, 7.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.25)(0.312579, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7.25)(0.312579, 7.5)(0, 7.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.5)(0, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7.5)(0.312579, 7.75)(0, 7.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.75)(0, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7.75)(0, 7.75)(0, 7.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.75)(0, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7.75)(0, 8)(0, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 7.5)(0.312579, 7.75)(0.312579, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.75)(0.93742, 6.5)(1.25, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.25)(1.56258, 5)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](1.56258, 5)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](1.875, 5.25)(1.56258, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5)(1.875, 5.25)(1.56258, 5.25)
\psline[linewidth=0.03,linecolor=black](1.875, 5.25)(1.56258, 5.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 5)(1.56258, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 5.25)(1.56258, 5)(1.56258, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.25)(1.56258, 5.5)(1.56258, 5.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 5.5)(1.56258, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5.5)(1.25, 5.25)(1.56258, 5.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 5.5)(1.25, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5.5)(1.25, 5.5)(1.25, 5.25)
\psline[linewidth=0.03,linecolor=black](1.25, 5.5)(1.25, 5.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 5.5)(1.25, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5.5)(1.56258, 5.75)(1.25, 5.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 5.75)(1.25, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 5.5)(1.56258, 5.75)(1.25, 5.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 5.75)(1.25, 5.75)
\psline[linewidth=0.03,linecolor=black](1.25, 5.5)(1.25, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5.75)(1.25, 5.5)(1.25, 5.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 5.75)(1.25, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 6)(0.93742, 5.75)(1.25, 5.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 5.75)(1.25, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6)(0.93742, 5.75)(1.25, 6)
\psline[linewidth=0.03,linecolor=black](0.93742, 6)(1.25, 6)
\psline[linewidth=0.03,linecolor=black](0.93742, 6)(0.93742, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5.75)(0.93742, 6)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.93742, 6)(0.625159, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6)(0.93742, 6.25)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.25)(0.625159, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.25)(0.625159, 6.25)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.25)(0.625159, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 6.25)(0.93742, 6.25)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 6.25)(0.625159, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6.5)(0.625159, 6.25)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.5)(0.625159, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6.75)(0.312579, 6.5)(0.625159, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 6.25)(0.93742, 6)(1.25, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5.75)(1.25, 6)(1.25, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 5.5)(0.93742, 5.5)(1.25, 5.25)
\psline[linewidth=0.03,linecolor=black](1.25, 5.5)(0.93742, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5.75)(0.93742, 5.5)(1.25, 5.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 5.75)(0.93742, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5.5)(0.93742, 5.75)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 5.75)(0.625159, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5.75)(0.625159, 5.75)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.75)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.75)(0.93742, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 5.75)(0.93742, 5.75)(0.625159, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 5.75)(0.312579, 5.75)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.75)(0.625159, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5.75)(0.625159, 5.75)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.75)(0.625159, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6)(0.312579, 5.75)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.312579, 6)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.75)(0.312579, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5.75)(0.312579, 6)(0, 6)
\psline[linewidth=0.03,linecolor=black](0, 6)(0.312579, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 6)(0.312579, 6)(0, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 6.25)(0.312579, 6)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.312579, 6)(0.625159, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6)(0.625159, 6.25)(0.312579, 6.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 6.25)(0.312579, 6.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 6)(0.312579, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6)(0.312579, 6.25)(0, 6.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.25)(0, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6.25)(0.312579, 6.5)(0, 6.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.5)(0, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6.5)(0, 6.5)(0, 6.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.5)(0, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6.5)(0.312579, 6.75)(0, 6.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.75)(0, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 6.75)(0, 6.75)(0, 6.5)
\psline[linewidth=0.03,linecolor=black](0, 6.75)(0.312579, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 6.75)(0.312579, 6.75)(0, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 6.25)(0.312579, 6.5)(0.312579, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5)(1.56258, 4.75)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](1.56258, 5)(1.56258, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 4.75)(1.56258, 5)(1.25, 5)
\psline[linewidth=0.03,linecolor=black](1.56258, 5)(1.25, 5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.75)(1.25, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4.75)(1.56258, 4.75)(1.25, 5)
\psline[linewidth=0.03,linecolor=black](1.25, 4.75)(1.25, 5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.75)(1.25, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 4.75)(1.25, 4.75)(1.25, 4.5)
\psline[linewidth=0.03,linecolor=black](1.25, 4.5)(1.25, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4.5)(1.25, 4.75)(0.93742, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5)(1.25, 4.75)(1.25, 5)
\psline[linewidth=0.03,linecolor=black](0.93742, 5)(1.25, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 4.75)(0.93742, 5)(0.93742, 4.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 5)(0.93742, 4.75)
\psline[linewidth=0.03,linecolor=black](1.25, 4.75)(0.93742, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 4.5)(1.25, 4.75)(0.93742, 4.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 4.5)(0.93742, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.75)(0.93742, 4.5)(0.93742, 4.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.75)(0.93742, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.75)(0.625159, 4.5)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.5)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.75)(0.625159, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.5)(0.625159, 4.75)(0.312579, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.5)(0.625159, 4.25)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.5)(0.625159, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.25)(0.625159, 4.5)(0.312579, 4.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.25)(0.312579, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4.25)(0.625159, 4.25)(0.312579, 4.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.25)(0.312579, 4.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.25)(0.625159, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.25)(0.312579, 4.25)(0.312579, 4)
\psline[linewidth=0.03,linecolor=black](0.312579, 4)(0.312579, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4)(0.312579, 4.25)(0, 4)
\psline[linewidth=0.03,linecolor=black](0.312579, 4)(0, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4)(0, 4)(0, 3.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4.25)(0.312579, 4.5)(0, 4.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.25)(0, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 4.25)(0.312579, 4.25)(0, 4.5)
\psline[linewidth=0.03,linecolor=black](0, 4.25)(0.312579, 4.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4.25)(0, 4.25)(0, 4)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5)(0.625159, 4.75)(0.93742, 4.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 5)(0.625159, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 5)(0.625159, 4.75)(0.93742, 5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5)(0.93742, 5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5)(0.625159, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5)(0.625159, 4.75)(0.625159, 5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5)(0.625159, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 4.75)(0.312579, 5)(0.312579, 4.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.75)(0.312579, 5)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.75)(0.312579, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4.5)(0.625159, 4.75)(0.312579, 4.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.5)(0.312579, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4.5)(0.312579, 4.75)(0, 4.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.5)(0, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4.5)(0, 4.75)(0, 4.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 4.75)(0.312579, 5)(0, 4.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 5.25)(0.625159, 5)(0.93742, 5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.25)(0.625159, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 5.25)(0.312579, 5)(0.625159, 5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5)(0.625159, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5)(0.625159, 5.25)(0.312579, 5.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.25)(0.312579, 5.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 5)(0.312579, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5)(0.312579, 5.25)(0, 5.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 5)(0, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5)(0, 5.25)(0, 5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5)(0, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 4.75)(0.312579, 5)(0, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 5.25)(0.312579, 5.5)(0.312579, 5.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.25)(0.312579, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5.25)(0.312579, 5.5)(0, 5.25)
\psline[linewidth=0.03,linecolor=black](0, 5.25)(0.312579, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 5.25)(0.312579, 5.5)(0, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 5)(1.25, 5.25)(1.25, 5)
\psline[linewidth=0.03,linecolor=black](1.25, 5.25)(1.25, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 5.25)(0.93742, 5)(1.25, 5)
\psline[linewidth=0.03,linecolor=black](1.25, 5.25)(0.93742, 5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5)(1.25, 5.25)(0.93742, 5.25)
\psline[linewidth=0.03,linecolor=black](1.25, 5.25)(0.93742, 5.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 5)(0.93742, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 5.25)(0.93742, 5)(0.93742, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 5.25)(0.93742, 5.5)(0.93742, 5.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 5.5)(0.93742, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 5.5)(0.625159, 5.25)(0.93742, 5.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.25)(0.93742, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 5.25)(0.93742, 5.5)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.25)(0.625159, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5.5)(0.625159, 5.25)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.5)(0.625159, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5.75)(0.312579, 5.5)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.5)(0.312579, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5.5)(0.312579, 5.75)(0, 5.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.75)(0, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5.75)(0, 5.75)(0, 5.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.75)(0, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 5.75)(0, 6)(0, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 5.25)(2.18752, 5.25)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.5, 5.25)(2.18752, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 5.5)(2.18752, 5.25)(2.5, 5.25)
\psline[linewidth=0.03,linecolor=black](2.5, 5.5)(2.18752, 5.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 5.25)(2.5, 5.5)(2.18752, 5.5)
\psline[linewidth=0.03,linecolor=black](2.5, 5.5)(2.18752, 5.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5.25)(2.18752, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.5)(2.18752, 5.25)(2.18752, 5.5)
\psline[linewidth=0.03,linecolor=black](1.875, 5.5)(2.18752, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.75)(1.875, 5.5)(2.18752, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 5.5)(2.5, 5.75)(2.18752, 5.5)
\psline[linewidth=0.03,linecolor=black](2.5, 5.75)(2.18752, 5.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 5.5)(2.5, 5.75)(2.18752, 5.75)
\psline[linewidth=0.03,linecolor=black](2.5, 5.75)(2.18752, 5.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 5.5)(2.18752, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.75)(2.18752, 5.5)(2.18752, 5.75)
\psline[linewidth=0.03,linecolor=black](1.875, 5.75)(2.18752, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6)(1.875, 5.75)(2.18752, 5.75)
\psline[linewidth=0.03,linecolor=black](1.875, 5.75)(2.18752, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 5.75)(2.18752, 6)(1.875, 6)
\psline[linewidth=0.03,linecolor=black](1.875, 6)(2.18752, 6)
\psline[linewidth=0.03,linecolor=black](1.875, 5.75)(1.875, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6)(1.875, 5.75)(1.875, 6)
\psline[linewidth=0.03,linecolor=black](1.56258, 6)(1.875, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6)(1.875, 6)(1.875, 6.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 6)(1.875, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6.25)(1.56258, 6)(1.875, 6.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.25)(1.875, 6.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 6)(1.56258, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6)(1.56258, 6.25)(1.25, 6.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.25)(1.25, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6.25)(1.56258, 6.5)(1.25, 6.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.5)(1.25, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 6.25)(1.56258, 6.5)(1.25, 6.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.5)(1.25, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6.5)(1.25, 6.75)(1.25, 6.5)
\psline[linewidth=0.03,linecolor=black](1.25, 6.75)(1.25, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 6.75)(0.93742, 6.75)(1.25, 6.5)
\psline[linewidth=0.03,linecolor=black](1.25, 6.75)(0.93742, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 7)(0.93742, 6.75)(1.25, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 6.5)(1.56258, 6.25)(1.875, 6.25)
\psline[linewidth=0.03,linecolor=black](1.875, 6.5)(1.56258, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 6.5)(1.56258, 6.5)(1.56258, 6.25)
\psline[linewidth=0.03,linecolor=black](1.875, 6.5)(1.56258, 6.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 6.5)(1.875, 6.75)(1.56258, 6.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.5)(1.875, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6.5)(1.875, 6.75)(1.56258, 6.75)
\psline[linewidth=0.03,linecolor=black](1.875, 6.75)(1.56258, 6.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.5)(1.56258, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6.5)(1.56258, 6.75)(1.25, 6.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.75)(1.25, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 6.75)(1.56258, 7)(1.25, 6.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 7)(1.25, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 7)(1.25, 7)(1.25, 6.75)
\psline[linewidth=0.03,linecolor=black](1.25, 7)(1.25, 6.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 7)(1.25, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 7)(1.56258, 7.25)(1.25, 7)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.25)(1.25, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 7)(1.56258, 7.25)(1.25, 7.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.25)(1.25, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.56258, 7.25)(1.25, 7.5)(1.25, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 7)(0.93742, 7)(1.25, 6.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 7)(1.25, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 7)(1.25, 7)(1.25, 7.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 7)(1.25, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 7.25)(0.93742, 7)(1.25, 7.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 7.25)(1.25, 7.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 7.25)(0.93742, 7)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 7)(0.93742, 7.25)(0.625159, 7.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 7.25)(0.625159, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 7.25)(0.625159, 7.5)(0.625159, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 7.5)(0.93742, 7.25)(1.25, 7.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 7.25)(1.25, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 7.5)(0.93742, 7.25)(1.25, 7.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 7.5)(1.25, 7.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 7.5)(0.93742, 7.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 7.5)(0.93742, 7.25)(0.93742, 7.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.5)(0.93742, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 7.5)(0.93742, 7.5)(0.93742, 7.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.5)(0.93742, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 7.75)(0.625159, 7.5)(0.93742, 7.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.75)(0.93742, 7.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.5)(0.625159, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 7.5)(0.625159, 7.75)(0.312579, 7.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.75)(0.312579, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 7.75)(0.625159, 8)(0.312579, 7.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.75)(0.625159, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 7.75)(0.625159, 8)(0.312579, 8)
\psline[linewidth=0.03,linecolor=black](0.625159, 8)(0.312579, 8)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.75)(0.312579, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 8)(0.312579, 7.75)(0.312579, 8)
\psline[linewidth=0.03,linecolor=black](0, 8)(0.312579, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.25)(0, 8)(0.312579, 8)
\psline[linewidth=0.03,linecolor=black](0, 8)(0.312579, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 8)(0.312579, 8.25)(0, 8.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.25)(0, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.25)(0, 8.5)(0, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 8)(0.312579, 8.25)(0.312579, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8)(0.625159, 7.75)(0.93742, 7.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 8)(0.625159, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8)(0.625159, 8)(0.625159, 7.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 8)(0.625159, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8)(0.93742, 8.25)(0.625159, 8)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.25)(0.625159, 8)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 8.25)(0.625159, 8.25)(0.625159, 8)
\psline[linewidth=0.03,linecolor=black](0.625159, 8.25)(0.625159, 8)
\psline[linewidth=0.03,linecolor=black](0.625159, 8.25)(0.93742, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 8.25)(0.93742, 8.25)(0.625159, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.625159, 8.25)(0.312579, 8.25)(0.625159, 8)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.25)(0.625159, 8.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.25)(0.625159, 8.25)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.25)(0.625159, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.5)(0.312579, 8.25)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.5)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.25)(0.312579, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.25)(0.312579, 8.5)(0, 8.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.5)(0, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.5)(0.312579, 8.75)(0, 8.5)
\psline[linewidth=0.03,linecolor=black](0, 8.5)(0.312579, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0, 8.5)(0.312579, 8.75)(0, 8.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.75)(0, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.75)(0, 9)(0, 8.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.312579, 8.75)(0.312579, 8.5)(0.625159, 8.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 7.75)(0.93742, 7.5)(1.25, 7.5)
\psline[linewidth=0.03,linecolor=black](1.25, 7.75)(0.93742, 7.5)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](0.93742, 7.5)(1.25, 7.75)(0.93742, 7.75)
\psline[linewidth=0.03,linecolor=black](1.25, 7.75)(0.93742, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.25, 7.75)(0.93742, 8)(0.93742, 7.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 6.75)(1.56258, 7)(1.56258, 6.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](1.875, 6)(2.18752, 6)(1.875, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 5.75)(2.5, 6)(2.18752, 5.75)
\psline[linewidth=0.03,linecolor=black](2.5, 6)(2.18752, 5.75)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.5, 6)(2.18752, 6)(2.18752, 5.75)
\psline[linewidth=0.03,linecolor=black](2.5, 6)(2.18752, 6)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6)(2.5, 6)(2.18752, 6.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 6)(2.18752, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6)(2.18752, 6.25)(1.875, 6.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.25)(1.875, 6.25)
\pspolygon[linestyle=none,fillcolor=disc4,fillstyle=solid](2.18752, 6.25)(1.875, 6.5)(1.875, 6.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 8.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 8.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 8.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 8)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 8)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 7.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 7.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 7.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 7.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 7.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 7)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 6.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 6.75)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 6.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 6.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 6.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 6)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 6)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 5.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 5.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 5.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 5.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 5.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 5.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 4.75)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 4.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 4.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 4.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 4.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 4.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 4.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 6.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 6)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 5.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 5.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 5.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 5.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 6.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 6.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 6)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 6)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 5.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 5.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 5.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 5.25)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 5.25)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 7.75)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 7.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 7.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 7.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 7)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 6.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 7.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 7)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 7)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 6.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 6.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 6.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 6.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 6.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 6.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 6.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 6)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 6)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 5.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 5.75)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 5.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 5.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 5.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 5.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 3.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 2.75)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 3)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 3)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 3.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 3.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 3.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 3.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 3.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 4)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 4)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 4.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 4)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 3.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 3.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 3.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 4)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 4.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 4)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 4.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 4.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 4.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 4.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 4.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 4.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 4.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 4.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 4.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 3.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 2)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 2.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 1.75)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 2)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 2.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 2.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 2.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 2.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 2.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 2.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 3)
\psdot[dotstyle=*,dotsize=0.11](1.25, 3)
\psdot[dotstyle=*,dotsize=0.11](1.25, 3.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 3.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 3.25)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 3.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 3.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 3.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 4)
\psdot[dotstyle=*,dotsize=0.11](1.875, 4.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 4.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 4.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 3.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 0.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 0.75)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 1)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 1.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 1.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 1.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 1.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 2)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 2.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 2.25)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 2.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 2.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 2.75)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 2.75)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 3)
\psdot[dotstyle=*,dotsize=0.11](1.875, 3)
\psdot[dotstyle=*,dotsize=0.11](1.875, 3.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 3.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 3.5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 3.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 4)
\psdot[dotstyle=*,dotsize=0.11](2.5, 3.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 4)
\psdot[dotstyle=*,dotsize=0.11](2.5, 4.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 1.75)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 0.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 0.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 0.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 0.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 0.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 1)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 1)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 1.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 1.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 1.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 1.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 2)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 2)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 2.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 2.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 2.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 2.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 2.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 2.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 3)
\psdot[dotstyle=*,dotsize=0.11](2.5, 2.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 3)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 3)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 3.25)
\psdot[dotstyle=*,dotsize=0.11](2.5, 3.25)
\psdot[dotstyle=*,dotsize=0.11](2.5, 3.5)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 3.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 3.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 3.75)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 3.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 4)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 4)
\psdot[dotstyle=*,dotsize=0.11](3.125, 3.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 1.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 1)
\psdot[dotstyle=*,dotsize=0.11](1.25, 1.25)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 1.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 1.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 1.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 2)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 2)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 2.25)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 1.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 0.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 0.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 0.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 0.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 0.25)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 0.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 0.75)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 1)
\psdot[dotstyle=*,dotsize=0.11](1.875, 1)
\psdot[dotstyle=*,dotsize=0.11](1.875, 1.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 1.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 1.5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 1.5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 1.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 2)
\psdot[dotstyle=*,dotsize=0.11](2.5, 2.25)
\psdot[dotstyle=*,dotsize=0.11](2.5, 2.5)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 2.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 2.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 2.5)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 2.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 2.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 3)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 3.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 2.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 3)
\psdot[dotstyle=*,dotsize=0.11](3.75, 3)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 3.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 3.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 3.5)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 3.5)
\psdot[dotstyle=*,dotsize=0.11](3.75, 3.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 3.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 4)
\psdot[dotstyle=*,dotsize=0.11](3.125, 4.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 4.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 4.5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 4.5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 4.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 1.5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 1.75)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 1.75)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 2)
\psdot[dotstyle=*,dotsize=0.11](3.125, 2)
\psdot[dotstyle=*,dotsize=0.11](3.125, 2.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 2.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 2.5)
\psdot[dotstyle=*,dotsize=0.11](3.75, 2.5)
\psdot[dotstyle=*,dotsize=0.11](3.75, 2.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 0.75)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 0.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 0.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 0.5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 0.5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 0.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 1)
\psdot[dotstyle=*,dotsize=0.11](2.5, 1)
\psdot[dotstyle=*,dotsize=0.11](2.5, 1.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 1.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 1.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 1.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 1.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 1.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 2)
\psdot[dotstyle=*,dotsize=0.11](3.75, 2)
\psdot[dotstyle=*,dotsize=0.11](3.75, 2.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 2.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 2.75)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 3)
\psdot[dotstyle=*,dotsize=0.11](4.375, 3.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 3)
\psdot[dotstyle=*,dotsize=0.11](5, 3.25)
\psdot[dotstyle=*,dotsize=0.11](6.25, 4.25)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 4)
\psdot[dotstyle=*,dotsize=0.11](5.625, 3.75)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 3.5)
\psdot[dotstyle=*,dotsize=0.11](5, 3.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 3.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 3.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 3.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 3.5)
\psdot[dotstyle=*,dotsize=0.11](4.375, 3.75)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 3.75)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 4)
\psdot[dotstyle=*,dotsize=0.11](3.75, 4)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 4.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 4.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 4.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 4.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 4.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 4.75)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 4.75)
\psdot[dotstyle=*,dotsize=0.11](5, 4.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 4.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 4.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 4.5)
\psdot[dotstyle=*,dotsize=0.11](5, 4.25)
\psdot[dotstyle=*,dotsize=0.11](6.875, 4.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 4.75)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 4.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 4.75)
\psdot[dotstyle=*,dotsize=0.11](6.25, 4.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 4.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 4.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 4.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 4)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 4.25)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 4)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 3.75)
\psdot[dotstyle=*,dotsize=0.11](5, 3.75)
\psdot[dotstyle=*,dotsize=0.11](5, 4)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 3.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 4)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 4.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 4)
\psdot[dotstyle=*,dotsize=0.11](4.375, 4.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 4.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 4.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 4.5)
\psdot[dotstyle=*,dotsize=0.11](3.75, 4.5)
\psdot[dotstyle=*,dotsize=0.11](3.75, 4.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 4.75)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 4.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 5)
\psdot[dotstyle=*,dotsize=0.11](5, 5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 4.5)
\psdot[dotstyle=*,dotsize=0.11](5, 4.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 4.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 5)
\psdot[dotstyle=*,dotsize=0.11](4.375, 4.75)
\psdot[dotstyle=*,dotsize=0.11](5, 5.25)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 5.25)
\psdot[dotstyle=*,dotsize=0.11](5, 5.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 5.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 5.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 5.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 5.5)
\psdot[dotstyle=*,dotsize=0.11](4.375, 5.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 5.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 5.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 5)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 5)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 4.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 7.75)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 9)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 8.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 8.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 8.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 8.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 8.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 8.25)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 8)
\psdot[dotstyle=*,dotsize=0.11](1.25, 8)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 8)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 7.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 7.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 6.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 7.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 7.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 7.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 7.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 7.25)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 7)
\psdot[dotstyle=*,dotsize=0.11](1.875, 7)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 7)
\psdot[dotstyle=*,dotsize=0.11](1.875, 6.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 6.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 6.5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 6.5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 6.25)
\psdot[dotstyle=*,dotsize=0.11](2.5, 6.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 7.5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 7.25)
\psdot[dotstyle=*,dotsize=0.11](2.5, 7.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 7)
\psdot[dotstyle=*,dotsize=0.11](2.5, 7)
\psdot[dotstyle=*,dotsize=0.11](2.5, 6.75)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 6.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 6.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 6.5)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 6.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 6.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 6.25)
\psdot[dotstyle=*,dotsize=0.11](3.125, 6)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 6)
\psdot[dotstyle=*,dotsize=0.11](2.5, 6)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 5.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 5.75)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 5.5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 5.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 5.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 5)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 5.25)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 5.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 5.25)
\psdot[dotstyle=*,dotsize=0.11](5.625, 5.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 5.5)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 5.75)
\psdot[dotstyle=*,dotsize=0.11](5, 5.75)
\psdot[dotstyle=*,dotsize=0.11](5, 6)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 5.5)
\psdot[dotstyle=*,dotsize=0.11](7.18748, 5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 5)
\psdot[dotstyle=*,dotsize=0.11](6.875, 5.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 5.25)
\psdot[dotstyle=*,dotsize=0.11](6.56248, 5.5)
\psdot[dotstyle=*,dotsize=0.11](6.25, 5.5)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 5.75)
\psdot[dotstyle=*,dotsize=0.11](5.625, 5.75)
\psdot[dotstyle=*,dotsize=0.11](5.93748, 6)
\psdot[dotstyle=*,dotsize=0.11](5.625, 6)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 6)
\psdot[dotstyle=*,dotsize=0.11](5.3125, 6.25)
\psdot[dotstyle=*,dotsize=0.11](5, 6.25)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 6.25)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 6)
\psdot[dotstyle=*,dotsize=0.11](4.375, 6)
\psdot[dotstyle=*,dotsize=0.11](4.375, 5.75)
\psdot[dotstyle=*,dotsize=0.11](5, 6.5)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 7)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 6.75)
\psdot[dotstyle=*,dotsize=0.11](4.6875, 6.5)
\psdot[dotstyle=*,dotsize=0.11](3.75, 7.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 9.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 9.5)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 9)
\psdot[dotstyle=*,dotsize=0.11](1.875, 9.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 9.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 9.5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 9.25)
\psdot[dotstyle=*,dotsize=0.11](2.5, 9)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 8.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 8.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 8.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 8.25)
\psdot[dotstyle=*,dotsize=0.11](3.125, 8)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 8)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 7.75)
\psdot[dotstyle=*,dotsize=0.11](3.75, 7.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 7.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 7.25)
\psdot[dotstyle=*,dotsize=0.11](4.375, 7.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 7.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 7)
\psdot[dotstyle=*,dotsize=0.11](4.375, 7)
\psdot[dotstyle=*,dotsize=0.11](4.375, 6.75)
\psdot[dotstyle=*,dotsize=0.11](4.375, 6.5)
\psdot[dotstyle=*,dotsize=0.11](4.375, 6.25)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 6)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 5.75)
\psdot[dotstyle=*,dotsize=0.11](3.75, 5.75)
\psdot[dotstyle=*,dotsize=0.11](3.75, 5.5)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 6.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 7.5)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 7.25)
\psdot[dotstyle=*,dotsize=0.11](3.125, 7.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 9.75)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 9.75)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 9.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 9.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 9.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 9.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 9)
\psdot[dotstyle=*,dotsize=0.11](2.5, 8.75)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 8.5)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 8.75)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 8.5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 8.5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 8.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 8.25)
\psdot[dotstyle=*,dotsize=0.11](2.5, 8)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 8)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 9.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 9)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 9)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 8.75)
\psdot[dotstyle=*,dotsize=0.11](1.875, 8.75)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 9.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 9.75)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 9.5)
\psdot[dotstyle=*,dotsize=0.11](1.25, 9.5)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 9.25)
\psdot[dotstyle=*,dotsize=0.11](1.25, 9.25)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 9.75)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 9.5)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 9.5)
\psdot[dotstyle=*,dotsize=0.11](0.312579, 9.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 9.25)
\psdot[dotstyle=*,dotsize=0.11](0.625159, 9)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 9)
\psdot[dotstyle=*,dotsize=0.11](1.25, 9)
\psdot[dotstyle=*,dotsize=0.11](0.93742, 8.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 8.75)
\psdot[dotstyle=*,dotsize=0.11](1.25, 8.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 8.5)
\psdot[dotstyle=*,dotsize=0.11](1.56258, 8.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 8.5)
\psdot[dotstyle=*,dotsize=0.11](1.875, 8.25)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 8.25)
\psdot[dotstyle=*,dotsize=0.11](1.875, 8)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 8)
\psdot[dotstyle=*,dotsize=0.11](2.18752, 7.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 7.75)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 7.75)
\psdot[dotstyle=*,dotsize=0.11](2.5, 7.5)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 7.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 7.5)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 7.25)
\psdot[dotstyle=*,dotsize=0.11](3.125, 7.25)
\psdot[dotstyle=*,dotsize=0.11](3.125, 7)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 7)
\psdot[dotstyle=*,dotsize=0.11](3.75, 7)
\psdot[dotstyle=*,dotsize=0.11](3.75, 6.75)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 6.75)
\psdot[dotstyle=*,dotsize=0.11](4.06252, 6.5)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 6.75)
\psdot[dotstyle=*,dotsize=0.11](3.75, 6.5)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 6.5)
\psdot[dotstyle=*,dotsize=0.11](3.75, 6.25)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 6.25)
\psdot[dotstyle=*,dotsize=0.11](3.75, 6)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 6)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 5.75)
\psdot[dotstyle=*,dotsize=0.11](3.125, 5.75)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 5.5)
\psdot[dotstyle=*,dotsize=0.11](3.43752, 5.25)
\psdot[dotstyle=*,dotsize=0.11](3.125, 5.5)
\psdot[dotstyle=*,dotsize=0.11](3.125, 5.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 5.25)
\psdot[dotstyle=*,dotsize=0.11](2.81252, 5)
\psdot[dotstyle=*,dotsize=0.11](2.5, 5.25)
\psdot[dotstyle=*,dotsize=0.11](2.5, 5)
\psline[linewidth=0.03,linecolor=black](2.18752, 6)(1.875, 6.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.5)(0.312579, 8.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 8.25)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 8)(0.93742, 7.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 8)(0.312579, 8.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.25)(0, 8.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.25)(0.312579, 8)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.75)(0.625159, 8)
\psline[linewidth=0.03,linecolor=black](0.93742, 7.5)(0.93742, 7.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.5)(0.93742, 7.25)
\psline[linewidth=0.03,linecolor=black](1.25, 7.5)(1.25, 7.25)
\psline[linewidth=0.03,linecolor=black](1.25, 7)(1.25, 7.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.75)(1.56258, 7)
\psline[linewidth=0.03,linecolor=black](1.875, 6.5)(1.875, 6.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 7)(1.25, 6.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.5)(1.25, 6.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 6.25)(1.56258, 6.5)
\psline[linewidth=0.03,linecolor=black](1.875, 6)(1.875, 6.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 6)(2.18752, 5.75)
\psline[linewidth=0.03,linecolor=black](1.875, 5.75)(2.18752, 5.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.25)(0.93742, 5.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.5)(0, 5.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.25)(0.312579, 5.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.25)(0, 5.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.25)(0.93742, 5)
\psline[linewidth=0.03,linecolor=black](0, 4.75)(0.312579, 5)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.75)(0, 4.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 5)(0.625159, 5)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.5)(0, 4.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.25)(0, 4)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.5)(0.312579, 4.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 4.5)(0.625159, 4.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.75)(0.93742, 4.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 5)(1.25, 5)
\psline[linewidth=0.03,linecolor=black](0.93742, 4.5)(1.25, 4.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.25)(0.312579, 6.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 6)(0, 6.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.75)(0, 6)
\psline[linewidth=0.03,linecolor=black](0.312579, 5.75)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 5.75)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.93742, 5.5)(0.625159, 5.5)
\psline[linewidth=0.03,linecolor=black](1.25, 5.25)(0.93742, 5.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.5)(0.312579, 6.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 6.25)(0.312579, 6.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 6.25)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.25)(0.93742, 6)
\psline[linewidth=0.03,linecolor=black](0.93742, 5.75)(0.625159, 6)
\psline[linewidth=0.03,linecolor=black](1.25, 6)(1.25, 5.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 5.75)(1.25, 5.5)
\psline[linewidth=0.03,linecolor=black](1.25, 5.25)(1.56258, 5)
\psline[linewidth=0.03,linecolor=black](1.25, 5.25)(1.56258, 5.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.75)(1.25, 6.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.5)(0.312579, 7.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.75)(0, 8)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.5)(0.312579, 7.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 7.5)(0.625159, 7.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 7.25)(0, 7.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 7)(0, 7.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.75)(0, 7)
\psline[linewidth=0.03,linecolor=black](0.312579, 6.75)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 7)(0.625159, 7.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 7)(0.625159, 7.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 6.75)(0.625159, 7)
\psline[linewidth=0.03,linecolor=black](0.93742, 7)(0.93742, 6.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.75)(0.93742, 6.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.25)(0.625159, 6.5)
\psline[linewidth=0.03,linecolor=black](1.25, 6.25)(1.25, 6.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 6.25)(1.25, 6)
\psline[linewidth=0.03,linecolor=black](1.56258, 6)(1.25, 6.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 5.75)(1.25, 6)
\psline[linewidth=0.03,linecolor=black](1.56258, 6)(1.875, 5.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 5.5)(1.56258, 5.75)
\psline[linewidth=0.03,linecolor=black](1.875, 5.75)(1.875, 5.5)
\psline[linewidth=0.03,linecolor=black](1.875, 5.25)(1.56258, 5.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5.25)(1.875, 5.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.75)(1.875, 5)
\psline[linewidth=0.03,linecolor=black](2.18752, 5.25)(2.5, 5)
\psline[linewidth=0.03,linecolor=black](0.93742, 3.25)(0.93742, 3.5)
\psline[linewidth=0.03,linecolor=black](1.25, 3.5)(1.25, 3.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.5)(0.312579, 2.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 3)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0, 2.75)(0.312579, 3)
\psline[linewidth=0.03,linecolor=black](0.625159, 3.25)(0.625159, 3)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.25)(0, 3)
\psline[linewidth=0.03,linecolor=black](0.625159, 3.25)(0.625159, 3.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 3.5)(0.93742, 3.75)
\psline[linewidth=0.03,linecolor=black](1.25, 4)(1.25, 3.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 3.75)(1.56258, 4)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.25)(1.56258, 4)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.5)(0, 3.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 4)(0, 3.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.25)(0.312579, 4)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.75)(0.312579, 3.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 3.5)(0.625159, 3.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 4)(0.312579, 3.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 4)(0.625159, 3.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 4.25)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](1.25, 4.25)(0.93742, 4)
\psline[linewidth=0.03,linecolor=black](0.93742, 4)(0.93742, 4.25)
\psline[linewidth=0.03,linecolor=black](1.25, 4.5)(0.93742, 4.5)
\psline[linewidth=0.03,linecolor=black](1.25, 4.25)(1.56258, 4.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 4.75)(1.25, 4.5)
\psline[linewidth=0.03,linecolor=black](1.875, 4.75)(1.56258, 4.75)
\psline[linewidth=0.03,linecolor=black](1.875, 4.25)(1.875, 4.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.5)(2.18752, 4.75)
\psline[linewidth=0.03,linecolor=black](1.875, 4.75)(2.18752, 5)
\psline[linewidth=0.03,linecolor=black](0.93742, 3.25)(0.93742, 3)
\psline[linewidth=0.03,linecolor=black](0.93742, 3.25)(1.25, 3.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 2)(0.625159, 1.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 2.25)(0.93742, 2.5)
\psline[linewidth=0.03,linecolor=black](0, 2.25)(0.312579, 2.5)
\psline[linewidth=0.03,linecolor=black](0, 1.5)(0.312579, 1.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.75)(0.312579, 2)
\psline[linewidth=0.03,linecolor=black](0, 2)(0.312579, 2.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 2.25)(0.312579, 2)
\psline[linewidth=0.03,linecolor=black](0.625159, 2.25)(0.625159, 2.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 2.5)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 2.5)(0.93742, 2.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 3)(0.625159, 2.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 3)(1.25, 3.25)
\psline[linewidth=0.03,linecolor=black](1.25, 2.75)(1.25, 3)
\psline[linewidth=0.03,linecolor=black](1.25, 3.5)(1.56258, 3.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 3)(1.56258, 3.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 3.25)(1.56258, 3.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 3.75)(1.875, 4)
\psline[linewidth=0.03,linecolor=black](1.875, 3.5)(1.875, 3.75)
\psline[linewidth=0.03,linecolor=black](1.875, 4)(1.875, 4.25)
\psline[linewidth=0.03,linecolor=black](1.875, 4)(2.18752, 4.25)
\psline[linewidth=0.03,linecolor=black](1.875, 4.25)(2.18752, 4.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 4.5)(2.5, 4.75)
\psline[linewidth=0.03,linecolor=black](1.875, 3.5)(1.875, 3.25)
\psline[linewidth=0.03,linecolor=black](1.875, 3.5)(2.18752, 3.75)
\psline[linewidth=0.03,linecolor=black](0, 0.25)(0.312579, 0.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.5)(0.312579, 0.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 0.75)(0.312579, 1)
\psline[linewidth=0.03,linecolor=black](0, 1)(0.312579, 1.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 1.5)(0.312579, 1.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.75)(0.312579, 1.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.5)(0.625159, 1.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 2)(0.625159, 1.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.25)(0.93742, 2)
\psline[linewidth=0.03,linecolor=black](0.93742, 2.25)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](1.25, 2)(1.25, 2.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.25)(1.56258, 2.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.75)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](1.25, 2.75)(1.25, 2.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 3)(1.25, 2.75)
\psline[linewidth=0.03,linecolor=black](1.875, 3.25)(1.56258, 3)
\psline[linewidth=0.03,linecolor=black](1.875, 3)(1.875, 2.75)
\psline[linewidth=0.03,linecolor=black](1.875, 3.25)(2.18752, 3.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 3)(2.18752, 3.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 4)(2.18752, 3.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 4)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](2.5, 3.5)(2.5, 3.75)
\psline[linewidth=0.03,linecolor=black](2.5, 4)(2.5, 3.75)
\psline[linewidth=0.03,linecolor=black](2.5, 4.5)(2.5, 4.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.75)(0.93742, 1.5)
\psline[linewidth=0.03,linecolor=black](1.25, 2)(0.93742, 1.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.75)(0.625159, 0.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 0)(0.312579, 0.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.5)(0.312579, 0.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 0)(0.625159, 0.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.5)(0.93742, 0.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 1)(0.625159, 0.75)
\psline[linewidth=0.03,linecolor=black](0.625159, 0.75)(0.625159, 1)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.25)(0.625159, 1)
\psline[linewidth=0.03,linecolor=black](0.625159, 1.25)(0.625159, 1)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.5)(0.625159, 1.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 1.5)(1.25, 1.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.75)(1.56258, 2)
\psline[linewidth=0.03,linecolor=black](1.25, 2)(1.56258, 2.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 2.25)(1.875, 2.5)
\psline[linewidth=0.03,linecolor=black](1.875, 2.25)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.25)(2.18752, 2.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.75)(1.875, 2.5)
\psline[linewidth=0.03,linecolor=black](1.875, 2.5)(1.875, 2.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 3)(1.875, 2.75)
\psline[linewidth=0.03,linecolor=black](2.5, 3.25)(2.18752, 3)
\psline[linewidth=0.03,linecolor=black](2.5, 2.75)(2.5, 2.5)
\psline[linewidth=0.03,linecolor=black](2.5, 2.75)(2.5, 3)
\psline[linewidth=0.03,linecolor=black](2.81252, 2.75)(2.81252, 3)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.25)(2.81252, 3)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.5)(2.5, 3.25)
\psline[linewidth=0.03,linecolor=black](2.5, 3.25)(2.5, 3.5)
\psline[linewidth=0.03,linecolor=black](2.5, 3.5)(2.81252, 3.75)
\psline[linewidth=0.03,linecolor=black](3.125, 3.5)(3.125, 3.25)
\psline[linewidth=0.03,linecolor=black](3.125, 3.75)(3.125, 3.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.75)(2.81252, 4)
\psline[linewidth=0.03,linecolor=black](2.81252, 3.75)(3.125, 4)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.25)(2.81252, 4)
\psline[linewidth=0.03,linecolor=black](3.125, 3)(3.125, 3.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.5)(3.125, 3.25)
\psline[linewidth=0.03,linecolor=black](1.25, 1.5)(1.25, 1.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.75)(1.25, 1.5)
\psline[linewidth=0.03,linecolor=black](1.25, 0.75)(1.25, 1)
\psline[linewidth=0.03,linecolor=black](1.25, 1.25)(1.25, 1)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.5)(1.25, 1.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 1.75)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](1.875, 1.5)(1.875, 1.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 2)(2.18752, 1.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 2.25)(1.875, 2)
\psline[linewidth=0.03,linecolor=black](2.5, 2.5)(2.18752, 2.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 1)(1.56258, 1.25)
\psline[linewidth=0.03,linecolor=black](1.875, 1.5)(1.56258, 1.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.5)(0.93742, 0.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.5)(1.25, 0.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.25)(0.625159, 0)
\psline[linewidth=0.03,linecolor=black](0.93742, 0.25)(1.25, 0.5)
\psline[linewidth=0.03,linecolor=black](1.25, 0.75)(1.56258, 1)
\psline[linewidth=0.03,linecolor=black](1.25, 0.25)(1.25, 0)
\psline[linewidth=0.03,linecolor=black](1.25, 0.25)(1.56258, 0.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 0.5)(1.56258, 0.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 1)(1.875, 1.25)
\psline[linewidth=0.03,linecolor=black](1.875, 0.75)(1.875, 1)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.25)(2.18752, 1)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.5)(2.18752, 1.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.75)(1.875, 1.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 1.75)(2.5, 2)
\psline[linewidth=0.03,linecolor=black](2.5, 2)(2.5, 2.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 2.75)(2.5, 2.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 2)(2.81252, 2.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 2.25)(2.81252, 2.5)
\psline[linewidth=0.03,linecolor=black](3.125, 2.25)(3.125, 2.5)
\psline[linewidth=0.03,linecolor=black](3.125, 2.75)(3.125, 2.5)
\psline[linewidth=0.03,linecolor=black](3.125, 3)(2.81252, 2.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.25)(3.125, 3)
\psline[linewidth=0.03,linecolor=black](3.43752, 2.5)(3.43752, 2.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 3)(3.43752, 2.75)
\psline[linewidth=0.03,linecolor=black](3.75, 3.25)(3.43752, 3)
\psline[linewidth=0.03,linecolor=black](3.75, 2.75)(3.75, 3)
\psline[linewidth=0.03,linecolor=black](4.06252, 3.25)(4.06252, 3)
\psline[linewidth=0.03,linecolor=black](3.75, 3.25)(3.75, 3.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 3.5)(3.43752, 3.75)
\psline[linewidth=0.03,linecolor=black](3.75, 3.75)(4.06252, 3.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4)(3.43752, 3.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 4)(3.125, 4.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.5)(2.81252, 4.25)
\psline[linewidth=0.03,linecolor=black](2.5, 1.5)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.5, 1.5)(2.5, 1.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.5)(2.81252, 1.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 2)(2.5, 1.75)
\psline[linewidth=0.03,linecolor=black](3.125, 2.25)(2.81252, 2)
\psline[linewidth=0.03,linecolor=black](3.125, 2)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](3.125, 2.25)(3.43752, 2.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 2)(3.43752, 2.25)
\psline[linewidth=0.03,linecolor=black](3.75, 2.5)(3.75, 2.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 2.5)(3.75, 2.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 3)(3.75, 2.75)
\psline[linewidth=0.03,linecolor=black](1.875, 0.75)(1.875, 0.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 1)(1.875, 0.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 0)(1.56258, 0.25)
\psline[linewidth=0.03,linecolor=black](1.875, 0.5)(1.56258, 0.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 0)(1.875, 0.25)
\psline[linewidth=0.03,linecolor=black](1.875, 0.5)(2.18752, 0.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 0.25)(2.18752, 0.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 1)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.5, 0.75)(2.5, 1)
\psline[linewidth=0.03,linecolor=black](2.81252, 1)(2.81252, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.5)(2.5, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1.5)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](3.125, 1.5)(3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.75)(3.43752, 1.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 2)(3.125, 1.75)
\psline[linewidth=0.03,linecolor=black](3.75, 2.25)(3.43752, 2)
\psline[linewidth=0.03,linecolor=black](3.75, 1.75)(3.75, 2)
\psline[linewidth=0.03,linecolor=black](3.75, 2.25)(4.06252, 2.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 2.75)(4.06252, 2.5)
\psline[linewidth=0.03,linecolor=black](4.375, 3.25)(4.06252, 3)
\psline[linewidth=0.03,linecolor=black](4.06252, 3.5)(4.375, 3.25)
\psline[linewidth=0.03,linecolor=black](4.375, 2.75)(4.375, 3)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.25)(4.375, 3)
\psline[linewidth=0.03,linecolor=black](5.3125, 3.25)(5, 3.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 4.5)(6.25, 4.25)
\psline[linewidth=0.03,linecolor=black](6.25, 4)(5.93748, 4)
\psline[linewidth=0.03,linecolor=black](5.93748, 3.75)(5.625, 3.75)
\psline[linewidth=0.03,linecolor=black](5.625, 3.5)(5.3125, 3.5)
\psline[linewidth=0.03,linecolor=black](5, 3.5)(5.3125, 3.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.25)(4.375, 3.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 3.5)(4.06252, 3.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 3.5)(5, 3.75)
\psline[linewidth=0.03,linecolor=black](4.375, 3.75)(4.6875, 3.5)
\psline[linewidth=0.03,linecolor=black](3.75, 4)(4.06252, 3.75)
\psline[linewidth=0.03,linecolor=black](4.375, 4)(4.06252, 4)
\psline[linewidth=0.03,linecolor=black](3.75, 4)(3.43752, 4.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.25)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](3.75, 4.25)(4.06252, 4.25)
\psline[linewidth=0.03,linecolor=black](3.75, 4.25)(3.43752, 4.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 4.75)(3.125, 4.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.75)(3.125, 4.75)
\psline[linewidth=0.03,linecolor=black](5.625, 4.75)(5.93748, 5)
\psline[linewidth=0.03,linecolor=black](5.3125, 4.75)(5.625, 4.75)
\psline[linewidth=0.03,linecolor=black](5, 4.5)(5.3125, 4.5)
\psline[linewidth=0.03,linecolor=black](6.25, 5)(5.93748, 4.75)
\psline[linewidth=0.03,linecolor=black](5.625, 4.5)(5.93748, 4.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 4.5)(5.625, 4.5)
\psline[linewidth=0.03,linecolor=black](5, 4.25)(5.3125, 4.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 4.25)(5, 4.25)
\psline[linewidth=0.03,linecolor=black](5.625, 4)(5.3125, 3.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.75)(6.875, 4.75)
\psline[linewidth=0.03,linecolor=black](6.875, 4.75)(6.56248, 4.75)
\psline[linewidth=0.03,linecolor=black](6.875, 4.5)(6.56248, 4.5)
\psline[linewidth=0.03,linecolor=black](6.25, 4.75)(6.56248, 4.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 4.5)(6.25, 4.5)
\psline[linewidth=0.03,linecolor=black](5.93748, 4.5)(6.25, 4.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 4.25)(6.25, 4.5)
\psline[linewidth=0.03,linecolor=black](5.625, 4.25)(5.93748, 4.5)
\psline[linewidth=0.03,linecolor=black](5.625, 4)(5.93748, 4.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 4.25)(5.625, 4.25)
\psline[linewidth=0.03,linecolor=black](5.625, 4)(5.3125, 4)
\psline[linewidth=0.03,linecolor=black](5, 4)(5.3125, 4.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 3.75)(5, 3.75)
\psline[linewidth=0.03,linecolor=black](5, 3.75)(4.6875, 3.75)
\psline[linewidth=0.03,linecolor=black](5, 4)(4.6875, 4)
\psline[linewidth=0.03,linecolor=black](4.375, 4)(4.6875, 3.75)
\psline[linewidth=0.03,linecolor=black](4.375, 4.25)(4.6875, 4.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.25)(4.375, 4)
\psline[linewidth=0.03,linecolor=black](3.75, 4.5)(4.06252, 4.25)
\psline[linewidth=0.03,linecolor=black](4.375, 4.5)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](4.375, 4.5)(4.06252, 4.5)
\psline[linewidth=0.03,linecolor=black](3.75, 4.75)(4.06252, 4.75)
\psline[linewidth=0.03,linecolor=black](3.75, 4.5)(3.43752, 4.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 4.75)(3.125, 5)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.75)(4.375, 4.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 4.75)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](5, 4.75)(5.3125, 5)
\psline[linewidth=0.03,linecolor=black](5.625, 5)(5.93748, 5)
\psline[linewidth=0.03,linecolor=black](5.625, 5)(5.3125, 5)
\psline[linewidth=0.03,linecolor=black](5.3125, 5)(5, 5)
\psline[linewidth=0.03,linecolor=black](5, 4.75)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](4.375, 4.75)(4.6875, 4.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5)(5, 4.75)
\psline[linewidth=0.03,linecolor=black](5, 4.75)(4.6875, 4.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 5)(4.375, 4.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.25)(4.375, 5)
\psline[linewidth=0.03,linecolor=black](5, 5.25)(5.3125, 5.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.25)(5, 5.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 5.25)(5.625, 5.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 5.25)(5, 5.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.25)(4.375, 5.25)
\psline[linewidth=0.03,linecolor=black](5, 5.75)(4.6875, 5.5)
\psline[linewidth=0.03,linecolor=black](5, 5.75)(4.6875, 5.75)
\psline[linewidth=0.03,linecolor=black](4.6875, 5.5)(4.375, 5.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.25)(4.375, 5.5)
\psline[linewidth=0.03,linecolor=black](3.75, 5.25)(4.06252, 5.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 5)(3.75, 5)
\psline[linewidth=0.03,linecolor=black](1.875, 8)(1.875, 7.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 9)(0, 9.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.75)(0, 9)
\psline[linewidth=0.03,linecolor=black](0.312579, 8.75)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 9)(0.625159, 8.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.5)(0.93742, 8.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.25)(0.625159, 8.5)
\psline[linewidth=0.03,linecolor=black](1.25, 8.25)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 8)(1.56258, 8.25)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.25)(0.93742, 8)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.25)(1.25, 8)
\psline[linewidth=0.03,linecolor=black](1.25, 7.75)(0.93742, 8)
\psline[linewidth=0.03,linecolor=black](1.56258, 8)(1.56258, 7.75)
\psline[linewidth=0.03,linecolor=black](1.875, 7.5)(1.56258, 7.75)
\psline[linewidth=0.03,linecolor=black](1.875, 6.5)(1.875, 6.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.25)(1.875, 6.5)
\psline[linewidth=0.03,linecolor=black](1.875, 7.25)(2.18752, 7)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.5)(1.25, 7.75)
\psline[linewidth=0.03,linecolor=black](1.25, 7.75)(1.25, 7.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 7.25)(1.25, 7.5)
\psline[linewidth=0.03,linecolor=black](1.875, 7.25)(1.56258, 7.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 7)(1.56258, 7.25)
\psline[linewidth=0.03,linecolor=black](1.875, 7.25)(1.875, 7)
\psline[linewidth=0.03,linecolor=black](1.875, 6.75)(1.56258, 7)
\psline[linewidth=0.03,linecolor=black](2.18752, 7)(2.18752, 6.75)
\psline[linewidth=0.03,linecolor=black](1.875, 6.75)(2.18752, 6.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 6.75)(2.5, 6.5)
\psline[linewidth=0.03,linecolor=black](2.5, 6.5)(2.5, 6.25)
\psline[linewidth=0.03,linecolor=black](2.5, 6)(2.18752, 6.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.75)(2.18752, 7.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.25)(2.18752, 7.5)
\psline[linewidth=0.03,linecolor=black](2.18752, 7.25)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.5, 7.5)(2.5, 7.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 7)(2.81252, 7.25)
\psline[linewidth=0.03,linecolor=black](2.5, 6.75)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.75)(2.5, 7)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.5)(2.5, 6.75)
\psline[linewidth=0.03,linecolor=black](3.125, 6.75)(3.125, 7)
\psline[linewidth=0.03,linecolor=black](3.125, 6.75)(3.125, 6.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.5)(2.81252, 6.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.5)(3.125, 6.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 6.25)(2.81252, 6)
\psline[linewidth=0.03,linecolor=black](3.125, 6)(3.43752, 6.25)
\psline[linewidth=0.03,linecolor=black](3.125, 5.75)(2.81252, 5.5)
\psline[linewidth=0.03,linecolor=black](2.5, 6)(2.5, 5.75)
\psline[linewidth=0.03,linecolor=black](2.5, 6)(2.81252, 5.75)
\psline[linewidth=0.03,linecolor=black](2.5, 5.75)(2.5, 5.5)
\psline[linewidth=0.03,linecolor=black](2.5, 5.5)(2.5, 5.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.25)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](4.375, 5.75)(4.06252, 5.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.5)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 6)(4.375, 5.75)
\psline[linewidth=0.03,linecolor=black](6.25, 5)(5.93748, 5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.25)(5.93748, 5)
\psline[linewidth=0.03,linecolor=black](6.875, 5)(6.56248, 5)
\psline[linewidth=0.03,linecolor=black](6.56248, 5)(6.25, 5)
\psline[linewidth=0.03,linecolor=black](5.93748, 5.25)(6.25, 5)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.25)(6.25, 5.25)
\psline[linewidth=0.03,linecolor=black](5.625, 5.25)(5.3125, 5.5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.5)(5.93748, 5.5)
\psline[linewidth=0.03,linecolor=black](5, 5.75)(5.3125, 5.5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.75)(5.3125, 5.75)
\psline[linewidth=0.03,linecolor=black](5, 5.75)(4.6875, 6)
\psline[linewidth=0.03,linecolor=black](5.3125, 6)(5, 6)
\psline[linewidth=0.03,linecolor=black](6.25, 5.5)(5.93748, 5.5)
\psline[linewidth=0.03,linecolor=black](5.625, 5.75)(5.93748, 5.5)
\psline[linewidth=0.03,linecolor=black](7.5, 5)(7.18748, 5)
\psline[linewidth=0.03,linecolor=black](6.875, 5)(7.18748, 5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.25)(6.875, 5.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.25)(6.875, 5)
\psline[linewidth=0.03,linecolor=black](6.25, 5.5)(6.56248, 5.25)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.5)(6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](6.25, 5.5)(5.93748, 5.75)
\psline[linewidth=0.03,linecolor=black](5.625, 5.75)(5.3125, 6)
\psline[linewidth=0.03,linecolor=black](5.93748, 6)(6.25, 5.75)
\psline[linewidth=0.03,linecolor=black](5.93748, 6)(5.625, 6)
\psline[linewidth=0.03,linecolor=black](5.625, 6.25)(5.3125, 6.25)
\psline[linewidth=0.03,linecolor=black](5.3125, 6)(5, 6.25)
\psline[linewidth=0.03,linecolor=black](5, 6.25)(4.6875, 6.25)
\psline[linewidth=0.03,linecolor=black](4.6875, 6)(4.375, 6)
\psline[linewidth=0.03,linecolor=black](4.375, 5.75)(4.06252, 5.75)
\psline[linewidth=0.03,linecolor=black](5, 6.5)(5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 6.5)(5, 6.5)
\psline[linewidth=0.03,linecolor=black](4.6875, 7)(4.6875, 7.25)
\psline[linewidth=0.03,linecolor=black](4.375, 7)(4.6875, 6.75)
\psline[linewidth=0.03,linecolor=black](4.375, 6.25)(4.6875, 6.5)
\psline[linewidth=0.03,linecolor=black](4.375, 7.5)(4.375, 7.25)
\psline[linewidth=0.03,linecolor=black](3.75, 8)(3.75, 7.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 7.5)(4.06252, 7.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 10)(2.5, 9.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 9.75)(2.5, 9.5)
\psline[linewidth=0.03,linecolor=black](2.5, 9.25)(2.81252, 9)
\psline[linewidth=0.03,linecolor=black](2.18752, 10)(2.18752, 9.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 10)(1.875, 9.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 9.75)(2.18752, 9.5)
\psline[linewidth=0.03,linecolor=black](2.5, 9.25)(2.18752, 9.5)
\psline[linewidth=0.03,linecolor=black](2.5, 9.25)(2.5, 9)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.75)(2.5, 9)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.5)(3.125, 8.25)
\psline[linewidth=0.03,linecolor=black](3.125, 8.75)(3.125, 8.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.25)(3.43752, 8.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 8)(3.43752, 8.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.25)(3.125, 8)
\psline[linewidth=0.03,linecolor=black](3.43752, 8)(3.43752, 7.75)
\psline[linewidth=0.03,linecolor=black](3.75, 7.5)(3.43752, 7.75)
\psline[linewidth=0.03,linecolor=black](4.06252, 7.5)(4.06252, 7.25)
\psline[linewidth=0.03,linecolor=black](4.375, 7.25)(4.375, 7)
\psline[linewidth=0.03,linecolor=black](3.75, 7.25)(3.43752, 7.5)
\psline[linewidth=0.03,linecolor=black](3.75, 7.25)(4.06252, 7)
\psline[linewidth=0.03,linecolor=black](4.375, 7)(4.375, 6.75)
\psline[linewidth=0.03,linecolor=black](4.375, 6.75)(4.375, 6.5)
\psline[linewidth=0.03,linecolor=black](4.375, 6.25)(4.06252, 6)
\psline[linewidth=0.03,linecolor=black](4.06252, 5.75)(3.75, 5.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.5)(3.75, 5.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.5)(4.06252, 6.25)
\psline[linewidth=0.03,linecolor=black](3.75, 6)(4.06252, 6.25)
\psline[linewidth=0.03,linecolor=black](3.125, 7.75)(3.43752, 7.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 7.25)(3.43752, 7.5)
\psline[linewidth=0.03,linecolor=black](3.75, 7)(3.43752, 7.25)
\psline[linewidth=0.03,linecolor=black](3.125, 7.75)(2.81252, 8)
\psline[linewidth=0.03,linecolor=black](3.125, 7.5)(3.125, 7.75)
\psline[linewidth=0.03,linecolor=black](1.875, 9.5)(2.18752, 9.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.75)(1.875, 9.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.75)(1.56258, 10)
\psline[linewidth=0.03,linecolor=black](1.25, 9.75)(1.25, 10)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.75)(1.56258, 9.5)
\psline[linewidth=0.03,linecolor=black](1.875, 9.5)(1.875, 9.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 9)(2.18752, 9.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 9)(2.5, 8.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.5)(2.5, 8.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 8.5)(2.81252, 8.25)
\psline[linewidth=0.03,linecolor=black](1.875, 9)(2.18752, 8.75)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.75)(2.5, 8.5)
\psline[linewidth=0.03,linecolor=black](1.875, 8.75)(2.18752, 8.5)
\psline[linewidth=0.03,linecolor=black](2.5, 8.5)(2.5, 8.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 8)(2.81252, 8.25)
\psline[linewidth=0.03,linecolor=black](2.5, 8)(2.18752, 8.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 8)(2.81252, 7.75)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.25)(1.25, 9.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 9.25)(1.875, 9)
\psline[linewidth=0.03,linecolor=black](1.875, 8.75)(1.875, 9)
\psline[linewidth=0.03,linecolor=black](1.56258, 9)(1.25, 9.25)
\psline[linewidth=0.03,linecolor=black](1.56258, 9)(1.56258, 8.75)
\psline[linewidth=0.03,linecolor=black](1.875, 8.75)(1.875, 8.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.75)(0.625159, 10)
\psline[linewidth=0.03,linecolor=black](0.312579, 10)(0.625159, 9.75)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.75)(1.25, 9.5)
\psline[linewidth=0.03,linecolor=black](0.93742, 9.75)(0.93742, 9.5)
\psline[linewidth=0.03,linecolor=black](1.25, 9.25)(1.25, 9.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.5)(0.93742, 9.25)
\psline[linewidth=0.03,linecolor=black](1.25, 9)(1.25, 9.25)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.75)(0.312579, 10)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.5)(0, 9.75)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.75)(0.625159, 9.5)
\psline[linewidth=0.03,linecolor=black](0.312579, 9.25)(0.312579, 9.5)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.5)(0.625159, 9.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 9)(0.312579, 9.25)
\psline[linewidth=0.03,linecolor=black](0.625159, 9.25)(0.93742, 9)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.75)(0.625159, 9)
\psline[linewidth=0.03,linecolor=black](1.25, 8.75)(1.25, 9)
\psline[linewidth=0.03,linecolor=black](0.93742, 8.75)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](1.25, 8.75)(1.56258, 8.5)
\psline[linewidth=0.03,linecolor=black](1.56258, 8.25)(1.25, 8.5)
\psline[linewidth=0.03,linecolor=black](1.875, 8)(1.56258, 8.25)
\psline[linewidth=0.03,linecolor=black](1.875, 8.5)(2.18752, 8.25)
\psline[linewidth=0.03,linecolor=black](1.875, 8.5)(1.875, 8.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 8.25)(2.18752, 8)
\psline[linewidth=0.03,linecolor=black](1.875, 8)(2.18752, 7.75)
\psline[linewidth=0.03,linecolor=black](2.5, 7.75)(2.18752, 8)
\psline[linewidth=0.03,linecolor=black](2.5, 7.5)(2.18752, 7.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 7.5)(2.81252, 7.75)
\psline[linewidth=0.03,linecolor=black](2.5, 7.5)(2.81252, 7.25)
\psline[linewidth=0.03,linecolor=black](3.125, 7.5)(3.125, 7.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 7.25)(3.125, 7)
\psline[linewidth=0.03,linecolor=black](3.125, 7.25)(3.43752, 7)
\psline[linewidth=0.03,linecolor=black](3.125, 7)(3.43752, 6.75)
\psline[linewidth=0.03,linecolor=black](3.75, 6.75)(3.75, 7)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.75)(3.75, 7)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.75)(4.06252, 6.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 6.5)(3.75, 6.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.5)(3.43752, 6.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.75)(3.75, 6.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.25)(3.43752, 6.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 6.25)(3.43752, 6)
\psline[linewidth=0.03,linecolor=black](3.75, 6)(3.43752, 5.75)
\psline[linewidth=0.03,linecolor=black](3.125, 5.75)(3.43752, 6)
\psline[linewidth=0.03,linecolor=black](3.125, 5.5)(3.125, 5.75)
\psline[linewidth=0.03,linecolor=black](3.43752, 5.25)(3.125, 5.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 5.25)(3.125, 5.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 5)(3.125, 5.25)


==> examples/cart/ddisc7.tex <==
\psline[linewidth=0.03,linecolor=black](0, 5.25)(0, 5)
\psdot[dotstyle=*,dotsize=0.13](0, 5)
\psdot[dotstyle=*,dotsize=0.13](0, 5.25)
\psline[linewidth=0.03,linecolor=black](0, 5.25)(0, 5.5)
\psdot[dotstyle=*,dotsize=0.13](0, 5.5)
\psline[linewidth=0.03,linecolor=black](0, 5.75)(0, 5.5)
\psdot[dotstyle=*,dotsize=0.13](0, 5.75)
\psline[linewidth=0.03,linecolor=black](0, 6)(0, 5.75)
\psdot[dotstyle=*,dotsize=0.13](0, 6)
\psline[linewidth=0.03,linecolor=black](0, 6)(0, 6.25)
\psdot[dotstyle=*,dotsize=0.13](0, 6.25)
\psline[linewidth=0.03,linecolor=black](0, 6.5)(0, 6.25)
\psdot[dotstyle=*,dotsize=0.13](0, 6.5)
\psline[linewidth=0.03,linecolor=black](0, 6.75)(0, 6.5)
\psdot[dotstyle=*,dotsize=0.13](0, 6.75)
\psline[linewidth=0.03,linecolor=black](0, 6.75)(0, 7)
\psdot[dotstyle=*,dotsize=0.13](0, 7)
\psline[linewidth=0.03,linecolor=black](0, 7.25)(0, 7)
\psdot[dotstyle=*,dotsize=0.13](0, 7.25)
\psline[linewidth=0.03,linecolor=black](0, 7.25)(0, 7.5)
\psdot[dotstyle=*,dotsize=0.13](0, 7.5)
\psline[linewidth=0.03,linecolor=black](0, 7.75)(0, 7.5)
\psdot[dotstyle=*,dotsize=0.13](0, 7.75)
\psline[linewidth=0.03,linecolor=black](0, 8)(0, 7.75)
\psdot[dotstyle=*,dotsize=0.13](0, 8)
\psline[linewidth=0.03,linecolor=black](0, 8)(0, 8.25)
\psdot[dotstyle=*,dotsize=0.13](0, 8.25)
\psline[linewidth=0.03,linecolor=black](0, 8.5)(0, 8.25)
\psdot[dotstyle=*,dotsize=0.13](0, 8.5)
\psline[linewidth=0.03,linecolor=black](0, 8.5)(0, 8.75)
\psdot[dotstyle=*,dotsize=0.13](0, 8.75)
\psline[linewidth=0.03,linecolor=black](0, 9)(0, 8.75)
\psdot[dotstyle=*,dotsize=0.13](0, 9)
\psline[linewidth=0.03,linecolor=black](0, 9.25)(0, 9)
\psdot[dotstyle=*,dotsize=0.13](0, 9.25)
\psline[linewidth=0.03,linecolor=black](0, 9.25)(0, 9.5)
\psdot[dotstyle=*,dotsize=0.13](0, 9.5)
\psline[linewidth=0.03,linecolor=black](0, 9.75)(0, 9.5)
\psdot[dotstyle=*,dotsize=0.13](0, 9.75)
\psline[linewidth=0.03,linecolor=black](0, 9.75)(0, 10)
\psline[linewidth=0.03,linecolor=black](0, 4.75)(0, 5)
\psdot[dotstyle=*,dotsize=0.13](0, 4.75)
\psline[linewidth=0.03,linecolor=black](0, 4.75)(0, 4.5)
\psdot[dotstyle=*,dotsize=0.13](0, 4.5)
\psline[linewidth=0.03,linecolor=black](0, 4.25)(0, 4.5)
\psdot[dotstyle=*,dotsize=0.13](0, 4.25)
\psline[linewidth=0.03,linecolor=black](0, 4.25)(0, 4)
\psdot[dotstyle=*,dotsize=0.13](0, 4)
\psline[linewidth=0.03,linecolor=black](0, 4)(0, 3.75)
\psdot[dotstyle=*,dotsize=0.13](0, 3.75)
\psline[linewidth=0.03,linecolor=black](0, 3.5)(0, 3.75)
\psdot[dotstyle=*,dotsize=0.13](0, 3.5)
\psline[linewidth=0.03,linecolor=black](0, 3.5)(0, 3.25)
\psdot[dotstyle=*,dotsize=0.13](0, 3.25)
\psline[linewidth=0.03,linecolor=black](0, 3.25)(0, 3)
\psdot[dotstyle=*,dotsize=0.13](0, 3)
\psline[linewidth=0.03,linecolor=black](0, 2.75)(0, 3)
\psdot[dotstyle=*,dotsize=0.13](0, 2.75)
\psline[linewidth=0.03,linecolor=black](0, 2.75)(0, 2.5)
\psdot[dotstyle=*,dotsize=0.13](0, 2.5)
\psline[linewidth=0.03,linecolor=black](0, 2.25)(0, 2.5)
\psdot[dotstyle=*,dotsize=0.13](0, 2.25)
\psline[linewidth=0.03,linecolor=black](0, 2)(0, 2.25)
\psdot[dotstyle=*,dotsize=0.13](0, 2)
\psline[linewidth=0.03,linecolor=black](0, 2)(0, 1.75)
\psdot[dotstyle=*,dotsize=0.13](0, 1.75)
\psline[linewidth=0.03,linecolor=black](0, 1.5)(0, 1.75)
\psdot[dotstyle=*,dotsize=0.13](0, 1.5)
\psline[linewidth=0.03,linecolor=black](0, 1.5)(0, 1.25)
\psdot[dotstyle=*,dotsize=0.13](0, 1.25)
\psline[linewidth=0.03,linecolor=black](0, 1)(0, 1.25)
\psdot[dotstyle=*,dotsize=0.13](0, 1)
\psline[linewidth=0.03,linecolor=black](0, 0.75)(0, 1)
\psdot[dotstyle=*,dotsize=0.13](0, 0.75)
\psline[linewidth=0.03,linecolor=black](0, 0.75)(0, 0.5)
\psdot[dotstyle=*,dotsize=0.13](0, 0.5)
\psline[linewidth=0.03,linecolor=black](0, 0.25)(0, 0.5)
\psdot[dotstyle=*,dotsize=0.13](0, 0.25)
\psline[linewidth=0.03,linecolor=black](0, 0.25)(0, 0)


==> examples/cart/ddisc8.tex <==
\psline[linewidth=0.03,linecolor=black](5, 7)(5, 6.75)
\psdot[dotstyle=*,dotsize=0.13](5, 6.75)
\psdot[dotstyle=*,dotsize=0.13](5, 7)
\psline[linewidth=0.03,linecolor=black](5, 7)(4.6875, 7.25)
\psdot[dotstyle=*,dotsize=0.13](4.6875, 7.25)
\psline[linewidth=0.03,linecolor=black](4.375, 7.5)(4.6875, 7.25)
\psdot[dotstyle=*,dotsize=0.13](4.375, 7.5)
\psline[linewidth=0.03,linecolor=black](4.375, 7.5)(4.06252, 7.75)
\psdot[dotstyle=*,dotsize=0.13](4.06252, 7.75)
\psline[linewidth=0.03,linecolor=black](3.75, 8)(4.06252, 7.75)
\psdot[dotstyle=*,dotsize=0.13](3.75, 8)
\psline[linewidth=0.03,linecolor=black](3.75, 8.25)(3.75, 8)
\psdot[dotstyle=*,dotsize=0.13](3.75, 8.25)
\psline[linewidth=0.03,linecolor=black](3.43752, 8.5)(3.75, 8.25)
\psdot[dotstyle=*,dotsize=0.13](3.43752, 8.5)
\psline[linewidth=0.03,linecolor=black](3.125, 8.75)(3.43752, 8.5)
\psdot[dotstyle=*,dotsize=0.13](3.125, 8.75)
\psline[linewidth=0.03,linecolor=black](3.125, 9)(3.125, 8.75)
\psdot[dotstyle=*,dotsize=0.13](3.125, 9)
\psline[linewidth=0.03,linecolor=black](3.125, 9)(2.81252, 9.25)
\psdot[dotstyle=*,dotsize=0.13](2.81252, 9.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 9.25)(2.81252, 9.5)
\psdot[dotstyle=*,dotsize=0.13](2.81252, 9.5)
\psline[linewidth=0.03,linecolor=black](2.81252, 9.75)(2.81252, 9.5)
\psdot[dotstyle=*,dotsize=0.13](2.81252, 9.75)
\psline[linewidth=0.03,linecolor=black](2.81252, 9.75)(2.81252, 10)
\psdot[dotstyle=*,dotsize=0.13](2.81252, 10)
\psline[linewidth=0.03,linecolor=black](2.81252, 10)(2.5, 10)
\psdot[dotstyle=*,dotsize=0.13](2.5, 10)
\psline[linewidth=0.03,linecolor=black](2.5, 10)(2.18752, 10)
\psdot[dotstyle=*,dotsize=0.13](2.18752, 10)
\psline[linewidth=0.03,linecolor=black](2.18752, 10)(1.875, 10)
\psdot[dotstyle=*,dotsize=0.13](1.875, 10)
\psline[linewidth=0.03,linecolor=black](1.875, 10)(1.56258, 10)
\psdot[dotstyle=*,dotsize=0.13](1.56258, 10)
\psline[linewidth=0.03,linecolor=black](1.56258, 10)(1.25, 10)
\psdot[dotstyle=*,dotsize=0.13](1.25, 10)
\psline[linewidth=0.03,linecolor=black](0.93742, 10)(1.25, 10)
\psdot[dotstyle=*,dotsize=0.13](0.93742, 10)
\psline[linewidth=0.03,linecolor=black](0.93742, 10)(0.625159, 10)
\psdot[dotstyle=*,dotsize=0.13](0.625159, 10)
\psline[linewidth=0.03,linecolor=black](0.625159, 10)(0.312579, 10)
\psdot[dotstyle=*,dotsize=0.13](0.312579, 10)
\psline[linewidth=0.03,linecolor=black](0.312579, 10)(0, 10)
\psline[linewidth=0.03,linecolor=black](5.3125, 6.75)(5, 6.75)
\psdot[dotstyle=*,dotsize=0.13](5.3125, 6.75)
\psline[linewidth=0.03,linecolor=black](5.3125, 6.75)(5.3125, 6.5)
\psdot[dotstyle=*,dotsize=0.13](5.3125, 6.5)
\psline[linewidth=0.03,linecolor=black](5.625, 6.25)(5.3125, 6.5)
\psdot[dotstyle=*,dotsize=0.13](5.625, 6.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.25)(5.625, 6.25)
\psdot[dotstyle=*,dotsize=0.13](5.93748, 6.25)
\psline[linewidth=0.03,linecolor=black](5.93748, 6.25)(6.25, 6)
\psdot[dotstyle=*,dotsize=0.13](6.25, 6)
\psline[linewidth=0.03,linecolor=black](6.25, 6)(6.25, 5.75)
\psdot[dotstyle=*,dotsize=0.13](6.25, 5.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.75)(6.25, 5.75)
\psdot[dotstyle=*,dotsize=0.13](6.56248, 5.75)
\psline[linewidth=0.03,linecolor=black](6.56248, 5.75)(6.875, 5.5)
\psdot[dotstyle=*,dotsize=0.13](6.875, 5.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.25)(6.875, 5.5)
\psdot[dotstyle=*,dotsize=0.13](7.18748, 5.25)
\psline[linewidth=0.03,linecolor=black](7.18748, 5.25)(7.5, 5)


==> examples/cart/ddisc9.tex <==
\psline[linewidth=0.03,linecolor=black](4.6875, 3)(5, 3)
\psdot[dotstyle=*,dotsize=0.13](5, 3)
\psdot[dotstyle=*,dotsize=0.13](4.6875, 3)
\psline[linewidth=0.03,linecolor=black](4.375, 2.75)(4.6875, 3)
\psdot[dotstyle=*,dotsize=0.13](4.375, 2.75)
\psline[linewidth=0.03,linecolor=black](4.375, 2.5)(4.375, 2.75)
\psdot[dotstyle=*,dotsize=0.13](4.375, 2.5)
\psline[linewidth=0.03,linecolor=black](4.06252, 2.25)(4.375, 2.5)
\psdot[dotstyle=*,dotsize=0.13](4.06252, 2.25)
\psline[linewidth=0.03,linecolor=black](4.06252, 2)(4.06252, 2.25)
\psdot[dotstyle=*,dotsize=0.13](4.06252, 2)
\psline[linewidth=0.03,linecolor=black](4.06252, 2)(3.75, 1.75)
\psdot[dotstyle=*,dotsize=0.13](3.75, 1.75)
\psline[linewidth=0.03,linecolor=black](3.75, 1.75)(3.43752, 1.5)
\psdot[dotstyle=*,dotsize=0.13](3.43752, 1.5)
\psline[linewidth=0.03,linecolor=black](3.43752, 1.5)(3.125, 1.25)
\psdot[dotstyle=*,dotsize=0.13](3.125, 1.25)
\psline[linewidth=0.03,linecolor=black](2.81252, 1)(3.125, 1.25)
\psdot[dotstyle=*,dotsize=0.13](2.81252, 1)
\psline[linewidth=0.03,linecolor=black](2.5, 0.75)(2.81252, 1)
\psdot[dotstyle=*,dotsize=0.13](2.5, 0.75)
\psline[linewidth=0.03,linecolor=black](2.5, 0.75)(2.5, 0.5)
\psdot[dotstyle=*,dotsize=0.13](2.5, 0.5)
\psline[linewidth=0.03,linecolor=black](2.5, 0.5)(2.18752, 0.25)
\psdot[dotstyle=*,dotsize=0.13](2.18752, 0.25)
\psline[linewidth=0.03,linecolor=black](2.18752, 0.25)(2.18752, 0)
\psdot[dotstyle=*,dotsize=0.13](2.18752, 0)
\psline[linewidth=0.03,linecolor=black](1.875, 0)(2.18752, 0)
\psdot[dotstyle=*,dotsize=0.13](1.875, 0)
\psline[linewidth=0.03,linecolor=black](1.56258, 0)(1.875, 0)
\psdot[dotstyle=*,dotsize=0.13](1.56258, 0)
\psline[linewidth=0.03,linecolor=black](1.56258, 0)(1.25, 0)
\psdot[dotstyle=*,dotsize=0.13](1.25, 0)
\psline[linewidth=0.03,linecolor=black](0.93742, 0)(1.25, 0)
\psdot[dotstyle=*,dotsize=0.13](0.93742, 0)
\psline[linewidth=0.03,linecolor=black](0.93742, 0)(0.625159, 0)
\psdot[dotstyle=*,dotsize=0.13](0.625159, 0)
\psline[linewidth=0.03,linecolor=black](0.312579, 0)(0.625159, 0)
\psdot[dotstyle=*,dotsize=0.13](0.312579, 0)
\psline[linewidth=0.03,linecolor=black](0.312579, 0)(0, 0)
\psline[linewidth=0.03,linecolor=black](5.3125, 3.25)(5, 3)
\psdot[dotstyle=*,dotsize=0.13](5.3125, 3.25)
\psline[linewidth=0.03,linecolor=black](5.625, 3.5)(5.3125, 3.25)
\psdot[dotstyle=*,dotsize=0.13](5.625, 3.5)
\psline[linewidth=0.03,linecolor=black](5.625, 3.5)(5.93748, 3.75)
\psdot[dotstyle=*,dotsize=0.13](5.93748, 3.75)
\psline[linewidth=0.03,linecolor=black](6.25, 4)(5.93748, 3.75)
\psdot[dotstyle=*,dotsize=0.13](6.25, 4)
\psline[linewidth=0.03,linecolor=black](6.25, 4)(6.56248, 4.25)
\psdot[dotstyle=*,dotsize=0.13](6.56248, 4.25)
\psline[linewidth=0.03,linecolor=black](6.875, 4.5)(6.56248, 4.25)
\psdot[dotstyle=*,dotsize=0.13](6.875, 4.5)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.75)(6.875, 4.5)
\psdot[dotstyle=*,dotsize=0.13](7.18748, 4.75)
\psline[linewidth=0.03,linecolor=black](7.18748, 4.75)(7.5, 5)


==> examples/cart/graph.tex <==
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 0.5)(10, 0.25)(10, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 0.25)(9.68742, 0.5)(9.68742, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 5.5)(9.37484, 5.25)(9.68742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 5.25)(9.68742, 5.5)(9.37484, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 5.5)(10, 5.25)(10, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 5.25)(9.68742, 5.5)(9.68742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 0.5)(1.25, 0.75)(0.93742, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 0.75)(0.93742, 0.5)(1.25, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5)(8.75, 5)(8.75, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.25)(8.43742, 5)(8.75, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.25)(1.56258, 5)(1.875, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5)(1.875, 5.25)(1.56258, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 5.25)(1.56258, 5)(1.56258, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5)(1.25, 5.25)(1.25, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 5.25)(0.93742, 5)(1.25, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5)(1.25, 5.25)(0.93742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.5)(8.125, 5.5)(8.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.25)(8.43742, 5.5)(8.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.5)(8.43742, 5.25)(8.75, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 5.5)(8.43742, 5.5)(8.75, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5.5)(9.37484, 5.25)(9.37484, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5.5)(9.06258, 5.25)(9.37484, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5.5)(8.75, 5.5)(8.75, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5.25)(9.06258, 5.5)(8.75, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 0.5)(5, 0.25)(5.3125, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 0.25)(5.3125, 0.5)(5, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 0.25)(3.43752, 0)(3.75, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 0)(3.75, 0.25)(3.43752, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 0.75)(0.312579, 0.75)(0, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0.75)(0.312579, 1)(0, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0)(0, 0.25)(0, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0)(0.312579, 0.25)(0, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0.25)(0.312579, 0)(0.625159, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0)(0.625159, 0)(0.625159, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 1)(0.312579, 1.25)(0, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1)(0.312579, 1.25)(0, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 1.25)(0.312579, 1.25)(0.625159, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1.25)(0.312579, 1)(0.625159, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 0.75)(0.93742, 1)(0.93742, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1)(1.25, 0.75)(1.25, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 2)(0.312579, 2.25)(0, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 2.25)(0, 2)(0.312579, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4.5)(0, 4.75)(0, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4.5)(0.312579, 4.75)(0, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 4.5)(1.25, 4.75)(0.93742, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4.5)(1.25, 4.75)(0.93742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5)(1.25, 4.75)(1.25, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4.75)(0.93742, 5)(0.93742, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4)(0, 4)(0, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.75)(0.312579, 4)(0, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3.75)(1.25, 4)(1.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4)(1.56258, 3.75)(1.56258, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 5.25)(9.68742, 5)(10, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 5)(10, 5.25)(9.68742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 5.25)(9.68742, 5)(9.68742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 5)(9.68742, 5)(9.37484, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 5)(9.06258, 5)(8.75, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5)(9.06258, 5.25)(8.75, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5.25)(9.06258, 5)(9.37484, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5)(9.37484, 5)(9.37484, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 5)(8.43742, 5)(8.43742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 5)(8.43742, 5.25)(8.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 0.25)(9.68742, 0)(10, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 0)(10, 0.25)(9.68742, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 0.5)(7.81248, 0.25)(7.81248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 0.25)(7.5, 0.5)(7.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 1.75)(7.5, 2)(7.18748, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2)(7.18748, 1.75)(7.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 9.25)(6.25, 9.5)(6.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 9.5)(6.56248, 9.25)(6.56248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9)(0, 9.25)(0, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9)(0.312579, 9.25)(0, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.75)(3.43752, 10)(3.43752, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 10)(3.75, 9.75)(3.75, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 9.25)(6.875, 9.5)(6.56248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9.5)(6.56248, 9.25)(6.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7.75)(0, 7.75)(0, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7.5)(0.312579, 7.75)(0, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7.75)(0, 8)(0, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 8)(0.312579, 7.75)(0.312579, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 7.25)(5, 7.25)(4.6875, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 7.5)(5, 7.25)(5, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7.25)(5.3125, 7.5)(5, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 7.5)(5, 7.25)(5.3125, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 7.75)(4.375, 7.75)(4.06252, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.75)(4.375, 8)(4.06252, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 9.5)(7.81248, 9.25)(7.81248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 9.25)(7.5, 9.5)(7.5, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 9.25)(6.875, 9.5)(6.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9.5)(7.18748, 9.25)(7.18748, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 9.5)(7.18748, 9.25)(7.5, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 9.25)(7.5, 9.5)(7.18748, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 9.5)(9.68742, 9.25)(10, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9.25)(10, 9.5)(9.68742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 9.75)(0.312579, 10)(0, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9.75)(0.312579, 10)(0, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 10)(0.312579, 9.75)(0.625159, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 10)(0.312579, 10)(0.625159, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9.5)(0, 9.75)(0, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9.5)(0.312579, 9.75)(0, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 9.25)(0.312579, 9.5)(0, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9.25)(0.312579, 9.5)(0, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 9.75)(2.5, 9.5)(2.81252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9.5)(2.81252, 9.75)(2.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 5)(2.18752, 4.75)(2.5, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 5)(2.5, 4.75)(2.5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4.75)(2.18752, 5)(1.875, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4.75)(2.18752, 5)(1.875, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 5.25)(0.312579, 5.5)(0, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5.25)(0.312579, 5.5)(0, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 5.25)(0.312579, 5.5)(0.312579, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5.5)(0.625159, 5.25)(0.625159, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 5.25)(0.93742, 5)(0.93742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 5.25)(0.625159, 5)(0.93742, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6.5)(0, 6.5)(0, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6.25)(0.312579, 6.5)(0, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.25)(8.125, 5)(8.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 5)(7.81248, 5.25)(7.81248, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 5.5)(7.81248, 5.25)(8.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.5)(7.81248, 5.25)(8.125, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 6.25)(6.56248, 6.5)(6.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6.5)(6.25, 6.25)(6.56248, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 5.75)(5.3125, 5.5)(5.3125, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 5.5)(5, 5.75)(5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 0.25)(5.3125, 0)(5.3125, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 0)(5, 0.25)(5, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 0.25)(4.6875, 0)(5, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0.25)(4.6875, 0)(5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 0)(4.6875, 0)(4.375, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0)(4.6875, 0.25)(4.375, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0.5)(5, 0.25)(5, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0.5)(4.6875, 0.25)(5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0.25)(4.06252, 0)(4.375, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0.25)(4.375, 0)(4.375, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0)(4.06252, 0.25)(3.75, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0.25)(3.75, 0.25)(3.75, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0.25)(3.75, 0.5)(3.75, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 0.5)(4.06252, 0.25)(4.06252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 0.25)(3.75, 0.5)(3.43752, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 0.5)(3.43752, 0.5)(3.43752, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 0)(2.81252, 0)(2.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 0)(2.81252, 0.25)(2.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 0)(3.125, 0.25)(3.125, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 0.25)(3.43752, 0)(3.43752, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 0.25)(2.81252, 0)(3.125, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 0)(3.125, 0.25)(2.81252, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 0.5)(3.125, 0.25)(3.43752, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 0.5)(3.125, 0.25)(3.43752, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 0.25)(3.125, 0.25)(2.81252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 0.25)(3.125, 0.5)(2.81252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0.5)(0, 0.75)(0, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0.5)(0.312579, 0.75)(0, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 0.25)(0.312579, 0.5)(0, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0.25)(0.312579, 0.5)(0, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1)(0.625159, 0.75)(0.93742, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 0.75)(0.93742, 1)(0.625159, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0.75)(0.625159, 0.75)(0.312579, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1)(0.625159, 0.75)(0.625159, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 0)(0.93742, 0.25)(0.625159, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 0)(0.93742, 0.25)(0.625159, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 0.25)(0.93742, 0)(1.25, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 0.25)(0.93742, 0.25)(1.25, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 0.5)(0.93742, 0.25)(1.25, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 0.25)(1.25, 0.25)(1.25, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1.25)(0.93742, 1)(1.25, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 1.25)(0.93742, 1.25)(1.25, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1.25)(0.625159, 1.25)(0.625159, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1)(0.93742, 1.25)(0.625159, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 1.5)(4.6875, 1.75)(4.6875, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1.75)(5, 1.5)(5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 2.5)(2.81252, 2.25)(2.81252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2.25)(2.5, 2.5)(2.5, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 2.25)(0.312579, 2.5)(0, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 2.25)(0.312579, 2.5)(0, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 2.5)(0, 2.75)(0, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 2.5)(0.312579, 2.75)(0, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 2.5)(0.625159, 2.5)(0.625159, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 2.75)(0.312579, 2.5)(0.625159, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 2.25)(1.56258, 2.25)(1.25, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2.25)(1.56258, 2.5)(1.25, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2.25)(1.875, 2.5)(1.56258, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 2.5)(1.56258, 2.25)(1.875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2.25)(1.56258, 2)(1.875, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 2.25)(1.56258, 2.25)(1.875, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 2.25)(1.25, 2.25)(1.25, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 2.5)(0.93742, 2.25)(1.25, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 4.25)(0.312579, 4.25)(0, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4.25)(0.312579, 4.5)(0, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4.25)(0, 4.25)(0, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4)(0.312579, 4.25)(0, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 4.75)(1.56258, 4.5)(1.875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4.75)(1.56258, 4.75)(1.875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 4.75)(1.25, 4.75)(1.25, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 4.5)(1.56258, 4.75)(1.25, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5)(1.56258, 4.75)(1.875, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 4.75)(1.875, 4.75)(1.875, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 4.75)(1.56258, 5)(1.25, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4.75)(1.56258, 4.75)(1.25, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 3.5)(1.56258, 3.75)(1.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3.75)(1.25, 3.5)(1.56258, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3.75)(1.25, 3.5)(1.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 3.5)(0.93742, 3.75)(0.93742, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 3.5)(0.93742, 3.75)(0.625159, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3.75)(0.625159, 3.5)(0.93742, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 3.5)(1.56258, 3.75)(1.56258, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3.75)(1.875, 3.5)(1.875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 3.5)(2.18752, 3.75)(1.875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3.75)(1.875, 3.5)(2.18752, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4.25)(1.25, 4)(1.56258, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 4.25)(1.25, 4.25)(1.56258, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4.25)(1.56258, 4.5)(1.25, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 4.5)(1.25, 4.25)(1.56258, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4.25)(1.25, 4.5)(0.93742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 4.25)(1.25, 4.25)(0.93742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4)(0.312579, 4)(0.312579, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4)(0.312579, 3.75)(0.625159, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.75)(4.06252, 3)(4.06252, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3)(4.375, 2.75)(4.375, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 4.5)(6.25, 4.75)(5.93748, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 4.75)(5.93748, 4.5)(6.25, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 4.5)(1.875, 4.25)(1.875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4.25)(1.56258, 4.5)(1.56258, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4.5)(2.18752, 4.75)(1.875, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4.5)(1.875, 4.75)(1.875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4.5)(2.5, 4.5)(2.5, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4.75)(2.18752, 4.5)(2.5, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4.25)(2.18752, 4.5)(1.875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4.5)(1.875, 4.25)(2.18752, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 4.5)(2.18752, 4.5)(2.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4.5)(2.18752, 4.25)(2.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4.5)(2.81252, 4.25)(3.125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 4.5)(2.81252, 4.25)(3.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4.25)(2.5, 4.5)(2.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4.25)(2.81252, 4.5)(2.5, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 0.75)(9.68742, 0.75)(10, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 0.75)(9.68742, 0.5)(10, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 0.75)(9.37484, 0.5)(9.68742, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 0.75)(9.37484, 0.75)(9.37484, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 1.25)(8.75, 1)(8.75, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 1)(8.43742, 1.25)(8.43742, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.25)(8.43742, 0)(8.75, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 0)(8.75, 0.25)(8.43742, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 0)(8.75, 0.25)(8.75, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.25)(9.06258, 0)(9.06258, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.25)(8.43742, 0.5)(8.43742, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 0.5)(8.75, 0.25)(8.75, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.5)(8.75, 0.25)(9.06258, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.25)(9.06258, 0.25)(9.06258, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 0.5)(9.37484, 0.25)(9.68742, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 0.5)(9.37484, 0.25)(9.68742, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 0.25)(9.37484, 0.25)(9.06258, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 0.25)(9.37484, 0.5)(9.06258, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 0.25)(9.68742, 0)(9.68742, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 0)(9.37484, 0.25)(9.37484, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 0.25)(9.06258, 0)(9.37484, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 0)(9.37484, 0.25)(9.06258, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 0)(8.125, 0.25)(8.125, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 0.25)(8.43742, 0)(8.43742, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 0.5)(8.125, 0.25)(8.43742, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 0.25)(8.43742, 0.5)(8.125, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 0.25)(8.125, 0.25)(7.81248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 0.5)(8.125, 0.25)(8.125, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 0)(7.81248, 0.25)(7.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 0)(7.81248, 0)(7.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 0.25)(7.81248, 0)(8.125, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 0)(8.125, 0.25)(7.81248, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 1)(9.06258, 1.25)(8.75, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.25)(8.75, 1)(9.06258, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 1.5)(9.68742, 1.25)(10, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1.5)(9.68742, 1.25)(10, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 1.25)(9.68742, 1.25)(9.37484, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1.25)(9.68742, 1.5)(9.37484, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 1.5)(8.43742, 1.25)(8.75, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 1.5)(8.43742, 1.5)(8.43742, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 2)(9.68742, 1.75)(10, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 2)(9.68742, 1.75)(10, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1.75)(10, 1.5)(10, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1.75)(9.68742, 1.5)(10, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1.5)(9.68742, 1.75)(9.37484, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1.75)(9.37484, 1.75)(9.37484, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 2.25)(10, 2)(10, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 2.25)(9.68742, 2)(10, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 2.25)(10, 2.25)(10, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 2.5)(9.68742, 2.25)(10, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.25)(8.75, 2)(8.75, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2)(8.43742, 2.25)(8.43742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 1.75)(6.56248, 2)(6.25, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1.75)(6.56248, 1.75)(6.25, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 10)(5.625, 9.75)(5.93748, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 10)(5.625, 10)(5.625, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 9.25)(4.375, 9.5)(4.06252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 9.5)(4.06252, 9.25)(4.375, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 10)(4.06252, 9.75)(4.375, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 10)(4.06252, 9.75)(4.375, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 9.75)(4.06252, 10)(3.75, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.75)(4.06252, 9.75)(3.75, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 9.5)(4.06252, 9.75)(4.06252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 9.75)(4.375, 9.5)(4.375, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 9.25)(4.375, 9)(4.375, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 9)(4.06252, 9.25)(4.06252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9)(4.6875, 8.75)(5, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 9)(4.6875, 8.75)(5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8.75)(5, 8.5)(5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8.75)(4.6875, 8.5)(5, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 9.5)(5.3125, 9.75)(5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 9.5)(5, 9.75)(5, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 9)(4.6875, 9.25)(4.375, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.25)(4.375, 9)(4.6875, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.25)(4.375, 9.5)(4.375, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 9.5)(4.6875, 9.25)(4.6875, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9)(3.43752, 9.25)(3.125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 9.25)(3.125, 9)(3.43752, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 10)(2.5, 10)(2.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 9.75)(2.81252, 10)(2.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9.75)(3.43752, 10)(3.125, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 10)(3.125, 9.75)(3.43752, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 10)(3.125, 9.75)(3.125, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9.75)(2.81252, 10)(2.81252, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9.75)(2.81252, 9.75)(2.81252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9.5)(3.125, 9.75)(2.81252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 9.75)(7.5, 9.5)(7.81248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 9.5)(7.81248, 9.75)(7.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8)(8.75, 7.75)(8.75, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 7.75)(8.43742, 8)(8.43742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 8.25)(8.43742, 8)(8.75, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8)(8.75, 8.25)(8.43742, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 8.75)(9.68742, 8.5)(10, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 8.75)(9.68742, 8.5)(10, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 8)(7.81248, 8.25)(7.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 8.25)(7.5, 8)(7.81248, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 8)(7.5, 8.25)(7.18748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 8)(7.5, 8)(7.18748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 8)(7.81248, 7.75)(7.81248, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 8)(7.5, 7.75)(7.81248, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 8)(7.18748, 8)(7.18748, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7.75)(7.5, 8)(7.18748, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.25)(6.56248, 8)(6.56248, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 8)(6.25, 8.25)(6.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 7.75)(6.56248, 8)(6.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.75)(6.56248, 8)(6.25, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 6.5)(6.25, 6.75)(5.93748, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 6.75)(5.93748, 6.5)(6.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 7.5)(1.25, 7.75)(1.25, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 7.75)(1.56258, 7.5)(1.56258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 8)(1.25, 7.75)(1.56258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 7.75)(1.56258, 8)(1.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.25)(5.93748, 8)(6.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 8)(6.25, 8.25)(5.93748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 8)(6.25, 7.75)(6.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 8)(5.93748, 7.75)(6.25, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7.75)(5.3125, 7.5)(5.3125, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 7.5)(5, 7.75)(5, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7.75)(4.6875, 7.5)(5, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7.75)(4.6875, 7.75)(4.6875, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.75)(2.5, 8)(2.18752, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 7.75)(2.5, 7.75)(2.18752, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.75)(2.81252, 8)(2.5, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8)(2.5, 7.75)(2.81252, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7.5)(3.43752, 7.75)(3.43752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 7.75)(3.75, 7.5)(3.75, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7.5)(4.06252, 7.75)(3.75, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7.5)(4.06252, 7.5)(4.06252, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 7.75)(4.375, 7.5)(4.6875, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.75)(4.375, 7.5)(4.6875, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.5)(4.375, 7.75)(4.06252, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 7.5)(4.375, 7.5)(4.06252, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.5)(4.6875, 7.25)(4.6875, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.5)(4.375, 7.25)(4.6875, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.5)(4.06252, 7.5)(4.06252, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.25)(4.375, 7.5)(4.06252, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.5)(2.5, 7.75)(2.18752, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.5)(2.18752, 7.75)(2.18752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.75)(2.5, 7.5)(2.81252, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.5)(2.81252, 7.5)(2.81252, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 7.5)(3.125, 7.75)(2.81252, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7.5)(3.125, 7.75)(2.81252, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 7.75)(3.125, 7.75)(3.43752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7.75)(3.125, 7.5)(3.43752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7.75)(2.81252, 8)(2.81252, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8)(3.125, 7.75)(3.125, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7.75)(3.43752, 8)(3.125, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8)(3.125, 7.75)(3.43752, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8.75)(3.75, 9)(3.43752, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8.75)(3.75, 9)(3.43752, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9)(4.06252, 8.75)(4.06252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9)(3.75, 8.75)(4.06252, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8)(2.81252, 8.25)(2.5, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 8)(2.81252, 8.25)(2.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.25)(2.81252, 8)(3.125, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 8.25)(2.81252, 8.25)(3.125, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8.75)(3.75, 8.5)(4.06252, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 8.75)(3.75, 8.5)(4.06252, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9.5)(7.81248, 9.75)(7.81248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 9.75)(8.125, 9.5)(8.125, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 8.5)(5.3125, 8.75)(5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8.5)(5.3125, 8.75)(5, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8.75)(5, 9)(5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8.75)(5.3125, 9)(5, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 9.75)(2.5, 9.5)(2.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9.5)(2.18752, 9.75)(2.18752, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 9.5)(2.18752, 9.75)(1.875, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 9.75)(1.875, 9.5)(2.18752, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9.75)(0.93742, 10)(0.625159, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9.75)(0.625159, 10)(0.625159, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 10)(0.93742, 9.75)(1.25, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9.75)(1.25, 9.75)(1.25, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9.75)(1.25, 9.5)(1.25, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 9.5)(0.93742, 9.75)(0.93742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 9.5)(0.93742, 9.5)(0.93742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 9.25)(1.25, 9.5)(0.93742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9.75)(1.875, 9.5)(1.875, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 9.5)(1.56258, 9.75)(1.56258, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 9.5)(1.56258, 9.75)(1.25, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9.75)(1.25, 9.5)(1.56258, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 9.25)(3.125, 9.5)(2.81252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9.5)(2.81252, 9.25)(3.125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9)(2.81252, 9.25)(2.81252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 9.25)(3.125, 9)(3.125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 5.5)(2.81252, 5.25)(2.81252, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 5.25)(2.5, 5.5)(2.5, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 5.25)(2.18752, 5)(2.5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 5.25)(2.18752, 5.25)(2.5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 5.25)(1.875, 5.25)(1.875, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 5)(2.18752, 5.25)(1.875, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 5.5)(2.18752, 5.25)(2.5, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 5.25)(2.5, 5.5)(2.18752, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 5.25)(1.875, 5.5)(1.875, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.5)(2.18752, 5.25)(2.18752, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5)(0, 5.25)(0, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5)(0.312579, 5.25)(0, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5)(0.625159, 5.25)(0.312579, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 5.25)(0.312579, 5)(0.625159, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 4.75)(0.312579, 5)(0, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4.75)(0.312579, 5)(0, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5)(0.625159, 4.75)(0.93742, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 5)(0.625159, 4.75)(0.93742, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5)(0.625159, 4.75)(0.625159, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.75)(0.312579, 5)(0.312579, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.75)(0.93742, 4.5)(0.93742, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.75)(0.625159, 4.5)(0.93742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4.5)(0.625159, 4.75)(0.312579, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.5)(0.625159, 4.75)(0.312579, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 5.25)(3.125, 5.5)(2.81252, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5.5)(2.81252, 5.25)(3.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 5.75)(4.6875, 5.5)(5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5.5)(5, 5.75)(4.6875, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 5.25)(0.93742, 5.5)(0.625159, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5.5)(0.625159, 5.25)(0.93742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 5.25)(0.93742, 5.5)(0.93742, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 5.5)(0.93742, 5.5)(1.25, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.25)(4.375, 7)(4.6875, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7)(4.6875, 7)(4.6875, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7)(4.6875, 6.75)(4.6875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6.75)(4.375, 7)(4.375, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6.75)(5, 7)(4.6875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7)(4.6875, 6.75)(5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7)(5, 7.25)(4.6875, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 7)(5, 7)(4.6875, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 6.75)(5, 6.5)(5.3125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 6.5)(5.3125, 6.75)(5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 6.25)(0.312579, 6.5)(0.312579, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6.5)(0.625159, 6.25)(0.625159, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 7.25)(0.312579, 7.25)(0, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7.25)(0.312579, 7.5)(0, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 7.75)(0.93742, 7.5)(1.25, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 7.5)(1.25, 7.75)(0.93742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 7.5)(0.93742, 7.25)(1.25, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 7.5)(0.93742, 7.25)(1.25, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 5.25)(7.81248, 5.25)(7.81248, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 5.25)(7.81248, 5.5)(7.5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5.25)(6.875, 5)(6.875, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 5)(6.56248, 5.25)(6.56248, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5.25)(6.875, 5.25)(6.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5.5)(6.56248, 5.25)(6.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 5.75)(4.6875, 5.5)(4.6875, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5.5)(4.375, 5.75)(4.375, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 5.75)(4.06252, 6)(4.06252, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6)(4.375, 5.75)(4.375, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5.5)(4.06252, 5.75)(3.75, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5.5)(3.75, 5.75)(3.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 5.75)(4.06252, 5.5)(4.375, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5.5)(4.375, 5.75)(4.06252, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 5.75)(3.43752, 5.75)(3.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5.75)(3.43752, 5.5)(3.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.25)(3.125, 6)(3.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 6)(2.81252, 6.25)(2.81252, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 6)(3.43752, 6.25)(3.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.25)(3.125, 6)(3.43752, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.75)(7.81248, 7)(7.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.75)(7.5, 7)(7.5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6.75)(8.75, 6.75)(8.75, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 7)(8.43742, 6.75)(8.75, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 5.5)(5.93748, 5.75)(5.93748, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 5.75)(6.25, 5.5)(6.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 5.5)(5.93748, 5.25)(6.25, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 5.5)(5.93748, 5.5)(5.93748, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 5.5)(6.56248, 5.25)(6.56248, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5.25)(6.25, 5.5)(6.25, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 5.5)(6.56248, 5.75)(6.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5.75)(6.25, 5.5)(6.56248, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5.75)(6.56248, 5.5)(6.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 5.75)(6.56248, 5.75)(6.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.75)(8.43742, 5.5)(8.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.75)(8.75, 5.5)(8.75, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.5)(8.43742, 5.75)(8.125, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.75)(8.125, 5.75)(8.125, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 5.75)(7.18748, 5.75)(7.5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.75)(7.18748, 5.5)(7.5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.75)(6.875, 5.75)(6.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.5)(7.18748, 5.75)(6.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 6)(5.93748, 5.75)(6.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 6)(5.93748, 6)(6.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6)(4.375, 5.75)(4.6875, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 5.75)(4.6875, 6)(4.375, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 5.75)(4.6875, 6)(4.6875, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6)(5, 5.75)(5, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6.5)(4.6875, 6.75)(4.375, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6.5)(4.375, 6.75)(4.375, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6.75)(4.6875, 6.5)(5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6.5)(5, 6.5)(5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.25)(5.3125, 0)(5.625, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 0)(5.625, 0.25)(5.3125, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 0)(5.625, 0.25)(5.625, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.25)(5.93748, 0)(5.93748, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.25)(5.3125, 0.5)(5.3125, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 0.5)(5.625, 0.25)(5.625, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.25)(5.93748, 0.5)(5.625, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.25)(5.93748, 0.25)(5.93748, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 0.25)(6.875, 0.25)(6.875, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 0.25)(6.875, 0.5)(6.56248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 0.5)(7.18748, 0.25)(7.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 0.25)(7.5, 0.5)(7.18748, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0.25)(7.18748, 0.25)(6.875, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0.5)(7.18748, 0.25)(7.18748, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 0.5)(4.06252, 0.25)(4.375, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0.25)(4.375, 0.5)(4.06252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0.25)(4.375, 0.5)(4.375, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0.5)(4.375, 0.5)(4.6875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1.25)(5, 1.5)(4.6875, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 1.5)(4.6875, 1.25)(5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.5)(4.06252, 1.75)(3.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.5)(3.75, 1.75)(3.75, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 0.5)(5.3125, 0.75)(5, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 0.75)(5, 0.75)(5, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0.75)(4.375, 0.5)(4.6875, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 0.5)(4.6875, 0.75)(4.375, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0.75)(4.6875, 0.5)(5, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 0.75)(4.6875, 0.75)(5, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 0.75)(2.18752, 1)(2.18752, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1)(2.5, 0.75)(2.5, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1)(2.5, 1)(2.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1.25)(2.18752, 1)(2.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1)(2.18752, 1.25)(1.875, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 1)(2.18752, 1)(1.875, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 1)(5.3125, 1)(5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1)(5.3125, 1.25)(5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 0.75)(5.3125, 1)(5, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 0.75)(5.3125, 1)(5, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 0.5)(3.125, 0.75)(2.81252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 0.75)(2.81252, 0.75)(2.81252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 0.5)(4.06252, 0.75)(4.06252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0.75)(4.375, 0.5)(4.375, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0.75)(3.75, 0.5)(4.06252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 0.5)(4.06252, 0.75)(3.75, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 1)(4.06252, 0.75)(4.375, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1)(4.06252, 0.75)(4.375, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 0.75)(4.06252, 0.75)(3.75, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 0.75)(4.06252, 1)(3.75, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 0.5)(0.93742, 0.5)(0.93742, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 0.75)(0.625159, 0.5)(0.93742, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 0.5)(0.625159, 0.5)(0.312579, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 0.5)(0.625159, 0.75)(0.312579, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 0.25)(0.625159, 0.5)(0.625159, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 0.5)(0.93742, 0.25)(0.93742, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 0.5)(0.312579, 0.25)(0.625159, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 0.5)(0.312579, 0.5)(0.312579, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 0.25)(2.5, 0.5)(2.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 0.5)(2.81252, 0.25)(2.81252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 0.5)(2.18752, 0.25)(2.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 0.25)(2.5, 0.5)(2.18752, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 0.75)(2.5, 0.5)(2.81252, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 0.75)(2.5, 0.5)(2.81252, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 0.5)(2.5, 0.75)(2.18752, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 0.5)(2.5, 0.5)(2.18752, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 0)(2.5, 0)(2.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 0.25)(2.18752, 0)(2.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0)(2.18752, 0)(1.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 0)(2.18752, 0.25)(1.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0)(1.25, 0.25)(1.25, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0)(1.56258, 0.25)(1.25, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0)(1.875, 0)(1.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0.25)(1.56258, 0)(1.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1.5)(1.25, 1.5)(1.25, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1.25)(1.56258, 1.5)(1.25, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2.25)(2.18752, 2)(2.5, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2.25)(2.5, 2)(2.5, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2.25)(1.875, 2.25)(1.875, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2)(2.18752, 2.25)(1.875, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 2.5)(2.18752, 2.25)(2.5, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2.25)(2.5, 2.5)(2.18752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2.25)(1.875, 2.5)(1.875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 2.5)(2.18752, 2.25)(2.18752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 2)(1.56258, 2.25)(1.25, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2.25)(1.25, 2)(1.56258, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 2.25)(1.25, 2)(1.25, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 2)(0.93742, 2.25)(0.93742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 2)(0.93742, 1.75)(1.25, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 2)(0.93742, 2)(0.93742, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1.5)(5, 1.5)(5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1.25)(5.3125, 1.5)(5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 1.75)(6.25, 1.75)(6.25, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 2)(5.93748, 1.75)(6.25, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.75)(4.06252, 2)(3.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 1.75)(4.06252, 2)(3.75, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 2)(4.375, 1.75)(4.375, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 2)(4.06252, 1.75)(4.375, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.25)(8.125, 2)(8.43742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 2.25)(8.125, 2)(8.43742, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 2)(8.125, 2)(7.81248, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 2)(8.125, 2.25)(7.81248, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 2.75)(5.93748, 2.5)(5.93748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 2.5)(5.625, 2.75)(5.625, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 2.75)(5.3125, 2.5)(5.625, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 2.75)(5.3125, 2.75)(5.3125, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 3)(8.43742, 3.25)(8.43742, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.25)(8.75, 3)(8.75, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 2.75)(0.312579, 3)(0, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 2.75)(0.312579, 3)(0, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 3)(0.312579, 3)(0.625159, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3)(0.312579, 2.75)(0.625159, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.75)(3.125, 2.5)(3.43752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.75)(3.43752, 2.5)(3.43752, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2.75)(1.875, 2.5)(2.18752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 2.5)(2.18752, 2.75)(1.875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 2.5)(2.18752, 2.75)(2.18752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 2.75)(2.18752, 2.75)(2.5, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 2.5)(0.93742, 2.75)(0.625159, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 2.5)(0.93742, 2.75)(0.625159, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 2.75)(0.93742, 2.5)(1.25, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 2.75)(0.93742, 2.75)(1.25, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 2.5)(1.56258, 2.75)(1.56258, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2.75)(1.875, 2.5)(1.875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2.5)(1.56258, 2.75)(1.25, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2.75)(1.25, 2.75)(1.25, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 2.5)(3.75, 2.75)(3.43752, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.5)(3.75, 2.75)(3.43752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 2.75)(3.75, 2.75)(4.06252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.75)(3.75, 2.5)(4.06252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.75)(3.43752, 3)(3.43752, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 3)(3.75, 2.75)(3.75, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3)(3.75, 2.75)(4.06252, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.75)(4.06252, 3)(3.75, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1.75)(2.81252, 2)(2.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2)(2.5, 2)(2.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2)(2.81252, 2)(3.125, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2)(2.81252, 1.75)(3.125, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2)(2.81252, 2.25)(2.5, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 2)(2.81252, 2)(2.5, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.25)(0.93742, 4.25)(0.93742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.5)(0.625159, 4.25)(0.93742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 4.25)(0.625159, 4.25)(0.312579, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.25)(0.625159, 4.5)(0.312579, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.25)(0.312579, 4.25)(0.312579, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4)(0.625159, 4.25)(0.312579, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 5)(2.81252, 5.25)(2.5, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 5)(2.5, 5.25)(2.5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 5.25)(2.81252, 5)(3.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 5)(3.125, 5)(3.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4)(2.18752, 3.75)(2.5, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 4)(2.18752, 4)(2.5, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4.25)(2.18752, 4)(2.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4)(2.5, 4)(2.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 3.5)(1.56258, 3.25)(1.56258, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3.25)(1.25, 3.5)(1.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 3.5)(2.18752, 3.75)(2.18752, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3.75)(2.5, 3.5)(2.5, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3.25)(1.25, 3.5)(0.93742, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 3.5)(0.93742, 3.25)(1.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 3.5)(0.93742, 3.25)(0.93742, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 3.25)(0.93742, 3.25)(0.625159, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4.25)(0.93742, 4)(1.25, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 4)(1.25, 4.25)(0.93742, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 4.25)(0.93742, 4)(0.93742, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 4)(0.625159, 4.25)(0.625159, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 4)(0.93742, 4)(1.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 4)(0.93742, 3.75)(1.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3.75)(0.93742, 4)(0.625159, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 4)(0.625159, 4)(0.625159, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 3)(3.125, 2.75)(3.43752, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 3)(3.125, 3)(3.43752, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 3.25)(3.125, 3)(3.43752, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 3)(3.43752, 3.25)(3.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.75)(4.6875, 3)(4.375, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3)(4.375, 2.75)(4.6875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 2.75)(4.6875, 3)(4.6875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3)(5, 2.75)(5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 2.75)(5, 2.75)(5.3125, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 2.5)(5, 2.75)(5, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 2.75)(5.3125, 3)(5.3125, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 3)(5.625, 2.75)(5.625, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 2.75)(5.3125, 3)(5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 3)(5, 2.75)(5.3125, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 3.25)(6.25, 3)(6.56248, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 3)(6.56248, 3.25)(6.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 4.5)(9.68742, 4.25)(10, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 4.25)(10, 4.5)(9.68742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 4.25)(10, 4)(10, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 4)(9.68742, 4.25)(9.68742, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 3.75)(10, 4)(9.68742, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 4)(9.68742, 4)(9.68742, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 4.25)(7.18748, 4.5)(7.18748, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4.5)(7.5, 4.25)(7.5, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 4.5)(6.25, 4.75)(6.25, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 4.75)(6.56248, 4.5)(6.56248, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 4.5)(6.25, 4.5)(6.25, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 4.25)(6.56248, 4.5)(6.25, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4.25)(3.125, 4.5)(3.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4.25)(3.43752, 4.5)(3.125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 3.5)(10, 3.75)(9.68742, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3.5)(10, 3.5)(9.68742, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 3.75)(4.6875, 3.5)(4.6875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3.5)(4.375, 3.75)(4.375, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 3.25)(6.25, 3.5)(6.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 3.5)(6.56248, 3.25)(6.56248, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 3.5)(5.93748, 3.25)(6.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 3.5)(5.93748, 3.5)(5.93748, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3.5)(5, 3.75)(4.6875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 3.75)(4.6875, 3.5)(5, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 3.75)(5, 3.5)(5.3125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 3.75)(5, 3.75)(5.3125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.75)(6.875, 5)(6.56248, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.75)(6.56248, 5)(6.56248, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.25)(7.5, 5)(7.81248, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 5.25)(7.5, 5)(7.81248, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 5.25)(5.3125, 5.5)(5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 5.25)(5.3125, 5.25)(5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 5.25)(5, 5.25)(5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 5)(5.3125, 5.25)(5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.75)(5.625, 5)(5.3125, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 4.75)(5.625, 4.75)(5.3125, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.75)(5.93748, 4.75)(5.93748, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5)(5.625, 4.75)(5.93748, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.75)(5, 4.5)(5.3125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.75)(5.3125, 4.5)(5.3125, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.75)(4.6875, 4.75)(4.6875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.5)(5, 4.75)(4.6875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.75)(5.3125, 5)(5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.75)(5.3125, 4.75)(5.3125, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5)(5, 4.75)(5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.75)(4.6875, 5)(4.6875, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.25)(5, 4.5)(4.6875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 4.25)(5, 4.25)(4.6875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.5)(5, 4.25)(5.3125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.25)(5.3125, 4.25)(5.3125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 5)(6.25, 4.75)(6.56248, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5)(6.25, 5)(6.56248, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 4.75)(6.25, 5)(5.93748, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 4.75)(6.25, 5)(5.93748, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5.25)(6.25, 5)(6.56248, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 5)(6.56248, 5.25)(6.25, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 5.25)(6.25, 5)(6.25, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 5)(6.25, 5)(5.93748, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 4.5)(5.93748, 4.25)(6.25, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 4.5)(5.93748, 4.25)(6.25, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 4.5)(2.81252, 4.75)(2.5, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4.5)(2.81252, 4.75)(2.5, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4.75)(2.81252, 4.5)(3.125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 4.75)(2.81252, 4.75)(3.125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 4.75)(2.81252, 4.75)(2.5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4.75)(2.81252, 5)(2.5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 5)(2.81252, 4.75)(3.125, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5)(2.81252, 4.75)(3.125, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4.25)(2.81252, 4)(3.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4)(3.125, 4)(3.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4)(2.81252, 4.25)(2.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 4)(2.81252, 4)(2.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 1)(9.68742, 1)(10, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1)(9.68742, 0.75)(10, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1)(10, 1)(10, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1.25)(9.68742, 1)(10, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 0.75)(5.93748, 0.5)(6.25, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 0.5)(6.25, 0.75)(5.93748, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 0.75)(6.25, 0.5)(6.56248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 0.75)(6.25, 0.75)(6.56248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 0.75)(7.81248, 0.5)(8.125, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 0.75)(7.81248, 0.75)(7.81248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.5)(9.37484, 1.25)(9.37484, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.5)(9.06258, 1.25)(9.37484, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.25)(9.06258, 1.5)(8.75, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.5)(8.75, 1.5)(8.75, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 1.75)(9.06258, 1.5)(9.37484, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.75)(9.06258, 1.5)(9.37484, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.5)(9.06258, 1.75)(8.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 1.5)(9.06258, 1.5)(8.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 1.5)(8.125, 1.25)(8.43742, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 1.5)(8.125, 1.25)(8.43742, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 2.25)(9.37484, 2.25)(9.06258, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2.25)(9.37484, 2.5)(9.06258, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2.25)(9.68742, 2.25)(9.68742, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2.5)(9.37484, 2.25)(9.68742, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.75)(9.06258, 2)(8.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 2)(8.75, 2)(8.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2)(9.06258, 2)(8.75, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 2)(9.06258, 2.25)(8.75, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 9.75)(5.3125, 10)(5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 9.75)(5.3125, 10)(5, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 10)(5.3125, 10)(5.625, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 10)(5.3125, 9.75)(5.625, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.75)(4.6875, 10)(4.375, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.75)(4.375, 10)(4.375, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 10)(4.6875, 9.75)(5, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.75)(5, 9.75)(5, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 9.5)(4.6875, 9.75)(4.375, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.75)(4.375, 9.5)(4.6875, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 9.75)(4.6875, 9.75)(5, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.75)(4.6875, 9.5)(5, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 10)(6.25, 9.75)(6.25, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 9.75)(5.93748, 10)(5.93748, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 9.75)(6.56248, 10)(6.25, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 10)(6.25, 9.75)(6.56248, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 9.5)(6.25, 9.75)(5.93748, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 9.5)(6.25, 9.75)(5.93748, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 9.75)(6.25, 9.5)(6.56248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 9.75)(6.25, 9.75)(6.56248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 10)(7.18748, 9.75)(7.5, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 10)(7.18748, 9.75)(7.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 9.5)(7.18748, 9.75)(7.18748, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 9.75)(7.5, 9.5)(7.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 9.5)(5.93748, 9.25)(6.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 9.25)(6.25, 9.5)(5.93748, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 9)(5, 9.25)(5, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 9.25)(5.3125, 9)(5.3125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 9.25)(4.6875, 9)(5, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 9.25)(4.6875, 9.25)(4.6875, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 9.25)(5.3125, 9.5)(5, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 9.5)(5, 9.25)(5.3125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.25)(5, 9.25)(4.6875, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 9.5)(5, 9.25)(5, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 8.75)(3.43752, 8.75)(3.43752, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9)(3.125, 8.75)(3.43752, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9.25)(1.875, 9.5)(1.56258, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 9.5)(1.56258, 9.25)(1.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9.25)(1.25, 9.5)(1.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 9.5)(1.56258, 9.25)(1.56258, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 9.25)(3.43752, 9.5)(3.125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 9.5)(3.125, 9.5)(3.125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 9.5)(3.125, 9.75)(3.125, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 9.75)(3.43752, 9.5)(3.43752, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 9.75)(7.81248, 10)(7.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 10)(7.5, 10)(7.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 10)(7.81248, 9.75)(8.125, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 10)(7.81248, 10)(8.125, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 9.75)(8.43742, 10)(8.125, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 9.75)(8.125, 10)(8.125, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 10)(8.43742, 9.75)(8.75, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 9.75)(8.75, 9.75)(8.75, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9.5)(8.43742, 9.75)(8.125, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 9.75)(8.125, 9.5)(8.43742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9.5)(8.43742, 9.75)(8.43742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 9.75)(8.75, 9.5)(8.75, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8)(8.125, 7.75)(8.43742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 8)(8.125, 7.75)(8.43742, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 7.75)(8.125, 7.75)(7.81248, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 7.75)(8.125, 8)(7.81248, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 7.75)(9.68742, 7.75)(10, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7.75)(9.68742, 7.5)(10, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7.75)(10, 7.75)(10, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 8)(9.68742, 7.75)(10, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 8.25)(9.68742, 8.25)(10, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 8.25)(9.68742, 8)(10, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 8.25)(10, 8.25)(10, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 8.5)(9.68742, 8.25)(10, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 7.75)(9.06258, 8)(8.75, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8)(8.75, 7.75)(9.06258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 8.5)(9.68742, 8.25)(9.68742, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 8.25)(9.37484, 8.5)(9.37484, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 8.5)(9.68742, 8.5)(9.68742, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 8.75)(9.37484, 8.5)(9.68742, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 8.25)(8.43742, 8)(8.43742, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 8.25)(8.125, 8)(8.43742, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 8.25)(7.81248, 8.25)(7.81248, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 8)(8.125, 8.25)(7.81248, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 8.5)(7.5, 8.5)(7.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 8.75)(7.18748, 8.5)(7.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 8.25)(7.18748, 8.5)(7.18748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 8.5)(7.18748, 8.5)(7.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 6.5)(9.68742, 6.5)(10, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 6.25)(9.68742, 6.5)(9.68742, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7.75)(0.625159, 8)(0.312579, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 7.75)(0.625159, 8)(0.312579, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 7.75)(1.875, 7.5)(2.18752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 7.75)(1.875, 7.5)(2.18752, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 7.5)(1.875, 7.5)(1.56258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 7.5)(1.875, 7.75)(1.56258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8)(2.18752, 7.75)(2.18752, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8)(1.875, 7.75)(2.18752, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8)(1.56258, 8)(1.56258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 7.75)(1.875, 8)(1.56258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 7.5)(5.625, 7.75)(5.3125, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.5)(5.625, 7.75)(5.3125, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 7.75)(5.625, 7.75)(5.93748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.75)(5.625, 7.5)(5.93748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8)(5.93748, 8)(5.93748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8.25)(5.625, 8)(5.93748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.75)(5.625, 8)(5.3125, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8)(5.3125, 8)(5.3125, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 8)(5.625, 8)(5.93748, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8)(5.625, 7.75)(5.93748, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 8)(5, 7.75)(5.3125, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8)(5, 8)(5.3125, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8.25)(5.625, 8)(5.625, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8)(5.3125, 8.25)(5.3125, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8.25)(5, 8)(5.3125, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 8)(5.3125, 8.25)(5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8.25)(5.3125, 8.5)(5, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 8.25)(5.3125, 8.25)(5, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8.5)(4.6875, 8.25)(5, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8.25)(5, 8.25)(5, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8)(3.43752, 8.25)(3.125, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8.25)(3.125, 8.25)(3.125, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8)(4.06252, 7.75)(4.06252, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 7.75)(3.75, 8)(3.75, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8)(3.43752, 7.75)(3.75, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8)(3.43752, 8)(3.43752, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 7)(1.25, 7)(1.25, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6.75)(1.56258, 7)(1.25, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7.5)(3.75, 7.25)(4.06252, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 7.5)(3.75, 7.25)(4.06252, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7.25)(3.75, 7.5)(3.43752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 7.25)(3.75, 7.25)(3.43752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 8.75)(3.43752, 8.5)(3.43752, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8.5)(3.125, 8.75)(3.125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8.5)(3.75, 8.75)(3.43752, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8.5)(3.75, 8.5)(3.75, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8.25)(3.43752, 8.5)(3.125, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8.5)(3.125, 8.5)(3.125, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.75)(4.06252, 8.75)(4.06252, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.5)(4.375, 8.75)(4.06252, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8.75)(4.375, 8.75)(4.6875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.75)(4.375, 8.5)(4.6875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.75)(4.375, 9)(4.06252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 8.75)(4.375, 8.75)(4.06252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.75)(4.6875, 8.75)(4.6875, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 9)(4.375, 8.75)(4.6875, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9.5)(8.125, 9.25)(8.43742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 9.5)(8.125, 9.25)(8.43742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 9.25)(8.125, 9.25)(7.81248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9.25)(8.125, 9.5)(7.81248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9.25)(8.75, 9.5)(8.43742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9.25)(8.43742, 9.5)(8.43742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 9.5)(8.75, 9.25)(9.06258, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9.5)(8.75, 9.25)(9.06258, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9.5)(9.68742, 9.25)(9.68742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9.5)(9.37484, 9.25)(9.68742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9.25)(9.37484, 9.5)(9.06258, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9.5)(9.06258, 9.5)(9.06258, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 8.5)(9.06258, 8.75)(8.75, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8.75)(8.75, 8.5)(9.06258, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8.75)(9.37484, 8.5)(9.37484, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 8.5)(9.06258, 8.75)(9.06258, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 9)(9.68742, 9)(10, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9)(9.68742, 8.75)(10, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9)(10, 9)(10, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9.25)(9.68742, 9)(10, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8.5)(8.125, 8.25)(8.43742, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 8.25)(8.43742, 8.5)(8.125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 8.25)(8.43742, 8.5)(8.43742, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 8.5)(8.43742, 8.5)(8.75, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8.5)(5.625, 8.25)(5.93748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 8.5)(5.625, 8.5)(5.93748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8.5)(5.3125, 8.25)(5.625, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8.25)(5.625, 8.5)(5.3125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.25)(6.25, 8.5)(5.93748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.5)(5.93748, 8.5)(5.93748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.5)(6.25, 8.25)(6.56248, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 8.5)(6.25, 8.5)(6.56248, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 10)(2.18752, 10)(2.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 10)(2.18752, 9.75)(2.5, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 9.75)(2.18752, 10)(1.875, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 10)(1.875, 10)(1.875, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 9.75)(1.56258, 10)(1.25, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9.75)(1.56258, 10)(1.25, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 10)(1.56258, 9.75)(1.875, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 10)(1.56258, 10)(1.875, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9.5)(0.625159, 9.5)(0.93742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 9.5)(0.625159, 9.25)(0.93742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 9.5)(0.312579, 9.5)(0.312579, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 9.25)(0.625159, 9.5)(0.312579, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 9.5)(0.93742, 9.75)(0.625159, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9.75)(0.625159, 9.5)(0.93742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9.75)(0.625159, 9.5)(0.625159, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9.5)(0.625159, 9.5)(0.312579, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 9.5)(2.18752, 9.25)(2.18752, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 9.25)(1.875, 9.5)(1.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 5.75)(2.5, 5.5)(2.81252, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 5.75)(2.5, 5.75)(2.81252, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 5.5)(2.5, 5.75)(2.18752, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 5.5)(2.5, 5.75)(2.18752, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5.5)(1.25, 5.25)(1.56258, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5.5)(1.25, 5.5)(1.25, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.25)(1.56258, 5.5)(1.56258, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.5)(1.56258, 5.5)(1.875, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6)(0.93742, 5.75)(1.25, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 6)(0.93742, 5.75)(1.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 5.75)(0.93742, 5.75)(0.625159, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5.75)(0.93742, 6)(0.625159, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5.75)(0.93742, 5.5)(1.25, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5.75)(1.25, 5.5)(1.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5.5)(0.93742, 5.75)(0.625159, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 5.75)(0.625159, 5.75)(0.625159, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 6)(0.312579, 6)(0, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6)(0.312579, 6.25)(0, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6)(0.625159, 6.25)(0.312579, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 6.25)(0.312579, 6)(0.625159, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5.25)(4.6875, 5.5)(4.375, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5.25)(4.375, 5.5)(4.375, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5.5)(4.6875, 5.25)(5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5.25)(5, 5.25)(5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5.25)(4.375, 5.25)(4.375, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5)(4.6875, 5.25)(4.375, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 5.25)(4.6875, 5.25)(5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5.25)(4.6875, 5)(5, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.75)(5.93748, 6.5)(5.93748, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.75)(5.625, 6.5)(5.93748, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.75)(5.3125, 6.75)(5.3125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.5)(5.625, 6.75)(5.3125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.75)(5.3125, 7)(5.3125, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 7)(5.625, 6.75)(5.625, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 7)(5, 7)(5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 6.75)(5.3125, 7)(5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7.25)(5.3125, 7)(5.3125, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7)(5.3125, 7)(5, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6)(1.56258, 6.25)(1.25, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6)(1.25, 6.25)(1.25, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6.25)(1.56258, 6)(1.875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6)(1.875, 6)(1.875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.25)(0.93742, 6)(1.25, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 6.25)(0.93742, 6.25)(1.25, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6)(0.93742, 6.25)(0.625159, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.25)(0.625159, 6.25)(0.625159, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.25)(1.25, 6.25)(1.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.5)(0.93742, 6.25)(1.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 6.25)(0.93742, 6.25)(0.625159, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.25)(0.93742, 6.5)(0.625159, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7)(0, 7.25)(0, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7)(0.312579, 7.25)(0, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7)(0.625159, 7)(0.625159, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7.25)(0.312579, 7)(0.625159, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7.25)(0.625159, 7.5)(0.312579, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 7.5)(0.312579, 7.25)(0.625159, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 7.5)(0.93742, 7.25)(0.93742, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 7.25)(0.625159, 7.5)(0.625159, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 7.5)(0.312579, 7.75)(0.312579, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 7.5)(0.625159, 7.75)(0.312579, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 7.5)(0.93742, 7.5)(0.93742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 7.75)(0.625159, 7.5)(0.93742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6.25)(1.56258, 6.5)(1.25, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 6.25)(1.56258, 6.5)(1.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6.5)(1.56258, 6.75)(1.25, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6.5)(1.25, 6.75)(1.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.75)(0.93742, 6.5)(1.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 6.75)(0.93742, 6.75)(1.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.5)(0.93742, 6.75)(0.625159, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.75)(0.625159, 6.75)(0.625159, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 7.25)(0.93742, 7)(1.25, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 7)(1.25, 7)(1.25, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 7)(0.93742, 7)(0.625159, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 7)(0.93742, 7.25)(0.625159, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 7)(0.93742, 7)(1.25, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 7)(0.93742, 6.75)(1.25, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 6.75)(0.93742, 7)(0.625159, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 6.75)(0.93742, 7)(0.625159, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6)(10, 6)(10, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6)(10, 6.25)(9.68742, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5.5)(9.06258, 5.75)(8.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 5.5)(9.06258, 5.75)(8.75, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 5)(7.18748, 5.25)(6.875, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.25)(6.875, 5)(7.18748, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.25)(7.5, 5)(7.5, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 5)(7.18748, 5.25)(7.18748, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 5.25)(7.18748, 5.25)(6.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.25)(7.18748, 5.5)(6.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.25)(7.5, 5.25)(7.5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.5)(7.18748, 5.25)(7.5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 6)(3.43752, 5.75)(3.75, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5.75)(3.75, 6)(3.43752, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6)(3.75, 6)(4.06252, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5.75)(3.75, 6)(3.75, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 6)(3.43752, 6.25)(3.43752, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.25)(3.75, 6)(3.75, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 6)(4.06252, 6.25)(3.75, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6.25)(3.75, 6)(4.06252, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5.5)(4.06252, 5.25)(4.375, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 5.5)(4.06252, 5.25)(4.375, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5.25)(4.06252, 5.5)(3.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 5.25)(4.06252, 5.25)(3.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 5.25)(4.06252, 5.25)(4.375, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5.25)(4.06252, 5)(4.375, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5.25)(3.75, 5.25)(3.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5)(4.06252, 5.25)(3.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5.5)(3.125, 5.75)(2.81252, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5.75)(2.81252, 5.75)(2.81252, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5.75)(3.125, 5.75)(3.43752, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5.75)(3.125, 5.5)(3.43752, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5.75)(3.125, 6)(2.81252, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5.75)(2.81252, 6)(2.81252, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 6)(3.125, 5.75)(3.43752, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5.75)(3.43752, 5.75)(3.43752, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.25)(3.43752, 6.5)(3.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.5)(3.125, 6.5)(3.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.5)(3.43752, 6.25)(3.75, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 6.5)(3.43752, 6.5)(3.75, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6.5)(6.56248, 6.75)(6.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6.75)(6.25, 6.75)(6.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 6.75)(6.56248, 6.75)(6.25, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6.75)(6.56248, 7)(6.25, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.5)(7.81248, 6.75)(7.5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 6.5)(7.81248, 6.5)(7.5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6.75)(8.75, 6.5)(8.75, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6.5)(8.75, 6.5)(8.43742, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 6.25)(7.5, 6.25)(7.5, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 6.25)(7.5, 6.5)(7.18748, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 5.5)(5.625, 5.75)(5.3125, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.5)(5.625, 5.75)(5.3125, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 5.75)(5.625, 5.75)(5.93748, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.75)(5.625, 5.5)(5.93748, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 6)(5.625, 5.75)(5.93748, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.75)(5.93748, 6)(5.625, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6)(6.56248, 5.75)(6.875, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6)(6.875, 5.75)(6.875, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 5.75)(6.56248, 6)(6.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6)(6.25, 6)(6.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 6.25)(6.56248, 6)(6.56248, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6)(6.25, 6.25)(6.25, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.75)(7.81248, 6)(7.5, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.75)(7.5, 6)(7.5, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.75)(8.125, 5.75)(8.125, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6)(7.81248, 5.75)(8.125, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.5)(7.81248, 5.75)(7.5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.75)(7.5, 5.75)(7.5, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 5.75)(7.81248, 5.5)(8.125, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 5.75)(7.81248, 5.75)(8.125, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.75)(5.3125, 6)(5.3125, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 6)(5.625, 5.75)(5.625, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 6)(5, 5.75)(5.3125, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 5.75)(5.3125, 6)(5, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 6.25)(4.6875, 6)(5, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6)(5, 6.25)(4.6875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 6)(5, 6.25)(5, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 6.25)(5.3125, 6)(5.3125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6.5)(5, 6.25)(5, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 6.25)(4.6875, 6.5)(4.6875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 6.5)(5, 6.25)(5.3125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 6.25)(5.3125, 6.25)(5.3125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.25)(5.3125, 6)(5.625, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 6)(5.625, 6.25)(5.3125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.25)(5.625, 6.5)(5.3125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 6.25)(5.625, 6.25)(5.3125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 6.25)(4.6875, 6.5)(4.375, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6.5)(4.375, 6.25)(4.6875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 6)(4.375, 6.25)(4.375, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 6.25)(4.6875, 6)(4.6875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 6.25)(4.06252, 6)(4.375, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 6.25)(4.06252, 6.25)(4.06252, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6.5)(4.375, 6.25)(4.375, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 6.25)(4.06252, 6.5)(4.06252, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6.25)(4.06252, 6.5)(3.75, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6.5)(3.75, 6.5)(3.75, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 0.25)(5.93748, 0)(6.25, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 0)(6.25, 0.25)(5.93748, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 0.25)(6.25, 0.25)(5.93748, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 0.5)(6.25, 0.25)(6.25, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 0.25)(6.56248, 0.25)(6.56248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 0.5)(6.25, 0.25)(6.56248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 0)(6.25, 0.25)(6.25, 0)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 0.25)(6.56248, 0)(6.56248, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 0.25)(6.56248, 0)(6.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 0)(6.875, 0)(6.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 0)(7.5, 0)(7.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 0.25)(7.18748, 0)(7.5, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 0)(7.18748, 0.25)(6.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0)(7.18748, 0)(6.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 1.5)(4.6875, 1.25)(4.6875, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1.25)(4.375, 1.5)(4.375, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1.75)(4.375, 1.5)(4.6875, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 1.5)(4.6875, 1.75)(4.375, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.5)(4.375, 1.5)(4.06252, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.75)(4.375, 1.5)(4.375, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 0.5)(5.625, 0.75)(5.625, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.75)(5.93748, 0.5)(5.93748, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.75)(5.3125, 0.5)(5.625, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.75)(5.3125, 0.75)(5.3125, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1)(4.6875, 0.75)(5, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1)(5, 0.75)(5, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 0.75)(4.6875, 1)(4.375, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1)(4.375, 1)(4.375, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1.25)(4.6875, 1)(5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1)(5, 1)(5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1)(4.6875, 1.25)(4.375, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 1)(4.6875, 1)(4.375, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 0.75)(1.56258, 1)(1.25, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0.75)(1.56258, 1)(1.25, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1)(1.25, 1.25)(1.25, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1)(1.56258, 1.25)(1.25, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1)(1.875, 1)(1.875, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1.25)(1.56258, 1)(1.875, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1)(1.875, 0.75)(2.18752, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0.75)(2.18752, 1)(1.875, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0.75)(1.56258, 1)(1.56258, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1)(1.875, 0.75)(1.875, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0.5)(1.25, 0.75)(1.25, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0.5)(1.56258, 0.75)(1.25, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 0.25)(1.56258, 0.5)(1.25, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0.25)(1.56258, 0.5)(1.25, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 1)(2.81252, 1)(2.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1)(2.81252, 1.25)(2.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1)(3.125, 1)(3.125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1.25)(2.81252, 1)(3.125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 0.75)(2.81252, 1)(2.5, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1)(2.5, 0.75)(2.81252, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 0.75)(2.81252, 1)(2.81252, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1)(3.125, 0.75)(3.125, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1)(5.625, 0.75)(5.93748, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 1)(5.625, 1)(5.93748, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1)(5.3125, 1)(5.3125, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 0.75)(5.625, 1)(5.3125, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1)(4.06252, 1.25)(3.75, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.25)(3.75, 1.25)(3.75, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.25)(4.06252, 1)(4.375, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.25)(4.375, 1)(4.375, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.25)(4.06252, 1.5)(3.75, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 1.25)(4.06252, 1.25)(3.75, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 1.5)(4.06252, 1.25)(4.375, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 1.25)(4.375, 1.5)(4.06252, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 0.5)(3.43752, 0.75)(3.43752, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 0.75)(3.75, 0.5)(3.75, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 0.75)(3.125, 0.5)(3.43752, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 0.75)(3.125, 0.75)(3.125, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1.5)(1.56258, 1.75)(1.25, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 1.5)(1.56258, 1.75)(1.25, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 2)(1.56258, 1.75)(1.56258, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1.75)(1.25, 2)(1.25, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2)(1.56258, 1.75)(1.875, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1.75)(1.875, 1.75)(1.875, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1.5)(2.18752, 1.25)(2.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 1.5)(2.18752, 1.5)(2.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1.5)(0.93742, 1.25)(1.25, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 1.5)(0.93742, 1.5)(1.25, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1.25)(0.93742, 1.5)(0.625159, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1.5)(0.625159, 1.5)(0.625159, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1.75)(0.93742, 1.5)(1.25, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1.5)(1.25, 1.5)(1.25, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1.5)(0.312579, 1.25)(0.625159, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 1.5)(0.312579, 1.5)(0.625159, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 2.25)(0.312579, 2.25)(0.312579, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 2)(0.625159, 2.25)(0.312579, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 2.25)(0.625159, 2.25)(0.93742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 2.25)(0.625159, 2)(0.93742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 2.5)(0.625159, 2.25)(0.625159, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 2.25)(0.312579, 2.5)(0.312579, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 2.25)(0.93742, 2.25)(0.93742, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 2.25)(0.93742, 2.5)(0.625159, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.25)(5.93748, 2)(6.25, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.25)(5.93748, 2.25)(5.93748, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 2)(6.25, 2.25)(6.25, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 2.25)(6.25, 2.25)(6.56248, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1)(5.625, 1.25)(5.3125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1)(5.625, 1.25)(5.3125, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.25)(5.625, 1)(5.93748, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 1.25)(5.625, 1.25)(5.93748, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.75)(5.93748, 1.75)(5.93748, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.75)(5.93748, 2)(5.625, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 3)(6.25, 2.75)(6.56248, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.75)(6.56248, 2.75)(6.56248, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.5)(7.5, 2.75)(7.18748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 2.5)(7.5, 2.5)(7.18748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 3.5)(9.68742, 3.25)(10, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3.25)(10, 3.5)(9.68742, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.25)(0, 3.25)(0, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3)(0.312579, 3.25)(0, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.25)(0.312579, 3)(0.625159, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 3.25)(0.312579, 3.25)(0.625159, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 2.75)(2.81252, 2.75)(2.5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2.75)(2.81252, 3)(2.5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 3)(2.81252, 2.75)(3.125, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2.75)(3.125, 3)(2.81252, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2.75)(2.5, 2.5)(2.81252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2.75)(2.5, 2.75)(2.5, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.75)(2.81252, 2.75)(3.125, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.5)(2.81252, 2.75)(2.81252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3)(2.18752, 2.75)(2.5, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3)(2.5, 2.75)(2.5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2.75)(2.18752, 3)(1.875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3)(1.875, 3)(1.875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3)(0.93742, 2.75)(1.25, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3)(1.25, 2.75)(1.25, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3)(0.625159, 3)(0.625159, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 2.75)(0.93742, 3)(0.625159, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3.25)(0.93742, 3)(1.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3)(1.25, 3)(1.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3)(0.93742, 3.25)(0.625159, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 3)(0.625159, 3.25)(0.625159, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 2.75)(1.56258, 3)(1.25, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 2.75)(1.56258, 3)(1.25, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3)(1.56258, 2.75)(1.875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 3)(1.56258, 3)(1.875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3)(1.56258, 3.25)(1.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 3)(1.56258, 3)(1.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 2)(3.75, 2.25)(3.75, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.25)(4.06252, 2)(4.06252, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.5)(3.75, 2.25)(4.06252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.25)(4.06252, 2.25)(4.06252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.25)(3.75, 2.5)(3.43752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 2.25)(3.75, 2.25)(3.43752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 2.25)(3.43752, 2)(3.75, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 2)(3.75, 2.25)(3.43752, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 2)(3.75, 1.75)(3.75, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 2)(3.43752, 1.75)(3.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 2)(3.125, 2)(3.125, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1.75)(3.43752, 2)(3.125, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.25)(2.81252, 2)(3.125, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2)(3.125, 2.25)(2.81252, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.25)(3.43752, 2)(3.43752, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 2)(3.125, 2.25)(3.125, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 2.25)(3.125, 2.25)(2.81252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.25)(3.125, 2.5)(2.81252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.5)(3.125, 2.25)(3.43752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 2.25)(3.43752, 2.25)(3.43752, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 2)(4.6875, 1.75)(5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 2)(4.6875, 2)(5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 1.75)(4.6875, 2)(4.375, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 1.75)(4.6875, 2)(4.375, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.25)(4.06252, 2)(4.375, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 2)(4.375, 2.25)(4.06252, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 2)(4.375, 2.25)(4.375, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.25)(4.6875, 2)(4.6875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 2.25)(4.6875, 2)(5, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 2)(5, 2.25)(4.6875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 2.25)(4.6875, 2.5)(4.6875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 2.5)(5, 2.25)(5, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 2.5)(5, 2.75)(4.6875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 2.75)(4.6875, 2.5)(5, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5)(3.43752, 5.25)(3.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5)(3.43752, 5.25)(3.125, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 5.25)(3.43752, 5.25)(3.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5.25)(3.43752, 5)(3.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5.25)(3.125, 5.5)(3.125, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 5.5)(3.43752, 5.25)(3.43752, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5.5)(3.43752, 5.25)(3.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5.25)(3.75, 5.25)(3.75, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4.25)(4.6875, 4.25)(4.6875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4.5)(4.375, 4.25)(4.6875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4.75)(3.125, 5)(3.125, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4.75)(3.43752, 5)(3.125, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 5)(3.43752, 4.75)(3.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4.75)(3.75, 4.75)(3.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4.5)(3.43752, 4.75)(3.125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4.75)(3.125, 4.75)(3.125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4.5)(3.43752, 4.75)(3.43752, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4.75)(3.43752, 4.75)(3.75, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3.75)(1.875, 4)(1.56258, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4)(1.56258, 3.75)(1.875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3.75)(1.875, 4)(1.875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 4)(1.875, 4)(2.18752, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4)(1.56258, 4.25)(1.56258, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4)(1.875, 4.25)(1.56258, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4.25)(1.875, 4)(2.18752, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 4)(2.18752, 4)(2.18752, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 3.5)(3.125, 3.75)(3.125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 3.75)(3.43752, 3.5)(3.43752, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 3.25)(3.43752, 3.5)(3.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 3.5)(3.125, 3.5)(3.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 3.75)(4.06252, 3.5)(4.375, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3.5)(4.375, 3.75)(4.06252, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 3.5)(3.75, 3.75)(3.43752, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 3.75)(3.43752, 3.5)(3.75, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 3.75)(4.06252, 3.5)(4.06252, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3.5)(3.75, 3.75)(3.75, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3)(1.875, 3.25)(1.875, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 3.25)(2.18752, 3)(2.18752, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 3.25)(1.56258, 3)(1.875, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3)(1.875, 3.25)(1.56258, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 3.5)(1.875, 3.25)(2.18752, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 3.25)(2.18752, 3.25)(2.18752, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 3.25)(1.875, 3.5)(1.56258, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 3.25)(1.875, 3.25)(1.56258, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.25)(3.125, 3)(3.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 3)(2.81252, 3.25)(2.81252, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 3.5)(2.81252, 3.5)(3.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.5)(2.81252, 3.25)(3.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 3)(5.3125, 3.25)(5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 3)(5.3125, 3.25)(5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 3.25)(5.3125, 3)(5.625, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 3.25)(5.3125, 3.25)(5.625, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 3.5)(5.3125, 3.25)(5.3125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 3.25)(5, 3.5)(5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3)(5.625, 2.75)(5.93748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 2.75)(5.93748, 3)(5.625, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3)(6.25, 2.75)(6.25, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.75)(5.93748, 3)(5.93748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3)(5.625, 3.25)(5.625, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3)(5.93748, 3.25)(5.625, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3)(6.25, 3)(6.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3.25)(5.93748, 3)(6.25, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 3.25)(6.875, 3.5)(6.56248, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3.5)(6.56248, 3.25)(6.875, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4.25)(9.37484, 4.5)(9.06258, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4.25)(9.06258, 4.5)(9.06258, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4.25)(9.68742, 4.25)(9.68742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4.5)(9.37484, 4.25)(9.68742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4.5)(6.875, 4.5)(7.18748, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.5)(6.875, 4.25)(7.18748, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.5)(6.56248, 4.5)(6.56248, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.25)(6.875, 4.5)(6.56248, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 4.5)(6.875, 4.5)(6.56248, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.5)(6.875, 4.75)(6.56248, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4)(3.43752, 4.25)(3.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 4)(3.43752, 4)(3.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4)(3.125, 3.75)(3.43752, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 3.75)(3.43752, 4)(3.125, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3.5)(7.81248, 3.25)(8.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3.5)(8.125, 3.25)(8.125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3.5)(7.5, 3.5)(7.5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3.25)(7.81248, 3.5)(7.5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 3.75)(7.81248, 3.5)(8.125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3.75)(7.81248, 3.5)(8.125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 3.5)(5.3125, 3.75)(5.3125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 3.5)(5.625, 3.75)(5.3125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 3.5)(5.3125, 3.25)(5.625, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 3.25)(5.625, 3.5)(5.3125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3.5)(5.625, 3.5)(5.93748, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3.25)(5.625, 3.5)(5.625, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 3.5)(5.93748, 3.75)(5.93748, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3.75)(6.25, 3.5)(6.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 3.5)(5.93748, 3.75)(5.625, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3.75)(5.625, 3.5)(5.93748, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 4.25)(7.81248, 4.5)(7.5, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4.5)(7.5, 4.25)(7.81248, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4.5)(7.81248, 4.25)(8.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 4.5)(7.81248, 4.5)(8.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 5)(7.81248, 4.75)(7.81248, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4.75)(7.5, 5)(7.5, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4.5)(7.81248, 4.75)(7.5, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4.75)(7.5, 4.75)(7.5, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 4.5)(8.75, 4.5)(9.06258, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4.5)(8.75, 4.25)(9.06258, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4.75)(7.18748, 4.5)(7.5, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 4.75)(7.18748, 4.75)(7.5, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4.75)(6.875, 4.5)(7.18748, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.5)(7.18748, 4.75)(6.875, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4.75)(7.5, 5)(7.18748, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 5)(7.18748, 4.75)(7.5, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.75)(7.18748, 4.75)(6.875, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 5)(7.18748, 4.75)(7.18748, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 5.5)(5.625, 5.25)(5.93748, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.5)(5.625, 5.25)(5.93748, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 5.25)(5.625, 5.25)(5.3125, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.25)(5.625, 5.5)(5.3125, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.25)(5.625, 5)(5.93748, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.25)(5.93748, 5)(5.93748, 5.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5.25)(5.3125, 5.25)(5.3125, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 5)(5.625, 5.25)(5.3125, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 4.75)(4.06252, 5)(3.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4.75)(4.06252, 4.75)(3.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 4.75)(3.75, 4.75)(3.75, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 4.75)(3.75, 4.5)(4.06252, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.5)(5.625, 4.75)(5.3125, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 4.5)(5.625, 4.5)(5.3125, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.5)(5.93748, 4.5)(5.93748, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.75)(5.625, 4.5)(5.93748, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.75)(2.5, 4)(2.5, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.75)(2.81252, 4)(2.5, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 4)(2.81252, 3.75)(3.125, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.75)(3.125, 3.75)(3.125, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 3.5)(2.81252, 3.75)(2.5, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.5)(2.81252, 3.75)(2.5, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 3.75)(2.81252, 3.75)(3.125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.75)(2.81252, 3.5)(3.125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 0.75)(9.37484, 1)(9.37484, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1)(9.37484, 1)(9.68742, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 1)(9.06258, 1.25)(9.06258, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 1.25)(9.37484, 1)(9.37484, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 1)(9.68742, 1.25)(9.37484, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 1)(9.68742, 1)(9.68742, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 0.75)(6.25, 1)(5.93748, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1)(5.93748, 1)(5.93748, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1)(5.93748, 1.25)(5.93748, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1)(6.25, 1.25)(5.93748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 0.5)(8.43742, 0.75)(8.125, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 0.75)(8.125, 0.75)(8.125, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 1.5)(8.43742, 1.75)(8.43742, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 1.75)(8.75, 1.5)(8.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 1.75)(8.125, 1.5)(8.43742, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 1.75)(8.125, 1.75)(8.125, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 1.75)(8.75, 2)(8.43742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2)(8.43742, 1.75)(8.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 2)(8.43742, 1.75)(8.43742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 1.75)(8.43742, 1.75)(8.125, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1.5)(8.125, 1.25)(8.125, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 1.25)(7.81248, 1.5)(7.81248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1.5)(7.5, 1.25)(7.81248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1.5)(7.5, 1.5)(7.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2)(9.68742, 1.75)(9.68742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 1.75)(9.37484, 2)(9.37484, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2)(9.06258, 1.75)(9.37484, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2)(9.06258, 2)(9.06258, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 2.25)(9.37484, 2)(9.68742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2.25)(9.37484, 2)(9.68742, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2)(9.37484, 2.25)(9.06258, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 2)(9.37484, 2)(9.06258, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2)(7.18748, 1.75)(7.18748, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2)(6.875, 1.75)(7.18748, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 1.75)(6.875, 2)(6.56248, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1.75)(6.875, 2)(6.56248, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 2.25)(6.875, 2)(7.18748, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2)(7.18748, 2.25)(6.875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2)(6.56248, 2.25)(6.56248, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 2.25)(6.875, 2)(6.875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9.75)(6.56248, 10)(6.56248, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 10)(6.875, 9.75)(6.875, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9.75)(7.18748, 10)(6.875, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9.75)(7.18748, 9.75)(7.18748, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9.5)(6.875, 9.75)(6.56248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9.75)(6.56248, 9.75)(6.56248, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9.75)(6.875, 9.5)(7.18748, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 9.75)(6.875, 9.75)(7.18748, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 9.25)(5.93748, 9)(6.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 9)(6.25, 9)(6.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 8.75)(2.5, 8.5)(2.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 8.5)(2.18752, 8.75)(2.18752, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9)(1.56258, 9.25)(1.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 9)(1.56258, 9)(1.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.75)(2.5, 9)(2.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9)(2.81252, 8.75)(2.81252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.75)(3.125, 9)(2.81252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.75)(3.125, 8.75)(3.125, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 9)(0.625159, 9)(0.312579, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 9)(0.625159, 9.25)(0.312579, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.75)(0, 9)(0, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.75)(0.312579, 9)(0, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.75)(0.625159, 9)(0.312579, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 9)(0.312579, 8.75)(0.625159, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 8.5)(0.312579, 8.75)(0, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.5)(0.312579, 8.75)(0, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 8.75)(0.312579, 8.75)(0.625159, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.75)(0.312579, 8.5)(0.625159, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 8.75)(1.56258, 9)(1.25, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9)(1.25, 8.75)(1.56258, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 9.75)(3.75, 9.5)(4.06252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.5)(4.06252, 9.75)(3.75, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.5)(3.75, 9.75)(3.43752, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 9.5)(3.75, 9.5)(3.43752, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9.75)(10, 9.75)(10, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 10)(9.68742, 9.75)(10, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9.75)(9.68742, 10)(9.37484, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9.75)(9.37484, 10)(9.37484, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 9.75)(9.68742, 9.75)(10, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 9.5)(9.68742, 9.75)(9.68742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9.75)(9.37484, 9.5)(9.68742, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9.5)(9.68742, 9.75)(9.37484, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 10)(9.06258, 9.75)(9.37484, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 10)(9.06258, 9.75)(9.37484, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9.75)(9.06258, 9.75)(8.75, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 9.75)(9.06258, 10)(8.75, 10)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9.5)(9.06258, 9.75)(9.06258, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 9.75)(9.37484, 9.5)(9.37484, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9.5)(9.06258, 9.75)(8.75, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 9.75)(8.75, 9.5)(9.06258, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 7.5)(8.125, 7.75)(7.81248, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 7.75)(7.81248, 7.5)(8.125, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.25)(5.3125, 7)(5.625, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 7)(5.625, 7.25)(5.3125, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.25)(5.3125, 7.5)(5.3125, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.25)(5.625, 7.5)(5.3125, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.5)(5.625, 7.25)(5.93748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.25)(5.93748, 7.25)(5.93748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 7.25)(5.93748, 7)(6.25, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 7.25)(5.93748, 7)(6.25, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 7)(5.625, 7.25)(5.625, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 7.25)(5.93748, 7)(5.93748, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 6.75)(5.93748, 7)(5.93748, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 7)(6.25, 6.75)(6.25, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 7)(5.625, 6.75)(5.93748, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.75)(5.93748, 7)(5.625, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 7.5)(9.06258, 7.5)(9.06258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 7.75)(8.75, 7.5)(9.06258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7.5)(9.06258, 7.5)(9.06258, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7.5)(9.06258, 7.25)(9.37484, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 8.25)(9.37484, 8)(9.68742, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 8)(9.68742, 8.25)(9.37484, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8.25)(9.37484, 8)(9.37484, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 8)(9.06258, 8.25)(9.06258, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8.25)(8.75, 8.25)(8.75, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8)(9.06258, 8.25)(8.75, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 8.5)(9.06258, 8.25)(9.37484, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8.25)(9.37484, 8.5)(9.06258, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 8.5)(9.06258, 8.25)(9.06258, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8.25)(8.75, 8.5)(8.75, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.25)(7.18748, 8)(7.18748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.25)(6.875, 8)(7.18748, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 8)(6.875, 8.25)(6.56248, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8)(6.875, 8.25)(6.56248, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 8.5)(6.875, 8.25)(7.18748, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.25)(7.18748, 8.5)(6.875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.25)(6.56248, 8.5)(6.56248, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 8.5)(6.875, 8.25)(6.875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 8)(6.875, 7.75)(7.18748, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8)(6.875, 7.75)(7.18748, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 7.75)(6.56248, 8)(6.56248, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 7.75)(6.875, 8)(6.56248, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 7.75)(7.18748, 7.5)(7.18748, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 7.75)(6.875, 7.5)(7.18748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7)(9.68742, 7.25)(9.37484, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7)(9.68742, 7.25)(9.37484, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 7.25)(9.68742, 7.25)(10, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7.25)(9.68742, 7)(10, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7.25)(9.37484, 7.5)(9.37484, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7.5)(9.68742, 7.25)(9.68742, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7.25)(10, 7.25)(10, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7.5)(9.68742, 7.25)(10, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 7)(9.68742, 6.75)(10, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7)(9.68742, 6.75)(10, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6.75)(9.68742, 7)(9.37484, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6.75)(9.68742, 6.75)(9.37484, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6.75)(10, 6.5)(10, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6.75)(9.68742, 6.5)(10, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6.75)(9.37484, 6.75)(9.37484, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6.5)(9.68742, 6.75)(9.37484, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 6.75)(9.06258, 7)(8.75, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 6.75)(9.06258, 7)(8.75, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 7)(9.37484, 6.75)(9.37484, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 7)(9.06258, 6.75)(9.37484, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 7.25)(9.06258, 7)(9.37484, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 7)(9.37484, 7)(9.37484, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 7.75)(0.93742, 8)(0.93742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8)(1.25, 7.75)(1.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8)(0.625159, 8)(0.625159, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8)(0.625159, 7.75)(0.93742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 7.25)(1.56258, 7.5)(1.25, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 7.25)(1.25, 7.5)(1.25, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 7)(1.56258, 7.25)(1.25, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 7)(1.56258, 7.25)(1.25, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7.75)(4.6875, 8)(4.375, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8)(4.375, 7.75)(4.6875, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 7.75)(4.6875, 8)(4.6875, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 8)(4.6875, 8)(5, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8)(5, 8)(5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8.25)(4.6875, 8)(5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.25)(4.375, 8.5)(4.06252, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 8.25)(4.375, 8.25)(4.06252, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.25)(4.6875, 8.25)(4.6875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.5)(4.375, 8.25)(4.6875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8)(4.375, 8.25)(4.06252, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.25)(4.06252, 8.25)(4.06252, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 8)(4.375, 8.25)(4.375, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 8.25)(4.6875, 8)(4.6875, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8.5)(3.75, 8.25)(4.06252, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8.25)(4.06252, 8.25)(4.06252, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 8.5)(3.75, 8.25)(3.75, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8.25)(3.43752, 8.5)(3.43752, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8.25)(3.75, 8)(4.06252, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 8.25)(3.75, 8.25)(4.06252, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8.25)(3.43752, 8.25)(3.43752, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 8)(3.75, 8.25)(3.43752, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7)(3.75, 7.25)(3.43752, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7)(3.43752, 7.25)(3.43752, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 8.25)(2.5, 8.5)(2.18752, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 8.5)(2.18752, 8.25)(2.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 8)(2.18752, 8.25)(2.18752, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 8.25)(2.5, 8)(2.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 8.25)(1.875, 8)(2.18752, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 8.25)(1.875, 8.25)(1.875, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8.5)(2.18752, 8.25)(2.18752, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 8.25)(1.875, 8.5)(1.875, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 8.75)(7.81248, 8.5)(8.125, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 8.75)(7.81248, 8.5)(8.125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 8.5)(7.81248, 8.5)(7.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 8.5)(7.81248, 8.75)(7.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 8.25)(7.81248, 8.5)(7.81248, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 8.5)(8.125, 8.25)(8.125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 8.25)(7.81248, 8.5)(7.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 8.5)(7.5, 8.5)(7.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8.75)(8.75, 8.5)(8.75, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8.75)(8.43742, 8.5)(8.75, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8.5)(8.43742, 8.75)(8.125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8.75)(8.125, 8.75)(8.125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8.75)(5.625, 8.5)(5.93748, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 8.75)(5.625, 8.75)(5.93748, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8.75)(5.3125, 8.75)(5.3125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8.5)(5.625, 8.75)(5.3125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9.5)(2.5, 9.25)(2.81252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9.25)(2.81252, 9.25)(2.81252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9.25)(2.5, 9.5)(2.18752, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 9.25)(2.5, 9.25)(2.18752, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 9.25)(2.5, 9.25)(2.81252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9.25)(2.5, 9)(2.81252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 6)(2.18752, 6)(1.875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6)(2.18752, 6.25)(1.875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5.5)(1.56258, 5.75)(1.25, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 5.5)(1.56258, 5.75)(1.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5.75)(1.25, 6)(1.25, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5.75)(1.56258, 6)(1.25, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5.75)(0, 6)(0, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5.75)(0.312579, 6)(0, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5.75)(0.625159, 5.75)(0.625159, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6)(0.312579, 5.75)(0.625159, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5.75)(0, 5.75)(0, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5.5)(0.312579, 5.75)(0, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 5.75)(0.312579, 5.5)(0.625159, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 5.75)(0.312579, 5.75)(0.625159, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 7.25)(3.125, 7.25)(3.43752, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7.25)(3.125, 7)(3.43752, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7.5)(3.125, 7.25)(3.43752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7.25)(3.43752, 7.25)(3.43752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 6.75)(0.312579, 6.75)(0, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6.75)(0.312579, 7)(0, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 7)(0.312579, 6.75)(0.625159, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6.75)(0.625159, 6.75)(0.625159, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6.75)(0, 6.75)(0, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6.5)(0.312579, 6.75)(0, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 6.75)(0.312579, 6.5)(0.625159, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 6.75)(0.312579, 6.75)(0.625159, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6.25)(1.875, 6.5)(1.875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6.5)(1.875, 6.5)(2.18752, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 6.5)(1.56258, 6.25)(1.875, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 6.5)(1.56258, 6.5)(1.56258, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6.5)(9.37484, 6.25)(9.68742, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6.25)(9.68742, 6.5)(9.37484, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 5.75)(9.06258, 5.5)(9.37484, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 5.75)(9.06258, 5.75)(9.06258, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 6.5)(7.18748, 6.75)(7.18748, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 6.75)(7.5, 6.5)(7.5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7)(7.18748, 6.75)(7.5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 7)(7.18748, 6.75)(7.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.25)(8.125, 6.5)(7.81248, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 6.5)(7.81248, 6.25)(8.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.25)(7.81248, 6.5)(7.5, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 6.25)(7.81248, 6.25)(7.5, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.25)(7.81248, 6)(8.125, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 6.25)(7.81248, 6.25)(8.125, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6)(7.81248, 6.25)(7.5, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.25)(7.5, 6.25)(7.5, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6.75)(9.06258, 6.5)(9.37484, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 6.75)(9.06258, 6.5)(9.37484, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 6.5)(9.06258, 6.5)(8.75, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 6.5)(9.06258, 6.75)(8.75, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 6.5)(9.37484, 6.25)(9.37484, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6.25)(9.06258, 6.5)(9.06258, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 6.5)(8.75, 6.25)(9.06258, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 6.25)(9.06258, 6.5)(8.75, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 6.25)(7.18748, 6)(7.5, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 6.25)(7.18748, 6)(7.5, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 5.75)(7.18748, 6)(6.875, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 5.75)(7.18748, 6)(6.875, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 6)(7.18748, 5.75)(7.5, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 6)(7.18748, 6)(7.5, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.25)(6.56248, 6)(6.875, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6)(6.875, 6.25)(6.56248, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.25)(7.18748, 6)(7.18748, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 6)(6.875, 6.25)(6.875, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.25)(6.56248, 6.5)(6.56248, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.25)(6.875, 6.5)(6.56248, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.25)(7.18748, 6.25)(7.18748, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.5)(6.875, 6.25)(7.18748, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 6.25)(5.93748, 6)(6.25, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 6.25)(5.93748, 6.25)(6.25, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 6)(5.93748, 6.25)(5.625, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 6.25)(5.625, 6.25)(5.625, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 6.25)(6.25, 6.25)(6.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 6.5)(5.93748, 6.25)(6.25, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.5)(5.93748, 6.25)(5.93748, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 6.25)(5.93748, 6.25)(5.625, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0.5)(2.18752, 0.5)(2.18752, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0.75)(1.875, 0.5)(2.18752, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0.5)(1.875, 0.75)(1.56258, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 0.5)(1.875, 0.5)(1.56258, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0.5)(2.18752, 0.25)(2.18752, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 0.25)(1.875, 0.5)(1.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0.5)(1.56258, 0.25)(1.875, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 0.5)(1.56258, 0.5)(1.56258, 0.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1)(3.75, 0.75)(3.75, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1)(3.43752, 0.75)(3.75, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 0.75)(3.43752, 1)(3.125, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 0.75)(3.43752, 1)(3.125, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 1.25)(3.43752, 1)(3.75, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1.25)(3.43752, 1)(3.75, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 1)(3.43752, 1)(3.125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1)(3.43752, 1.25)(3.125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 1.5)(1.56258, 1.5)(1.56258, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 1.5)(1.56258, 1.25)(1.875, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1.25)(1.875, 1.5)(1.875, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1.5)(1.875, 1.5)(2.18752, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 1.5)(1.56258, 1.75)(1.56258, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 1.75)(1.875, 1.5)(1.875, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1.75)(2.18752, 1.5)(2.5, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1.75)(2.5, 1.5)(2.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1.75)(1.875, 1.5)(2.18752, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 1.5)(2.18752, 1.75)(1.875, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 2)(2.18752, 1.75)(2.5, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 2)(2.18752, 1.75)(2.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 1.75)(2.18752, 2)(1.875, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 1.75)(2.18752, 1.75)(1.875, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1.25)(0, 1.5)(0, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1.5)(0, 1.5)(0.312579, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 1.5)(0.312579, 1.75)(0, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1.75)(0, 1.5)(0.312579, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1.75)(0, 2)(0, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 2)(0.312579, 1.75)(0.312579, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.5)(5.625, 1.25)(5.93748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.5)(5.93748, 1.25)(5.93748, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.5)(5.3125, 1.5)(5.3125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.25)(5.625, 1.5)(5.3125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.75)(5.625, 1.5)(5.93748, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 1.75)(5.625, 1.5)(5.93748, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 1.5)(5.3125, 1.75)(5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1.5)(5.3125, 1.75)(5, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 1.5)(5.3125, 1.75)(5.3125, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1.75)(5.625, 1.5)(5.625, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1.75)(5, 2)(5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1.75)(5.3125, 2)(5, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 1.75)(5.625, 1.75)(5.625, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 2)(5.3125, 1.75)(5.625, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 2.25)(6.875, 2.5)(6.875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 2.5)(6.875, 2.5)(7.18748, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2.5)(6.56248, 2.25)(6.875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2.5)(6.56248, 2.5)(6.56248, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2.5)(7.18748, 2.5)(7.18748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2.75)(6.875, 2.5)(7.18748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2.5)(6.875, 2.75)(6.56248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 2.5)(6.875, 2.5)(6.56248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.25)(6.25, 2.5)(5.93748, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.5)(5.93748, 2.5)(5.93748, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.5)(6.25, 2.25)(6.56248, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 2.5)(6.25, 2.5)(6.56248, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 2.5)(6.25, 2.5)(5.93748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.5)(6.25, 2.75)(5.93748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.75)(6.25, 2.5)(6.56248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 2.5)(6.56248, 2.5)(6.56248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.25)(7.5, 2.5)(7.18748, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.25)(7.18748, 2.5)(7.18748, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.25)(7.81248, 2)(7.81248, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.25)(7.5, 2)(7.81248, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2)(7.5, 2.25)(7.18748, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.25)(7.18748, 2.25)(7.18748, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3)(9.68742, 3.25)(9.37484, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3)(9.37484, 3.25)(9.37484, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3)(10, 3)(10, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3.25)(9.68742, 3)(10, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 3.25)(9.06258, 3)(9.37484, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3.25)(9.06258, 3)(9.37484, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 3)(9.06258, 3)(8.75, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3)(9.06258, 3.25)(8.75, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 2.75)(9.68742, 2.5)(10, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 2.75)(9.68742, 2.75)(9.68742, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3)(10, 2.75)(10, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 2.75)(9.68742, 3)(9.68742, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3)(7.5, 3)(7.5, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3)(7.5, 2.75)(7.81248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3)(7.81248, 3.25)(7.5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 3)(7.81248, 3)(7.5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.75)(7.18748, 3)(7.18748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 3)(7.18748, 3)(7.5, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 3)(7.5, 3)(7.5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 3.25)(7.18748, 3)(7.5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.5)(0.625159, 3.25)(0.625159, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.5)(0.312579, 3.25)(0.625159, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.5)(0, 3.5)(0, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.25)(0.312579, 3.5)(0, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.5)(0.625159, 3.5)(0.625159, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.75)(0.312579, 3.5)(0.625159, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 3.5)(0.312579, 3.75)(0, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 3.5)(0.312579, 3.5)(0, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 2.25)(5, 2.25)(5, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 2)(5.3125, 2.25)(5, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 2.25)(5.3125, 2.5)(5, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 2.25)(5.3125, 2.25)(5, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 2.25)(4.375, 2.5)(4.06252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.25)(4.375, 2.5)(4.06252, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.5)(4.375, 2.25)(4.6875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 2.5)(4.375, 2.5)(4.6875, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.5)(4.375, 2.75)(4.06252, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.5)(4.06252, 2.75)(4.06252, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.75)(4.375, 2.5)(4.6875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 2.5)(4.6875, 2.5)(4.6875, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4.25)(3.75, 4.25)(3.43752, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4.25)(3.75, 4.5)(3.43752, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 3.25)(2.5, 3.5)(2.18752, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3.25)(2.5, 3.25)(2.18752, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.5)(2.5, 3.25)(2.81252, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 3.25)(2.81252, 3.5)(2.5, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 3.25)(2.18752, 3)(2.5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 3)(2.5, 3.25)(2.18752, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3)(2.5, 3.25)(2.5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 3.25)(2.5, 3.25)(2.81252, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 3.25)(3.43752, 3)(3.75, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 3.25)(3.43752, 3.25)(3.43752, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3)(3.75, 3.25)(3.75, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3.25)(3.75, 3.25)(4.06252, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 3.25)(3.43752, 3.5)(3.43752, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 3.5)(3.75, 3.25)(3.75, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 3.25)(4.06252, 3.5)(3.75, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 3.25)(4.06252, 3.25)(4.06252, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 3.25)(4.06252, 3)(4.375, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 3.25)(4.06252, 3.25)(4.06252, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3.5)(4.375, 3.25)(4.375, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3.25)(4.375, 3.25)(4.06252, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 3.5)(7.18748, 3.5)(7.5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 3.5)(7.18748, 3.25)(7.5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 3.5)(6.875, 3.5)(6.875, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 3.25)(7.18748, 3.5)(6.875, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 4)(8.43742, 4)(8.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4)(8.43742, 4.25)(8.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4.25)(4.375, 4)(4.6875, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4)(4.6875, 4)(4.6875, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 3.75)(4.375, 4)(4.06252, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 3.75)(4.375, 4)(4.06252, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4)(4.375, 3.75)(4.6875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 4)(4.375, 4)(4.6875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 5)(8.125, 4.75)(8.43742, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 4.75)(8.43742, 4.75)(8.43742, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 4.75)(8.125, 5)(7.81248, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4.75)(8.125, 4.75)(7.81248, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 4.75)(7.81248, 4.5)(8.125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 4.75)(7.81248, 4.75)(7.81248, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5)(8.75, 4.75)(8.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4.75)(8.75, 4.75)(8.43742, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4.75)(9.06258, 5)(8.75, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4.75)(9.06258, 4.75)(9.06258, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4.75)(8.75, 4.5)(9.06258, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 4.75)(8.75, 4.75)(9.06258, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5)(9.37484, 4.75)(9.37484, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 4.75)(9.37484, 4.75)(9.06258, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4.5)(9.37484, 4.75)(9.06258, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4.75)(9.06258, 4.75)(9.06258, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 4.75)(8.43742, 4.5)(8.43742, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4.5)(8.125, 4.75)(8.125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4.5)(8.75, 4.75)(8.43742, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4.75)(8.43742, 4.5)(8.75, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4.5)(8.125, 4.5)(8.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4.25)(8.43742, 4.5)(8.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4.5)(8.43742, 4.5)(8.75, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4.5)(8.43742, 4.25)(8.75, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 5)(4.375, 4.75)(4.6875, 4.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4.75)(4.6875, 5)(4.375, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 5)(4.375, 4.75)(4.375, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 4.75)(4.375, 4.75)(4.06252, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 4.75)(4.375, 4.75)(4.6875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4.75)(4.375, 4.5)(4.6875, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4.75)(4.06252, 4.75)(4.06252, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4.5)(4.375, 4.75)(4.06252, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 4.25)(5.625, 4.25)(5.3125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.25)(5.625, 4.5)(5.3125, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.25)(5.93748, 4.25)(5.93748, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.5)(5.625, 4.25)(5.93748, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 1)(6.25, 0.75)(6.56248, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 1)(6.25, 1)(6.25, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1)(6.56248, 1)(6.25, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1.25)(6.56248, 1)(6.56248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 0.75)(8.125, 1)(8.125, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 1)(8.43742, 0.75)(8.43742, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 0.75)(8.125, 1)(7.81248, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 1)(7.81248, 1)(7.81248, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 1.25)(8.125, 1)(8.43742, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 1.25)(8.125, 1)(8.43742, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 1)(8.125, 1.25)(7.81248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1)(8.125, 1)(7.81248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 1)(7.5, 1.25)(7.18748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 1)(7.5, 1)(7.18748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 1.25)(7.5, 1)(7.81248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 1)(7.81248, 1)(7.81248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.75)(8.43742, 0.5)(8.75, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.75)(8.43742, 0.75)(8.43742, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.75)(8.75, 1)(8.43742, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 0.75)(8.75, 0.75)(8.43742, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1.5)(7.81248, 1.75)(7.5, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 1.5)(7.81248, 1.75)(7.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 1.75)(7.81248, 1.75)(8.125, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1.75)(7.81248, 1.5)(8.125, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1.75)(7.5, 2)(7.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2)(7.81248, 1.75)(7.81248, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1.75)(8.125, 2)(7.81248, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1.75)(8.125, 1.75)(8.125, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 1.75)(6.25, 1.5)(6.25, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1.5)(5.93748, 1.75)(5.93748, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1.5)(6.56248, 1.75)(6.25, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1.5)(6.56248, 1.5)(6.56248, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1.25)(6.25, 1.5)(5.93748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 1.25)(6.25, 1.5)(5.93748, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 1.5)(6.25, 1.25)(6.56248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 1.5)(6.25, 1.5)(6.56248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 1.75)(7.18748, 1.5)(7.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 1.5)(7.5, 1.5)(7.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 1.5)(7.18748, 1.5)(7.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 1.25)(7.18748, 1.5)(7.18748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9.5)(5.93748, 9.25)(5.93748, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9.5)(5.625, 9.25)(5.93748, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9.5)(5.3125, 9.5)(5.3125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9.25)(5.625, 9.5)(5.3125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9.75)(5.625, 9.5)(5.93748, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9.5)(5.93748, 9.5)(5.93748, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 9.5)(5.625, 9.5)(5.3125, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 9.75)(5.625, 9.5)(5.625, 9.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 9)(6.56248, 9.25)(6.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 9)(6.56248, 9)(6.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 9.25)(6.56248, 9)(6.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 9)(6.875, 9)(6.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 9)(7.18748, 9.25)(6.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 9)(7.18748, 9)(6.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 9)(6.25, 8.75)(6.25, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.75)(5.93748, 9)(5.93748, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.75)(6.56248, 9)(6.25, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 9)(6.25, 8.75)(6.56248, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.5)(6.25, 8.75)(5.93748, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.75)(5.93748, 8.75)(5.93748, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 8.75)(6.25, 8.5)(6.56248, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 8.75)(6.25, 8.75)(6.56248, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.75)(7.18748, 9)(6.875, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 9)(6.875, 8.75)(7.18748, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 9)(6.875, 8.75)(6.875, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.75)(6.56248, 9)(6.56248, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.75)(7.18748, 8.5)(7.18748, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 8.5)(6.875, 8.75)(6.875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.75)(6.56248, 8.5)(6.875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 8.75)(6.56248, 8.75)(6.56248, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 9)(2.18752, 8.75)(2.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9)(2.18752, 9)(2.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 9)(2.5, 9.25)(2.18752, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 9.25)(2.18752, 9)(2.5, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 8.75)(2.81252, 8.5)(3.125, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.75)(2.81252, 8.5)(3.125, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 8.5)(2.81252, 8.5)(2.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.5)(2.81252, 8.75)(2.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.5)(2.81252, 8.25)(3.125, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 8.5)(2.81252, 8.5)(3.125, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.25)(2.81252, 8.5)(2.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 8.5)(2.5, 8.5)(2.5, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9)(1.25, 9.25)(0.93742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9)(1.25, 9)(1.25, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 9.25)(0.93742, 9)(0.93742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 9)(0.93742, 9)(0.625159, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.25)(4.06252, 9.25)(4.06252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.5)(3.75, 9.25)(4.06252, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.25)(3.43752, 9.5)(3.43752, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.25)(3.75, 9.5)(3.43752, 9.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 9.25)(3.75, 9.25)(4.06252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.25)(3.75, 9)(4.06252, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9.25)(3.43752, 9.25)(3.43752, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 9)(3.75, 9.25)(3.43752, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 7.75)(6.25, 7.5)(6.25, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 7.5)(5.93748, 7.75)(5.93748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 7.25)(6.25, 7.5)(5.93748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 7.5)(5.93748, 7.25)(6.25, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 7.75)(8.43742, 7.5)(8.43742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 7.5)(8.125, 7.75)(8.125, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 7.5)(8.75, 7.75)(8.43742, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 7.5)(8.75, 7.5)(8.75, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 7.5)(9.37484, 7.75)(9.06258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7.5)(9.37484, 7.75)(9.06258, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 7.75)(9.37484, 7.75)(9.68742, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7.75)(9.37484, 7.5)(9.68742, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7.75)(9.06258, 8)(9.06258, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7.75)(9.37484, 8)(9.06258, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 7.75)(9.68742, 7.75)(9.68742, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 8)(9.37484, 7.75)(9.68742, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.25)(0, 8.5)(0, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.25)(0.312579, 8.5)(0, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.5)(0.312579, 8.25)(0.625159, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.25)(0.625159, 8.25)(0.625159, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0, 8)(0.312579, 8.25)(0, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 8.25)(0, 8)(0.312579, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 8)(0.312579, 8.25)(0.312579, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 8.25)(0.312579, 8.25)(0.625159, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.25)(1.25, 8.25)(1.25, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.5)(0.93742, 8.25)(1.25, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 8.25)(0.93742, 8.25)(0.625159, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.25)(0.93742, 8.5)(0.625159, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.25)(0.93742, 8)(1.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 8.25)(0.93742, 8.25)(1.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8)(0.93742, 8.25)(0.625159, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.25)(0.625159, 8.25)(0.625159, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 7.25)(2.5, 7.5)(2.18752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.5)(2.18752, 7.25)(2.5, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.25)(2.18752, 7.25)(2.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 7.25)(2.18752, 7)(2.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 7)(4.375, 7.25)(4.06252, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 7)(4.375, 7)(4.375, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7.25)(4.06252, 7)(4.06252, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 7)(4.06252, 7)(3.75, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 8.75)(1.875, 8.75)(2.18752, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8.75)(1.875, 8.5)(2.18752, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 8.75)(1.56258, 8.5)(1.56258, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 8.5)(1.25, 8.75)(1.25, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8.75)(1.56258, 8.5)(1.875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 8.5)(1.875, 8.75)(1.56258, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9)(8.43742, 8.75)(8.75, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8.75)(8.75, 9)(8.43742, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 8.75)(8.75, 9)(8.75, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 9)(8.75, 9)(9.06258, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9)(8.75, 9.25)(8.43742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9)(8.43742, 9.25)(8.43742, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9.25)(8.75, 9)(9.06258, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 9)(9.06258, 9)(9.06258, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9)(9.37484, 8.75)(9.68742, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 9)(9.37484, 9)(9.68742, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9)(9.06258, 8.75)(9.37484, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9)(9.06258, 9)(9.06258, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9.25)(9.37484, 9)(9.68742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9)(9.68742, 9)(9.68742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 9)(9.37484, 9.25)(9.06258, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 9)(9.37484, 9)(9.06258, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 8.75)(5.625, 9)(5.3125, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 8.75)(5.625, 9)(5.3125, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9)(5.625, 8.75)(5.93748, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 9)(5.625, 9)(5.93748, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 9)(5.625, 9)(5.3125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9)(5.625, 9.25)(5.3125, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9)(5.93748, 9)(5.93748, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 9.25)(5.625, 9)(5.93748, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 6)(2.5, 5.75)(2.81252, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6)(2.5, 6)(2.81252, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 5.75)(2.5, 6)(2.18752, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 6)(2.18752, 6)(2.18752, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.25)(2.5, 6)(2.81252, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 6)(2.81252, 6.25)(2.5, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6)(2.5, 6)(2.18752, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6.25)(2.5, 6)(2.5, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.75)(1.875, 5.5)(2.18752, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.75)(2.18752, 5.5)(2.18752, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.75)(1.56258, 5.5)(1.875, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.75)(1.56258, 5.75)(1.56258, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 5.75)(2.18752, 6)(1.875, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6)(1.875, 5.75)(2.18752, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6)(1.875, 5.75)(1.875, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 5.75)(1.875, 5.75)(1.56258, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 7.5)(2.81252, 7.25)(2.81252, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 7.25)(2.5, 7.5)(2.5, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 7.25)(3.125, 7.5)(2.81252, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 7.25)(3.125, 7.25)(3.125, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 7.25)(2.5, 7.25)(2.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 7)(2.81252, 7.25)(2.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7.25)(2.81252, 7.25)(3.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 7.25)(2.81252, 7)(3.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 7)(2.18752, 6.75)(2.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6.75)(2.5, 6.75)(2.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6.75)(2.5, 6.5)(2.5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 6.5)(2.18752, 6.75)(2.18752, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 6.5)(2.18752, 6.5)(2.18752, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 6.5)(2.18752, 6.25)(2.5, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6)(9.37484, 6.25)(9.06258, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6)(9.06258, 6.25)(9.06258, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6)(9.68742, 6)(9.68742, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6.25)(9.37484, 6)(9.68742, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 5.75)(9.37484, 6)(9.06258, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5.75)(9.37484, 6)(9.06258, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 6.25)(8.75, 6)(9.06258, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 6.25)(8.75, 6)(9.06258, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 5.75)(8.75, 6)(8.75, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 6)(9.06258, 5.75)(9.06258, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6.25)(8.125, 6.5)(8.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 6.5)(8.43742, 6.25)(8.43742, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6.25)(8.75, 6.5)(8.43742, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6.25)(8.75, 6.25)(8.75, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 6)(9.68742, 5.75)(10, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 6)(9.68742, 5.75)(10, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 6)(9.68742, 5.75)(9.68742, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 5.75)(9.37484, 6)(9.37484, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 5.75)(9.68742, 5.75)(10, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 5.75)(9.68742, 5.5)(10, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 5.5)(9.68742, 5.75)(9.37484, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 5.75)(9.37484, 5.75)(9.37484, 5.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.75)(6.56248, 6.75)(6.56248, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.5)(6.875, 6.75)(6.56248, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 6.75)(6.875, 6.75)(7.18748, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.75)(6.875, 6.5)(7.18748, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 6.75)(6.875, 6.75)(6.56248, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7)(6.875, 6.75)(6.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.75)(7.18748, 6.75)(7.18748, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 6.75)(7.18748, 7)(6.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.5)(8.125, 6.75)(7.81248, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 6.5)(8.125, 6.75)(7.81248, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 6.75)(8.43742, 6.5)(8.43742, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 6.75)(8.125, 6.5)(8.43742, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 6.75)(8.125, 6.75)(7.81248, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 7)(8.125, 6.75)(8.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 6.75)(8.43742, 6.75)(8.43742, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 6.75)(8.43742, 7)(8.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1.5)(2.81252, 1.75)(2.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 1.5)(2.81252, 1.5)(2.5, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1.75)(2.81252, 1.5)(3.125, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1.5)(3.125, 1.5)(3.125, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1.25)(2.81252, 1.5)(2.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1.5)(2.5, 1.5)(2.5, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 1.5)(2.81252, 1.25)(3.125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 1.5)(2.81252, 1.5)(3.125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 1.75)(3.43752, 1.5)(3.75, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1.75)(3.43752, 1.5)(3.75, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1.5)(3.43752, 1.75)(3.125, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 1.5)(3.43752, 1.5)(3.125, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1.5)(3.75, 1.25)(3.75, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1.5)(3.43752, 1.25)(3.75, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1.25)(3.43752, 1.5)(3.125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 1.5)(3.125, 1.5)(3.125, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 1.5)(0.625159, 1.75)(0.625159, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 1.75)(0.93742, 1.5)(0.93742, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 1.75)(0.312579, 1.5)(0.625159, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 1.75)(0.312579, 1.75)(0.312579, 1.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 2)(0.625159, 1.75)(0.93742, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 2)(0.625159, 1.75)(0.93742, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.625159, 1.75)(0.625159, 2)(0.312579, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.312579, 1.75)(0.625159, 1.75)(0.312579, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.25)(7.81248, 2.5)(7.5, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 2.5)(7.5, 2.25)(7.81248, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 2.25)(7.81248, 2.5)(7.81248, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 2.5)(7.81248, 2.5)(8.125, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.5)(7.81248, 2.5)(7.5, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 2.75)(7.81248, 2.5)(7.81248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 2.5)(8.125, 2.5)(8.125, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 2.5)(8.125, 2.75)(7.81248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.5)(8.125, 2.25)(8.43742, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.5)(8.125, 2.5)(8.125, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2.75)(9.37484, 2.5)(9.68742, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 2.75)(9.37484, 2.75)(9.68742, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2.5)(9.37484, 2.75)(9.06258, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2.75)(9.06258, 2.75)(9.06258, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 2.75)(9.68742, 3)(9.37484, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3)(9.37484, 2.75)(9.68742, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3)(9.37484, 2.75)(9.37484, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 2.75)(9.37484, 2.75)(9.06258, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2.75)(9.06258, 3)(8.75, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2.75)(9.06258, 2.75)(9.06258, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 3)(7.81248, 3)(7.81248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 2.75)(8.125, 3)(7.81248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.25)(8.125, 3)(8.43742, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 3)(8.43742, 3.25)(8.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3.25)(8.125, 3)(8.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3)(8.125, 3)(7.81248, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 2.75)(6.875, 3)(6.56248, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 2.75)(6.875, 3)(6.56248, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3)(6.875, 2.75)(7.18748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 3)(6.875, 3)(7.18748, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3)(6.56248, 3.25)(6.56248, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 3.25)(6.875, 3)(6.875, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3)(7.18748, 3)(7.18748, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3)(7.18748, 3.25)(6.875, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 2.25)(5.625, 2.25)(5.93748, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 2)(5.625, 2.25)(5.625, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 2.25)(5.3125, 2)(5.625, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 2.25)(5.3125, 2.25)(5.3125, 2)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 2.25)(5.93748, 2.5)(5.625, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 2.5)(5.625, 2.25)(5.93748, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 2.5)(5.625, 2.25)(5.625, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 2.25)(5.625, 2.25)(5.3125, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 4.25)(4.375, 4)(4.375, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 4)(4.06252, 4.25)(4.06252, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 4.25)(4.375, 4.25)(4.375, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 4.25)(4.375, 4.5)(4.06252, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4.5)(4.06252, 4.25)(4.06252, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4.25)(4.06252, 4.25)(3.75, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 4.25)(3.75, 4)(4.06252, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4)(4.06252, 4.25)(3.75, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 4)(3.75, 4)(3.43752, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4)(3.75, 4.25)(3.43752, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4)(3.75, 3.75)(4.06252, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4)(4.06252, 3.75)(4.06252, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 3.75)(3.75, 4)(3.43752, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 4)(3.43752, 4)(3.43752, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3.25)(4.6875, 3)(5, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3.25)(5, 3)(5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3)(4.6875, 3.25)(4.375, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3.25)(4.375, 3.25)(4.375, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3.5)(4.6875, 3.25)(5, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 3.5)(4.6875, 3.25)(5, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 3.25)(4.6875, 3.5)(4.375, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 3.25)(4.6875, 3.25)(4.375, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 4.25)(9.37484, 4)(9.68742, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4.25)(9.37484, 4)(9.68742, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 3.25)(8.43742, 3.5)(8.125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.25)(8.43742, 3.5)(8.125, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.5)(8.43742, 3.25)(8.75, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 3.5)(8.43742, 3.5)(8.75, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 3.5)(9.68742, 3.25)(9.68742, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 3.25)(9.37484, 3.5)(9.37484, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.75)(8.43742, 4)(8.125, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.75)(8.125, 4)(8.125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.75)(8.125, 3.75)(8.125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.5)(8.43742, 3.75)(8.125, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.75)(8.43742, 3.5)(8.75, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.75)(8.75, 3.5)(8.75, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 3.75)(6.25, 3.5)(6.56248, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 3.5)(6.56248, 3.75)(6.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4)(7.81248, 3.75)(8.125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 4)(7.81248, 4)(8.125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4.25)(7.81248, 4)(8.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4)(8.125, 4)(8.125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 4.25)(7.81248, 4)(7.81248, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 4)(7.81248, 4)(7.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 4)(7.5, 3.75)(7.81248, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 3.75)(7.81248, 4)(7.5, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 3.5)(7.5, 3.75)(7.5, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 3.75)(7.81248, 3.5)(7.81248, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 3.75)(7.18748, 3.5)(7.5, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 3.75)(7.18748, 3.75)(7.18748, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.25)(7.18748, 4)(7.18748, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4)(6.875, 4.25)(6.875, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4)(7.5, 4.25)(7.18748, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4)(7.5, 4)(7.5, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4)(7.5, 3.75)(7.5, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 3.75)(7.18748, 4)(7.18748, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 4.75)(10, 4.75)(10, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 5)(9.68742, 4.75)(10, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 4.75)(9.68742, 5)(9.37484, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4.75)(9.68742, 4.75)(9.37484, 5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 4.75)(9.68742, 4.75)(10, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](10, 4.5)(9.68742, 4.75)(9.68742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 4.75)(9.37484, 4.5)(9.68742, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 4.75)(9.37484, 4.75)(9.37484, 4.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1)(7.18748, 1)(7.18748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1.25)(6.875, 1)(7.18748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 1)(6.875, 1)(6.56248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1)(6.875, 1.25)(6.56248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 1)(7.5, 0.75)(7.81248, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 1)(7.5, 0.75)(7.81248, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 0.75)(7.5, 1)(7.18748, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 0.75)(7.5, 0.75)(7.18748, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 0.75)(7.5, 0.5)(7.81248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 0.75)(7.5, 0.75)(7.81248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 0.5)(7.5, 0.75)(7.18748, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 0.75)(7.18748, 0.75)(7.18748, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 0.75)(9.06258, 0.75)(9.37484, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 0.5)(9.06258, 0.75)(9.06258, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 0.75)(8.75, 0.5)(9.06258, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 0.75)(8.75, 0.75)(8.75, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 1)(9.06258, 0.75)(9.37484, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 0.75)(9.37484, 1)(9.06258, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 1)(9.06258, 0.75)(9.06258, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 0.75)(9.06258, 0.75)(8.75, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1.5)(6.875, 1.75)(6.56248, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 1.5)(6.875, 1.5)(6.56248, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1.75)(6.875, 1.5)(7.18748, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1.5)(7.18748, 1.5)(7.18748, 1.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1.5)(6.56248, 1.5)(6.56248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1.25)(6.875, 1.5)(6.56248, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 1.5)(6.875, 1.5)(7.18748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1.5)(6.875, 1.25)(7.18748, 1.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 9.25)(7.5, 9)(7.5, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 9)(7.5, 9)(7.18748, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 9)(7.18748, 8.75)(7.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 9)(7.18748, 9)(7.18748, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.75)(0.625159, 9)(0.625159, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.75)(0.93742, 9)(0.625159, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.75)(1.25, 8.75)(1.25, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 9)(0.93742, 8.75)(1.25, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.75)(0.625159, 8.75)(0.625159, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.5)(0.93742, 8.75)(0.625159, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](0.93742, 8.75)(0.93742, 8.5)(1.25, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 8.75)(0.93742, 8.75)(1.25, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 7.75)(6.56248, 7.5)(6.875, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.5)(6.875, 7.75)(6.56248, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.5)(6.56248, 7.75)(6.25, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 7.5)(6.56248, 7.5)(6.25, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 7)(7.5, 7.25)(7.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 7.25)(7.5, 7.25)(7.81248, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 7.25)(1.875, 7.5)(1.56258, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 7.25)(1.875, 7.25)(1.56258, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 7.5)(1.875, 7.25)(2.18752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 7.25)(2.18752, 7.25)(2.18752, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 7.25)(1.56258, 7.25)(1.56258, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 7.25)(1.56258, 7)(1.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 7.25)(1.875, 7.25)(2.18752, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 7)(1.875, 7.25)(1.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 7)(4.06252, 6.75)(4.375, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 7)(4.06252, 6.75)(4.375, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6.75)(4.06252, 7)(3.75, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 6.75)(4.06252, 6.75)(3.75, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.375, 6.75)(4.06252, 6.75)(4.375, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6.75)(4.06252, 6.5)(4.375, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6.5)(4.06252, 6.75)(3.75, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.06252, 6.75)(3.75, 6.75)(3.75, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 7)(3.43752, 6.75)(3.43752, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 6.75)(3.43752, 6.75)(3.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.75)(3.75, 7)(3.43752, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.75)(3.75, 6.75)(3.75, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.5)(3.43752, 6.75)(3.125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.75)(3.125, 6.75)(3.125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.43752, 6.75)(3.43752, 6.5)(3.75, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.75, 6.75)(3.43752, 6.75)(3.75, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 9)(1.56258, 9)(1.56258, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8.75)(1.875, 9)(1.56258, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 9)(1.875, 9)(2.18752, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 9)(1.875, 8.75)(2.18752, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9.25)(1.875, 9)(1.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 9)(1.875, 9)(1.56258, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 9)(2.18752, 9.25)(1.875, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 9)(2.18752, 9)(2.18752, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.25, 8.25)(1.56258, 8.25)(1.25, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 8.25)(1.56258, 8.5)(1.25, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8.5)(1.56258, 8.25)(1.875, 8.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 8.5)(1.56258, 8.25)(1.875, 8.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 8)(1.56258, 8.25)(1.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 8.25)(1.25, 8.25)(1.25, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8)(1.56258, 8.25)(1.56258, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 8.25)(1.56258, 8.25)(1.875, 8)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 6.5)(1.875, 6.75)(1.56258, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 6.5)(1.875, 6.75)(1.56258, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 6.75)(1.875, 6.5)(2.18752, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.18752, 6.75)(1.875, 6.75)(2.18752, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 6.75)(1.56258, 7)(1.56258, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.56258, 7)(1.875, 6.75)(1.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 6.75)(2.18752, 6.75)(2.18752, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](1.875, 6.75)(2.18752, 7)(1.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 7)(2.81252, 6.75)(3.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.75)(3.125, 6.75)(3.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.75)(2.81252, 7)(2.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 6.75)(2.81252, 6.75)(2.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 5.75)(8.43742, 6)(8.125, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 5.75)(8.43742, 6)(8.125, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6)(8.43742, 5.75)(8.75, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 6)(8.43742, 6)(8.75, 5.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6)(8.125, 6.25)(8.125, 6)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6)(8.43742, 6.25)(8.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6)(8.75, 6)(8.75, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 6.25)(8.43742, 6)(8.75, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2.5)(9.06258, 2.25)(9.06258, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 2.25)(8.75, 2.5)(8.75, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2.5)(8.43742, 2.25)(8.75, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2.5)(8.43742, 2.5)(8.43742, 2.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 2.75)(8.75, 2.5)(9.06258, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2.75)(8.75, 2.5)(9.06258, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.75)(8.125, 3)(8.125, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 3)(8.43742, 2.75)(8.43742, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.75)(8.75, 3)(8.43742, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.75)(8.75, 2.75)(8.75, 3)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 2.5)(8.43742, 2.75)(8.125, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.5)(8.43742, 2.75)(8.125, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 2.5)(8.43742, 2.75)(8.43742, 2.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 2.75)(8.75, 2.5)(8.75, 2.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.68742, 4)(9.37484, 3.75)(9.68742, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 4)(9.37484, 3.75)(9.68742, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 3.75)(9.68742, 3.5)(9.68742, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 3.75)(9.37484, 3.5)(9.68742, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 3.75)(8.75, 4)(8.43742, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4)(8.43742, 3.75)(8.75, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4)(8.75, 4)(8.43742, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 4.25)(8.75, 4)(8.75, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3.25)(9.06258, 3.5)(8.75, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3.5)(8.75, 3.5)(8.75, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3.5)(9.06258, 3.25)(9.37484, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 3.5)(9.06258, 3.5)(9.37484, 3.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 3.5)(9.06258, 3.5)(8.75, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3.5)(9.06258, 3.75)(8.75, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 3.75)(9.06258, 3.5)(9.37484, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3.5)(9.37484, 3.75)(9.06258, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 3.5)(6.875, 3.75)(6.875, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 3.75)(6.875, 3.75)(7.18748, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3.5)(6.875, 3.75)(6.56248, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3.75)(6.56248, 3.75)(6.56248, 3.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3.75)(7.18748, 4)(6.875, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 4)(6.875, 3.75)(7.18748, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 4)(6.875, 3.75)(6.875, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 3.75)(6.56248, 4)(6.56248, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 4)(6.875, 4.25)(6.56248, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 4.25)(6.56248, 4)(6.875, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 3.75)(5.625, 4)(5.625, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 4)(5.625, 4)(5.93748, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 3.75)(5.625, 4)(5.3125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4)(5.3125, 4)(5.3125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4.25)(5.625, 4)(5.93748, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4)(5.93748, 4)(5.93748, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.625, 4)(5.625, 4.25)(5.3125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 4)(5.625, 4)(5.3125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 3.75)(5, 4)(4.6875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4)(4.6875, 4)(4.6875, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4)(5, 3.75)(5.3125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.3125, 4)(5, 4)(5.3125, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4)(5, 4.25)(4.6875, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](4.6875, 4)(5, 4)(4.6875, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4.25)(5, 4)(5.3125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5, 4)(5.3125, 4)(5.3125, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0.75)(6.56248, 1)(6.56248, 0.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0.75)(6.875, 1)(6.56248, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 1)(6.875, 0.75)(7.18748, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0.75)(7.18748, 0.75)(7.18748, 1)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0.5)(6.875, 0.75)(6.56248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0.75)(6.56248, 0.75)(6.56248, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 0.75)(6.875, 0.5)(7.18748, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 0.75)(6.875, 0.75)(7.18748, 0.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 9)(7.81248, 9.25)(7.5, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 9)(7.81248, 9)(7.5, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 8.75)(7.81248, 9)(7.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 9)(7.5, 9)(7.5, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.25)(6.25, 7.5)(6.25, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.25)(6.56248, 7.5)(6.25, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.5)(6.56248, 7.25)(6.875, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.25)(6.875, 7.25)(6.875, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7)(6.56248, 7.25)(6.25, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.25)(6.25, 7.25)(6.25, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 7.25)(6.56248, 7)(6.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 7.25)(6.56248, 7.25)(6.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 7)(7.18748, 7.25)(6.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 7.25)(6.875, 7.25)(6.875, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 7.25)(7.18748, 7)(7.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7.25)(7.18748, 7.25)(7.5, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 7.5)(7.18748, 7.25)(7.18748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.875, 7.25)(7.18748, 7.25)(6.875, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7.5)(7.18748, 7.25)(7.5, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 7.25)(7.5, 7.5)(7.18748, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7.5)(7.5, 7.25)(7.81248, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7.5)(7.81248, 7.25)(7.81248, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7.5)(7.5, 7.75)(7.18748, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.18748, 7.5)(7.5, 7.5)(7.18748, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7.75)(7.5, 7.5)(7.81248, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.5, 7.5)(7.81248, 7.5)(7.81248, 7.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 7.25)(7.81248, 7)(8.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 7.25)(7.81248, 7.25)(7.81248, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 7)(8.125, 7.25)(8.125, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 7.25)(8.125, 7.25)(8.43742, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 7.5)(8.125, 7.25)(8.125, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 7.25)(8.125, 7.25)(7.81248, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 7.25)(8.43742, 7.5)(8.125, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 7.25)(8.43742, 7.25)(8.43742, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 7)(8.75, 7.25)(8.75, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 7.25)(9.06258, 7)(9.06258, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 7.25)(8.43742, 7)(8.75, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 7.25)(8.43742, 7.25)(8.43742, 7)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 7.5)(8.75, 7.25)(9.06258, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 7.5)(8.75, 7.25)(9.06258, 7.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 7.5)(8.75, 7.25)(8.75, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 7.25)(8.75, 7.25)(8.43742, 7.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 6.75)(2.81252, 6.5)(3.125, 6.5)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.75)(2.81252, 6.5)(3.125, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.5, 6.5)(2.81252, 6.5)(2.5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.5)(2.81252, 6.75)(2.5, 6.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.5)(2.81252, 6.25)(3.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](3.125, 6.5)(2.81252, 6.5)(3.125, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.25)(2.81252, 6.5)(2.5, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](2.81252, 6.5)(2.5, 6.5)(2.5, 6.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 4)(9.37484, 3.75)(9.37484, 4)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.37484, 3.75)(9.06258, 4)(9.06258, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 4)(8.75, 4)(8.75, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 3.75)(9.06258, 4)(8.75, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 4)(9.37484, 4.25)(9.06258, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](9.06258, 4)(9.37484, 4)(9.37484, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4.25)(9.06258, 4)(9.06258, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.75, 4)(9.06258, 4)(8.75, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 4)(5.93748, 3.75)(6.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 4)(5.93748, 4)(5.93748, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 3.75)(6.25, 4)(6.25, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.56248, 4)(6.25, 4)(6.56248, 3.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 4.25)(6.25, 4)(6.25, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](5.93748, 4)(6.25, 4)(5.93748, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 4)(6.56248, 4.25)(6.25, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](6.25, 4)(6.56248, 4)(6.56248, 4.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9.25)(8.125, 9)(8.43742, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 9.25)(8.125, 9)(8.43742, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9)(8.125, 9.25)(7.81248, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](7.81248, 9)(8.125, 9)(7.81248, 9.25)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.43742, 8.75)(8.125, 9)(8.125, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9)(8.43742, 8.75)(8.43742, 9)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9)(7.81248, 8.75)(8.125, 8.75)
\pspolygon[linewidth=0.1pt,fillcolor=white,fillstyle=solid](8.125, 9)(7.81248, 9)(7.81248, 8.75)

